The Realizability of Theta Graphs as Reconfiguration Graphs of Minimum Independent Dominating Sets

The independent domination number $i(G)$ of a graph $G$ is the minimum cardinality of a maximal independent set of $G$, also called an $i(G)$-set. The $i$-graph of $G$ is the graph whose vertices correspond to the $i(G)$-sets, and where two $i(G)$-sets are adjacent if and only if they differ by two adjacent vertices. Not all graphs are $i$-graph realizable, that is, given a target graph $H$, there does not necessarily exist a source graph $G$ such that $H$ is the $i$-graph of $G$. We consider a class of graphs called "theta graphs": a theta graph is the union of three internally disjoint nontrivial paths with the same two distinct end vertices. We characterize theta graphs that are $i$-graph realizable, showing that there are only finitely many that are not. We also characterize those line graphs and claw-free graphs that are $i$-graphs, and show that all $3$-connected cubic bipartite planar graphs are $i$-graphs.

==> ConcM.tex <==

\chapter{Conclusion}

\label{ch:conc}





In this dissertation, we provided new results on the slide graph model of reconfiguration graphs for domination parameters. 


In Chapter \ref{ch:slater}, we defined several variations on the $\gamma$-graph using other  parameters such as  total domination number, the paired domination number,  the irredundance number, and the identification number, and showed that in each case all graphs are $\pi$-graphs for their respective parameters $\pi$.  The singular exception was the Roman dominating graph, where we demonstrated that $K_2$ is not a $\gamma_R$-graph.



In Chapter \ref{ch:igraphs}, we showed that unlike the graphs of  Chapter \ref{ch:slater}, not all graphs are $i$-graph realizable.  We built a series of tools to show that known $i$-graphs can be used to construct new $i$-graphs and applied these results to build other classes of $i$-graphs, such as block graphs, hypercubes, forests, and unicyclic graphs.  We also showed that a chordal graph is $i$-graph realizable if and only if it is diamond-free.


In Chapter \ref{ch:pathcycles}, we determined the structure of the $i$-graphs of paths and cycles, and in the case of cycles, determined exactly which cycles have Hamiltonian or Hamiltonian traceable $i$-graphs. 

In Chapter \ref{ch:comp} we used graph complements to construct the $i$-graph seeds for certain classes of line graphs, theta graphs, and maximal planar graphs.  In doings so, we characterized the line graphs and theta graphs that are $i$-graphs.   
The results concerning the $i$-graph realizability of theta graph are listed in Table \ref{tab:c:thetaLong}.

We conclude this dissertation with a list of open problems, some of which were previously mentioned in the text.




\section*{Open Problems}


%---- S: {op:forbidSubG}

Of the open problems presented in this dissertation, we believe the following to be the most important:

\begin{problem}\label{op:forbidSubG}
	Does there exist a finite forbidden subgraph characterization of $i$-graph realizable graphs?
\end{problem}


\noindent We now list the remaining open problems in the order in which their associated topic was discussed in the dissertation.




%================= SLATER PROBLEMS

\begin{problem}
	Determine conditions on the graph $G$ under which each $\gamma$-graph
	variation is connected/disconnected. 
\end{problem}	

\begin{problem}
	Let $\pi$ be any of the above-mentioned domination-related parameters for which every graph is a $\pi$-graph.
	Is it true that every \textbf{bipartite} graph is the $\pi$-graph of a
	\textbf{bipartite }graph?
\end{problem}

\begin{problem}
	If $H$ is $i$-graph realizable, does there exist a well-covered seed graph $G$ such that $\ig{G}\cong H$?  
\end{problem}

\begin{problem} 
	We have already seen that classes of graphs trees, cycles, and, more generally, block graphs, are $i$-graphs.  As we build new graphs from these families of $i$-graphs, using tree structures, which of those are also $i$-graphs?  
	For example, are cycle-trees $i$-graphs?  Path-trees?  For what families of graphs $H$ are $H$-trees $i$-graphs?
\end{problem}


\begin{problem} \label{con:op:tree}
	Determine the structure of  $i$-graphs of various families of trees.  For example, consider caterpillars in which every vertex has degree 1 or 3.  
	
\end{problem}



\begin{problem} \label{con:op:ham}
	Find more classes of $i$-graphs that are Hamiltonian, or Hamiltonian traceable.
\end{problem}


\begin{problem} \label{con:op:domChain}
	Let $\pi$ be any of the previously mentioned domination-related parameters.  Suppose $G_1, G_2,\dots$ are graphs such that $\pi(G_1) \cong G_2$, $\pi(G_2)\cong G_3$, $\pi(G_3) \cong G_4, \dots$  Under which conditions does there exist an integer $k$ such that $\pi(G_k) \cong G_1$?
	
	%Hedetniemi Domination - Chain type questions
\end{problem}

As a special case of Problem \ref{con:op:domChain},  we saw in Chapter \ref{ch:igraphs}  that for any $n\geq 1$, $\ig{K_n} \cong K_n$, and that for $k \equiv 2 \Mod{3}$, $\ig{C_k} \cong C_k$.   

\begin{problem} 
	Determine for which graphs $G$, $\ig{G} \cong G$.
\end{problem}

==> PathcycleM.tex <==
\chapter{The $i$-Graphs of Paths and Cycles}
\label{ch:pathcycles}



%%%% COMMENTED Note:  WTF is the following for? Why is it here?

%$S_1=\{v_1,v_4, v_7, v_{10},\dots, v_{3k+1}\}$.

%$\edge{S_1, v_1,v_2,S_2} \adedge{v_4,v_5,S_3}  \adedge{v_7,v_8,S_4} \dots \edge{S_{k+1},v_{3k+1},v_{3k+2},S_{k+2}}$



% +++++++++++++++++++++++++++  PRE INFO / REFERENCES  BLAH BLAH +++++++++++++++++



In our previous chapters, we have explored whether a given graph $H$ is $i$-graph realizable.  That is, does there exist a graph $G$ such that $\ig{G} = H$?  We now move to the opposing question: given a graph $G$, what is the structure of $\ig{G}$?  As we have already observed, although not every graph is $i$-graph realizable, every graph does have an $i$-graph.  The exact structure of the resulting $i$-graph can vary among families of graphs from the simplest isolated vertex to surprisingly complex structures.  


In this chapter, we examine the $i$-graphs of two of the most famous classes of graphs: paths and cycles.  To  begin, we use generating functions to count the distinct $i$-sets of the path $P_n$ and the cycle $C_n$.  That is, we determine $ \left|  V \left(\ig{P_n} \right)  \right|$ for $n\geq 1$  and $\left|  V \left(\ig{C_n} \right)  \right|$ for $n \geq 3$.  




% +++++++++++++++++++++++++++  PRE INFO / REFERENCES  BLAH BLAH +++++++++++++++++


\section{The Number of $i$-Sets of Paths} \label{sec:i:numbPaths}

For the remainder of this chapter, we assume that the vertices of the path $P_{n}$  are labelled as $P_{n} = (v_1,v_2,\dots, v_{n})$. 
Given that we are discussing $i$-sets, which are both independent and dominating, if $X$ is an $i$-set of $P_n$, then two consecutive vertices of $X$ are separated by one or two vertices of $P_n-X$; the different interval lengths between these consecutive vertices of $X$ therefore correspond to the different $i$-sets of $P_n$.  This provides our method for counting the distinct $i$-sets of $P_n$.



To begin, recall the following well-known result regarding the  independent domination number for both paths and cycles.



%>>> S: Lemma {lem:i:iPC}
\begin{lemma} \label{lem:i:iPC} \cite{GH13}
	For the path and cycle, $i(P_n) = i(C_n) = \left \lceil n/3 \right \rceil $.
\end{lemma}
% <<< E: Lemma {lem:i:iPC}

\noindent 
Thus, deleting the vertices of an arbitrary $i$-set $X$ of $P_n$ divides $V(P_n)-X$ into $t=i(P_n)+1$ subsets $X_1, X_2,\dots,X_t$, where $X_1$ and $X_t$ could be empty or consist of a single vertex, and where $1 \leq |X_j| \leq 2$ for $ j \neq \{1,t\}$.  An example for $P_{10}$ with sets $X_1, X_2, \dots, X_5$ is given below in Figure \ref{fig:i:GF}.  In particular, notice that $X_1 = \varnothing$.  




%>>> S: Figure {fig:i:GF}	
\begin{figure}[H] \centering	
	\begin{tikzpicture}			 		
		
		%%%% REQUIRED TO FIX THE OVER BRACKET TEXT LABEL
		%% https://tex.stackexchange.com/questions/34446/how-to-join-underbrace-overbrace-between-nodes
		\tikzset{
			position label/.style={
				above = 1pt,
				text height = 1ex,
				text depth = 1ex
			},
			brace/.style={
				decoration={brace, mirror},
				decorate
			}
		}
		
		
		%---------- REF-------------------
		\coordinate (cent) at (0,0) {};
		\coordinate (v0) at (0,0) {};
		
		\foreach \i / \j in {1,2,3,4,5,6,7,8,9,10}
		{
			\path(cent) ++(0: \i*10 mm) node[std,label={ 270:$v_{\i}$}]  (v\i) {};
		}
		\draw[thick] (v1)--(v10);		
		
		
		\foreach \i / \j in {1,3,6,9}
		\node[bred] (w\i) at (v\i) {};
		
		
		
		\foreach \i / \j in {0,1,2,3,4,5,6,7,8,9,10}
		{
			\path(v\i) ++(-3mm,2mm) coordinate (l\i) {};
			\path(v\i) ++(3mm,2mm) coordinate (r\i) {};
		}
		
		\draw [decoration={brace}, decorate, color=blue] (l0.north) -- node [position label, pos=0.5] {$X_1$} (l1.north);
		\draw [decoration={brace}, decorate, color=blue] (r1.north) -- node [position label, pos=0.5] {$X_2$} (l3.north);
		\draw [decoration={brace}, decorate, color=blue] (r3.north) -- node [position label, pos=0.5] {$X_3$} (l6.north);
		\draw [decoration={brace}, decorate, color=blue] (r6.north) -- node [position label, pos=0.5] {$X_4$} (l9.north);
		\draw [decoration={brace}, decorate, color=blue] (r9.north) -- node [position label, pos=0.5] {$X_5$} (r10.north);		
	\end{tikzpicture}   
	
	\caption{The sets $X_1,X_2,\dots,X_5$ of $P_{10}$.}
	\label{fig:i:GF}	
\end{figure}	
% <<< E: Figure {fig:i:GF}	

The number of $i$-sets, therefore, equals the number of integer solutions to the following equation, where $r=|V(P) - X| = n - i(P_n) = n -  \left \lceil n/3 \right \rceil $, and where $x_j = |X_j|$:

\vspace{-1cm}
\begin{align}\label{eq:i:pathEq}
	x_1 + \dots + x_t = r, \text{ where } 0 \leq x_1, x_t \leq 1, \text{ and } 1 \leq x_j \leq 2 \text{ for } j \in \{2,\dots,t-1\}.
\end{align}

\noindent The corresponding generating function is
\begin{align} \label{eq:i:pathGF}
	(1+x)^2(x+x^2)^{t-2} = x^{t-2}(1+x)^t.
\end{align}
\begin{enumerate}[label=$\bullet$]
	\item If $n=3k+1$ then $t=i(P_n)+1=k+2$ and $r=2k$.  Thus we want to the coefficient of $2k$ in  (\ref{eq:i:pathGF}), that is, the coefficient of $x^k$ in $(1+x)^{k+2}$, which is $\binom{k+2}{k}$.
	
	\item If $n=3k+2$, then $t=k+2$ and $r=2k+1$.  Here we want the coefficient of $x^{k+1}$ in $(1+x)^{k+2}$, which is $\binom{k+2}{k+1} = k+2$.
	
	\item If $n=3k+3$, then $t=k+2$ and $r=2k+2$.  Here we want the coefficient of $x^{k+2}$ in $(1+x)^{k+2}$, which is $1$.
\end{enumerate}
\noindent We summarize  the above results in the following lemma. 


%>>> S: Lemma {lem:i:pathSize}
\begin{lemma} \label{lem:i:pathSize}
	For $n \geq 1$, the order of $\ig{P_n}$ is 	
	\begin{align*}
		\left|  V \left(\ig{P_n} \right)  \right|  = 
		\begin{cases}
			1 & \text{ if } \ n = 3k\\ 
			\binom{k+2}{k} & \text{ if }  \ n = 3k+1 \\
			k+2 & \text{ if }  \ n=3k+2.
		\end{cases}
	\end{align*}
\end{lemma}
% <<< E: Lemma {lem:i:pathSize}





% +++++++++++++++++++++++++++  LATTICE GRAPH  +++++++++++++++++

\section{The $i$-Graph of $P_n$} \label{sec:i:Pn}


We remind the reader that the vertices of the path $P_{n}$  are labelled as $P_{n} = (v_1,v_2,\dots, v_{n})$.   As we return to our token-sliding model for $i$-graphs, notice that the $i$-set tokens on $P_n$ that are free to slide are very limited.  

For example, in Figure \ref{fig:i:P10}	below, we have two different $i$-sets on $P_{10}$.  In the first case, the token at $v_6$ which is surrounded on each side by two consecutive non-$i$-set vertices is frozen; a slide in either direction would leave either $v_5$ or $v_7$ undominated.   That is, in this first configuration $|X_3|=|X_4|=2$.   Similarly, near the end of the path, the token at $v_9$ is frozen.  Indeed, the only  token that can slide is $v_3$.  Thus the $i$-graph vertex  associated with the $i$-set in the first figure would have only degree 1.  On the other hand, in the second $i$-set of Figure \ref{fig:i:P10}, we see that there are 4 possible token slides, corresponding to an $i$-graph vertex of degree four.  Indeed, we see  that due to the limited availability of slack between $i$-set vertices, the maximum degree of an $i$-graph vertex of $P_n$ is 4, as we now explain.  Moving the token between $X_i$ and $X_{i+1}$ to the right, we increase $|X_i|$ by one, and decrease $|X_{i+1}|$ by one.




%>>> S: Figure {fig:i:P10}	
\begin{figure}[H] \centering	
	\begin{tikzpicture}			
		%---------- REF-------------------
		\coordinate (cent) at (0,0) {};
		
		\foreach \i / \j in {1,2,3,4,5,6,7,8,9,10}
		{
			\path(cent) ++(0: \i*8 mm) node[std,,label={ 270:$v_{\i}$}]  (v\i) {};
		}
		\draw[thick] (v1)--(v10);		
		
		
		\foreach \i / \j in {1,3,6,9}
		\node[bred] (w\i) at (v\i) {};
		
		\draw[ltteal,thick, ->]  (v3) to [out=45,in=135]  (v4);
		
		
	\end{tikzpicture} 
	
	\vspace{1cm}
	
	\begin{tikzpicture}			
		%---------- REF-------------------
		\coordinate (cent) at (0,0) {};
		
		\foreach \i / \j in {1,2,3,4,5,6,7,8,9,10}
		{
			\path(cent) ++(0: \i*8 mm) node[std,,label={ 270:$v_{\i}$}]  (v\i) {};
		}
		\draw[thick] (v1)--(v10);		
		
		
		\foreach \i / \j in {2,4,7,9}
		\node[bred] (w\i) at (v\i) {};
		
		\draw[ltteal,thick, <-]  (v1) to [out=45,in=135]  (v2);
		\draw[ltteal,thick, ->]  (v4) to [out=45,in=135]  (v5);
		\draw[ltteal,thick, <-]  (v6) to [out=45,in=135]  (v7);
		\draw[ltteal,thick, ->]  (v9) to [out=45,in=135]  (v10);
		
	\end{tikzpicture} 
	
	\caption{Two $i$-sets of $P_{10}$.}
	\label{fig:i:P10}
\end{figure}	
% <<< E: Figure {fig:i:P10}

Thus, a token between $X_i$ and $X_{i+1}$ can slide to the right if and only if 
\begin{align*}
	|X_i| = \begin{cases} 0 & \text{ if } i=0 \\ 1 &  \text{ if }  i \neq 0 \end{cases}  \ \hspace{3mm} \text { and } \  \hspace{3mm}
	|X_{i+1}| = \begin{cases} 1 & \text{ if }    i=t \\ 2 & \text{ if } i \neq t. \end{cases}
\end{align*}

\noindent Similarly, a token between $X_i$ and $X_{i+1}$ can slide to the left if and only if 
\begin{align*}
	|X_i| = \begin{cases} 1 & \text{ if } i=0 \\ 2 &  \text{ if }  i \neq 0 \end{cases}  \ \hspace{3mm}  \text { and } \  \hspace{3mm}
	|X_{i+1}| = \begin{cases} 0 & \text{ if }    i=t \\ 1 & \text{ if } i \neq t. \end{cases}
\end{align*}

\noindent With these results in mind, we can now consider the actual structure of $\ig{P_n}$. 


From Lemma \ref{lem:i:pathSize}, the $i$-graphs of $P_n$ for $n=3k$ and $n=3k+2$ $(k\geq 0$) are immediate.  In particular, a token can move only if it is adjacent to some $X_i$ when $x_i=|X_i|$ is at its lower bound in (\ref{eq:i:pathEq}).  For $n=3k$, there are no such $X_i$, so all tokens are frozen, and $\ig{P_n}=K_1$.  If $n=3k+2$, then exactly one  $X_i$ is at its lower bound.  If $i=0$ or $t$, then one token can move.  Otherwise, $1 \leq i \leq t-1$ and $X_i$ has both a left and right token that can move. Hence $\Delta(\ig{P_{3k+2}}) \leq  2$.  It is easy to confirm that $\ig{P_{3k+2}} = P_{k+2}$.



%>>> S: Lemma {lem:i:2Pn}
\begin{lemma} \label{lem:i:2Pn}
	For $n \geq 1$, $k \geq 0$,		
	\begin{align*}
		\ig{P_n} = 	
		\begin{cases}
			K_1 & \text{ if } n=3k \\
			P_{k+2} & \text{ if } n=3k+2.
		\end{cases}
	\end{align*}
\end{lemma}
% <<< E: Lemma {lem:i:2Pn}

\noindent It is only the third case where $n=3k+1$ that remains to be described.   Using the fact that two $X_i$ are at their lower bound, we get $\Delta(\ig{P_n}) \leq 4$. In order to eventually determine the structure of $\ig{P_{3k+1}}$, we first detour slightly to define a new class of graphs.

%\noindent \textbf{Definition} \\
We define the \emph{worn $k$-lattice graph} $\wlat_k$ to be the graph with $1+2+\dots+k +(k+1)=  \binom{k+2}{2} $ vertices, such that  $V(\wlat_k) = \{w_{i,j}: 0 \leq j \leq i \leq k\}$, and where the vertex $w_{a,b}$ is adjacent to vertex $w_{c,d}$  if and only if one of the following holds:

\begin{enumerate}[label=(\roman*)]
	\item  $a = c-1$ and $b=d \text{ or } d-1$, or
	\item  $a=c+1$ and $b=d \text{ or } d+1$.
\end{enumerate}	

\noindent The graph $\wlat_3$ is given as an example below in Figure \ref{fig:i:wlat3}.	






%>>> S: Figure {fig:i:wlat3}
\begin{figure}[H] \centering	
	\begin{tikzpicture}[scale=1.2]
		
		
		%---------- REF-------------------
		\coordinate (cent) at (0,0) {};
		
		\path (cent) ++(-90: 15 mm) coordinate (centL1);
		\path (centL1) ++(270: 15 mm) coordinate (centL2);
		
		%--------- Level 0
		\node[std,label={ 0: $w_{1,1}$}] (z) at (cent) {}; 
		
		%--------- Level 1
		\path (centL1) ++(180: 15 mm) node[std,label={ 0:  $w_{2,1}$}] (a1) {};
		\path (a1) ++(0: 30 mm) node[std,label={ 0:  $w_{2,2}$}](a2) {};
		
		
		%--------- Level 2
		\path (centL2) ++(180: 30 mm) node[std,label={ 270: $w_{3,1}$}] (b1) {};
		
		
		\path (b1) ++(0: 30 mm) node[std,label={ 270: $w_{3,2}$}] (b2) {};	
		\path (b1) ++(0: 60 mm) node[std,label={ 270: $w_{3,3}$}] (b3) {};	
		
		
		%============================ D LINES
		
		\path (a1) ++(90: 30 mm) node[std,label={ 0: $w_{0,0}$}] (d1) {};
		\path (z) ++(180: 30 mm) node[std,label={ 0: $w_{1,0}$}] (d2) {};
		\path (a1) ++(180: 30 mm) node[std,label={ 0: $w_{2,0}$}] (d3) {};
		\path (b1) ++(180: 30 mm) node[std,label={ 270: $w_{3,0}$}](d4) {};
		
		%--------- Paths
		\draw[thick](z)--(a1)--(b1);
		\draw[thick](z)--(a2)--(b3);
		\draw[thick](a1)--(b2)--(a2);
		\draw[thick](z)--(d1)--(d2)--(d3)--(d4);
		\draw[thick](d2)--(a1);
		\draw[thick](d3)--(b1);
		
	\end{tikzpicture} 
	
	\caption{The worn lattice graph $\wlat_3$.}
	\label{fig:i:wlat3}	
\end{figure}	
% <<< E: Figure {fig:i:wlat3}	





The observant reader will have already noted several similarities to $\wlat_k$ and the structure of $\ig{P_{3k+1}}$.  Notably, recall from Lemma \ref{lem:i:pathSize} that $\ig{P_{3k+1}}$ also has $\binom{k+2}{2}$ vertices.  We have also noted that for each $v\in V(\ig{P_k})$, $\deg(v) \leq 4$.  In Lemma  \ref{lem:i:p3k1} below, we show exactly this connection, with a key observation being that just as one can imagine growing $P_{3k+1}$ into $P_{3(k+1)+1}$ by adding a \emph{tail} of three additional vertices to the end of $P_{3k+1}$, so can we grow $\wlat_k$ into $\wlat_{k+1}$ by adding an additional path of $(k+1)+1$ vertices down one outer-diagonal. We call these vertices the \emph{path tail}  vertices of $\wlat_{k+1}$.

%\begin{m} \label{thm:i:p3k1} cc
% For $k \geq 1$, $\ig{P_{3k+1}} = \wlat_{k-1}$.
%\end{theorem}









The cases for $k=1$ and $k=2$ (i.e. with $P_4$ and $P_7$) are illustrated in Figures \ref{fig:i:P4ig} and  \ref{fig:i:P7ig} below.  Here the vertices  of $\wlat_k$ are labelled with the subscripts of the vertices of an $i$-set of $P_{3k+1}$.  So, for example, the vertex labelled ``$1,4$" at the top of $\wlat_{1}$ corresponds to the $i$-set $\{v_1,v_4\}$ of $P_4$, while the vertex labelled ``$2,4$" corresponds to the $i$-set $\{v_2,v_4\}$.  Cases $k=3$ ($P_{10}$) and $k=4$ ($P_{13}$) are given in Figures \ref {fig:i:P10ig} and \ref {fig:i:P13ig}, respectively, and the added path tail vertices highlighted in green and blue.




%>>> S: Figure {fig:i:P4ig}	
\begin{figure}[H] \centering	
	
	\begin{tikzpicture}			
		%---------- REF-------------------
		\coordinate (cent) at (0,0) {};
		
		\foreach \i / \j in {1,2,3,4}
		{
			\path(cent) ++(0: \i*8 mm) node[std,,label={ 270:$v_{\i}$}]  (v\i) {};
		}
		\draw[thick] (v1)--(v4);		
	\end{tikzpicture} 	\hspace{1cm}
	\begin{tikzpicture}			
		\node[broadArrow,fill=white, draw=black, ultra thick, text width=6mm] at (0,0){};	
	\end{tikzpicture} \hspace{1cm}
	\begin{tikzpicture}			
		
		%---------- REF-------------------
		\coordinate (cent) at (0,0) {};
		
		\path (cent) ++(-90: 15 mm) coordinate (centL1);
		%	\path (centL1) ++(270: 15 mm) coordinate (centL2);
		
		%--------- Level 0
		\node[std,label={ 0:\scriptsize$1,4$}] (z) at (cent) {}; 
		
		%--------- Level 1
		\path (centL1) ++(180: 15 mm) node[std,label={ 0:\scriptsize$2,4$}] (a1) {};
		\path (a1) ++(0: 30 mm) node[std,label={ 0:\scriptsize$1,3$}] (a2) {};	 
		
		%--------- Paths
		\draw[thick](a1)--(z)--(a2);		
		
	\end{tikzpicture} 
	
	\caption{$\ig{P_4} \cong \wlat_{1}$.}
	\label{fig:i:P4ig}	
\end{figure}	
% <<< E: Figure {fig:i:P4ig}	


%>>> S: Figure {fig:i:P7ig}	
\begin{figure}[H] \centering	 
	\begin{tikzpicture}	
		
		
		%---------- REF-------------------
		\coordinate (cent) at (0,0) {};
		
		\path (cent) ++(-90: 15 mm) coordinate (centL1);
		\path (centL1) ++(270: 15 mm) coordinate (centL2);
		
		%--------- Level 0
		\node[std,label={ 0:\scriptsize$1,4,7$}] (z) at (cent) {}; 
		
		%--------- Level 1
		\path (centL1) ++(180: 15 mm) node[std,label={ 0:\scriptsize$2,4,7$}] (a1) {};
		\path (a1) ++(0: 30 mm) node[std,label={ 0:\scriptsize$1,4,6$}] (a2) {};
		
		
		%--------- Level 2
		\path (centL2) ++(180: 30 mm) node[std,label={ 270:\scriptsize$2,5,7$}] (b1) {};
		
		
		\path (b1) ++(0: 30 mm) node[std,label={ 270:\scriptsize$2,4,6$}] (b2) {};	
		\path (b1) ++(0: 60 mm) node[std,label={ 270:\scriptsize$1,3,6$}] (b3) {};	
		
		%--------- Paths
		\draw[thick](z)--(a1)--(b1);
		\draw[thick](z)--(a2)--(b3);
		\draw[thick](a1)--(b2)--(a2);
		
		
		
		
		
	\end{tikzpicture} 
	
	\caption{$\ig{P_7} \cong \wlat_{2}$.}
	\label{fig:i:P7ig}	
\end{figure}	
% <<< E: Figure {fig:i:P7ig}	






%>>> S: Figure {fig:i:P10ig}
\begin{figure}[H] \centering	
	\begin{tikzpicture}	
		
		
		%---------- REF-------------------
		\coordinate (cent) at (0,0) {};
		
		\path (cent) ++(-90: 15 mm) coordinate (centL1);
		\path (centL1) ++(270: 15 mm) coordinate (centL2);
		
		%--------- Level 0
		\node[std,label={ 0:\scriptsize $1,4,7, {\color{forGreen}9}$}] (z) at (cent) {}; 
		
		%--------- Level 1
		\path (centL1) ++(180: 15 mm) node[std,label={ 0:\scriptsize$2,4,7,{\color{forGreen}9}$}] (a1) {};
		\path (a1) ++(0: 30 mm) node[std,label={ 0:\scriptsize$1,4,6,{\color{forGreen}9}$}] (a2) {};
		
		
		%--------- Level 2
		\path (centL2) ++(180: 30 mm) node[std,label={ 270:\scriptsize$2,5,7,{\color{forGreen}9}$}] (b1) {};
		
		
		\path (b1) ++(0: 30 mm) node[std,label={ 270:\scriptsize$2,4,6,{\color{forGreen}9}$}] (b2) {};	
		\path (b1) ++(0: 60 mm) node[std,label={ 270:\scriptsize$1,3,6,{\color{forGreen}9}$}] (b3) {};	
		
		
		%============================ D LINES
		
		\path (a1) ++(90: 30 mm) node[bgreen,label={ 0:\scriptsize $1,4,7, {\color{forGreen}10}$}] (d1) {};
		\path (z) ++(180: 30 mm) node[bgreen,label={ 0:\scriptsize$2,4,7,{\color{forGreen}10}$}] (d2) {};
		\path (a1) ++(180: 30 mm) node[bgreen,label={ 0:\scriptsize$2,5,7,{\color{forGreen}10}$}] (d3) {};
		\path (b1) ++(180: 30 mm) node[bgreen,label={ 270:\scriptsize$2,5,8,{\color{forGreen}10}$}] (d4) {};
		
		%--------- Paths
		\draw[thick](z)--(a1)--(b1);
		\draw[thick](z)--(a2)--(b3);
		\draw[thick](a1)--(b2)--(a2);
		\draw[forGreen, thick](z)--(d1)--(d2)--(d3)--(d4);
		\draw[forGreen, thick](d2)--(a1);
		\draw[forGreen, thick](d3)--(b1);
		
	\end{tikzpicture} 
	
	\caption{$\ig{P_{10}} \cong \wlat_{3}$.}
	\label{fig:i:P10ig}	
\end{figure}	
% <<< E: Figure {fig:i:P10ig}	




%>>> S: Figure {fig:i:P13ig}
\begin{figure}[H] \centering	
	\begin{tikzpicture}			
		
		%---------- REF-------------------
		\coordinate (cent) at (0,0) {};
		
		\path (cent) ++(-90: 15 mm) coordinate (centL1);
		\path (centL1) ++(270: 15 mm) coordinate (centL2);
		
		%--------- Level 0
		\node[std,label={ 0:\scriptsize $1,4,7,  {\color{forGreen}9},  {\color{blue}12}$}] (z) at (cent) {}; 
		
		%--------- Level 1
		\path (centL1) ++(180: 15 mm) node[std,label={ 0:\scriptsize$2,4,7, {\color{forGreen}9},  {\color{blue}12}$}] (a1) {};
		\path (a1) ++(0: 30 mm) node[std,label={ 0:\scriptsize$1,4,6, {\color{forGreen}9},  {\color{blue}12}$}] (a2) {};		
		
		%--------- Level 2
		\path (centL2) ++(180: 30 mm) node[std,label={ 270:\scriptsize$2,5,7, {\color{forGreen}9},  {\color{blue}12}$}] (b1) {};		
		
		\path (b1) ++(0: 30 mm) node[std,label={ 270:\scriptsize$2,4,6,  {\color{forGreen}9},  {\color{blue}12}$}] (b2) {};	
		\path (b1) ++(0: 60 mm) node[std,label={ 270:\scriptsize$1,3,6, {\color{forGreen}9},  {\color{blue}12}$}] (b3) {};			
		
		%============================ D LINES
		\path (a1) ++(90: 30 mm) node[bgreen,label={ 0:\scriptsize $1,4,7, {\color{forGreen}10},  {\color{blue}12}$}] (d1) {};
		\path (z) ++(180: 30 mm) node[bgreen,label={ 0:\scriptsize$2,4,7, {\color{forGreen}10},  {\color{blue}12}$}] (d2) {};
		\path (a1) ++(180: 30 mm) node[bgreen,label={ 0:\scriptsize$2,5,7, {\color{forGreen}10},  {\color{blue}12}$}] (d3) {};
		\path (b1) ++(180: 30 mm) node[bgreen,label={ 270:\scriptsize$2,5,8, {\color{forGreen}10},  {\color{blue}12}$}] (d4) {};
		
		%============================ F LINES
		\path (d2) ++(90: 30 mm) node[bblue,label={ 0:\scriptsize $1,4,7, {\color{forGreen}10},  {\color{blue}13}$}] (f1) {};
		\path (d1) ++(180: 30 mm) node[bblue,label={ 0:\scriptsize$2,4,7, {\color{forGreen}10},  {\color{blue}13}$}] (f2) {};
		\path (d2) ++(180: 30 mm) node[bblue,label={ 0:\scriptsize$2,5,7, {\color{forGreen}10},  {\color{blue}13}$}] (f3) {};
		\path (d3) ++(180: 30 mm) node[bblue,label={ 0:\scriptsize$2,5,8, {\color{forGreen}10},  {\color{blue}13}$}] (f4) {};
		\path (d4) ++(180: 30 mm) node[bblue,label={ 270:\scriptsize$2,5,8, {\color{forGreen}11},  {\color{blue}13}$}] (f5) {};
		
		%--------- Paths
		\draw[thick](z)--(a1)--(b1);
		\draw[thick](z)--(a2)--(b3);
		\draw[thick](a1)--(b2)--(a2);
		\draw[forGreen, thick](z)--(d1)--(d2)--(d3)--(d4);
		\draw[forGreen, thick](d2)--(a1);
		\draw[forGreen, thick](d3)--(b1);
		\draw[blue,thick](f1)--(f2)--(f3)--(f4)--(f5);
		\draw[blue,thick](f1)--(d1);
		\draw[blue,thick](f2)--(d2);
		\draw[blue,thick](f3)--(d3);
		\draw[blue,thick](f4)--(d4);
		
	\end{tikzpicture} 
	
	\caption{$\ig{P_{13}} \cong \wlat_{4}$.}
	\label{fig:i:P13ig}
\end{figure}	
% <<< E: Figure {fig:i:P13ig}







%>>> S: Lemma {lem:i:p3k1} 
\begin{lemma} \label{lem:i:p3k1} 
	For $k\geq 1$, $\ig{P_{3k+1}} \cong \wlat_{k}$.  
\end{lemma}	



%============================ RICK ATTEMPT
\begin{proof}
	We proceed by induction on $k$.  The base cases with $k \in \{1,2,3,4\}$ are given explicitly above in Figures \ref{fig:i:P4ig} - \ref{fig:i:P13ig}.  Assume that $\ig{P_{3k+1}} \cong \wlat_k$.  We now consider $\ig{P_{3k+4}}$.  Observe that every $i$-set of $P_{3k+4}$ contains $v_{3k+3}$ or $v_{3k+4}$.  
	
	%	In our induction, we include the following claims for each value of $k \geq 1$:
	
	%	\begin{enumerate}[label=(\roman*)]
		%	\item 
		%		The $i$-sets down the (pictured as left) side of the $\wlat_k$ correspond to the $i$-sets:
		
		%		\begin{align*} w_{\ell,0} =  \bigcup_{j=0}^{\ell-1} \{v_{3j+2}\} \  \cup  \ \ \bigcup_{j=\ell}^{k} \{v_{3j+1}\}. \end{align*}
		
		%	\item 
		
		
		
		%	\end{enumerate}
	
	
	
	Let $S$ be some $i$-set of ${P_{3k+1}}$, and define  in $P_{3k+4}$ the set $S' = S \cup \{v_{3k+3}\}$.  Then $S'$ is both independent and dominating in $P_{3k+4}$, and since $i(P_{3k+4}) = i(P_{3k+1}) +1 = k+2$,  $S'$ is an $i$-set of $P_{3k+4}$ (and corresponds to a vertex of $\ig{P_{3k+4}}$).  Conversely, given an $i$-set of $P_{3k+4}$ containing $v_{3k+3}$, say $S'$, the set $S = S' - \{v_{3k+3}\}$ is an $i$-set of $P_{3k+1}$.  This follows since $N[v_{3k+3}] = \{v_{3k+2}, v_{3k+3}, v_{3k+4}\}$.
	
	
	
	
	
	
	
	%>>> S: Figure {fig:i:P3k4}
	\begin{figure}[H] \centering	
		\begin{tikzpicture}			
			%---------- REF-------------------
			\coordinate (cent) at (0,0) {};
			
			
			\coordinate (v1) at (cent) {};
			\path(cent) ++(0: 1.3 cm) coordinate  (v2) {};
			\path(v2) ++(0:  2.3  cm) coordinate  (v3k) {};
			
			\foreach \i in {1,2,3,4}
			{
				\path(v3k) ++(0: \i*1.3 cm) node[std,label={ 270:$v_{3k+\i}$}]  (v3k\i) {};
			}
			
			\draw[draw=gray, fill=lgray] \convexpath{v1,v3k1}{7mm};		
			
			\node[std, label={ 270:$v_1$}] (v1x) at (v1) {};
			\node[std, label={ 270:$v_2$}] (v2x) at (v2) {};
			%\node[std, label={ 270:$v_3$}] (v3x) at (v3) {};
			\node[std, label={ 270:$v_{3k}$}] (v3kx) at (v3k) {};
			\node[std, label={ 270:$v_{3k+1}$}] (v3k1x) at (v3k1) {};
			
			
			
			\path(v2) ++(0:  0.6 cm) coordinate (v2a) {};
			\path(v3k) ++(0:  -0.6  cm) coordinate (v3ka) {};
			
			
			\draw[thick] (v1)--(v2a);
			\draw[thick] (v3ka)--(v3k4);
			\draw[thick, dashed] (v3ka)--(v2a);
			
			\node[bgreen] (v3k3G) at (v3k3) {};
			
			
			%	\coordinate (P3k) at ($(v1)!0.5!(v3k1)$) {};	
			%	\path(P3k) ++(90: 1 cm) node  (P3kL) {\color{mgray}$P_{3k+1}$};
			
			%	\foreach \i / \j in {1,3,6,9}
			%	\node[bred] (w\i) at (v\i) {};
			
			%	\draw[ltteal,thick, ->]  (v3) to [out=45,in=135]  (v4);
			
		\end{tikzpicture} 
		\caption{$P_{3k+4}$.}
		\label{fig:i:P3k4}
	\end{figure}	
	% <<< E: Figure {fig:i:P3k4}
	
	
	
	
	
	
	Moreover, if $S_1$ and $S_2$ are $i$-sets of $P_{3k+1}$,  
	we have that $\onlyedge{S_1,S_2}$ if and only if $\onlyedge{S_1',S_2'}$.  It follows that $\ig{P_{3k+4}}$ contains an induced copy of $\ig{P_{3k+1}} = \wlat_k$.  This accounts for $\binom{k+2}{2}$ of the $\binom{k+3}{2}$ vertices in $\ig{P_{3k+4}}$.  
	These are precisely the $i$-sets of $P_{3k+4}$ containing $v_{3k+3}$ (these correspond to the black and green vertices in Figure \ref{fig:i:P13ig}).
	
	Now, consider some $i$-set of $P_{3k+4}$ containing $v_{3k+4}$, say $S'$.  We observe $S'$ must contain either $v_{3k+1}$ or $v_{3k+2}$.  We consider the former first.   Let $S= S'-\{v_{3k+4}\}$.  Then $S$ dominates $\{v_1,v_2,\dots,v_{3k+1}\}$, is independent, and has size $k$.  So, $S$ is an $i$-set of $P_{3k+1}$.  
	
	Conversely, given an $i$-set of $P_{3k+1}$ containing the vertex $v_{3k+1}$, say $S$, the set $S' = S \cup \{v_{3k+4}\}$ is an $i$-set of $P_{3k+4}$.  Finally, given two such sets $S_1$ and $S_2$ and the corresponding $S_1'$ and $S_2'$, we have that $\onlyedge{S_1,S_2}$ if and only if $\onlyedge{S_1',S_2'}$.  This accounts for $k+1$ $i$-sets of $P_{3k+4}$.  We emphasize that these sets are all different from the $\binom{k+2}{2}$ $i$-sets mentioned above.
	
	%	\nts{RE Kieka Note: I don't know.  This entire proof is terrible.}
	
	Let $S_1'$ be an $i$-set of $P_{3k+4}$ containing $v_{3k+4}$ and not $v_{3k+2}$.  Then, let $S_2' = \left\lbrace S_1' \cup \{v_{3k+3}\}\right\rbrace - \{v_{3k+4}\}$.  Now $S_2'$ is  an independent dominating set of size $k+1$ and clearly $\onlyedge{S_1', S_2'}$.  Further, $S_2=S_2' - \{v_{3k+3}\}$ is a dominating set of $P_{3k+1}$ containing $v_{3k+1}$, and so $S_2$ is a path-tail vertex of $\wlat_k$.  Thus, $S_2$ is a path-tail vertex the left-hand side of the copy of $\wlat_k$ inside of $\wlat_{k+1}$ constructed above.    These correspond to the blue vertices matched to the green vertices in Figure \ref{fig:i:P13ig}.  
	
	
	The only remaining $i$-set of $P_{3k+4}$ has both $v_{3k+2}$ and $v_{3k+4}$.  This set is precisely $\{v_2, v_5, \dots, v_{3k+2}, v_{3k+4}\}$.  
	This is the lower left blue vertex in Figure \ref{fig:i:P13ig}, and is adjacent only to  $\{v_2, v_5, \dots, v_{3k+1}, v_{3k+4}\}$, thus forming the (unique) path-tail vertex of $\wlat_{k+1}$ of degree 1.  
	
	Note there are $\binom{k+2}{2}+(k+1)+1 = \binom{k+3}{2}$ $i$-sets, which accounts for all the $i$-sets of $P_{3k+4}$.  
	We emphasize that the $i$-sets of $P_{3k+4}$ containing $v_{3k+4}$ are precisely the path-tail vertices of $\wlat_{k+1}$ (down the left-hand side), verifying the invariant for $k+1$.  The result follows by induction.  
\end{proof}



Bringing Lemmas \ref{lem:i:2Pn} and \ref{lem:i:p3k1}  together yields the following theorem.

%>>> S: Theorem {thm:i:Pn}
\begin{theorem} \label{thm:i:Pn}
	For $n \geq 1$, $k \geq 0$,	and $\wlat_k$ as  defined	in Section \ref{sec:i:Pn},
	\begin{align*}
		\ig{P_n} = 	
		\begin{cases}
			K_1 & \text{ if } n=3k, \\
			\wlat_k & \text{ if } n=3k+1, \\
			P_{k+2} & \text{ if } n=3k+2.
		\end{cases}
	\end{align*}
\end{theorem}
% <<< E: Theorem {thm:i:Pn}


\section{The Number of $i$-Sets of Cycles}	\label{sec:i:numCycles}

Our methods for counting the $i$-sets of cycles are similar to paths, but with an added complication.  Although one might be 
tempted to use the equation in Equation (\ref{eq:i:pathEq})  (restated here for reference)  with the constraints $1 \leq x_j \leq 2$ for $j \in \{1, \dots, t\}$,  this method does not take the rotational symmetries of the $i$-sets of $C_n$ into account: 

\vspace{-1cm}
\begin{align} \label{eq:i:pathEq2}
	x_1 + \dots + x_t = r, \text{ where } 0 \leq x_1, x_t \leq 1, \text{ and } 1 \leq x_j \leq 2 \text{ for } j \in \{2,\dots,t-1\}.
\end{align}




For example, it will count only one $i$-set of $C_n$, $n \equiv 0 \Mod{3}$, whereas $C_n$ has three $i$-sets in this case. Moreover, different $i$-sets have different types of rotational symmetries, and so we cannot simply proceed as above and then multiply the answer by a constant.  

Let $e=v_0v_{n-1}$ be an edge of $C_n$ and consider $P_n = C_n - e = (v_0, \dots, v_{n-1})$.  Any $i$-set $X$ of $C_n$ corresponds to either an $i$-set of $P_n$ or to a ``near $i$-set of $P_n$'', in which 

\begin{enumerate}[label=(\roman*)]
	\item $v_2$ is the first vertex and $v_{n-1}$ is the last vertex of $X$ on $P_n$, or
	\item $v_0$ is the first vertex and $v_{n-3}$ is the last vertex of $X$ on $P_n$.
\end{enumerate}

These three varieties of $i$-sets are pairwise disjoint; therefore, we count the number of $i$-sets by using Equation (\ref{eq:i:pathGF})
with different conditions on the integer variables.  The number of $i$-sets of $C_n$ equals the sum of the number of integer solutions to the following equations, where $r$, $t$ and $x_j$ are defined as in Section \ref{sec:i:numbPaths}:
\begin{align} \label{eq:i:cycleEQ}
	x_1 + \dots + x_t = r, & \text{ where } x_1=0 \text{ and } 1 \leq x_j \leq 2 \text{ for } j \in \{ 2,\dots,t \},\\
	x_1 + \dots + x_t = r, & \text{ where } x_t=0 \text{ and } 1 \leq x_j \leq 2 \text{ for } j \in \{1,\dots,t-1\},\\
	x_1 + \dots + x_t = r, & \text{ where } x_1=x_t=1 \text{ and } 1 \leq x_j \leq 2 \text{ for } j \in \{2,\dots,t-1\}.
\end{align}

The corresponding generating function is 
\begin{align} \label{eq:i:cycleGF}
	(x + x^2)^{t-1} + (x+x^2)^{t-1} + x^2(x+x^2)^{t-2} = 2x^{t-1}(1+x)^{t-1} + x^t(1+x)^{t-2}.
\end{align}

\begin{enumerate}[label=$\bullet$]
	\item If $n=3k+1$, then $t = i(P_n) + 1 = k+2$ and $r=2k$.  Thus, we require the coefficient of $2k$ in (\ref{eq:i:cycleGF}),  that is, in $2x^{k+1}(1+x)^{k+1} + x^{k+2}(1+x)^k$, which is $2 \binom{k+1}{k-1} + \binom{k}{k-2} = k(3k+1)/2$.
	
	\item If $n = 3k+2$, then $t=k+2$ and $r=2k+1$.  Thus, we require the coefficient of $2k+1$ in $2x^{k+1}(1+x)^{k+1}+x^{k+2}(1+x)^k$, which is $2\binom{k+1}{k} + \binom{k}{k-1} = 3k+2 = n$.
	
	\item If $n=3k+3$, then $t=k+2$ and $r=2k+2$.  Thus, we require the coefficient of $2k+2$ in $2x^{k+1}(1+x)^{k+1} + x^{k+2}(1+x)^k$, which is 3.
	
\end{enumerate}

We summarize this result in the lemma below.

%>>> S: Lemma {lem:i:cycleSize}
\begin{lemma} \label{lem:i:cycleSize}
	For $n \geq 3$, the order of $\ig{C_n}$ is 
	
	\begin{align*}
		\left|  V \left(\ig{C_n} \right)  \right|  = 
		\begin{cases}
			3 & \text{ if } \ n = 3k\\ 
			k(3k+1)/2 & \text{ if }  \ n = 3k+1 \\
			n & \text{ if }  \ 3k+2.
		\end{cases}
	\end{align*}
\end{lemma}
% <<< E: Lemma {lem:i:cycleSize}





%---------------------------------------SECTION: $i$-graphs of cycles ----------------
\section{The $i$-Graphs of Cycles}	\label{sec:i:cycles}


Contrary to our conventions in the previous sections on paths, we assume that all cycles have labelled vertices $V(C_n) = (v_0,v_1,\dots,v_{n-1})$.  

Immediately, we discover that some of the $i$-graphs for $C_n$ are fairly straight-forward.  For a $C_{3}$, this is a complete graph, and hence $\ig{C_3} = \ig{K_3} = C_3$.  For $C_{3k}$ with  $3k \geq 6$,  $|V(C_{3k})|$ is divisible by 3, and hence there are three distinct $i$-sets of $C_{3k}$, in which each $i$-set vertex has two non-$i$-set vertices between it and the next $i$-set vertex; thus each $i$-set vertex is frozen, and hence $\ig{C_n}$ consists of three singletons.   

For $C_{n}$ with $n \equiv 2 \Mod{3}$, say $n=3k+2$, each $i$-set of $C_n$ contains exactly one pair of vertices $v_{j-1}$ and $v_{j+1}$ that are separated by exactly one vertex, $v_j$, not in the $i$-set (the common neighbour of these two vertices), while all other pairs  of consecutive $i$-set vertices are separated by exactly two vertices not in the $i$-set.  Hence, the $i$-set has exactly two vertices, namely $v_{j-1}$ and $v_{j+1}$, that are not frozen, and each of them can slide in only one direction.  The vertex $v_{j-1}$ can move to $v_{j-2}$, and $v_{j+1}$ can move to $v_{j+2}$.  In the former case,  the vertex that has two neighbours  in the $i$-set is now $v_{j-3}$, while in the latter, it is $v_{j+3}$.  As a result, $\ig{C_n}$ is 2-regular and since 3 is coprime to $n$, the sequence $v_j$, $v_{j+3}$, $v_{j+6}$, $\dots$, of the vertex dominated by two vertices in the $i$-set will visit each vertex in $C_n$  after $n$-slides.  Thus, each $i$-set is generated; that is, $\ig{C_n}$ is connected.  As it is 2-regular and connected, we conclude it is a cycle.




We provide examples of $C_5$ and $C_8$ in Figures \ref{fig:i:C5} and \ref{fig:i:C8} below.  




%>>> S: Figure {fig:i:C5}	
\begin{figure}[H] \centering
	\begin{subfigure}{.4\textwidth}
		\begin{tikzpicture}			
			%---------- REF-------------------
			\coordinate (cent) at (0,0) {};
			
			
			%=========  MAIN CYCLE W/O BOXED NODES
			\foreach \i  in {0,1,2,3,4} 
			{
				\node[std,label={90-\i*72: ${v_{\i}}$}] (v\i) at (90-\i*72:2cm) {}; 
			}
			
			
			\draw[thick] (v0)--(v1)--(v2)--(v3)--(v4)--(v0);
			
			%======== RED NODES 
			\foreach \i  in {1,3} 
			{
				\node[regRed] (r\i) at (v\i) {};
			}
		\end{tikzpicture} 
		\caption{$C_5$ with the $i$-set $\{v_1,v_3\}$ in red.}
		\label{subfig:i:C5}
	\end{subfigure}
	\hspace{10mm}
	\begin{subfigure}{.4\textwidth}
		\begin{tikzpicture}			
			%---------- REF-------------------
			\coordinate (cent) at (0,0) {};
			
			
			%=========  MAIN CYCLE W/O BOXED NODES
			\foreach \i / \x / \y  in {0/0/2,1/0/3,2/1/3,3/1/4,4/2/4} 
			{
				\node[std,label={90-\i*72: $\{v_{\x},v_{\y}\}$}] (v\i) at (90-\i*72:2cm) {}; 
			}	
			
			\draw[thick] (v0)--(v1)--(v2)--(v3)--(v4)--(v0);
			
			%======== RED NODES 
			\foreach \i  in {2} 
			{
				\node[regRed] (r\i) at (v\i) {};
			}
		\end{tikzpicture} 
		\caption{$\ig{C_5}$ with the vertex corresponding to the $i$-set $\{v_1,v_3\}$ in red. }
		\label{subfig:i:C5i}
	\end{subfigure}
	\caption{$C_5$ and its $i$-graph.}
	\label{fig:i:C5}
\end{figure}
% <<< E: Figure {fig:i:C5}


%>>> S: Figure {fig:i:C8}	
\begin{figure}[H] \centering
	\begin{subfigure}{.4\textwidth}
		\begin{tikzpicture}			
			%---------- REF-------------------
			\coordinate (cent) at (0,0) {};
			
			
			%=========  MAIN CYCLE W/O BOXED NODES
			\foreach \i  in {0,1,2,3,4,5,6,7} 
			{
				\node[std,label={90-\i*45: ${v_{\i}}$}] (v\i) at (90-\i*45:2cm) {}; 
			}
			
			
			\draw[thick] (v0)--(v1)--(v2)--(v3)--(v4)--(v5)--(v6)--(v7)--(v0);
			
			%======== RED NODES 
			\foreach \i  in {1,3,6} 
			{
				\node[regRed] (r\i) at (v\i) {};
			}
		\end{tikzpicture} 
		\caption{$C_8$ with the $i$-set $\{v_1,v_3,v_6\}$ in red.}
		\label{subfig:i:C8}
	\end{subfigure}
	\hspace{6mm}
	\begin{subfigure}{.5\textwidth}
		\begin{tikzpicture}			
			%---------- REF-------------------
			\coordinate (cent) at (0,0) {};
			
			
			%=========  MAIN CYCLE W/O BOXED NODES
			\foreach \i / \x / \y / \z in {0/0/2/5,1/0/3/5,2/0/3/6,3/1/3/6,4/1/4/6,5/1/4/7,6/2/4/7,7/2/5/7} 
			{
				\node[std,label={90-\i*45: $\{v_{\x},v_{\y},v_{\z}\}$}] (v\i) at (90-\i*45:2cm) {}; 
			}	
			
			\draw[thick] (v0)--(v1)--(v2)--(v3)--(v4)--(v5)--(v6)--(v7)--(v0);
			
			%======== RED NODES 
			\foreach \i  in {3} 
			{
				\node[regRed] (r\i) at (v\i) {};
			}
		\end{tikzpicture} 
		\caption{$\ig{C_8}$ with the vertex corresponding to the $i$-set $\{v_1,v_3,v_6\}$ in red. }
		\label{subfig:i:C8i}
	\end{subfigure}
	\caption{$C_8$ and its $i$-graph.}
	\label{fig:i:C8}
\end{figure}
% <<< E: Figure {fig:i:C8}





We summarize these results in the lemma below.  
% <<< E: Lemma {lem:i:2Cn}
%>>> S: Lemma {lem:i:2Cn}
\begin{lemma} \label{lem:i:2Cn}
	For $n \geq 3$, $k \geq 0$,	
	\begin{align*}
		\ig{C_n} \cong 	
		\begin{cases}
			K_3 & \text{ if } n=3 \\
			3K_1 & \text{ if } n=3k \geq 6 \\
			C_n & \text{ if } n \equiv 2 \Mod{3}.
		\end{cases}
	\end{align*}
\end{lemma}
% <<< E: Lemma {lem:i:2Cn}




%\nts{Does third case of above $\ig{C_n} \cong C_n$ need more of a formal proof than the "frozen token" explanation on the previous page?}


Once again, the case that requires deeper analysis is $n = 3k+1$ for $k \geq 1$.  To help us tackle this final case, we first introduce a new notation for referencing the $i$-sets of cycles.  

For cycles $C_{3k+1}$, given any $i$-set $X$, there are exactly two vertices in $C_{3k+1} - X$ that are doubly dominated (that is, are adjacent to two different vertices of $X$).  Rather than referring to the $i$-set by its elements, which given a large $k$, could be numerous, we instead refer to the $i$-sets by these two unique vertices.  For clarity, we use a wide-angled bracketed notation when using this convention.  Figure \ref{fig:i:C13}	below illustrates this system:  for (a), rather than calling the $i$-set $X=\{v_1,v_3,v_6,v_9,v_{12}\}$, we refer to it as $\left\langle 0,2\right\rangle = \left\langle 2,0\right\rangle $.  Similarly in (b), instead of $Y=\{v_1,v_4,v_6,v_9,v_{12}\}$, we denote the $i$-set as $\left\langle 0,5\right\rangle $.





%>>> S: Figure {fig:i:C13}	
\begin{figure}[H] \centering	
	
	\begin{subfigure}{.35\textwidth}
		\begin{tikzpicture}			
			%---------- REF-------------------
			\coordinate (cent) at (0,0) {};
			
			
			%=========  MAIN CYCLE W/O BOXED NODES
			\foreach \i  in {1,3,4,5,6,7,8,9,10,11,12} 
			{
				\node[std,label={90-\i*27.6923: ${\i}$}] (v\i) at (90-\i*27.6923:2cm) {}; 
			}
			
			
			%========= BOXED NODES
			\foreach \i  in {0,2} 
			{
				
				\node[std,label={90-\i*27.6923: $\color{blue} \fbox{{\i}}$}] (v\i) at (90-\i*27.6923:2cm) {}; 
				
			}	
			
			\draw[thick] (v0)--(v1)--(v2)--(v3)--(v4)--(v5)--(v6)--(v7)--(v8)--(v9)--(v10)--(v11)--(v12)--(v0);
			
			%======== RED NODES 
			\foreach \i  in {1,3,6,9,12} 
			{
				\node[regRed] (r\i) at (v\i) {};
			}
		\end{tikzpicture} 
		\caption{$X=\{v_1,v_3,v_6,v_9,v_{12}\}$, \\ denoted as $\left\langle 0,2\right\rangle$.}
		\label{subfig:i:C13b}
	\end{subfigure}
	\hspace{3cm}
	\begin{subfigure}{.35\textwidth}
		\begin{tikzpicture}			
			%---------- REF-------------------
			\coordinate (cent) at (0,0) {};
			
			
			%=========  MAIN CYCLE W/O BOXED NODES
			\foreach \i  in {1,2,3,4,6,7,8,9,10,11,12} 
			{
				\node[std,label={90-\i*27.6923: ${\i}$}] (v\i) at (90-\i*27.6923:2cm) {}; 
			}
			
			
			%========= BOXED NODES
			\foreach \i  in {0,5} 
			{
				
				\node[std,label={90-\i*27.6923: $\color{blue} \fbox{{\i}}$}] (v\i) at (90-\i*27.6923:2cm) {}; 
				
			}	
			
			\draw[thick] (v0)--(v1)--(v2)--(v3)--(v4)--(v5)--(v6)--(v7)--(v8)--(v9)--(v10)--(v11)--(v12)--(v0);
			
			%======== RED NODES 
			\foreach \i  in {1,4,6,9,12} 
			{
				\node[regRed] (r\i) at (v\i) {};
			}
		\end{tikzpicture} 
		\caption{$Y=\{v_1,v_4,v_6,v_9,v_{12}\}$, \\ denoted as $\left\langle 0,5\right\rangle$.}
		\label{subfig:i:C13a}
	\end{subfigure}
	\caption{Two $i$-sets of $C_{13}$.}
	\label{fig:i:C13}
\end{figure}	
% <<< E: Figure {fig:i:C13}


%----------------

With this new labelling in place, we move now to a proposed family of graphs that we have dubbed \emph{bracelet graphs}, $\bcl_{k}$.
The vertex set of $\bcl_{k}$ consists of all distinct $2$-subsets
$\{j,\ell\}$ of $\{0,1,\dots,3k\}$ such that $0\leq j\leq3k$ and $\ell\equiv
j+3s+2(\operatorname{mod}\ 3k+1)$, $s\in\{0,1,\dots,k-1\}$. For example, the
subsets containing $0$ are $\{0,2\},\{0,5\},\dots,\{0,3k-4\},\{0,3k-1\}$.

To simplify notation, assume the vertices of $C_{3k+1}$ are labelled $0,1,\dots,3k$ in clockwise
order, as illustrated in Figure \ref{fig:i:C13}. In $\mathfrak{B}_{k}$, the neighbours of
the vertex $\{j,\ell\}$ are described below.
\begin{enumerate}
	\item Suppose $j-\ell\equiv2$ or $-2\ (\operatorname{mod}\ 3k+1)$. Assume
	without loss of generality that $j$ precedes $\ell$ in clockwise order around
	$C_{3k+1}$. (Thus, for the subsets $\{0,2\}$ and $\{11,0\}$ of $C_{13}$, for
	example, $0$ precedes $2$, while $11$ precedes $0$.) With arithmetic performed
	modulo $3k+1$, the neighbours of $\{j,\ell\}$ are $\{j,\ell+3\}$ and
	$\{j-3,\ell\}$, and $\{j,\ell\}$ has degree $2$ in $\mathfrak{B}_{k}$. (Thus,
	$\{0,2\}$ is adjacent to $\{0,5\}$ and $\{10,2\}$ in $\mathfrak{B}_{4}$, while
	$\{11,0\}$ is adjacent to $\{11,3\}$ and $\{8,0\}$.)
	
	\item Suppose $j-\ell\not \equiv 2$ or $-2\ (\operatorname{mod}\ 3k+1)$. Then
	the neighbours of $\{j,\ell\}$ in $\mathfrak{B}_{k}$ are $\{j-3,\ell
	\},\{j+3,\ell\},\{j,\ell-3\}$ and $\{j,\ell+3\}$ (arithmetic modulo $3k+1$),
	and $\{j,\ell\}$ has degree $4$ in $\mathfrak{B}_{k}$. (For example, the
	neighbours, in $\mathfrak{B}_{4}$, of $\{0,5\}$ are $\{10,5\},\{3,5\},\{0,2\}$
	and $\{0,8\}$).
\end{enumerate}



\begin{comment}
	
	For $k \geq 1$, define the graphs $\bcl_{k}$ as follows. The vertex set of $\bcl_{k}$ consists of all distinct 2-subsets
	$\cid{j,\ell}$ of $\{0,1,\dots,3k\}$ such that $0 \leq j \leq 3k$ and $\ell \equiv j+3s+2 \Mod{3k+1}$, $s \in \{0,1,\dots,k-1\}$.  
	Note that $\bcl_{k}$ has order $\frac{1}{2} k (3k+1)$.  For $r\in \{1,2\}$, define $j_r$ and $\ell_r$ to be the least residues
	
	
	
	\begin{align*}
		\ell_1 \equiv \ell+3 \Mod{3k+1}, \ell_2 \equiv \ell-3 \Mod {3k+1} \\
		j_1 \equiv j+3 \Mod{3k+1}, j_2 \equiv j-3 \Mod{3k+1}.
	\end{align*}
	
	The neighbours in $\bcl_k$ of the vertex $\{j,\ell\}$ are all vertices in the set
	
	\begin{align*}
		\{\{j,\ell_1\}, \{j, \ell_2\} \in V(F_k): |\ell_r -j| \notin \{1,3k\}, \  r \in \{1,2\}  \} \cup  \\
		\{\{j_1,\ell\}, \{j_2, \ell\} \in V(F_k): |\ell -j_r| \notin \{1,3k\}, \  r \in \{1,2\}  \} .
	\end{align*}
	
\end{comment}

%\nts{RB: Include a small example $\{0,2\},\{0,5\},...$}


%\nts{Stuck on notation here. Bracelets should exist independently outside of the context of i-graphs  and hence use a $\{a,b\}$ notation.  But when specify the i-graph of a cycle (which so happens to be bracelet) we want $\bk{a,b}$ to make it clear that $\{a,b\}$ is not the $i$-set itself.}

We emphasize that the sets $\bk{j,\ell}$ are unordered.  For example, the neighbours of $\bk{2,7}$ in $\bcl_3$ are $\bk{2,0} = \bk{0,2}, \bk{2,4},\bk{9,7} = \bk{7,9}$ and $\bk{5,7}$.  Examples of these graphs are given in Figures \ref{fig:i:iC7},	\ref{fig:i:iC10},  \ref{fig:i:iC13},  and \ref{fig:i:iC16} below, but where the set braces are removed to reduce visual clutter.  			

The two-number identifiers on the vertices of a bracelet graph and the $i$-sets of a cycle $C_{3k+1}$ are no coincidence; in the following series of lemmas and observations, we show that they are one and the same.  That is, we show that the vertex $\{i,j\}$ in the bracelet graph $\bcl_k$ corresponds to the $i$-set of $C_{3k+1}$ represented by $\cid{i,j}$, and hence that $\ig{C_{3k+1}} \cong \bcl_k$.

%\nts{Still need to fix this}.



%......................  SUB SECTION:  theta (1,k,l) .........................
%\subsection{$\thet{1,k,\ell}$}  \label{subsec:c:1kl}

% +++++++++++++++++++++++++++  LABELLING +++++++++++++++++

%>>> S: Figure {fig:i:iC7}	
\begin{figure}[H] \centering	 	 
	\begin{tikzpicture}			
		%---------- REF-------------------
		%	\coordinate (cent) at (0,0) {};			
		
		%----- TOP LINE
		\foreach \c / \i / \j in {
			0/	0	/	2	,
			1/	3	/	5	,
			2/	6	/	1	,
			3/	2	/	4		
		}
		{
			\node[std,label={0: \scriptsize ${\i,\j}$}] (v\c) at (2*\c, 2) {}; 					
		}				
		
		%----- BOTTOM LINE
		\foreach \c / \i / \j in {
			0/	0	/	5	,
			1/	3	/	1	,
			2/	6	/	4								
		}
		{
			\node[std,label={0: \scriptsize ${\i,\j}$}] (z\c) at (1+2*\c, 0) {}; 					
		}			
		
		%----- EDGES		
		\foreach \i / \j in {0/1,1/2,2/3}
		{
			\draw (z\i)--(v\j);
			\draw (z\i)--(v\i);
		}
		
		\draw (v0) to [out=270,in=160]  (1,-1) to [out=0, in=180]  (5,-1)  to [out=10,in=270]  (v3); 
		%	\draw (z0) to [out=-55,in=-45]  (w4); 
		
	\end{tikzpicture} 
	\caption{$\bcl_2 \cong \ig{C_{7}}$.}
	\label{fig:i:iC7}		 
\end{figure}
% <<< E: Figure {fig:i:iC7}



%>>> S: Figure {fig:i:iC10}	
\begin{figure}[H] \centering	 	 
	\begin{tikzpicture}			\hspace{3mm}
		%---------- REF-------------------
		%	\coordinate (cent) at (0,0) {};			
		
		%----- TOP LINE
		\foreach \c / \i / \j in {
			0/	7	/	9	,
			1/	0	/	2	,
			2/	3	/	5	,
			3/	6	/	8	,
			4/	1	/	9	}
		{
			\node[std,label={0: \scriptsize ${\i,\j}$}] (v\c) at (2*\c, 2) {}; 					
		}				
		
		%----- MID LINE
		\foreach \c / \i / \j in {
			0/	2	/	7	,
			1/	0	/	5	,
			2/	3	/	8	,
			3/	1	/	6	,
			4/	4	/	9									
		}
		{
			\node[std,label={0: \scriptsize ${\i,\j}$}] (w\c) at (1+2*\c, 1) {}; 					
		}	
		
		%----- BOTTOM LINE
		\foreach \c / \i / \j in {
			0/	2	/	4	,
			1/	5	/	7	,
			2/	0	/	8	,
			3/	1	/	3	,
			4/	4	/	6							
		}
		{
			\node[std,label={0: \scriptsize ${\i,\j}$}] (z\c) at (2*\c, 0) {}; 					
		}			
		
		%----- EDGES
		\draw	(v0)--(w0)--(z0);
		\draw	(v1)--(w1)--(z1);
		\draw	(v2)--(w2)--(z2);
		\draw	(v3)--(w3)--(z3);
		\draw	(v4)--(w4)--(z4);
		
		\draw	(v1)--(w0)--(z1);
		\draw	(v2)--(w1)--(z2);
		\draw	(v3)--(w2)--(z3);
		\draw	(v4)--(w3)--(z4);
		
		\draw (v0) to [out=55,in=45]  (w4); 
		\draw (z0) to [out=-55,in=-45]  (w4); 
		
	\end{tikzpicture} 
	\caption{$\bcl_3 \cong \ig{C_{10}}$.}
	\label{fig:i:iC10}		 
\end{figure}
% <<< E: Figure {fig:i:iC10}


%>>> S: Figure {fig:i:C13}	
\begin{figure}[H]  \begin{minipage}{0.1\textwidth} 
	\begin{tikzpicture}		\hspace{-13mm}	
		%---------- REF-------------------
		%	\coordinate (cent) at (0,0) {};				
		
		%----- TOP LINE - T
		\foreach \c / \i / \j in {
			0/	0	/	2	,
			1/	3	/	5	,
			2/	6	/	8	,
			3/	9	/	11	,
			4/	1	/	12	,
			5/	2	/	4	
		}
		{
			\node[std,label={0: \scriptsize ${\i,\j}$}] (t\c) at (1+2*\c, 3) {}; 					
		}				
		
		%----- MID 1 LINE - V
		\foreach \c / \i / \j in {
			0/	2	/	10	,
			1/	0	/	5	,
			2/	3	/	8	,
			3/	6	/	11	,
			4/	1	/	9	,
			5/	4	/	12	,
			6/	2	/	7										
		}
		{
			\node[std,label={0: \scriptsize ${\i,\j}$}] (v\c) at (2*\c, 2) {}; 					
		}	
		
		%----- MID 2 LINE - W
		\foreach \c / \i / \j in {
			0/	5	/	10	,
			1/	0	/	8	,
			2/	3	/	11	,
			3/	1	/	6	,
			4/	4	/	9	,
			5/	7	/	12									
		}
		{
			\node[std,label={0: \scriptsize ${\i,\j}$}] (w\c) at (1+2*\c, 1) {}; 					
		}					
		
		%----- MID 3 LINE - Z
		\foreach \c / \i / \j in {
			0/	5	/	7	,
			1/	8	/	10	,
			2/	0	/	11	,
			3/	1	/	3	,
			4/	4	/	6	,
			5/	7	/	9	,
			6/	10	/	12										
		}
		{
			\node[std,label={0: \scriptsize ${\i,\j}$}] (z\c) at (2*\c, 0) {}; 					
		}			
		
		%----- EDGES
		\draw	(t0)--(v0)--(w0)--(z0);
		\draw	(t1)--(v1)--(w1)--(z1);
		\draw	(t2)--(v2)--(w2)--(z2);
		\draw	(t3)--(v3)--(w3)--(z3);
		\draw	(t4)--(v4)--(w4)--(z4);
		\draw	(t5)--(v5)--(w5)--(z5);
		
		\draw	(t0)--(v1)--(w0)--(z1);
		\draw	(t1)--(v2)--(w1)--(z2);
		\draw	(t2)--(v3)--(w2)--(z3);
		\draw	(t3)--(v4)--(w3)--(z4);
		\draw	(t4)--(v5)--(w4)--(z5);
		\draw	(t5)--(v6)--(w5)--(z6);			
		
		\draw (v0) to [out=135,in=45]  (v6); 
		\draw[very thick,red] (v0) to [out=-135,in=160]  (0.2,-1) to [out=-20,in=210] (z6); 
		\draw[very thick,red] (v6) to [out=-25,in=30]  (13,-0.5) to [out=210,in=-30] (z0); 
		
		
		%---- RED HAMIL EDGES
		\foreach \i / \j in {0/1,1/2,2/3,3/4,4/5,5/6}
		{
			\draw[very thick,red] (t\i)--(v\j);
			\draw[very thick,red] (t\i)--(v\i);
		}		
		
		\foreach \i / \j in {0/1,1/2,2/3,3/4,4/5,5/6}
		{
			\draw[very thick,red] (w\i)--(z\j);
			\draw[very thick,red] (z\i)--(w\i);
		}		
		
		
	\end{tikzpicture} 
\end{minipage}
	\caption{$\bcl_4 \cong \ig{C_{13}}$ with Hamiltonian cycle in red.}
	\label{fig:i:iC13}
\end{figure}
% <<< E: Figure {fig:i:iC13}


%>>> S: Figure {fig:i:C16}	
\begin{figure}[H] 	 \centering
	\begin{tikzpicture}	[scale=0.9]	 %	\hspace{-3cm}	
		%---------- REF-------------------
		%	\coordinate (cent) at (0,0) {};				
		
		%----- TOP LINE
		\foreach \c / \i / \j in {
			0/	0	/	2	,
			1/	3	/	5	,
			2/	6	/	8	,
			3/	9	/	11	,
			4/	12	/	14	,
			5/	1	/	15	,
			6/	2	/	4	,
			7/	5	/	7			
		}
		{
			\node[std,label={0: \scriptsize ${\i,\j}$}] (r\c) at (2*\c, 4) {}; 					
		}			
		
		%----- Mid1 LINE
		\foreach \c / \i / \j in {
			0/	0	/	5	,
			1/	3	/	8	,
			2/	6	/	11	,
			3/	9	/	14	,
			4/	1	/	12	,
			5/	4	/	15	,
			6/	2	/	7	,
			7/	5	/	10				
		}
		{
			\node[std,label={0: \scriptsize ${\i,\j}$}] (t\c) at (1+2*\c, 3) {}; 					
		}		
		
		%----- MID 2 LINE
		\foreach \c / \i / \j in {
			0/	5	/	13	,
			1/	0	/	8	,
			2/	3	/	11	,
			3/	6	/	14	,
			4/	1	/	9	,
			5/	4	/	12	,
			6/	7	/	15	,
			7/	2	/	10										
		}
		{
			\node[std,label={0: \scriptsize ${\i,\j}$}] (v\c) at (2*\c, 2) {}; 					
		}	
		
		%----- MID 3 LINE
		\foreach \c / \i / \j in {
			0/	8	/	13	,
			1/	0	/	11	,
			2/	3	/	14	,
			3/	1	/	6	,
			4/	4	/	9	,
			5/	7	/	12	,
			6/	10	/	15	,
			7/	2	/	13												
		}
		{
			\node[std,label={0: \scriptsize ${\i,\j}$}] (w\c) at (1+2*\c, 1) {}; 					
		}					
		
		%----- MID 3 LINE
		\foreach \c / \i / \j in {
			0/	8	/	10	,
			1/	11	/	13	,
			2/	0	/	14	,
			3/	1	/	3	,
			4/	4	/	6	,
			5/	7	/	9	,
			6/	10	/	12	,
			7/	13	/	15										
		}
		{
			\node[std,label={0: \scriptsize ${\i,\j}$}] (z\c) at (2*\c, 0) {}; 					
		}			
		
		%----- EDGES
		\draw	(r0)--(t0)--(v0)--(w0)--(z0);
		\draw	(r1)--(t1)--(v1)--(w1)--(z1);
		\draw	(r2)--(t2)--(v2)--(w2)--(z2);
		\draw	(r3)--(t3)--(v3)--(w3)--(z3);
		\draw	(r4)--(t4)--(v4)--(w4)--(z4);
		\draw	(r5)--(t5)--(v5)--(w5)--(z5);
		\draw	(r6)--(t6)--(v6)--(w6)--(z6);
		\draw	(r7)--(t7)--(v7)--(w7)--(z7);
		
		\draw	(r1)--(t0)--(v1)--(w0)--(z1);
		\draw	(r2)--(t1)--(v2)--(w1)--(z2);
		\draw	(r3)--(t2)--(v3)--(w2)--(z3);
		\draw	(r4)--(t3)--(v4)--(w3)--(z4);
		\draw	(r5)--(t4)--(v5)--(w4)--(z5);
		\draw	(r6)--(t5)--(v6)--(w5)--(z6);
		\draw	(r7)--(t6)--(v7)--(w6)--(z7);		
		
		
		\draw (v0) to [out=155,in=190]  (0.8,5) to [out=10, in=180]  (8,5.5)  to [out=0,in=35]  (t7);    
		\draw[red] (v0) to [out=-155,in=-190]  (0.8,-1) to [out=-10, in=180]  (8,-1.5)  to [out=0,in=-35]  (w7);    		
		
		
		\draw[color=blue] (r0) to [out=70,in=190]  (3,6) to [out=10, in=160]  (15,5.5)  to [out=-20,in=25]  (w7);    
		\draw[color=ForestGreen] (z0) to [out=-70,in=170]  (3,-2) to [out=-10, in=200]  (15,-1.5)  to [out=20,in=-25]  (t7);    		
		
	\end{tikzpicture} 
	\caption{$\bcl_5 \cong \ig{C_{16}}$.}
	\label{fig:i:iC16}	
\end{figure}
% <<< E: Figure {fig:i:iC16}


% +++++++++++++++++++++++++++  OBSERVATIONS  +++++++++++++++++





%>>> S: Lemma {lem:i:bcl}
\begin{lemma} \label{lem:i:bcl}
	For $k \geq 1$,		
	%	\begin{align*}
		$	\ig{C_{3k+1}} \cong 	\bcl_{k}$.
		%	\end{align*}
\end{lemma}
% <<< E: Lemma {lem:i:bcl}


To prove Lemma \ref{lem:i:bcl}, we first establish several lemmas, beginning with a formulation of the observation from page \pageref{sec:i:cycles}, for the case $n=3k+1$.  Going forward, we assume that all arithmetic in the $i$-set notation is performed modulo $3k+1$.


%>>> S: OBS {obs:i:2ver}
\begin{obs} \label{obs:i:2ver}
	Each $i$-set $X$ of $C_{3k+1}$ contains exactly two pairs of vertices, say $v_{j-1},v_{j+1}$ and $v_{\ell-1},v_{\ell+1}$,
	such that each pair has a common neighbour in $C_{3k+1}-X$; all other pairs of consecutive
	vertices of $X$ on $C_{3k+1}$ are separated by two vertices of $C_{3k+1}-X$. 
\end{obs}
% <<< E: OBS {obs:i:2ver}


%\nts{notation splits here - vertex in $C_n$ is $v_1,v_2,...$, with represented by ``short gap" $i$-set at, say $v_4$ and $v_6$ to be $\cid{4,6}$. - vertex is $v_k$ not $k$.}


%>>> S: Lemma {lem:i:Fdegree}
\begin{lemma} \label{lem:i:Fdegree}
	Each vertex of $\ig{C_{3k+1}}$ has degree 2 or 4.  
\end{lemma}


\begin{proof}
	For each $i$-set $X$ of $C_{3k+1}$, we  deduce from Observation \ref{obs:i:2ver} that $X$ is one of two types (with notation as in Observation \ref{obs:i:2ver}):
	
	\begin{enumerate}[label=]
		\item \textbf{Type 1:}\ $\{v_{j-1},v_{j+1}\}\cap\{v_{\ell-1},v_{\ell+1}\}\neq\varnothing$; in this case
		$|\{v_{j-1},v_{j+1}\}\cap\{v_{\ell-1},v_{\ell+1}\}|=1$. Say ${j+1}={\ell-1}$. In our wide-angled notation, Type 1
		$i$-sets are of the form $X=\left\langle j,j+2 \right\rangle$. %\ (\operatorname{mod}%
		%\ 3k+1)\right\rangle $. 
		%If $v_{j-1},v_{j+1},v_{\ell+1}$ occur in this order in a clockwise
		%direction on $C_{3k+1}$, 
		Then the subpath $(v_{j-1},v_j,v_{j+1},v_{j+2},v_{j+3})$  of $C_{3k+1}$ has tokens on $v_{j-1}, v_{j+1},$ and $v_{j+3}$. A
		token on $v_{j-1}$ can only slide counterclockwise to $v_{j-2}$, a token on $v_{j+3}$ can only slide clockwise to $v_{j+4}$, and a token on $v_{j+1}$ is frozen. Hence $X$ has degree $2$ in $\ig{C_{3k+1}}$ (all other tokens are frozen).
		
		\item \textbf{Type 2:}\ $\{v_{j-1},v_{j+1}\}\cap\{v_{\ell-1},v_{\ell+1}\}=\varnothing$. When $X$ is a Type 2
		$i$-set, and $v_{j-1},v_{j+1},v_{\ell-1},$ and $v_{\ell+1}$ occur in this order in a clockwise direction on
		$C_{3k+1}$, then each of $v_{j-1}$ and $v_{\ell-1}$ is immediately preceded
		(counterclockwise) by two vertices of $C_{3k+1}-X$, and each of $v_{j+1}$ and $v_{\ell+1}$ is
		immediately followed (clockwise) by two vertices of $C_{3k+1}-X$. Hence tokens
		on $v_{j-1}$ and $v_{\ell-1}$ can slide counterclockwise to $v_{j-2}$
		and $v_{\ell-1}$, respectively, while tokens on $v_{j+1}$ and
		$v_{\ell+1}$ can slide clockwise to $v_{j+2}$ and
		$v_{\ell+2}$, respectively. Hence $X$ has degree $4$ in
		$\ig{C_{3k+1}}$.
	\end{enumerate}
\end{proof}

% <<< E: Lemma {lem:i:Fdegree}



The following is straightforward from the above proof, but we include a proof here for completeness.

\newpage

%>>> S: Lemma {lem:i:bkNeigh}
\begin{lemma} \label{lem:i:bkNeigh}   
	
	Let $X$ be an $i$-set of $C_{3k+1}$.	
	\begin{enumerate}[label=(\roman*)]
		\item  \label{lem:i:bkNeigh:i}    If $X=\left\langle j,j+2\right\rangle $ for some $j\in
		\{0,...,3k\}$, then the neighbours of $X$ in $\ig{C_{3k+1}}$ are
		$\left\langle j,j+5\right\rangle $ and $\left\langle j-3,j+2\right\rangle $. 
		
		\item \label{lem:i:bkNeigh:ii}  If $X=\left\langle j,\ell\right\rangle $ for some $j\in
		\{0,...,3k\}$ and some $\ell$, where $j-\ell\not \equiv 2$ or
		$-2\ (\operatorname{mod}\ 3k+1)$, then $\ell=j+2+3s$, where $s\in
		\{1,...,k-2\}$. The neighbours of $X$ in $\ig{C_{3k+1}}$ are
		$\left\langle j,\ell+3\right\rangle ,\left\langle j,\ell-3\right\rangle
		,\left\langle j+3,\ell\right\rangle ,$ and $\left\langle j-3,\ell\right\rangle
		$.
	\end{enumerate}
\end{lemma}


\begin{proof} We prove the statement for $j=0$; the general
	cases follow by symmetry.	
	\begin{enumerate} [label=(\roman*)]
		\item Consider the $i$-set $X=\left\langle
		0,2\right\rangle $. Then $X$ is a Type 1  $i$-set (see Lemma \ref{lem:i:Fdegree}) of $C_{3k+1}$. Then
		$\{v_{-1},v_1,v_3\}\subseteq X$. By Lemma \ref{lem:i:Fdegree}, the token on $v_1$ is frozen, the token on $v_{-1}$ can slide to $v_{-2}$,
		creating the $i$-set $\left\langle -3,2\right\rangle $, and the token on $v_3$
		can slide to $v_4$, creating the $i$-set $\left\langle 0,5\right\rangle$.
		
		\item Consider the $i$-set $X=\left\langle
		0,\ell\right\rangle $, where $\ell\not \equiv 2$ or $-2\ (\operatorname{mod}%
		\ 3k+1)$. Then $X$ is a Type 2 $i$-set of $C_{3k+1}$, and there are tokens on
		$v_{-1},v_1,v_{\ell-1}$, and $v_{\ell+1}$. Moreover, since $v_{0}$ and $v_{\ell}$ are the only
		vertices that have two neighbours in $X$, the other vertices, in a clockwise
		direction from $v_{1}$, contained in $X$ are $v_{4},v_{7},...,v_{\ell-1}$, which shows that
		$\ell=3s+2$ for some $s\geq1$. Since $X$ is a Type 2 $i$-set, $\ell\neq3k-1$,
		that is, $s\neq k-1$. Hence $\ell=3s+2$, where $s\in\{1,...,k-2\}$.
		
		Similarly to the above, the token on $v_{-1}$ can slide to $v_{-2}$,
		forming the $i$-set $\left\langle -3,\ell\right\rangle $, the token on $v_{1}$ can
		slide to $v_{2}$, forming the $i$-set $\left\langle 3,\ell\right\rangle $, the
		token on $v_{\ell-1}$ can slide to $v_{\ell-2}$, forming the $i$-set $\left\langle
		0,\ell-3\right\rangle $, and the token on $v_{\ell+1}$ can slide to $v_{\ell+2}$,
		forming the $i$-set $\left\langle 0,\ell+3\right\rangle $. 		
	\end{enumerate}	
\end{proof}


% <<< E: Lemma {lem:i:bkNeigh}


This completes the proof of Lemma \ref{lem:i:bcl}.  Finally, combining Lemma \ref{lem:i:2Cn} and Lemma \ref{lem:i:bcl} reveals the full result for $i$-graphs of cycles.




%\emph{Now you can say something about a 1-1 correspondence between the
	%	vertices of }$\mathfrak{B}_{k}$ \emph{and the }$i$\emph{-sets in }$C_{3k+1}%
%$,\emph{ and that the neighbours of each i-set correspond to the neighbours of
	%	the corresponding vertex of }$\mathfrak{B}_{k}$\emph{. This proves that
	%}$\mathcal{I}(C_{3k+1})\cong\mathfrak{B}_{k}$.

% <<< E: Lemma {lem:i:bkNeigh}


\begin{comment}
	
	%>>> S: Lemma {lem:i:Fcon}
	\begin{lemma} \label{lem:i:Fcon}
		$\ig{C_{3k+1}}$  is connected.
	\end{lemma}
	% <<< E:Lemma {lem:i:Fcon}
	
	
	\nts{This is still all wrong.}
	
	%\textbf{Claim:}  
	If $\cid{a,b}$ and $\cid{a,c}$ are $i$-sets of $C_{3k+1}$, then $\cid{a,b}$ and $\cid{a,c}$ are in the same component of $\ig{C_{3k+1}}$.  That is, the $i$-set corresponding to the labelling $\cid{a,b}$ can be transformed into the $i$-set corresponding to $\cid{a,c}$ through a series of token slides.
	
	
	
	If $\cid{a,b}$ is an $i$-set, then $a-b \equiv 2 \Mod{3}$ and $b = a + 2 + 3n \Mod{3k +1}$.
	
	
	We  claim that if there is $a'$ and $b'$ such that $\cid{a,a'}$ and $\cid{b,b'}$ are $i$-sets, then $a'\neq b'$.  
	Notice $a'=b+3j \Mod{3k+1}$ and $b'=a+3\ell \Mod{3k+1}$
	
	Suppose not.  Then, 
	
	\begin{align*}
		a'&=b'\\
		b+3j &= a+3\ell \\
		b-a &= 3\ell -3j
	\end{align*}
	
	Then, $b-a \equiv 2 \Mod{3}$ but $3\ell-3j \equiv 0 \Mod{3}$.  
	
\end{comment}




%Bringing Lemmas \ref{lem:i:2Cn} and \ref{lem:i:bcl} together yields the following.

%>>> S: Theorem {thm:i:Cn}
\begin{theorem} \label{thm:i:Cn}
	For $n \geq 3$, $k \geq 0$,		
	\begin{align*}
		\ig{C_n} = 	
		\begin{cases}
			K_3 & \text{ if } n=3 \\
			3K_1 & \text{ if } n=3k \geq 6 \\
			\bcl_{k} & \text{ if } n = 3k+1\\
			C_n & \text{ if } n \equiv 2 \Mod{3}.
		\end{cases}
	\end{align*}
\end{theorem}
% <<< E:Theorem {thm:i:Cn}



%---------------------------------------SECTION: $i$-graphs of cycles ----------------
\section{Hamiltonicity of $\ig{C_n}$}	\label{sec:i:hamCycle}

In some of the figures presented in Section \ref{sec:i:cycles}, a Hamiltonian cycle or path is easily found; in others, it is not.  This leads to the problem of determining for which values of  $n$ $\ig{C_n}$ is Hamiltonian or Hamilton traceable (i.e. has a Hamiltonian path).  In most cases, this is not too difficult to determine, as we show next.  

%>>> S: Theorem {thm:i:Ham}
\begin{theorem} \label{thm:i:Ham}  For $n\geq 3$,
	\begin{enumerate}[label=$\bullet$]
		\item If $n \equiv 0 \Mod{3}$, $\ig{C_n}$ is disconnected.
		\item If $n \equiv 2 \Mod{3}$, $\ig{C_n}$ is trivially Hamiltonian.
		\item If $n  \equiv 4 \Mod{6}$, $\ig{C_n}$ is neither Hamiltonian nor Hamilton traceable.
	\end{enumerate}
\end{theorem}
% <<< E: Theorem {thm:i:Ham}


\begin{proof}	
	The first two cases are trivial, and so assume that $n \equiv 4 \Mod{6}$. Since $\ig{C_4} = \overline{K_2}$, it is non-Hamiltonian;
	hence, assume $n >4$, say $n = 6k+4$, $k \geq 1$.   With notation as above, we first count the
	number of vertices $\cid{j, \ell}$ of $\ig{C_n}$ such that $j \equiv \ell \Mod{2}$.  For $j=0$, the set of these
	vertices is
	\begin{align*}
		\mathscr{X}_0 = \{\cid{0,2}, \cid{0,8}, \dots, \cid{0,6k+2}\}
	\end{align*}	
	and $| \mathscr{X}_0| = k+1$.   Similarly, 	
	\begin{align*}
		\mathscr{X}_j = \{\cid{j,j+2}, \cid{j,j+8}, \dots, \cid{j,j+6k+2}\}
	\end{align*}	
	and
	\begin{align*}
		\sum^{6k+3}_{j=0} |\mathscr{X}_j| = (k+1)(6k+4).
	\end{align*}	
	But each vertex $\cid{j,\ell}, j \equiv \ell \Mod{2}$  occurs in exactly two sets, namely $\mathscr{X}_j$ and $\mathscr{X_{\ell}}$.	
	Hence,
	\begin{align*}
		\left| \bigcup_{j=0}^{6k+3} \mathscr{X}_j \right| = (k+1)(3k+2).
	\end{align*}
	
	\noindent Since 
	\begin{align*}
		V(\ig{C_n}) = \frac{n(n-1)}{6} = (3k+2)(2k+1),
	\end{align*}
	$\ig{C_n}$ has $k(3k+2)$ vertices $\cid{j,\ell}$ such that $j \not\equiv \ell \Mod{2}$.  
	%To show that $\ig{C_n}$ is non-Hamiltonian, we need the following result.
	
	
	
	%>>> S: Theorem {thm:i:HamComp}
	%\begin{theorem} \label{thm:i:HamComp} \cite{CLZ}   If $G$ is a Hamiltonian graph, then for every nonempty proper
	%	subset $S$ of $V(G)$, the number of components of $G-S$ does not exceed $|S|$
	%\end{theorem}
	% <<< E: Theorem {thm:i:HamComp}
	
	
	
	%>>> S: Theorem {thm:i:C6k4Ham}
	%\begin{theorem} \label{thm:i:C6k4Ham} For $n=6k+4$, $\ig{C_n}$ is neither Hamiltonian nor Hamilton traceable.
	%\end{theorem}
	% <<< E: Theorem {thm:i:C6k4Ham}
	
	
	
	%>>> S: Proof of Theorem {thm:i:Ham}
	%\begin{proof}
	We show next that each vertex $\cid{j,\ell}$ such that $j \equiv \ell \Mod{2}$ is adjacent only to vertices $\cid{j',\ell'}$ such that $j' \not\equiv \ell' \Mod{2}$, and vice versa.  
	
	
	Let $\cid{j,\ell}$ be any vertex of $\ig{C_n}$ such that $j \equiv \ell \Mod{2}$.  Then, with arithmetic in
	the subscripts performed modulo $n$, 
	\begin{align*}
		N(\cid{j,\ell}) = \begin{cases}
			\{  \cid{j, \ell+3},  \cid{j, \ell-3},  \cid{j+3, \ell},  \cid{j-3, \ell}  \} & \text{ if } \ell -j \not\equiv \pm 2 \Mod{n} \\
			\{  \cid{j, \ell+3},   \cid{j-3, \ell}  \} & \text{ if } \ell -j \equiv  2 \Mod{n} \\
			\{    \cid{j, \ell-3},  \cid{j+3, \ell} \} & \text{ if } \ell -j \equiv -2 \Mod{n}, \\			
		\end{cases}
	\end{align*}
	
	
	
	\noindent	where, since $n$  is even, $j \not\equiv \ell \pm 3  \Mod{2}$ and  $\ell \not\equiv j \pm 3 \Mod{2}$. Hence each vertex $\cid{j,\ell}$ of
	$\ig{C_n}$ such that $j \equiv \ell \Mod{2}$  is adjacent only to vertices  $\cid{j',\ell'}$ such that $j' \not\equiv \ell' \Mod{2}$.  
	
	
	Therefore, $\ig{C_n}$ is bipartite with $(k+1)(3k+2)$ vertices in one partite set, and $k(3k+2)$ in the other.   Since the cardinalities of the partite sets differ by more than one, the result follows.  
\end{proof}

%	Let $S= \{\cid{j,\ell} : j \not\equiv \ell \Mod{2} \}$.  Then $|S| = k(3k+2)$ and $G-S$ consists of the $(k+1)(3k+2)$ isolated vertices $\cid{j,\ell}$, $j \equiv \ell \Mod{2}$.  By (the contrapositive of) Theorem \ref{thm:i:HamComp}, $\ig{C_n}$ is non-Hamiltonian.  
%\end{proof}


The case for $n \equiv 1 \Mod{6}$ is more complicated.   From Figures \ref{fig:i:iC7} and \ref{fig:i:iC13} given above, $\ig{C_7}$ and $\ig{C_{13}}$ are Hamiltonian:  $\ig{C_7}$ trivially so,  and for  $\ig{C_{13}}$, illustrated in red.    For $n \equiv 1 \Mod{6}$ with $n \geq 19$, we claim that $\ig{C_n}$ is not Hamiltonian.  Consider $\ig{C_{19}}$ given in Figure \ref{fig:i:iC19} below.   Any Hamiltonian cycle on $\ig{C_{19}}$ would include all of the vertices of degree 2 and their  degree 4 neighbours, as highlighted in red in Figure \ref{fig:i:iC19}.  However, this (proper) subset of vertices induces a cycle in $\ig{C_{19}}$, and so $\ig{C_{19}}$ is not Hamiltonian.  A similar argument follows for larger $n$  with $n \equiv 1 \Mod{6}$, as we show next.

% <<< E:  Proof of Theorem {thm:i:Ham}

%>>> S: Figure {fig:i:iC19}	
\begin{figure}[H] \centering	 	 
	\begin{tikzpicture}[scale=0.88]			
		%---------- REF-------------------
		%	\coordinate (cent) at (0,0) {};			
		
		%----- TOP LINE - V
		\foreach \c / \i / \j in {
			0/	0	/	2	,
			1/	3	/	5	,
			2/	6	/	8	,
			3/	9	/	11	,
			4/	12	/	14	,
			5/	15	/	17	,
			6/	18	/	1	,
			7/	2	/	4	,
			8/	5	/	7	,
			9/	8	/	10	,
			10/	11	/	13	,
			11/	14	/	16	
		}
		{
			\node[std,label={0: \scriptsize ${\i,\j}$}] (v\c) at (1.5*\c, 5) {}; 					
		}				
		
		%----- MID 1  - W
		\foreach \c / \i / \j in {
			0/	0	/	5	,
			1/	3	/	8	,
			2/	6	/	11	,
			3/	9	/	14	,
			4/	12	/	17	,
			5/	15	/	1	,
			6/	18	/	4	,
			7/	2	/	7	,
			8/	5	/	10	,
			9/	8	/	13	,
			10/	11	/	16										
		}
		{
			\node[std,label={0: \scriptsize ${\i,\j}$}] (w\c) at (0.75+1.5*\c, 4) {}; 					
		}			
		
		%----- MID 2 - T
		\foreach \c / \i / \j in {
			0/	0	/	8	,
			1/	3	/	11	,
			2/	6	/	14	,
			3/	9	/	17	,
			4/	12	/	1	,
			5/	15	/	4	,
			6/	18	/	7	,
			7/	2	/	10	,
			8/	5	/	13	,
			9/	8	/	16							
		}
		{
			\node[std,label={0: \scriptsize ${\i,\j}$}] (t\c) at (1.5+1.5*\c, 3) {}; 					
		}	
		
		
		%----- MID 3 - Y
		\foreach \c / \i / \j in {
			0/	0	/	11	,
			1/	3	/	14	,
			2/	6	/	17	,
			3/	9	/	1	,
			4/	12	/	4	,
			5/	15	/	7	,
			6/	18	/	10	,
			7/	2	/	13	,
			8/	5	/	16			
		}
		{
			\node[std,label={0: \scriptsize ${\i,\j}$}] (y\c) at (2.25+1.5*\c, 2) {}; 					
		}
		
		
		%----- MID 4 - X
		\foreach \c / \i / \j in {
			0/	0	/	14	,
			1/	3	/	17	,
			2/	6	/	1	,
			3/	9	/	4	,
			4/	12	/	7	,
			5/	15	/	10	,
			6/	18	/	13	,
			7/	2	/	16			
		}
		{
			\node[std,label={0: \scriptsize ${\i,\j}$}] (x\c) at (3+1.5*\c, 1) {}; 					
		}		
		
		
		%----- BOTTOM LINE - Z
		\foreach \c / \i / \j in {
			0/	0	/	17	,
			1/	3	/	1	,
			2/	6	/	4	,
			3/	9	/	7	,
			4/	12	/	10	,
			5/	15	/	13	,
			6/	18	/	16							
		}
		{
			\node[std,label={0: \scriptsize ${\i,\j}$}] (z\c) at (3.75+1.5*\c, 0) {}; 		
		}			
		
		%----- EDGES
		
		\foreach \c in {0,1,2,3,4,5,6}
		{\draw	(v\c)--(w\c)--(t\c)--(y\c)--(x\c)--(z\c);
		}
		
		\draw (v7)--(w7)--(t7)--(y7)--(x7);
		\draw (v8)--(w8)--(t8)--(y8);
		\draw (v9)--(w9)--(t9);
		\draw (v10)--(w10);
		
		\draw (v11)--(w10)--(t9)--(y8)--(x7)--(z6);
		\draw (v10)--(w9)--(t8)--(y7)--(x6)--(z5);
		\draw (v9)--(w8)--(t7)--(y6)--(x5)--(z4);
		\draw (v8)--(w7)--(t6)--(y5)--(x4)--(z3);
		\draw (v7)--(w6)--(t5)--(y4)--(x3)--(z2);	
		\draw (v6)--(w5)--(t4)--(y3)--(x2)--(z1);
		\draw (v5)--(w4)--(t3)--(y2)--(x1)--(z0);
		\draw (v4)--(w3)--(t2)--(y1)--(x0);
		\draw (v3)--(w2)--(t1)--(y0);
		\draw (v2)--(w1)--(t0);
		\draw (v1)--(w0);
		
		%	\draw	(v2)--(w2)--(z2);
		%	\draw	(v3)--(w3)--(z3);
		%	\draw	(v4)--(w4)--(z4);
		
		%	\draw	(v1)--(w0)--(z1);
		%	\draw	(v2)--(w1)--(z2);
		%	\draw	(v3)--(w2)--(z3);
		%	\draw	(v4)--(w3)--(z4);
		
		
		
		% --- RED CYCLE EDGES 
		\draw[very thick,red] (v0) to [out=250,in=160]  (3,-1) to [out=0, in=180]  (13.5,-1)  to [out=10,in=-35]  (x7);    		
		
		\draw[very thick,red]  (v11) to [out=300,in=20]  (13.5,-2.5) to [out=180, in=0]  (4.5,-2.5)  to [out=170,in=215]  (x0);    
		
		\foreach \i / \j in {0/1,1/2,2/3,3/4,4/5,5/6,6/7,7/8,8/9,9/10,10/11}
		{
			\draw[very thick,red] (w\i)--(v\j);
			\draw[very thick,red] (v\i)--(w\i);
		}
		
		
		\foreach \i / \j in {0/1,1/2,2/3,3/4,4/5,5/6,6/7}
		{
			\draw[very thick,red] (z\i)--(x\j);
			\draw[very thick,red] (z\i)--(x\i);
		}
		
		
		%--- secondary curved edges
		\draw[thick,blue]  (t0) to [out=250,in=160]  (3,-1.5) to [out=0, in=180]  (13.5,-1.5)  to [out=10,in=-35]  (t9); 
		\draw (w0) to [out=250,in=160]  (3,-1.7) to [out=0, in=180]  (13.5,-1.7)  to [out=10,in=-35]  (y8); 
		\draw (y0) to [out=250,in=160]  (3,-1.9) to [out=0, in=180]  (13.5,-1.9)  to [out=10,in=-35]  (w10);   
		
		%---- PURPLE FOR HPATH
		\foreach \i / \j in {0/1,1/2,2/3,3/4,4/5,5/6,6/7,7/8,8/9}
		{
			\draw[thick,blue] (y\i)--(t\j);
			\draw[thick,blue] (y\i)--(t\i);
		}			
		%	\draw[color=red] (r0) to [out=70,in=190]  (3,6) to [out=10, in=160]  (15,5.5)  to [out=-20,in=25]  (w7);    
		%	\draw[color=red] (z0) to [out=-70,in=170]  (3,-2) to [out=-10, in=200]  (15,-1.5)  to [out=20,in=-25]  (t7);    		
		
		%	\draw[ultra thick,green, dashed] (x7)--(y8);
		
	\end{tikzpicture} 
	\caption{$\ig{C_{19}}$.}
	\label{fig:i:iC19}		 
\end{figure}
% <<< E: Figure {fig:i:iC19}


%As a consolation, although not Hamiltonian, $\ig{C_{19}}$ does contain a Hamilton path.  In Figure \ref{fig:i:iC19}, start at the vertex for $\cid{0,2}$ and move along the red path at the top of the graph through $\cid{3,5}$, $\cid{3,8} \dots  \cid{14,16}$.  Then, take the red edge down to the bottom left of the graph to 
%$\cid{0,14}$ and follow the red path along the bottom of the graph through $\cid{0,17}$, $\cid{3,17}$, \dots, $\cid{2,16}$.  From there,  take the green edge up to $\cid{5,16}$, and follow the blue path through $\cid{ 8,16}$, and then around the long blue edge to the left side of the graph to $\cid{0,8}$, through the blue path and finally ending at $\cid{5,13}$.
%We claim that for all  $n \equiv 1 \Mod{6}$, $\ig{C_{n}}$ contains a Hamilton path, constructed similarly to the path in Figure \ref{fig:i:iC19}: traversing first the outer alternating degree 2 (red) pathway and then moving through the inner (blue) cycles one level at a time.  

%>>> S: Figure {thm:i:1m6nonHam}
\begin{theorem} \label{thm:i:1m6nonHam}
	If $n\geq 19$ and $n \equiv 1 \Mod{6}$, then $\ig{C_n}$ is not Hamiltonian.
\end{theorem}
% <<< E: Figure {thm:i:1m6nonHam}

%We know what happens if $k\leq3$, so assume $k\geq4$.\bigskip

\begin{proof}
	As shown in Lemma \ref{lem:i:bkNeigh} \ref{lem:i:bkNeigh:i}, the neighbours of the $i$-set
	$X=\cid{0,2}$ in $\ig{C_{6k+1}}$ are
	$\cid{-3,2}$ and $\cid{ 0,5}$. On the
	other hand, the neighbours of $\cid{0,5}$ are
	$\cid{0,2}$, $\cid{0,8}$,
	$\cid{ 3,5}$ and $\cid{-3,5}$. Note
	that $\cid{0,2}$ and $\cid{3,5}$ are
	Type 1 vertices while $\cid{0,8}$ and $\cid{
		-3,5}$ are Type 2. Similarly, $\cid{-3,2}$
	has Type 1 neighbours $\cid{0,2}$ and $\cid{
		-3,-1}$, and Type 2 neighbours $\cid{ -3,5}$
	and $\cid{-6,2}$. A similar remark holds for any $i$-set
	$\cid{j,j+5},\ j\in\{0,...,3k\}$. We call these $i$-sets
	\emph{Type 2a} $i$-sets.
	
	Consider the $i$-set $X=\left\langle 0,2+3s\right\rangle $, where
	$s\in\{2,...,2k-3\}$ (hence $k\geq 3$). As proved in Lemma  \ref{lem:i:bkNeigh} \ref{lem:i:bkNeigh:ii}, the neighbours of $X$ in $\ig{C_{6k+1}}$ are the Type 2
	$i$-sets
	\[
	\cid{ 0,2+3(s+1)},\cid{ 0,2+3(s-1)}
	,\cid{ 3,2+3s},\cid{ -3,2+3s}.
	\]
	Observe that for the given range of $s$, these are all Type 2 $i$-sets. A
	similar remark holds for any $i$-set $\cid{ j,j+2+3s}$,
	where $s\in\{2,...,k-3\}$. We call these $i$-sets \emph{Type 2b} $i$-sets.
	
	Therefore there are exactly $6k+1$ Type 1 $i$-sets of $C_{6k+1}$ and the same
	number of Type 2a $i$-sets, and each Type 1 $i$-set has exactly two neighbours
	in $\ig{C_{6k+1}}$, both of which are Type 2a $i$-sets, and,
	conversely, each Type 2a $i$-set has two Type 1 neighbours in $\ig{C_{6k+1}}$. We deduce that the subgraph of $\ig{C_{6k+1}}$ induced by
	its Type 1 vertices and their neighbours consists of only Type 1 and Type 2a
	vertices, and is $2$-regular. Hence if $\ig{C_{6k+1}}$ has Type 2b
	vertices, that is, if $k\ge3$, then $\ig{C_{6k+1}}$ is
	non-Hamiltonian. 
	%This leaves only the case where $k=4$, and a Hamiltonian
	%cycle of $\ig{C_{13}}$ is depicted in Figure \ref{fig:i:C13}.
\end{proof}



%--------------------


%--------------------
\subsection*{Traceability of $\ig{C_{6k+1}}$, where $k\geq3$.}  \label{subsec:i:C3k1Trac}

When $k\geq 3$ and $n=6k+1$, we have previously established that $\ig{C_{n}}$ has no Hamiltonian cycle.  We now instead prove that it has a Hamilton path.


%>>> S: E: Theorem {thm:i:C6r1}
\begin{theorem} \label{thm:i:C6r1}
	For $n=6k+1$, $k \geq 3$, $\ig{C_n}$ is Hamilton traceable.
\end{theorem}


\begin{proof}	
	Say $k\geq3$, and consider $C_{6k+1}$ and an $i$-set $\cid{j,\ell} $. The distance from $j$ to $\ell$ on $C_{6k+1}$ is the length of the shorter path, thus $d(j,\ell)\in
	\{2,5,8, \dots ,3k-1\}$.
	
	\begin{enumerate}[label=$\bullet$]
		\item If $k$ is even, say $k=2k^{\prime}$, then, in $C_{12k^{\prime}+1}$, we
		see that $d(j,\ell)\in\{2,5,8, \dots ,6k^{\prime}-1\}$. This set contains an equal
		number of even and odd integers.
		
		\item If $k$ is odd, say $k=2k^{\prime}+1$, then, in $C_{12k^{\prime}+7}$, we
		see that $d(j,\ell)\in\{2,5,8, \dots ,6k^{\prime}+2\}$. This set contains more even
		than odd integers.
	\end{enumerate}
	
	Consider, again, the subgraph of $\ig{C_{6k+1}}$ induced by its Type 1
	vertices and their neighbours, which is $2$-regular (as above) and has order
	$2(6k+1)$. Denote this graph by $\mathcal{H}_{2,5}$. 
	In Figure \ref{fig:i:iC19}, $\mathcal{H}_{2,5}$ is the subgraph induced by the vertices: 
	\begin{align*} \{\cid{0,2}, \cid{0,5}, \cid{3,5}, \cid{3,8}, \cid{6,8} \dots, \cid{2,16} \}. 
	\end{align*}
	
	\noindent We argue below that
	$\mathcal{H}_{2,5}$ is in fact connected; that is, $\mathcal{H}_{2,5}$ is a cycle.
	
	%\bigskip
	
	Note that, with arithmetic modulo $6k+1$,
	\begin{align*}
		\mathcal{W}_{2,5}  = 
		&\cid{ 0,2}, \cid{0,2+3}, \cid{3,2+3}, \cid{3,2+2\cdot3}, \cid{ 2\cdot3,2+2\cdot3},  \\
		& \dots, \cid{3x,2+3x}, \cid{3x, 2+3(x+1)} \dots
	\end{align*}	
	\noindent is a walk in $\mathcal{H}_{2,5}$. When does $\cid{ 0,2} $
	recur? There are two cases to consider, each having two subcases.
	
	%\bigskip
	
	\noindent\textbf{Case 1}:\textbf{\hspace{0.1in}}When $\cid{
		0,2} $ recurs for the first time, an even cycle is formed. Then
	$\cid{ 0,2} =\cid{ 3x,2+3x} $ for some
	integer $x$. Since $\cid{ 0,2} =\cid{
		2,0} $, there are two subcases.\smallskip
	
	\noindent\textbf{Case 1.1}:\hspace{0.1in}$3x\equiv2\ (\operatorname{mod}%
	\ 6k+1)$ and $2+3x\equiv0\ (\operatorname{mod}\ 6k+1)$, that is,
	$3x\equiv-2\ (\operatorname{mod}\ 6k+1)$. But then $2\equiv
	-2\ (\operatorname{mod}\ 6k+1)$, which is impossible because $k>0$.\smallskip
	
	\noindent\textbf{Case 1.2}:\hspace{0.1in}$3x\equiv0\ (\operatorname{mod}%
	\ 6k+1)$ and $2+3x\equiv2\ (\operatorname{mod}\ 6k+1)$. Since $\gcd
	(3,6k+1)=1$, $x\equiv0\ (\operatorname{mod}\ 6k+1)$. Then the first time
	$\cid{ 0,2} $ recurs on $\mathcal{W}_{2,5}$ is therefore
	when $x=6k+1$. It follows that $\mathcal{W}_{2,5}$ contains the cycle
	\begin{align*}
		\cid{0,2}, \cid{0,2+3}, \cid{3,2+3}, \cid{3, 2+2 \cdot 3}, \cid{2\cdot3,2+2\cdot3}, \dots, \cid{0,2}
	\end{align*}	
	of length $2(6k+1)=|V(\mathcal{H}_{2,5})|$. Therefore $\mathcal{H}_{2,5}\cong
	C_{12k+2}$.
	
	%	\bigskip
	
	\noindent\textbf{Case 2}:\textbf{\hspace{0.1in}}When $\cid{
		0,2} $ recurs for the first time, an odd cycle is formed. Then
	$\cid{ 0,2} =\cid{ 3x,2+3(x+1)} $ for
	some integer $x$. Again there are two subcases.\smallskip
	
	\noindent\textbf{Case 2.1}:\textbf{\hspace{0.1in}}$3x\equiv
	2\ (\operatorname{mod}\ 6k+1)$ and $2+3(x+1)\equiv0\ (\operatorname{mod}%
	\ 6k+1)$. Then $7\equiv0\ (\operatorname{mod}\ 6k+1)$, which is impossible
	because $k>1$.\smallskip
	
	\noindent\textbf{Case 2.2}:\textbf{\hspace{0.1in}}$3x\equiv
	0\ (\operatorname{mod}\ 6k+1)$ and $2+3(x+1)\equiv2\ (\operatorname{mod}%
	\ 6k+1)$. This is likewise impossible.
	
	Therefore, we conclude in all cases that $\mathcal{H}_{2,5} \cong C_{12k+2}$.
	
	
	%	\bigskip
	
	In general, for fixed $\ell\equiv2\ (\operatorname{mod}\ 6)$ and $2\leq
	\ell\leq3k-1$, denote the subgraph of $\ig{C_{6k+1}}$ induced by the
	$i$-sets of the form $\cid{ j,j+\ell} $ and $\cid{
		j,j+\ell+3} $, where $j\in\{0,...,6k\}$, by $\mathcal{H}_{\ell,\ell+3}$.
	
	Then	
	\begin{align*} 
		\mathcal{W}_{\ell, \ell+3} & = \cid{0,\ell}, \cid{0,\ell+3}, \cid{3, \ell+3}, \cid{3,\ell+2\cdot3}, \cid{2\cdot3, \ell+2\cdot3}, \\ 
		& \dots, \cid{3x, \ell+3x}, 
		\cid{3x, \ell+3(x+1)} \dots
	\end{align*}	
	is a walk in $\mathcal{H}_{\ell,\ell+3}$. When does $\cid{ 0,\ell} $
	recur? Again there are two cases to consider.
	
	\bigskip
	
	\noindent\textbf{Case 3}:\textbf{\hspace{0.1in}} When $\cid{ 0,\ell} $ recurs for the first time, an
	even cycle is formed. Then $\cid{ 0,\ell} =\cid{
		3x,\ell+3x} $ for some integer $x$. Since $\cid{
		0,\ell} =\cid{ \ell,0} $, there are two
	subcases.\smallskip
	
	\noindent\textbf{Case 3.1}:\textbf{\hspace{0.1in}}$3x\equiv
	\ell\ (\operatorname{mod}\ 6k+1)$ and $\ell+3x\equiv0\ (\operatorname{mod}\ 6k+1)$,
	that is, $3x\equiv-\ell\ (\operatorname{mod}\ 6k+1)$. Then $2\ell\equiv
	0\ (\operatorname{mod}\ 6k+1)$ and, since $\gcd(2,6k+1)=1$, $\ell\equiv
	0\ (\operatorname{mod}\ 6k+1)$. Since $2\leq \ell\leq3k-1$, this is
	impossible.\smallskip
	
	\noindent\textbf{Case 3.2}:\textbf{\hspace{0.1in}}$3x\equiv
	0\ (\operatorname{mod}\ 6k+1)$ and $\ell+3x\equiv \ell\ (\operatorname{mod}\ 6k+1)$,
	i.e., $x\equiv0\ (\operatorname{mod}\ 6k+1)$. Therefore the first time
	$\cid{ 0,\ell} $ recurs on $\mathcal{W}_{\ell,\ell+3}$ is when
	$x=6k+1$. It follows that $\mathcal{W}_{\ell,\ell+3}$ contains the cycle
	\begin{align*}
	\cid{ 0,\ell} ,\cid{ 0,\ell+3} ,\cid{
		3,\ell+3} ,...,\cid{ 3(x-1),\ell+3x} ,\cid{
		0,\ell}
	\end{align*}
	of length $2(6k+1)=|V(\mathcal{H}_{\ell,\ell+3})|$. Therefore $\mathcal{H}%
	_{\ell,\ell+3}\cong C_{12k+2}$.
	
	\bigskip
	
	\noindent\textbf{Case 4}:\textbf{\hspace{0.1in}}When $\cid{
		0,\ell} $ recurs for the first time, an odd cycle is formed. Then
	$\cid{ 0,\ell} =\cid{ 3x,\ell+3(x+1)} $ for
	some integer $x$.\smallskip
	
	\noindent\textbf{Case 4.1}:\textbf{\hspace{0.1in}}$3x\equiv
	\ell\ (\operatorname{mod}\ 6k+1)$ and $\ell+3(x+1)\equiv0\ (\operatorname{mod}%
	\ 6k+1)$. Then $2\ell+3\equiv0\ (\operatorname{mod}\ 6k+1)$, or $2\ell\equiv
	-3\equiv6k-2\ (\operatorname{mod}\ 6k+1)$. This implies that $\ell\equiv
	3k-1\ (\operatorname{mod}\ 6k+1)$ and the restrictions on $\ell$ show that
	$\ell=3k-1$. That is, there is exactly one value of $\ell$ for which these
	congruences hold. Moreover, $6x+3\equiv0\ (\operatorname{mod}\ 6k+1)$, i.e.,
	$2x\equiv-1\equiv6k\ (\operatorname{mod}\ 6k+1)$. Hence $x=3k$. 
	
	Therefore $\mathcal{W}_{\ell,\ell+3}$ contains the cycle%
	\begin{align*}
	\cid{ 0,\ell} ,\cid{ 0,\ell+3} ,\cid{
		3,\ell+3} ,...,\cid{ 3x,\ell+3x} ,\cid{
		\ell,0}
	\end{align*}
	of length $2x+1=6k+1$. Consider the distances $d(0,3k-1)$ and $d(0,3k+2)$ on
	$C_{6k+1}$. Observe that $d(0,\ell)=d(0,3k-1)=3k-1$ and
	$d(0,\ell+3)=d(0,3k+2)=6k+1-(3k+2)=3k-1$. It follows that $\mathcal{H}_{\ell,\ell+3}$
	consists of all $i$-sets $\cid{ p,q} $ such that, on
	$C_{6k+1}$, $d(p,q)=3k-1$, and there are exactly $6k+1$ such $i$-sets. Hence
	$|V(\mathcal{H}_{\ell,\ell+3})|=6k+1$, that is, $\mathcal{H}_{\ell,\ell+3}$ is exactly the
	cycle $\cid{ 0,\ell} ,\cid{ 0,\ell+3}
	,\cid{ 3,\ell+3} ,...,\cid{ 3x,\ell+3x}
	,\cid{ \ell,0} $. 
	
	Since $\ell=3k-1$ and $\ell\equiv2\ (\operatorname{mod}\ 6)$, we deduce that $k$ is
	odd; say $k=2k^{\prime}+1$, where $k^{\prime}\geq1$. Then $\ell=6k^{\prime}+2$.
	The smallest cycle $C_{6k+1}$ where $k\geq3$ for which this case occurs is
	$C_{19}$, in which case $\ell=8$ (see Figure \ref{fig:i:iC19}).
	
	\noindent\textbf{Case 4.2}:\textbf{\hspace{0.1in}}$3x\equiv
	0\ (\operatorname{mod}\ 6k+1)$ and $\ell+3(x+1)\equiv \ell\ (\operatorname{mod}%
	\ 6k+1)$. From the first congruence, $x\equiv0\ (\operatorname{mod}\ 6k+1)$,
	and so, from the second congruence, $3\equiv0\ (\operatorname{mod}\ 6k+1)$.
	This is impossible.
	
	\paragraph*{To summarize:}
	
	Fix $\ell\in\{2,5,8,...,3k-1\}$.  	
	\begin{enumerate}[label=$\bullet$]
		\item If $k=2k^{\prime}$, then by (1) and Cases 3 and 4, the subgraphs
		$\mathcal{H}_{2,5},...,\mathcal{H}_{6k^{\prime}-4,6k^{\prime}-1}$ of
		$\ig{C_{12k^{\prime}+1}}$ all have order $24k^{\prime}+2$, and
		$\mathcal{H}_{2,5}\cong\cdots\cong\mathcal{H}_{6k^{\prime}-4,6k^{\prime}%
			-1}\cong C_{24k^{\prime}+2}$.
		
		\item If $k=2k^{\prime}+1$, then by (2) and Cases 3 and 4, the subgraphs
		$\mathcal{H}_{2,5},...,\mathcal{H}_{6k^{\prime}-4,6k^{\prime}-1}$ of
		$\ig{C_{12k^{\prime}+7}}$ all have order $24k^{\prime}+14$, and
		$\mathcal{H}_{2,5}\cong\cdots\cong\mathcal{H}_{6k^{\prime}-4,6k^{\prime}%
			-1}\cong C_{24k^{\prime}+14}$. However, the subgraph $\mathcal{H}_{6k^{\prime
			}+2,6k^{\prime}+5}$ of $\ig{C_{12k^{\prime}+7}}$ has order
		$12k^{\prime}+7$ and, as for the subgraph $\mathcal{H}_{8,11}$ of
		$\ig{C_{19}}$, is a cycle, that is, $\mathcal{H}_{6k^{\prime
			}+2,6k^{\prime}+5}\cong C_{12k^{\prime}+7}$.
	\end{enumerate}	
	\noindent 	In either case, each vertex of $\ig{C_{6k+1}}$ belongs to $H_{\ell,\ell+3}$
	for some $\ell\equiv2\ (\operatorname{mod}\ 6)$. 
	
	\subsubsection*{Connecting the Subgraphs $\mathcal{H}_{\ell,\ell+3}$ to Form a
		Hamilton Path of $\ig{C_{6k+1}}$}
	
	Denote the subgraph of $\ig{C_{6k+1}}$ that consists of the union of
	the cycles $\mathcal{H}_{\ell,\ell+3}$ by $\mathcal{H}$, and the set of edges of
	$\ig{C_{6k+1}}$ that do not belong to $\mathcal{H}$ by $\mathcal{E}$.
	Since each vertex of $\ig{C_{6k+1}}$ belongs to $H_{\ell,\ell+3}$ for some
	$\ell\equiv2\ (\operatorname{mod}\ 6)$, $\mathcal{H}$ is a spanning subgraph of
	$\ig{C_{6k+1}}$. We consider two cases, depending on whether $k$ is
	even or odd.  
	
		
	\noindent\textbf{Case 1:\hspace{0.1in}}$k=2k^{\prime}$. Then
	\begin{align*}
	\mathcal{P}:\cid{ 0,2} ,\cid{ 0,5}
	,\cid{ 0,8} ,...,\cid{ 0,6k^{\prime}-4}
	,\cid{ 0,6k^{\prime}-1}
	\end{align*}
	is a path in $\ig{C_{12k^{\prime}+1}}$ whose edges belong alternately
	to $\mathcal{H}$ and to $\mathcal{E}$, beginning with the edge $(\cid{
		0,2} ,\cid{ 0,5} )$ in $\mathcal{H}_{2,5}$ and
	ending with the edge $(\cid{ 0,6k^{\prime}-4} ,\cid{
		0,6k^{\prime}-1} )$ in $\mathcal{H}_{6k^{\prime}-4,6k^{\prime}-1}%
	$. Moreover, $\mathcal{P}$ contains at least one vertex of each $\mathcal{H}%
	_{\ell,\ell+3}$. Let $\mathcal{T}$ be the subgraph of $\ig{C_{12k^{\prime
			}+1}}$ obtained by deleting all edges of $\mathcal{P}$ from $\mathcal{H}$,
	then adding the edges of $E(\mathcal{P})\cap\mathcal{E}$. Observe that
	$\mathcal{T}$ is a spanning subgraph of $\ig{C_{12k^{\prime}+1}}$.
	Since the edges of $\mathcal{P}$ were alternately deleted and added, all
	vertices of $\mathcal{T}$ have degree $2$, except for $\cid{
		0,2} $ and $\cid{ 0,6k^{\prime}-1} $, which
	have degree $1$. Also, by construction, $\mathcal{T}$ is connected. Therefore,
	$\mathcal{T}$ is a Hamiltonian path of $\ig{C_{12k^{\prime}+1}}$.
	
	
	
	\noindent\textbf{Case 2:\hspace{0.1in}}$k=2k^{\prime}+1$. The argument is similar.
	
	
	Therefore, in all cases $\ig{C_{6k+1}}, k\geq 3$ is Hamilton traceable.
\end{proof}

This completes the characterization of which cycles have Hamiltonian or Hamiltonian
traceable $i$-graphs.



==> SlaterM.tex <==
%\documentclass[12pt]{article}%

%\input{LTthesisCmd.tex}

%=================================START DOCUMENT ======================
%\begin{document}


\chapter{Variations on the $\gamma$-Graph}






\label{ch:slater}

The following chapter is taken from \cite{MT18}, except for  Section \ref{sec:s:roman}, which contains new results regarding Roman and total-Roman dominating graphs.  




%>>>S Theorem {thm:sl:gammaGraph}
\begin{theorem}
	\label{thm:sl:gammaGraph} \emph{\cite{CHH10}}  For any graph $H$, there
	exists some graph $G$ such that $G(\gamma) \cong H$.  That is, every graph is
	the $\gamma$-graph of some graph. 
\end{theorem}
%<<<E Theorem{thm:sl:gammaGraph}

%\section{The $\ir$, $\gamma_{t}$, $\gamma_{pr}$ and $\gamma_{c}$-graphs}


To begin, we examine four domination-related parameters and their respective
extensions of Theorem \ref{thm:sl:gammaGraph}. A vertex set $S$ is said to
\emph{totally-dominate} a graph $G$ if it is dominating and for each $v\in S$
there exists $u\in S$ such that $u$ and $v$ are adjacent. The cardinality of a
smallest total-dominating set is the \emph{total-domination number}
$\gamma_{t}(G)$, as first introduced by Cockayne et al. in \cite{CDH80}.
Closely related, a \emph{paired-dominating} set $S$ is a total-dominating set with
the additional requirement that the induced subgraph $G[S]$ has a perfect
matching. The \emph{paired-domination number} $\gamma_{pr}(G)$ was defined
similarly by Haynes and Slater in \cite{HS98}. Since every paired-dominating
set is also a total-dominating set, for every graph $G$ without isolated
vertices, $\gamma(G)\leq\gt(G)\leq\gpr(G)$ \cite{HHS1}. A
\emph{connected-dominating} set $S$ is a dominating set where $G[S]$ is
connected, and the cardinality of a smallest connected-dominating set is the
\emph{connected-domination number} $\gamma_{c}(G)$, as defined by Sampathkumar
and Walikar \cite{SW79}. For all nontrivial connected graphs $G$,
$\ir(G)\leq\gamma(G)\leq\gamma_{t}(G)\leq\gamma_{c}(G)$ and $\gamma
(G)\leq2\ir(G)-1$ \cite{HHS1}.

We say the $\ir$\emph{-}$\emph{graph}$, the \emph{$\gamma_{t}$-graph}, the
\emph{$\gamma_{pr}$-graph}, and the \emph{$\gamma_{c}$-graph} of $G$ are the
graphs with vertices representing the minimum-cardinality maximal irredundant,
total-dominating, paired-dominating, and connected dominating sets of $G$,
respectively, and where adjacency is defined using the vertex-slide model.
Using the same construction as Connelly et al. in \cite{CHH10} and restated
below, we find a result analogous to Theorem \ref{thm:sl:gammaGraph} for
the $\ir$-graph, $\gamma_{t}$-graph, $\gamma_{pr}$-graph, and $\gamma_{c}$-graph.

\begin{theorem}
	\label{thm:prGraph} Every graph $H$ is the $\ir$-graph, $\gamma_{pr}$-graph,
	$\gamma_{t}$-graph, and $\gamma_{c}$-graph of infinitely many graphs.
\end{theorem}

\noindent For reference, we restate Connelly et al.'s construction for a graph
$G$ with $G(\gamma)\cong H$.

\noindent\underline{Construction:} Given some graph $H$ with $V(H) =
\{v_{1},v_{2},\dots, v_{n}\}$, to construct a graph $G$ with $G(\gamma)\cong
H$, begin with a copy of $H$ and attach vertices $a,b,c$ to every vertex of
$H$. Then, add two (or more) pendant vertices to $c$, labelled as $c_{1}$ and
$c_{2}$ (see Figure \ref{fig:gprConst}).

%XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX


%~~~~~~~~~~~~~~~~~~~~~~~~~FIG START~~~~~~~~~~~~~~~~~~~~~~
\begin{figure}[H]
	\centering
	\begin{tikzpicture}					
		%---------- H CORE  --------------- 		
		\fill[lgray, dashed] (0,0) circle (1.7cm);
		
		\node [std](v1) at (45:1cm) {};
		\path (v1) ++(45:4 mm) node (x1L) {$v_1$};
		\node [std](v2) at (135:1cm){};
		\path (v2) ++(135:4 mm) node (x2L) {$v_2$};
		\node [std](v3) at (225:1cm) {};
		\path (v3) ++(270:4 mm) node (x3L) {$v_3$};
		\node [std](v4) at (315:1cm){};
		\path (v4) ++(270:4 mm) node (x4L) {$v_4$};
		\draw[mgray](v1)--(v2)--(v3)--(v4)--(v1)--(v3);
		
		\draw[gray, dashed] (0,0) circle (1.7cm);
		\node (H) at (0,-1.4) [color=gray](L){$H$};	
		%--------- A B C ----------------------					
		
		\node [std](a) at (175:25mm)[label=left:$a$]  {};			
		\node [std](b) at (185:25mm)[label=left:$b$]  {};	
		
		
		\node [std](c) at (0:25mm)[label=below:$c$]  {};	
		
		\foreach \i in {1,2,3,4}
		{\draw(a)--(v\i)--(b);
			\draw(c)--(v\i);}
		
		\foreach \i / \j in {1/20, 2/-20}
		{ \path (c) ++(\j:10 mm) node (c\i) [std] {};
			\path (c\i) ++(0:5 mm) node (cL\i)  {$c_{\i}$};	
			\draw(c)--(c\i);
		}
		
	\end{tikzpicture}
	\caption{The graph $G$ constructed from $H$ from \cite{CHH10}.}%
	\label{fig:gprConst}%
\end{figure}
%~~~~~~~~~~~~~~~~~~~~~~~~~FIG END~~~~~~~~~~~~~~~~~~~~~~


From the pendant vertices, $c$ is in every $\gamma$-set of $G$; however, as
$a$ and $b$ remain undominated, $\{c\}$ is not itself a $\gamma$-set. Thus,
$\gpr(G) \geq\gamma(G) \geq2$ (likewise $\gamma_{c}(G) \geq\gt(G) \geq
\gamma(G) \geq2$). It follows that for each $v_{i}\in V(H)$, the set
$S_{i}=\{c,v_{i}\}$ is a $\gamma$-set. Since $\ir(G) \leq2 = \gamma(G) \leq2
\ir(G)-1$, it follows that $S_{i}$ is an $\ir$-set. Moreover, since $cv_{i}
\in E(G)$, each $S_{i}$ is also a $\gpr$-set, a $\gt$-set, and $\gamma_{c}%
$-set. Since neither $\{c,a\}$ nor $\{ c,b\}$ is dominating, the collection
$\{S_{i}: 1 \leq i \leq n\}$ consists of all the $\ir$, $\gamma$, $\gt$,
$\gpr$, $\gamma_{c}$-sets of $G$.

%-----	GAMMA + ID GRAPH PROOF ---

\section{The $\gid$-Graph}

\label{subsec:GIDExist}

A popular variation on domination is the topic of identifying codes. A vertex
set $S$ is an \emph{identifying code} (ID-code) of a graph $G$ if for each $v \in V$, the
closed neighbourhood of $v$ and $S$ have a unique, nonempty intersection. The
\emph{intersection set} of a vertex $v$ with respect to a vertex subset $S$ is
the set $I_{S}(v) = N[v]\cap S$. Thus, $S$ is an identifying code of $G$ if
all of its intersection sets are unique and nonempty.  The
cardinality of a minimum ID-code is denoted $\gid(G)$, and an ID-code with
cardinality $\gid(G)$ is called an $\gid$-\emph{set}. If $\gid(G)$ is finite,
$G$ is said to be \emph{identifiable} (or \emph{distinguishable}); otherwise,
$G$ is not identifiable, and $\gid(G)$ is defined to be $\gid(G)=\infty$. 

Originally introduced by Karpovsky et al. in 1998 \cite{KCL98}, ID-codes were
proposed as a model for the positioning of fault-detection units on
multiprocessor systems (for additional references, see Lobstein's extensive
bibliography \cite{Biblio}). Consider now the problem of migrating the
detecting units from one configuration to another, such that only one
detecting unit can be moved at time to an adjacent processor, and at each step
the configuration remains an ID-code. When given a certain starting
configuration, what other configurations are reachable under these conditions?
How many steps are required to move between them? Are there multiple routes
from start to destination, or are we stuck with a single path? To aid in
addressing this family of questions, we define the $\gid$-\emph{graph of a
	graph $G$}, $G(\gid)=(V(\gid),E(\gid))$, similarly to the $\gamma$-graph, but
where the vertices now correspond to the $\gid$-sets in $G$ instead.

As a first result, we extend Theorem \ref{thm:sl:gammaGraph} to
$\gid$-graphs. The construction and proof are similar; however, in
consideration of the additional identification requirements, multiple copies
of the graph $\mathcal{C} = C_{4}\circleddash K_{1}$, the \emph{depleted
	corona of $C_{4}$}, in Figure \ref{fig:gidHand} are used to force certain
vertices into the $\gid$-set. Given any graph $G^{\prime}$, we construct a new
graph $G$ by adding an edge between $x_{1} \in V(\mathcal{C})$ and some $v\in
V(G^{\prime})$; we say $\mathcal{C}$ is \emph{attached to $G^{\prime}$ at $v$}.

%~~~~~~~~~~~~~~~~~~~~~~~~~FIG START~~~~~~~~~~~~~~~~~~~~~~
\begin{figure}[tbh]
	\centering
	\begin{tikzpicture}				
		
		%-----------X PATH ------------------								
		\foreach \i/\x in {1/1.5, 2/2.5,3/3.5,4/4.5}
		\node [std](x\i) at (\x,1.5)[label=below:$x_\i$] {};	
		
		\draw(x1)--(x2)--(x3)--(x4);		
		
		%---------- Y LEAVES  --------------- 									
		\foreach \i/\x in {1/1.5, 2/2.5,3/3.5}
		\node [std](y\i) at (\x,2.5)[label=above:$y_\i$] {};							
		
		\foreach \i/\x in {1/1.5, 2/2.5,3/3.5}
		\draw (y\i)--(x\i);
		
		\draw(x1) to [out=30,in=150](x4);								
		
	\end{tikzpicture}
	\caption{The graph $\mathbf{\mathcal{C}}$ in Lemmas \ref{lem:C} and
		\ref{lem:gidHand}.}%
	\label{fig:gidHand}%
\end{figure}
%~~~~~~~~~~~~~~~~~~~~~~~~~FIG END~~~~~~~~~~~~~~~~~~~~~~


\begin{lemma}
	\label{lem:C}  The vertex set $X=\{x_{1},x_{2},x_{3}\}$ is the unique
	$\gid$-set of $\mathcal{C}$.
\end{lemma}

%### Proof Start


\begin{proof}
	Suppose that $\mathcal{C}$ has a $\gid$-set $S$. Since the vertices in
	$Y=\{y_{1},y_{2},y_{3}\}$ are all pendant vertices in $\mathcal{C}$, for each
	$1 \leq i \leq3$, either $x_{i}$ or $y_{i}$ is in $S$. Since $X$ is
	identifying, it follows that $\gid(\mathcal{C}) = 3$ and that $X$ is a
	$\gid$-set of $\mathcal{C}$.
	
	Notice that since $|S|=3$ and each $y_{i}$ is pendant, $S\subseteq X\cup Y$
	and $x_{4}\notin S$. To dominate $x_{4}$, either $x_{1}$ or $x_{3}$ is in $S$.
	Without loss of generality, say $x_{1} \in S$. To show uniqueness, we need
	only verify that the sets $S_{2}=\{x_{1},y_{2},x_{3}\}$, $S_{3}=\{x_{1}%
	,x_{2},y_{3}\}$ and $S_{2,3}=\{x_{1},y_{2},y_{3}\}$ are not identifying. For
	$S_{2}$, $I_{S_{2}}(x_{3})= I_{S_{2}}(y_{3})=\{x_{3}\}$ and is therefore not
	identifying. Likewise for $S_{2,3}$, $I_{S_{2,3}}(x_{3})= I_{S_{2,3}}%
	(y_{3})=\{y_{3}\}$. Finally for $S_{3}$, $I_{S_{3}}(x_{4})= I_{S_{3}}%
	(y_{1})=\{x_{1}\}$. It follows that $S=X =\{x_{1},x_{2},x_{3}\}$ is the unique
	$\gid$-set of $\mathcal{C}$.
\end{proof}

%### Proof End


\begin{lemma}
	\label{lem:gidHand}  Let $G^{\prime}$ be any graph, and construct $G$ by
	attaching $\mathcal{C}$ to $G^{\prime}$ at some $v\in V(G^{\prime})$. If $S$
	is any $\gid$-set of $G$, then $\{x_{1},x_{2},x_{3}\} \subseteq S$. Moreover,
	if $S^{\prime}$ is a $\gid$-set of $G^{\prime}$, then $S^{\prime}\cup
	\{x_{1},x_{2},x_{3}\}$ is identifying in $G$.
\end{lemma}

%### Proof Start


\begin{proof}
	Let $V(G^{\prime}) = \{v_{1},v_{2},\dots,v_{n}\}$, and suppose that $G$ was
	constructed by attaching $\mathcal{C}$ to $G^{\prime}$ at $v_{n}$. Suppose
	that $G$ has an $\gid$-set $S$. Regardless of whether $v_{n} $ is in $S$ or
	not, each vertex of $Y=\{y_{1},y_{2},y_{3}\}$ remains pendant and so for each
	$1 \leq i \leq3$, either $x_{i}$ or $y_{i}$ is in $S$. Using the same
	arguments as in Lemma \ref{lem:C}, $\{x_{1},x_{2},x_{3}\} \subseteq S$.
	
	Now suppose that $S^{\prime}$ is a $\gid$-set of $G^{\prime}$ and consider
	$S=S^{\prime}\cup\{x_{1},x_{2},x_{3}\}$ in $G$. Since $S^{\prime}$ is
	identifying, for each $v_{i} \in V(G^{\prime})$, the intersection set
	$I_{S^{\prime}}(v_{i})$ in $G^{\prime}$ is unique. In $G$, all intersection
	sets of $v_{1}, v_{2}, \dots, v_{n-1}$ remain the same. The intersection set
	of $v_{n}$ becomes $I_{S}(v_{n}) = I_{S^{\prime}}(v_{n}) \cup\{x_{1}\} \neq
	I_{s}(y_{1})$. From the first portion of this lemma, the sets $I_{S}(x_{i})$
	for $1 \leq i \leq4$ are also unique. It follows that $S$ is identifying in
	$G$.
\end{proof}

%### Proof End


Notice that the converse of the second portion of Lemma \ref{lem:gidHand} does
not hold. For a counterexample, consider the graph $G$ in Figure
\ref{fig:leCE} constructed by attaching $\mathcal{C}$ to a copy of $C_{4}$
with $V(C_{4}) =\{v_{1},v_{2},v_{3},v_{4}\}$. Although $\{v_{1},v_{3}%
,x_{1},x_{2},x_{3}\}$ is a $\gid$-set of $G$, $\{v_{1},v_{3}\}$ is not a
$\gid$-set of $C_{4}$.



%~~~~~~~~~~~~~~~~~~~~~~~~~FIG START~~~~~~~~~~~~~~~~~~~~~~
\begin{figure}[H]
	\centering
	\begin{tikzpicture}					
		%---------- H CORE  --------------- 								
		\node [std](v1) at (45:1cm) {};
		\path (v1) ++(45:4 mm) node (x1L) {$v_1$};
		\node [wstd](v2) at (135:1cm){};
		\path (v2) ++(135:4 mm) node (x2L) {$v_2$};
		\node [std](v3) at (225:1cm) {};
		\path (v3) ++(270:4 mm) node (x3L) {$v_3$};
		\node [wstd](v4) at (315:1cm){};
		\path (v4) ++(270:4 mm) node (x4L) {$v_4$};
		\draw(v1)--(v2)--(v3)--(v4)--(v1);								
		
		%---------- X ------------------					
		\foreach \label/\rad in {1/10,2/20,3/30,4/40}
		\path (v4) ++(0:\rad mm) node (x\label) [std]  {};
		\draw(v4)--(x4);
		
		\foreach \i in {1, 2,3,4}
		\path (x\i) ++(-90:4 mm) node (xL\i) {$x_{\i}$};				
		
		%-----------Y -------------------					
		\foreach \i/\x in {1,2,3}
		{	\path (x\i) ++(90:10 mm) node (y\i) [wstd]  {};
			\draw (y\i)--(x\i);			
			\path (y\i) ++(90:4 mm) node (yL\i) {$y_{\i}$};	
		}
		
		\draw(x1) to [out=30,in=150](x4);			
		\node [wstd](x4w) at (x4){};										
		
	\end{tikzpicture}
	\caption{Counterexample to the converse of Lemma \ref{lem:gidHand}.}%
	\label{fig:leCE}%
\end{figure}
%~~~~~~~~~~~~~~~~~~~~~~~~~FIG END~~~~~~~~~~~~~~~~~~~~~~


\begin{theorem}
	\label{thm:gamma-ID}  Every graph $H$ is the $\gid$-graph of some graph.
\end{theorem}

%### Proof START


\begin{proof}
	Let $H = (V(H),E(H))$ be any nonempty graph with $V(H) = \{v_{1},v_{2}%
	,\dots,v_{n}\}$. We construct a new graph $G$ such that $G(\gid) \cong H$.
	
	\noindent\underline{Construction:} Begin with a copy of $H$ and for each
	$v_{i} \in V(H)$, attach two copies of the graph $\mathcal{C}$ from Figure
	\ref{fig:gidHand} to $H$ at $v_{i}$, labelled as $\mathcal{C}_{i}$ and
	$\mathcal{C}_{i}^{*}$ with 	
	\begin{align*}
	V(\mathcal{C}_{i}) = \{x_{i,1},x_{i,2},x_{i,3},x_{i,4}, y_{i,1}, y_{i,2}, y_{i,3}\}, \text{ and } 
	V(\mathcal{C}_{i}^{*}) = \{x_{i,1}^{*},x_{i,2}^{*},x_{i,3}^{*}, x_{i,4}^{*}, y_{i,1}^{*}, y_{i,2}^{*},
	y_{i,3}^{*}\}. 
	\end{align*}
	\noindent Now, add vertices $a$ and $b$ so that $av_{i} \in E(G)$ and
	$bv_{i} \in E(G)$ for all $i=1,2,\dots, n$. Finally, attach two more copies of
	$\mathcal{C}$, $\mathcal{C}_{a}$ and $\mathcal{C}_{b}$, at $a$ and $b$,
	respectively (see Figure \ref{fig:gidConst}).
	
	\noindent Consider the vertex set,
	\begin{align*}
		X = \left( \bigcup\limits_{\substack{1 \leq j \leq n \\1 \leq k \leq3}}
		\{x_{j,k}, x_{j,k}^{*}\}\right)  \cup\left( \bigcup\limits_{1\leq k \leq3}
		\{x_{a,k},x_{b,k}\}\right) .
	\end{align*}
	In particular, notice that $X$ consists of all the vertices within the various
	$\mathcal{C}$ graphs that Lemma \ref{lem:gidHand} demonstrates are in every
	$\gid$-set of $G$.
	
	%~~~~~~~~~~~~~~~~~~~~~~~~~FIG START~~~~~~~~~~~~~~~~~~~~~~
	\begin{figure} 
		\centering %\scalebox{0.85}{
			\begin{tikzpicture}				
				%---------- H CORE  --------------- 		
				\fill[lgray, dashed] (0,0) circle (1.7cm);
				
				\node [std](v1) at (45:1cm)[label=above:$v_1$] {};
				\node [std](v2) at (135:1cm)[label=above:$v_2$] {};
				\node [std](v3) at (225:1cm)[label=below:$v_3$] {};
				\node [std](v4) at (315:1cm)[label=below:$v_4$] {};
				\draw[mgray](v1)--(v2)--(v3)--(v4)--(v1)--(v3);
				
				\draw[gray, dashed] (0,0) circle (1.7cm);
				\node (H) at (0,-1.4) [color=gray](L){$H$};			
				
				%---------- X Stems  --------------- 									
				\node (x31) at (215:25mm) [label=above:$x_{3,1}$] {};
				\node (x41) at (305:25mm) [label=left:$x_{4,1}$] {};
				
				\draw(v3)--(x31);
				\draw(v4)--(x41);
				%---------- X* Stems  --------------- 									
				\node (x31*) at (235:25mm)[label=right:$x_{3,1}^*$] {};
				\node (x41*) at (325:25mm) [label=above:$x_{4,1}^*$]{};	
				\draw(v3)--(x31*);
				\draw(v4)--(x41*);
				
				%-----------X1 PATHS ------------------
				\path (v1) ++(25:20 mm) node (x11) [std]  {};
				\draw(v1)--(x11);
				
				\foreach \label/\rad in {2/8,3/16,4/24}
				\path (x11) ++(25:\rad mm) node (x1\label) [std]  {};
				\draw(x11)--(x14);
				
				\foreach \x/\i in {1/2, 2/2,3/2,4/2}
				\path (x1\x) ++(115:3 mm) node (x1L\x) {$x_{1,\x}$};										
				
				\foreach \x/\y in {1/1, 2/2, 3/3}
				\path (x1\x) ++(-65:6mm) node (y1\y) [std]  {};
				\foreach \x/\y in {1/1, 2/2,3/3}
				\draw(x1\x)--(y1\y);	
				
				\foreach \y/\i in {1/2, 2/2,3/2}
				\path (y1\y) ++(-65:4 mm) node (y1L\y) {$y_{1,\y}$};								
				
				\draw(x11) to [out=0,in=240](x14);	
				
				%-----------X1* PATHS ------------------
				\path (v1) ++(65:20 mm) node (x11*) [std]  {};
				\draw(v1)--(x11*);
				
				\foreach \label/\rad in {2/8,3/16,4/24}
				\path (x11*) ++(65:\rad mm) node (x1\label*) [std]  {};
				\draw(x11*)--(x14*);							
				
				\foreach \x/\i in {1/2, 2/2,3/2,4/2}
				\path (x1\x*) ++(-25:5 mm) node (x1L\x*) {$x_{1,\x}^*$};									
				
				\foreach \x/\y in {1/1, 2/2, 3/3}
				\path (x1\x*) ++(155:6mm) node (y1\y*) [std]  {};
				\foreach \x/\y in {1/1, 2/2,3/3}
				\draw(x1\x*)--(y1\y*);				
				
				\foreach \y/\i in {1/2, 2/2,3/2}
				\path (y1\y*) ++(155:5 mm) node (y1L\y*) {$y_{1,\y}^*$};										
				
				\draw(x11*) to [out=90,in=220](x14*);
				%-----------X2 PATHS ------------------
				\path (v2) ++(115:20 mm) node (x21) [std]  {};
				\draw(v2)--(x21);
				
				\foreach \label/\rad in {2/8,3/16,4/24}
				\path (x21) ++(115:\rad mm) node (x2\label) [std]  {};
				\draw(x21)--(x24);
				
				\foreach \x/\i in {1/2, 2/2,3/2,4/2}
				\path (x2\x) ++(205:5 mm) node (x2L\x) {$x_{2,\x}$};										
				
				\foreach \x/\y in {1/1, 2/2, 3/3}
				\path (x2\x) ++(25:6mm) node (y2\y) [std]  {};
				\foreach \x/\y in {1/1, 2/2,3/3}
				\draw(x2\x)--(y2\y);	
				
				\foreach \y/\i in {1/2, 2/2,3/2}
				\path (y2\y) ++(25:5 mm) node (y2L\y) {$y_{2,\y}$};								
				
				\draw(x21) to [out=90,in=330](x24);	
				
				%-----------X2* PATHS ------------------
				\path (v2) ++(155:20 mm) node (x21*) [std]  {};
				\draw(v2)--(x21*);
				
				\foreach \label/\rad in {2/8,3/16,4/24}
				\path (x21*) ++(155:\rad mm) node (x2\label*) [std]  {};
				\draw(x21*)--(x24*);							
				
				\foreach \x/\i in {1/2, 2/2,3/2,4/2}
				\path (x2\x*) ++(65:4 mm) node (x2L\x*) {$x_{2,\x}^*$};									
				
				\foreach \x/\y in {1/1, 2/2, 3/3}
				\path (x2\x*) ++(245:6mm) node (y2\y*) [std]  {};
				\foreach \x/\y in {1/1, 2/2,3/3}
				\draw(x2\x*)--(y2\y*);				
				
				\foreach \y/\i in {1/2, 2/2,3/2}
				\path (y2\y*) ++(245:4 mm) node (y2L\y*) {$y_{2,\y}^*$};										
				
				\draw(x21*) to [out=180,in=300](x24*);	
				
				%--------- A ----------------------			
				\node [std](a) at (180:25mm)[label=below:$a$]  {};			
				
				\foreach \i in {1,2,3,4}
				\draw(a)--(v\i);
				
				\path (a) ++(180:15 mm) node (xa1) [std]  {};
				\draw(a)--(xa1);
				
				\foreach \label/\rad in {2/8,3/16,4/24}
				\path (xa1) ++(180:\rad mm) node (xa\label) [std]  {};
				\draw(xa1)--(xa4);
				
				\foreach \x in {1, 2,3,4}
				\path (xa\x) ++(90:3 mm) node (xaL\x) {$x_{a,\x}$};										
				
				\foreach \x/\y in {1/1, 2/2, 3/3}
				\path (xa\x) ++(270:6mm) node (ya\y) [std]  {};
				\foreach \x/\y in {1/1, 2/2,3/3}
				\draw(xa\x)--(ya\y);	
				
				\foreach \y/\i in {1/2, 2/2,3/2}
				\path (ya\y) ++(270:4 mm) node (yaL\y) {$y_{a,\y}$};								
				
				\draw(xa1) to [out=210,in=-30](xa4);	
				
				%--------- B ----------------------						
				\node [std](b) at (0:25mm)[label=below:$b$]  {};					
				
				\foreach \i in {1,2,3,4}
				\draw(b)--(v\i);
				
				\draw(b)--(v1);
				\draw(b)--(v2);
				\draw(b)--(v3);
				\draw(b)--(v4);
				
				\path (b) ++(0:15 mm) node (xb1) [std]  {};
				\draw(b)--(xb1);
				
				\foreach \label/\rad in {2/8,3/16,4/24}
				\path (xb1) ++(0:\rad mm) node (xb\label) [std]  {};
				\draw(xb1)--(xb4);
				
				\foreach \x in {1, 2,3,4}
				\path (xb\x) ++(90:3 mm) node (xbL\x) {$x_{b,\x}$};										
				
				\foreach \x/\y in {1/1, 2/2, 3/3}
				\path (xb\x) ++(270:6mm) node (yb\y) [std]  {};
				\foreach \x/\y in {1/1, 2/2,3/3}
				\draw(xb\x)--(yb\y);	
				
				\foreach \y/\i in {1/2, 2/2,3/2}
				\path (yb\y) ++(270:4 mm) node (ybL\y) {$y_{b,\y}$};								
				
				\draw(xb1) to [out=-30,in=210](xb4);														
				
				% ----------- BLOBS ---------------------
				% Z3 - Blob
				\path (x31) ++(215:4 mm) node (x31C){};
				\fill[lgray] (x31C) circle (4mm);
				\draw[gray] (x31C) circle (4mm){};
				\node[std] at (x31){};
				\node at  (x31C) [color=gray]{$\mathcal{C}_3$};	
				
				% Z3* - Blob	
				\path (x31*) ++(235:4 mm) node (x31C*){};
				\fill[lgray] (x31C*) circle (4mm);
				\draw[gray] (x31C*) circle (4mm){};
				\node[std] at (x31*){};
				\node at  (x31C*) [color=gray]{$\mathcal{C}_3^*$};							
				
				% Z4 - Blob
				\path (x41) ++(305:4 mm) node (x41C){};
				\fill[lgray] (x41C) circle (4mm);
				\draw[gray] (x41C) circle (4mm){};
				\node[std] at (x41){};
				\node at  (x41C)[color=gray]{$\mathcal{C}_4$};
				
				% Z4* - Blob
				\path (x41*) ++(325:4 mm) node (x41C*){};
				\fill[lgray] (x41C*) circle (4mm);
				\draw[gray] (x41C*) circle (4mm){};
				\node[std] at (x41*){};
				\node at  (x41C*)[color=gray]{$\mathcal{C}_4^*$};
				
			\end{tikzpicture} %}
		\caption{The graph $G$ constructed from $H$ in Theorem \ref{thm:gamma-ID}. }%
		\label{fig:gidConst}% 
	\end{figure}
	%~~~~~~~~~~~~~~~~~~~~~~~~~FIG END~~~~~~~~~~~~~~~~~~~~~~
	
	
	We first show that for each $1 \leq i \leq n$, the vertex set $S_{i} =
	\{v_{i}\}\cup X$ is a $\gid$-set of $G$. From the construction of $G$, it is
	clear that $S_{i}$ dominates $G$. Furthermore, from Lemma \ref{lem:gidHand},
	we know that each vertex within a $\mathcal{C}$ subgraph is identified by
	$S_{i}$. For vertices within $H$, the identifying set $I_{S_{i}}(v_{j})$ of
	the vertex $v_{j}$ contains the unique pair $\{x_{j,1},x_{j,1}^{*}\}$,
	ensuring that each $v_{j}$ is identified in $S_{i}$. Finally, $a$ and $b$ also
	have the unique identifying sets $I_{S_{i}}(a)=\{x_{a,1}, v_{i}\}$ and
	$I_{S_{i}}(b) = \{x_{b,1}, v_{i}\}$, respectively. It follows that $S_{i}$ is
	identifying and dominating in $G$.
	
	We now show that $S_{i}$ is a $\gid$-set. Notice that there are $2n+6$ pendant
	vertices in $G$, and so $\gamma(G) \geq2n+6$. Indeed, it is easy to see that
	$X=S_{i}-\{v_{i}\}$ is dominating in $G$, so $\gamma(G) = 2n+6$. Moreover,
	$\gid(G) \geq\gamma(G) = 2n+6$. Again, by Lemma \ref{lem:gidHand}, we know
	that any $\gid$-set of $G$ contains all of $X$; however $X$ is not identifying
	as $I_{X}(a) = \{x_{a,1}\} = I_{X}(y_{a,1})$, and so, $\gid(G) \geq(2n+6)+1$.
	Since $|S_{i}|=2n+7$ and $S_{i}$ is identifying, it follows that $S_{i}$ is a
	$\gid$-set for all $\leqn$.
	
	Let $\mathcal{S}_{\gid}=\{S_{1},S_{2},\dots,S_{n}\}$. We claim that
	$\mathcal{S}_{\gid}$ is the collection of all $\gid$-sets of $G$. Since we
	have already established that $\gid(G)=2n+7$ and that in every $\gid$-set,
	$2n+6$ of the vertices are from $X$, every $\gid$-set of $G$ can viewed as
	\textquotedblleft$X$-plus-one\textquotedblright. However, there is no single
	vertex $w\in V(G)-V(H)$ such that $X\cup\{w\}$ identifies both pairs
	$\{a,y_{a,1}\}$ and $\{b,y_{b,1}\}$. The set $S_{a}=\{a\}\cup X$ with $|S_{a}|=2n+7$
	has $I_{S_{a}}(b)=\{x_{b,1}\}=I_{S_{a}}(y_{b,1})$ and is therefore not
	identifying. Similarly, $S_{b}=\{b\}\cup X$ is not identifying. Thus,
	$\mathcal{S}_{\gid}$ is the collection of all $\gid$-sets.
	
	Consider now $G(\gid) = (V(\ggid),E(\ggid))$. By the above arguments,
	$V(\ggid)$ $= \{v_{1}^{\prime},v_{2}^{\prime},\dots,v_{n}^{\prime}\}$, where
	the vertex $v_{i}^{\prime}$ corresponds to the set $S_{i} \in\mathcal{S}%
	_{\gid}$ for each $\leqn$. Since $v_{i}^{\prime}$ and $v_{j}^{\prime}$ in
	$V(\ggid)$ are adjacent in $\ggid$ if and only if there exist $w_{i}\in S_{i}$
	and $w_{j} \in S_{j}$ with $w_{i}w_{j}\in E(G)$ such that $S_{i} = (S_{j}
	-\{w_{j}\}) \cup\{w_{i}\}$ and $S_{i}$ and $S_{j}$ differ at exactly one
	vertex (that is, $v_{i}$ versus $v_{j}$), it follows that $v_{i}^{\prime}%
	v_{j}^{\prime}\in E(\gid)$ if and only if $v_{i}v_{j} \in E(G)$. Therefore,
	$\ggid \cong H$ as required.
\end{proof}

%### Proof End


In the construction of the graph $G$ in the proof of Theorem
\ref{thm:gamma-ID}, if instead of attaching only two copies of the graph
$\mathcal{C}$ to each vertex of the graph $H$, we attached three or more
copies, the same $\gid$-graph $H$ is obtained. This leads immediately to the
following corollary.

\begin{coro}
	Every graph $H$ is the $\gid$-graph of infinitely many graphs.
\end{coro}

%----------------------SUBSEC: Locating ----------------------------------------------------
\section{The $\gamma_{L}$ and $\gamma_{t}^{L}$-Graphs}

Introduced by Slater in 1988 \cite{Slater87, Slater88}, a \emph{locating-dominating set}
$S$ of graph $G=(V,E)$ is a dominating set such that for each $v\in V-S$, the
set $N[v] \cap S$ is unique. In contrast to identifying codes,
locating-dominating sets do not require that the vertices of the dominating
set have unique neighbourhood intersection with the dominating set itself. The
minimum cardinality of a locating-dominating set, denoted by $\gamma_{L}(G)$,
is the \emph{locating-domination number} of a graph $G$. A \emph{$\gamma_{L}%
	$-set} of a graph is a minimum locating-dominating vertex subset. Since all
identifying codes are also locating-dominating sets, it follows that
$\gamma_{L} \leq\gid$ for all graphs. We reuse the notation of the
intersection set of a vertex $v$ and set $S$ from ID-codes; however, for
locating-dominating sets, the sets $I_{S}(v)$ need only be unique for $v\notin S$.

We define the \emph{$\gamma_{L}$-graph of a graph $G$}, $G(\gamma
_{L})=(V(\gamma_{L}),E(\gamma_{L}))$, to the be graph where the vertex set
$V(\gamma_{L})$ is the collection of $\gamma_{L}$-sets of $G$. As with the
$\gamma$-graph, $u,w \in V(\gamma_{L})$ associated with $\gamma_{L}$-sets
$S_{u}$ and $S_{w}$ are adjacent in $G(\gamma_{L})$ if and only if there exist
$v_{u} \in S_{u}$ and $v_{w} \in S_{w}$ with $v_{u}v_{w}\in E(G)$, such that
$S_{u} = (S_{w} - \{v_{w}\}) \cup\{v_{u}\}$.

Given the similarities between ID-codes and locating-dominating sets, it is
not surprising that a similar result to Theorem \ref{thm:gamma-ID} exists for
$\gamma_{L}$-graphs.

\begin{theorem}
	\label{thm:gammaL} Every graph $H$ is the $\gamma_{L}$-graph of infinitely
	many graphs.
\end{theorem}

Since $\mathcal{C}$ does not have a unique $\gamma_{L}$-set (for example,
$\{x_{1},x_{2},x_{3}\}$ and $\{x_{1},x_{2},y_{3}\}$ are $\gamma_{L}$-sets), we
cannot use it in the construction to prove Theorem \ref{thm:gammaL}. Instead,
we use the very similar \emph{Bull graph}, $\bull$, as pictured in Figure
\ref{fig:gLhand}. Notice that $S=\{x_{1},x_{2}\}$ is a $\gamma_{L}$-set in
$\bull$. Moreover, since $S_{1}=\{x_{1}, y_{2}\}$ and $S_{2}=\{y_{1},x_{2}\}$
give $I_{S_{1}}(y_{1})=\{x_{1}\}=I_{S_{1}}(x_{3})$, and $I_{S_{2}}%
(y_{2})=\{x_{2}\}=I_{S_{2}}(x_{3})$, $S$ is the only $\gamma_{L}$-set of
$\bull$. The proof to Theorem \ref{thm:gammaL} then proceeds identically to
that of Theorem \ref{thm:gamma-ID}, substituting the use of $\bull$ for
$\mathcal{C}$.



%~~~~~~~~~~~~~~~~~~~~~~~~~FIG START~~~~~~~~~~~~~~~~~~~~~~
\begin{figure}[H]
	\centering
	\begin{tikzpicture}				
		
		%-----------X PATH ------------------								
		\foreach \i/\x in {1/1.5, 2/2.5,3/3.5}
		\node [std](x\i) at (\x,1.5)[label=below:$x_\i$] {};	
		
		\draw(x1)--(x2)--(x3);		
		
		%---------- Y LEAVES  --------------- 									
		\foreach \i/\x in {1/1.5, 2/2.5}
		\node [std](y\i) at (\x,2.5)[label=above:$y_\i$] {};							
		
		\foreach \i/\x in {1/1.5, 2/2.5}
		\draw (y\i)--(x\i);
		
		\draw(x1) to [out=30,in=150](x3);								
		
	\end{tikzpicture}
	\caption{The Bull graph $\bull$ used in the construction of Theorem
		\ref{thm:gammaL}.}%
	\label{fig:gLhand}%
\end{figure}
%~~~~~~~~~~~~~~~~~~~~~~~~~FIG END~~~~~~~~~~~~~~~~~~~~~~

A variant of locating-dominating sets, a vertex subset $S$ is a
\emph{locating-total dominating set} (LTDS) of a graph $G$ if $S$ a
locating-dominating set and if each vertex in $V(G)$ is adjacent to some
vertex in $S$. The \emph{locating-total domination number} $\gamma_{t}^{L}(G)$
is the minimum cardinality of a LTDS \cite{HHH06}. We define the $\gamma
_{t}^{L}$-graph of a graph $G$ analogously to the $\gamma_{L}$-graph. Since in
the construction of Theorem \ref{thm:gammaL}, there were no independent
vertices in the $\gamma_{L}$-sets, the following corollary is immediate.

\begin{coro}
	Any graph $H$ is the $\gamma_{t}^{L}$-graph of infinitely many graphs.
\end{coro}

%----------------------SUBSEC: BIG GAMMA  ----------------------------------------


\section{The $\Gamma$-Graph}

The next domination parameter we examine is $\Gamma(G)$, the
\emph{upper domination number} of a graph $G$, defined to be the cardinality
of a largest minimal dominating set. The \emph{$\Gamma$-graph of a graph $G$}
and its associated parameters are defined analogously to $G(\gamma)$. Once
again, this variation requires the use of a new gadget: the graph
$\mathcal{Z}$ in Figure \ref{fig:Z}.

%~~~~~~~~~~~~~~~~~~~~~~~~~FIG START~~~~~~~~~~~~~~~~~~~~~~
\begin{figure}[H] 
	\centering
	\begin{tikzpicture}								
		
		%---------- Add on------------------
		\node [std](z) at (0,0)[label=below:$z$]  {};						
		
		\path (z) ++(0:10 mm) node (x2) [std] {};
		\draw(z)--(x2);	
		
		\foreach \i / \j in {1/90, 3/-90}
		{ \path (x2) ++(\j:8 mm) node (x\i) [std] {};
			\draw(z)--(x\i);
		}							
		
		\draw(x1)--(x3);	
		\draw(x1) to [out=-120,in=120](x3);		
		
		\foreach \i / \j  in {1/30, 2/30, 3/30}
		{
			\path (x\i) ++(0:15 mm) node (y\i) [std] {};
			\path (y\i) ++(\j:5 mm) node (yL\i)  {$y_{\i}$};
			\path (x\i) ++(\j:5 mm) node (xL\i)  {$x_{\i}$};		
			\draw(x\i)--(y\i);									
		}	
		
		\draw(y1)--(y3);	
		\draw(y1) to [out=-120,in=120](y3);		
		
	\end{tikzpicture} 
	\caption{The graph $\mathcal{Z}$ used in Theorem \ref{thm:bigGamma}.}%
	\label{fig:Z}%
\end{figure}
%~~~~~~~~~~~~~~~~~~~~~~~~~FIG END~~~~~~~~~~~~~~~~~~~~~~


\begin{theorem}
	\label{thm:bigGamma} Every graph $H$ is the $\Gamma$-graph of infinitely many graphs.
\end{theorem}

%## START PROOF


\begin{proof}
	\underline{Construction:} The construction of a graph $G$ with $G(\Gamma
	)\cong H$ is similar to the previous results. Begin with a copy of the graph
	$H$ with $V(H)=\{v_{1}, v_{2}, \dots, v_{n}\}$, and to each $v_{i}$, attach a
	copy of the graph $\mathcal{Z}$ in Figure \ref{fig:Z} labelled $\mathcal{Z}%
	_{i}$ with $V(Z_{i})=\{z_{i},x_{i,1},x_{i,2},x_{i,3}, y_{i,1}, y_{i,2},
	y_{i,3}\}$ at vertex $x_{i,1}$ to $v_{i}$. Attach a final copy of
	$\mathcal{Z}$ labelled $\mathcal{Z^{*}}$ ($V(\mathcal{Z}^{*})=\{z^{*}%
	,x_{1}^{*},x_{2}^{*},x_{3}^{*}, y_{1}^{*}, y_{2}^{*}, y_{3}^{*}\}$) by joining
	each $v_{i}$ to $z^{*}$.
	
	\noindent For reference, we define $X_{i} = \{x_{i,1}, x_{i,2}, x_{i,3}\}$,
	$Y_{i} = \{y_{i,1}, y_{i,2}, y_{i,3}\}$, $X^{*} = \{x_{1}^{*}, x_{2}^{*},
	x_{3}^{*}\}$, and $Y^{*} = \{y_{1}^{*}, y_{2}^{*}, y_{3}^{*}\}$.
	
	We claim that the $\Gamma$-sets of $G$ are $S_{1}, S_{2}, \dots, S_{n}$ where
	for each $1 \leq i \leq n$,
	\begin{align}
		S_{i} = \{v_{i}\} \cup\left( \bigcup_{1\leq j \leq n} X_{j} \right)  \cup
		Y^{*}.
	\end{align}
	
	
	%~~~~~~~~~~~~~~~~~~~~~~~~~FIG START~~~~~~~~~~~~~~~~~~~~~~
	\begin{figure}
		\centering \scalebox{0.9}{
			\begin{tikzpicture}					
				%---------- H CORE  --------------- 		
				\fill[lgray, dashed] (0,0) circle (1.7cm);
				
				\node [std](v1) at (45:1cm) {};
				\path (v1) ++(100:4 mm) node (x1L) {$v_1$};
				\node [std](v2) at (135:1cm){};
				\path (v2) ++(80:4 mm) node (x2L) {$v_2$};
				\node [std](v3) at (225:1cm) {};
				\path (v3) ++(280:4 mm) node (x3L) {$v_3$};
				\node [std](v4) at (315:1cm){};
				\path (v4) ++(260:4 mm) node (x4L) {$v_4$};
				\draw[mgray](v1)--(v2)--(v3)--(v4)--(v1)--(v3);
				
				\draw[gray, dashed] (0,0) circle (1.7cm);
				\node (H) at (0,-1.4) [color=gray](L){$H$};	
				%---------- X Stems  --------------- 		
				\path (v3) ++(225:15 mm) node (x31) [std][label=right:$x_{3,1}$] {};								
				\path (v4) ++(-45:15 mm) node (x41) [std][label=left:$x_{4,1}$] {};		
				
				\draw(v3)--(x31);
				\draw(v4)--(x41);
				
				% Z3 - Blob
				\path (x31) ++(225:5 mm) node (x31C){};
				\fill[lgray] (x31C) circle (5mm);
				\draw[gray] (x31C) circle (5mm){};
				\node[std] at (x31){};
				\node at  (x31C) [color=gray]{$\mathcal{Z}_3$};							
				
				% Z4 - Blob
				\path (x41) ++(-45:5 mm) node (x41C){};
				\fill[lgray] (x41C) circle (5mm);
				\draw[gray] (x41C) circle (5mm){};
				\node[std] at (x41){};
				\node at  (x41C)[color=gray]{$\mathcal{Z}_4$};
				%---------- Z1 ------------------
				
				\path (v1) ++(60:15 mm) node (x11) [std] {};
				
				\foreach \i / \j in {2/8, 3/16}
				{ \path (x11) ++(0: \j mm) node (x1\i) [std] {};
					\draw(x11)--(x1\i);								
				}
				
				\path (x12) ++(-90:8 mm) node (z1) [std] [label=below:$z_1$] {};
				\draw (x11)--(z1)--(x13);
				\draw(z1)--(x12);															
				
				\draw(x11)--(x13);	
				\draw(x11) to [out=-30,in=210](x13);		
				
				\foreach \i / \j  in {1/45, 2/45, 3/45}
				{
					\path (x1\i) ++(90:15 mm) node (y1\i) [std] {};
					\path (y1\i) ++(\j:5 mm) node (yL1\i)  {$y_{1,\i}$};							
					\draw(x1\i)--(y1\i);									
				}	
				
				\foreach \i / \j  in {1/45, 2/45, 3/45}	
				\path (x1\i) ++(\j:5 mm) node (xL1\i)  {$x_{1,\i}$};							
				
				\draw(y11)--(y13);	
				\draw(y11) to [out=-30,in=210](y13);						
				
				\draw(v1)--(x11);
				
				
				%---------- Z2 ------------------
				
				\path (v2) ++(120:15 mm) node (x21) [std] {};
				
				\foreach \i / \j in {2/8, 3/16}
				{ \path (x21) ++(180: \j mm) node (x2\i) [std] {};
					\draw(x21)--(x2\i);								
				}
				
				\path (x22) ++(-90:8 mm) node (z2) [std] [label=below:$z_2$] {};
				\draw (x21)--(z2)--(x23);
				\draw(z2)--(x22);															
				
				\draw(x21)--(x23);	
				\draw(x21) to [out=210,in=-30](x23);		
				
				\foreach \i / \j  in {1/135, 2/135, 3/135}
				{
					\path (x2\i) ++(90:15 mm) node (y2\i) [std] {};
					\path (y2\i) ++(\j:5 mm) node (yL2\i)  {$y_{2,\i}$};							
					\draw(x2\i)--(y2\i);									
				}	
				
				\foreach \i / \j  in {1/135, 2/135, 3/135}	
				\path (x2\i) ++(\j:5 mm) node (xL2\i)  {$x_{2,\i}$};							
				
				\draw(y21)--(y23);	
				\draw(y21) to [out=210,in=-30](y23);		
				\draw(v2)--(x21);							
				
				%---------- Z* ------------------												
				
				\node [std](z) at (0:25mm)[label=below:$z^*$]  {};		
				\foreach \i in {1, 2, 3, 4}
				\draw(z)--(v\i);								
				
				\path (z) ++(0:10 mm) node (x2) [std] {};
				\draw(z)--(x2);	
				
				\foreach \i / \j in {1/90, 3/-90}
				{ \path (x2) ++(\j:8 mm) node (x\i) [std] {};
					\draw(z)--(x\i);
				}							
				
				\draw(x1)--(x3);	
				\draw(x1) to [out=-120,in=120](x3);		
				
				\foreach \i / \j  in {1/30, 2/30, 3/30}
				{
					\path (x\i) ++(0:15 mm) node (y\i) [std] {};
					\path (y\i) ++(\j:5 mm) node (yL\i)  {$y_{\i}^*$};
					\path (x\i) ++(\j:5 mm) node (xL\i)  {$x_{\i}^*$};		
					\draw(x\i)--(y\i);									
				}	
				
				\draw(y1)--(y3);	
				\draw(y1) to [out=-120,in=120](y3);						
				
		\end{tikzpicture}}
		\caption{The graph $G$ constructed from $H$ in Theorem \ref{thm:bigGamma}.}%
		\label{fig:bigGamma}%
	\end{figure}
	%~~~~~~~~~~~~~~~~~~~~~~~~~FIG END~~~~~~~~~~~~~~~~~~~~~~
	
	
	\noindent To begin, notice that $S_{i}$ is minimal dominating with $|S_{i}| =
	3(n+1)+1=3n+4$; for each $1 \leq j \leq3$, $pn[x_{i,j},S_{i}] =\{y_{i,j}\}$,
	$pn[y_{j}^{*},S_{i}] = \{x_{j}^{*}\}$, and $pn[v_{i},S_{i}] = \{z^{*}\}$. We
	proceed with a series of claims to demonstrate that the collection
	$\mathcal{S}=\{S_{1}, S_{2},\dots,S_{n}\}$ contains the only $\Gamma$-sets of
	$G$.
	
	\begin{enumerate}[label=(\roman*)]
		\setlength{\parindent}{1pt} \setlength{\parskip}{1pt}
		
		\item \emph{If $S$ is a minimal dominating set, then for each $1 \leq i \leq
			n$ and $1 \leq j \leq3$, \\ $\{z_{i}, x_{i,j}\} \not \subseteq S$. Likewise,
			$\{z^{*}, x_{j}^{*}\} \not \subseteq S$}\newline Since $N[z_{i}] \subseteq
		N[x_{i,j}]$, either $X_{i} \cap S = \varnothing$, or one of the $x_{i,j}$
		annihilates the private neighbourhood of $z_{i}$ in $S$.
		
		\item \emph{If $S$ is a minimal dominating set, and $x_{i,1} \notin S$, then
			$|S\cap V(\mathcal{Z}_{i})| = 2$.}\newline If $z_{i} \in S$, then by (i),
		$X_{i} \cap S = \varnothing$. To dominate $Y_{i}$ minimally, exactly one
		$y_{i,j} \in S$, and thus $|V(\mathcal{Z}_{i}) \cap S|=2$. Suppose instead
		that $z_{i} \notin S$ and that $z_{i}$ is externally dominated. Then $|X_{i}
		\cap S| \geq1$, say without loss of generality, $x_{i,2} \in S$. To dominate
		$y_{i,1}$ minimally, some $y_{i,k}$ is also in $S$. Then $\mathcal{Z}_{i}$ is
		dominated by $\{x_{i,2}, y_{i,k}\}$ and again $|V(\mathcal{Z}_{i}) \cap S|=2$.
		
		\item \emph{If $S$ is a minimal dominating set, then for $1\leq i\leq n$,
			$|S\cap V(\mathcal{Z}_{i})|\leq3$, and \linebreak $|S\cap V(\mathcal{Z}^{\ast})|\leq3$}.
		\newline As in (ii), if $z_i \in S$ then $|S\cap V(\mathcal{Z}_{i})| = 2$. For $1 \leq j \leq 3$, if $y_{i,j}\in S$, then to dominate $z_i$, either 	$z_i \in S$ (and $|S\cap V(\mathcal{Z}_{i})| = 2$), or  $x_{i,k} \in S$ for some $1\leq k \leq 3$, in which case $\{x_{i,k}, y_{i,j}\}$ dominates $\mathcal{Z}_i$, and again, $|S\cap V(\mathcal{Z}_{i})| = 2$.  Otherwise, $z_i \notin S$, and $Y_i\cap S=\varnothing$, which implies $X_i\cap S \neq \varnothing$.  Since only $x_{i,j}$ externally dominates $y_{i,j}$, it follows that  $X_i \subseteq S$, and hence $|S\cap V(\mathcal{Z}_i)|=3$.
		
			
		%If $z_i \in S$, then by (i), $x_{i,j} \notin S$ for $1 \leq j \leq 3$.
		
		%Notice that for $1\leq j \leq 3$, $\{z_i,y_{i,j}\}$ minimally dominates $\mathcal{Z}_i$.
		%Likewise, as was
		
		
	%	\newline As in (ii), if some $x_{i,j}\in S$ and some $y_{i,k}\in S$, then
	%	$|V(\mathcal{Z}_{i})\cap S|=2$. Thus, the largest intersection of
	%	$\mathcal{Z}_{i}$ and $S$ occurs when $z_{i}\notin S$ and $S\cap
	%	Y_{i}=\varnothing$; that is, when $V(\mathcal{Z}_{i})\cap S=X_{i}$.
		
		\item \emph{If $S$ is a $\Gamma$-set of $G$, then $|V(H)\cap S|\leq1$%
			.}\newline Suppose to the contrary that $|V(H)\cap S|=m\geq2$; say without
		loss of generality that $v_{1},...,v_{m}\in S$. For each $i=1,...,m$,
		$z^{\ast}\notin pn[v_{i},S]$. Since $z_{i}$ is dominated (by a vertex in
		$\{z_{i},x_{i,1},x_{i,2},x_{i,3}\}\cap S$), $x_{i,1}\notin pn[v_{i},S]$. Hence
		either $v_{i}\in pn[v_{i},S]$ or $v_{j}\in pn[v_{i},S]$ for some $j>m$. In the
		former case, $x_{i,1}\notin S$ and $|V(\mathcal{Z}_{i})\cap S|=2$, and in the
		latter case, $x_{j,1}\notin S$ and $|V(\mathcal{Z}_{j})\cap S|=2$. Thus, for
		each $i\in\{1,...,m\}$ there exists a unique $j$ such that $x_{j,1}\notin S$.
		By (ii), then, for each $i\in\{1,...,m\}$ there exists a unique $j$ such that
		$|S\cap V(\mathcal{Z}_{j})|=2$. Hence $|S\cap(V(H)\cup(\bigcup_{i=1}%
		^{n}\mathcal{Z}_{i}))|\leq3n$. By (iii), $|S\cap V(\mathcal{Z}^{\ast})|\leq3$.
		Hence $|S|\leq3n+3<\Gamma(G)$, a contradiction.
	\end{enumerate}
	
	\noindent From (i)-(iv), $\mathcal{S}$ consists of all the $\Gamma$-sets of
	$G$. The proof proceeds as in Theorem \ref{thm:gamma-ID}. To construct other
	graphs with a $\Gamma$-graph of $H$, attach additional copies of $\mathcal{Z}$
	to any vertex of $V(H)$.
\end{proof}

%------------

\begin{comment}
	\section{Open problems}
	
	\nts{These are the same open problems as in paper. Update and add to Conclusion instead.}
	
	We concluded with a few open problems for future consideration.
	
	\begin{enumerate}
		\setlength{\parindent}{1pt} \setlength{\parskip}{1pt} 
		
		\item Determine conditions on the graph $G$ under which each $\gamma$-graph
		variation is connected/disconnected. 
		
		\item \emph{Reconfiguration problems} are a well-studied class of problems
		which examine the step-by-step transformation from one feasible solution to
		another, where feasibility is maintained at each intermediate step (see
		\cite{IDHPSUU11}). These problems are often represented as
		\emph{reconfiguration graphs}, where each vertex represents a feasible
		solution. As they represent the movement from one $\gamma$-set to another with
		each intermediate step also being a $\gamma$-set, $\gamma$-graphs and the
		variations presented in this paper are reconfiguration graphs. In the context
		of graph problems where the vertices of the reconfiguration graph
		$\mathcal{G}$ represent vertex subsets of a graph $G$, a vertex $v\in V(G)$ in
		a solution set $S$ is said to be \emph{stuck} if in $\mathcal{G}$, each
		neighbor $v_{S^{\prime}}$ of the vertex $v_{S}$ corresponding to $S$ in $G$
		has $v\in S^{\prime}$. A vertex $v\in S$ is \emph{frozen} if all vertices in
		the same component of $\mathcal{G}$ as $v_{S}$ correspond to sets also
		containing $v$. Under what conditions is a vertex stuck or frozen in each of
		the $\gamma$-graph variations? Moreover, when is $v$ in every $\gamma$-graph
		variation?
		%\item Characterize the graphs $G$ with the property that $|V(G(\gamma))| > |V(G)|$.
		
		
		\item Let $\pi$ be any of the above-mentioned domination-related parameters.
		Is it true that every \textbf{bipartite} graph is the $\pi$-graph of a
		\textbf{bipartite }graph?
		
		\item Study the nature of $i$-graphs, $\operatorname{IR}$-graphs, and $\alpha
		$-graphs, where $\operatorname{IR}(G)$ is the upper irredundance number and
		$i(G)$ and $\alpha(G)$ are the independent domination and independence numbers
		of $G$, respectively. (Depending on $H$, the graph $G$ constructed in the
		proof of Theorem \ref{thm:bigGamma} could have more $\operatorname{IR}$-sets
		than the order of $H$, and possibly also $\operatorname{IR}(G)>\Gamma(G)$.) In
		particular, determine whether all graphs are $i$-graphs, $\alpha$-graphs, or
		$\operatorname{IR}$-graphs. Consider other domination variations like Roman
		and Italian domination.
	\end{enumerate}
	
\end{comment}

%============================= SECTION : ROMAN / NEW WORK ======================================





\section{Roman and Total Roman Domination} \label{sec:s:roman}

%\nts{NEW STUFF: Roman works, total roman does not (and stops half way through proof).  Does suggested fix work?  Or change total roman to ``connected Roman"?  Or abandon?}


The final two variants of the $\gamma$-graph we examine are derived from the reconfiguration of Roman and Total Roman dominating functions.  These are new results, not found in \cite{MT18}.



Roman domination was first presented by Ian Stewart in 1999 in the popular science magazine \emph{Scientific American} \cite{Stew99}.  Stewart asked how the 4th-century Emperor Constantine could distribute the fewest of his Roman legions about the empire so that each settlement either had a legion stationed within it or was adjacent to a city with two legions. Thus, in the event of an attack, a city was either already protected, or could request aid from a neighbouring settlement with a spare legion. 



Unlike the previous domination variants we have  examined, Roman domination is not a set-inclusion problem.  Instead, a \emph{Roman dominating function} of a graph $G$ is a function $f: V(G)\rightarrow \{0,1,2\}$ such that each vertex $v$ has either $f(v) \geq 1$ or there exists some $w\in N(v)$ such that $f(w) =2$.  The \emph{cost} of a Roman   
dominating function $f$ is $c(f)  = \sum_{v\in V(G)} f(v)$, and the \emph{Roman domination number} is the minimum cost of a Roman dominating function $\gamma_R =  \min\{c(f):f \text{ is a Roman dominating function}\}$.  Going forward, we will assume all Roman dominating functions to be of minimum cost.  See \cite{CDHH04} for additional definitions and introductory results on Roman domination.

Since Roman domination is not a set-inclusion problem, we must alter our strategy for creating an analogous version of the $\gamma$-graph.  Each vertex of the \emph{$\gamma_R$-graph} corresponds to a (minimum cost) Roman dominating function $f$.  Two vertices of the graph are adjacent if and only if they correspond to Roman dominating functions $f$ and $g$ such that for some pair of adjacent vertices $u, w \in V(G)$, 
\begin{align*}
	\begin{cases}
		f(v) = g(v),		& \text{ if }	v\in  V(G) - \{u, w\}\\
		|f(v) - g(v)|=1,	   &	 \text{ if } v \in \{u, w\}.
	\end{cases}
\end{align*}


The token-sliding model becomes particularly useful here.  Since each vertex $v$ has $f(v) \in \{0,1,2\}$, we now allow for the possibility of 0, 1, or 2 tokens (representing that number of legions) to occupy a single vertex.  Each vertex of $G(\gamma_R)$ corresponds to a token configuration, where each vertex either has at least one token on it, or is adjacent to a vertex with two tokens on it.  Two vertices of $G(\gamma_R)$ are adjacent if their corresponding token configurations can be transformed from one into the other by sliding a single token along an edge of $G$.




% The  \emph{$\gamma_R$-graph of a graph $G$}, $G(\gamma_R)$ has $V(G(\gamma_R))$ 
% the \emph{$\gamma_R$-graph of a graph $G$}, $G(\gamma_R)$ similarly to $G(\gamma)$  
%The token-sliding model is also slightly modified: we now allow for the possibility of several tokens (representing several legions) to occupy a single vertex.  


Before we consider the realizability of $\gamma_R$-graphs, we first note the following observation regarding minimum cost Roman dominating functions.


%>>>Start: Obs {obs:s:ord2}
\begin{obs}\label{obs:s:ord2}
	Suppose that $f$ is a Roman dominating function of a graph $G$ of minimum cost and $uw$ is an edge in $G$.  If $f(u)=2$, then $f(w)\neq 1$.  Likewise, if $f(u)=1$, then $f(w) \neq 2$.
\end{obs}
% <<< E: Prop  {obs:s:ord2}

\noindent 
To see the observation, suppose otherwise.  If $f(u)=2$ and $f(w)=1$, then  each $v\in N[w] \backslash N[u]$, either has $f(v)=1$ or is adjacent to some $z \in V(G)$ such that $f(z)=2$.  That is, no vertex in the neighbourhood of $w$ is dominated by $w$ alone.  Thus, the function $g$ where for $v\neq w$, $g(v) =f(v)$ and $g(w)=0$, is also Roman dominating, and at lower cost, contradicting the minimality of $f$.  The second statement follows similarly.

Returning to the $\gamma_R$-graph, we finally depart from the trend of the rest of Chapter \ref{ch:slater}, and encounter a parameter where not every graph is realizable as a $\gamma_R$-graph.


%>>>Start: Prop {prop:s:notRomK2}
\begin{prop}\label{prop:s:notRomK2}
	$K_2$ is not a $\gamma_R$-graph.
\end{prop}


\begin{proof}
	Suppose to the contrary that there is some graph $G$ such that $G(\gamma_R) \cong K_2$.  Applying the token-sliding model, $K_2$ corresponds to two configurations of tokens on the vertices of $G$, say $f$ and $g$, where a single token slides from a vertex $u\in V(G)$ (under configuration $f$), to the vertex $w \in V(G)$ (under configuration $g$).  That is, $f(u) - g(u)=1$ and $f(w) - g(w)=-1$.
	
	If $f(u) = 1$, then by Observation \ref{obs:s:ord2}, $f(w)\neq 2$; likewise, for  each $v\in N(u)$, $f(v) \neq 2$.  If $f(w)=0$, then a token slide from $u$ to $w$ gives   $g(u)=0$, $g(w)=1$, and for each $v\in N(u) - \{w\}$ $g(v)\neq 2$, thus leaving $u$ not Roman-dominated by $g$.   Hence, we conclude that if $f(u)=1$, then $f(w)=1$.
	After the token slide, this leaves $g(u)=0$ and $g(w)=2$.  
	
	Since we have supposed (for contradiction) that a token move between $f$ and $g$ does exist, then there is no $v \in N(w) - \{u\}$ such that $v$ is Roman-dominated only by the two tokens at $w$ under $g$; otherwise, $f$ is not a Roman-dominating function.
	Therefore, instead of sliding the token at $u$ to $w$ in configuration $f$, nothing prevents the opposite: we  slide the token from $w$ to $u$, creating a third (Roman dominating) token configuration $h$, where $h(u)=2$, $h(w)=0$, and $h(v)=f(v)$ for all $v\in V(G) - \{u,w\}$. 
	Thus, the $\gamma_R$-graph of $G$ has at least three vertices, contradicting  that $G(\gamma_R) \cong K_2$.
	
	%If $f(u)=2$, then again by Observation \ref{obs:s:ord2}, for  each $v\in N(u)$, $f(v) \neq 2$, including $f(w)\neq 2$.
	
	Similar arguments show that if $f(u) = 2$, then  $f(w)=0$, and so $g(u)=1$, and $g(w)=1$, and once again, there exists some third configuration $h$, where $h(u)=0$, $h(w)=2$ and $h(v)=f(v)$ for all $v\in V(G) - \{u,w\}$. Again, this is  a contradiction. 
	We conclude that there is no graph $G$ such that  $G(\gamma_R) \cong K_2$.	
\end{proof}
% <<< E: Prop {prop:s:notRomK2}




Although Proposition \ref{prop:s:notRomK2} shows that not every graph is a $\gamma_R$-graph, examining a more restrictive variation of Roman domination leads to a surprisingly different outcome.  


A function $f: V(G)\rightarrow \{0,1,2\}$ is a \emph{total Roman dominating function} of a graph $G$ if it is a Roman dominating function and has the additional property that the subgraph of $G$ induced by $V^+_f := \{v \in V(G): f(v) > 0\}$ has no isolated vertices.  The \emph{cost} of a total Roman  dominating function $f$ is similarly defined as $c(f)  = \sum_{v\in V(G)} f(v)$, and the \emph{total Roman domination number} is the minimum cost of a total Roman dominating function $\gamma_{tR} =  \min\{c(f):f \text{ is a total Roman dominating function}\}$.  Going forward, we again assume all total Roman dominating functions to be of minimum cost.  

Now that the token-bearing vertices induce a  subgraph without isolated vertices, there is no result analogous to Observation \ref{obs:s:ord2} for total Roman dominating functions, and without that key observation, nothing prevents every graph from being a $\gamma_{tR}$-graph.


%>>>Start: Theorem {thm:s:totRom}
\begin{theorem} \label{thm:s:totRom}
	Every graph is the $\gamma_{tR}$-graph of some graph.
	
\end{theorem}	









%--- Start proof
\begin{proof}
	Given a graph $H$, we construct a graph $G$ such that $G(\gamma_{tR})\cong H$.	
	
	\noindent \underline{Construction:} The construction of a graph $G$ with  $G(\gamma_{tR})\cong H$ is similar to those given previously in this chapter (and in \cite{MT18}).
	Begin with a copy of the graph $H$ with $V(H)=\{v_{1}, v_{2}, \dots, v_{n}\}$.  For each $v_{i}$, add two copies of the star $K_{1,3}$ with vertices labelled $\mathcal{Z}_i=\{x_i, y_{i,1}, y_{i,2}, y_{i,3}\}$ and $\mathcal{Z}_i^*=\{x_i^*, y_{i,1}^*, y_{i,2}^*, y_{i,3}^*\}$, such that $x_i$ and $x_i^*$ are the centres of the stars with degree 3.  Then, for each $i\in \{1, 2,\dots, n\}$ connect each $v_i$ to each $x_i$ and $x_i^*$ with an edge.  Finally, add $2$ more vertices labelled $a$ and $b$, and connect every vertex in $H$ to both.  An example of this construction  is given in Figure \ref{fig:s:trCons}.
	
	
	%~~~~~~~~~~~~~~~~~~~~~~~~~FIG START~~~~~~~~~~~~~~~~~~~~~~
	\begin{figure}[H]
		\centering \scalebox{0.9}{
			\begin{tikzpicture}					
				%---------- H CORE  --------------- 		
				\node (cent) at (0,0) {};
				\fill[lgray, dashed] (0,0) circle (1.7cm);
				
				
				\foreach \i / \j in {1,2,3,4}
				{
					\path(cent) ++( \i*90-45: 14 mm) node[std]  (v\i) {};
					%					,label={  \i*90-45:$v_{\i}$}
				}	
				
				\draw[mgray](v1)--(v2)--(v3)--(v4)--(v1)--(v3);
				
				\draw[gray, dashed] (0,0) circle (1.7cm);
				\node (H) at (0,-1.4) [color=gray](L){$H$};				
				
				%---------- X Stems  --------------- 
				\foreach \i  in {1,2,3,4}
				{
					\path(v\i) ++( \i*90-55: 15 mm) node[std]  (x\i) {};
					\draw(x\i)--(v\i);
					
					%	\path(v\i) ++( \i*90-55: 25 mm) node[std]  (y\i2) {};
					%	\draw(x\i)--(y\i2);
					%,label={\i*90-45:$x_{\i}$}
					\foreach \j in {1,3}
					{						
						\path(v\i) ++( \i*90-45: 25 mm) node[std,label={ \i*90-65:$y_{\i,1}$}]  (y\i1) {};
						\path(v\i) ++( \i*90-55: 25 mm) node[std,label={ \i*90-75:$y_{\i,2}$}]  (y\i2) {};
						\path(v\i) ++( \i*90-65: 25 mm) node[std,label={ \i*90-85:$y_{\i,3}$}]  (y\i3) {};
						%	\path(x\i) ++( \i*90-105+\j*24: 10 mm) node[std,label={\i*90-105+\j*24:$y_{\i,\j}$}]  (y\i\j) {};
						\draw(x\i)--(y\i1);
						\draw(x\i)--(y\i2);
						\draw(x\i)--(y\i3);
					}					
				}	
				
				
				%---------- X* Stems  --------------- 
				\foreach \i  in {1,2,3,4}
				{
					\path(v\i) ++( \i*85: 15 mm) node[std]  (xs\i) {};
					%	,label={\i*90-45:$x^*_{\i}$}
					\draw(xs\i)--(v\i);
					
					%	\foreach \j in {1,2,3}
					%	{
						%		\path(xs\i) ++( \i*90-85+\j*24: 10 mm) node[std,label={\i*90-85+\j*24:$y^*_{\i,\j}$}]  (ys\i\j) {};
						%		\draw(xs\i)--(ys\i\j);
						%	}					
					
					\path(v\i) ++( \i*85-10: 25 mm) node[std]  (ys\i1) {};
					%				,label={ \i*85-10:$y_{\i,1}^*$}
					\path(v\i) ++( \i*85-12: 30 mm) node   (Lys\i1) {$y_{\i,1}^*$};
					%	\path (v1) ++(150:4mm)  node (Lv1) {$v_{1}$};
					\path(v\i) ++( \i*85: 25 mm) node[std]  (ys\i2) {};
					%				,label={ \i*85:$y_{\i,2}^*$}
					\path(v\i) ++( \i*85: 30 mm) node  (Lys\i2) {$y_{\i,2}^*$};
					\path(v\i) ++( \i*85+10: 25 mm) node[std]  (ys\i3) {};
					%				,label={ \i*85+10:$y_{\i,3}^*$}
					\path(v\i) ++( \i*85+12: 30 mm) node  (Lys\i3) {$y_{\i,3}^*$};
					%	\path(x\i) ++( \i*90-105+\j*24: 10 mm) node[std,label={\i*90-105+\j*24:$y_{\i,\j}$}]  (y\i\j) {};
					\draw(xs\i)--(ys\i1);
					\draw(xs\i)--(ys\i2);
					\draw(xs\i)--(ys\i3);
					
					
				}	
				
				%---------- Z* ------------------		
				\node (z) at (0:35mm) {};		
				
				\foreach \i/\j in {1/90, 2/270}
				{
					\path (z) ++(\j:2mm)  node[std ] (z\i) {};
					
					\foreach \j in {1, 2, 3, 4}
					{
						\draw(z\i)--(v\j);
					}
					
				}	
				
				
				%---------- LABEL FIX------------------
				\path (z1) ++(0:4 mm)  node (La) {$a$};
				\path (z2) ++(0:4 mm)  node (Lb) {$b$};
				
				
				\path (v1) ++(150:4mm)  node (Lv1) {$v_{1}$};
				\path (v2) ++(30:4mm)  node (Lv2) {$v_{2}$};
				\path (v3) ++(140:4mm)  node (Lv3) {$v_{3}$};
				\path (v4) ++(210:4mm)  node (Lxv4) {$v_{4}$};				
				
				\path (x1) ++(270:4mm)  node (Lx1) {$x_{1}$};
				\path (x2) ++(0:4mm)  node (Lx2) {$x_{2}$};
				\path (x3) ++(90:3mm)  node (Lx3) {$x_{3}$};
				\path (x4) ++(180:4mm)  node (Lx4) {$x_{4}$};
				
				\path (xs1) ++(180:3mm)  node (Lxs1) {$x_{1}^*$};
				\path (xs2) ++(260:4mm)  node (Lxs2) {$x_{2}^*$};
				\path (xs3) ++(0:4mm)  node (Lxs3) {$x_{3}^*$};
				\path (xs4) ++(90:4mm)  node (Lxs4) {$x_{4}^*$};
				
				
		\end{tikzpicture}}
		\caption{The graph $G$ constructed from $H$ in Theorem \ref{thm:s:totRom}.}%
		\label{fig:s:trCons}%
	\end{figure}
	%~~~~~~~~~~~~~~~~~~~~~~~~~FIG END~~~~~~~~~~~~~~~~~~~~~~
	
	
	
	%---------------
	We define the family of functions $\mathcal{F}=\{f_1, f_2, \dots, f_n\}$ for $1 \leq k \leq n$ by  
	
	\vspace{-5mm}
	
	\begin{align*}
		f_k(v) = \begin{cases} 2 & \text{ for }v  \in \{x_i, x_i^*\}, i=1,2,\dots,n, \\
			2 	&  \text{ for } v=v_k,\\
			1	& \text{ for } v=v_i, \text{ for } i\neq k,\\
			0&  \text{ for } v\in \{a,b\}.\\
		\end{cases}
	\end{align*}
	
	%$f_k(x_i)=f_k(x_i^*) = 2$ for each $i=1,2, \dots, n$, $f(a)=f(b)=0$, $f_k(v_k)=2$, and $f_k(v_i)=1$ for $i \neq k$.  
	\noindent 
	Then $c(f_k) = 5n+1$, and $f_k$ is  total Roman dominating.  We claim that the family $\mathcal{F}$ are all the least cost total Roman dominating functions of $G$.
	
	Let $g$ be a minimum total Roman dominating function, so that $c(g) \leq c(f_k)$.  To begin, we determine $g(v_i)$.
	Suppose $g(v_i)=0$ for some $i$.   Then, to totally Roman dominate the star $\mathcal{Z}_i$, $\sum_{v\in \mathcal{Z}_i} g(v) \geq 3$, and likewise $\sum_{v\in \mathcal{Z}_i^*} g(v) \geq 3$.  Define a function $g^*$ by
	
	\begin{align*}
		g^*(v) = \begin{cases} f_k(v) & \text{ for } v\in \mathcal{Z}_i \cup \mathcal{Z}_i^*, \\
			1 & \text{ for } v=v_i,\\
			g(v)  & \text{ otherwise.} \\
		\end{cases}
	\end{align*}
	
	
	\noindent Then $g^*$ is a total Roman dominating function of lower cost than $g$, contradicting that $g$ is of minimum cost.  Therefore, $g(v_i) \geq 1$ for each $i$.
	
	Suppose $g(v_i)=1$ for each $v_i$.  Then, to totally Roman dominate $a$ and $b$,  $g(a), g(b) \geq 1$.   Setting $g^*(a)=g^*(b)=0$, and $g^*(v_i)=2$ for any $i$, gives a total Roman dominating function of lower cost.  Therefore, $g(v_i)=2$ for at least one $i\in \{1,2,\dots,n\}$.
	
	
	%yields a total Roman dominating function $g^*$ of lower cost, a contradiction.
	
	
	Next, we determine $g(x_i)$.  Suppose now that	$g(x_i) < 2$.  Then, $\sum_{1\leq j \leq 3} g(y_{i,j}) \geq 3$.    Again, setting $g^*(x_i) = 2$ and $ g^*(y_{i,j}) =0$ for each $1\leq j \leq 3$, gives a total Roman dominating function of lower cost.  Hence $g(x_i)=2$, and similarly, $g(x_i^*)=2$ for each $i$.
	
	
	
	Since  $c(g) \leq c(f_k)$, it now follows easily that $g=f_k$ for some $k \in \{1,2,\dots,n\}$.  
	Thus,  $\gamma_{tR}(G) = 5n+1$, and that	$\mathcal{F}$ consists of all total Roman dominating functions of $G$.  Moreover, the vertex corresponding to $f_i$ in $\gamma_{tR}(G)$ is adjacent to the vertex corresponding to $f_j$ if and only if $v_i$ is adjacent to $v_j$ in $H$.  It follows that $G(\gamma_{tR})\cong H$ as required.	
\end{proof}

	In this chapter, we examined several variations on the $\gamma$-graph.  In each case, with the exception  of the $\gamma_R$-graph, we demonstrated that all graphs are $\pi$-graphs for their respective parameters $\pi$. 
Thus, the natural question to explore is what other parameters $\pi$ are like $\gamma_R$, in that not every graph is a $\pi$-graph?
For example, for the upper irredundance number $IR$, Mynhardt and Roux have shown that not all connected graphs are $IR$-graphs, but that all disconnected graphs are $IR$-graphs \cite{MR22B, MR22A}.	
For remainder of this dissertation we focus on a single such $\gamma$-graph variation, the $i$-graph, which like the $\gamma_R$-graph and the $IR$-graph, is not realizable for all graphs.



==> iGraphM.tex <==
\chapter{Introduction to $i$-Graphs}

\label{ch:igraphs}

%================================== SECTION: INTRO  =============================	
%\section{Introduction} \label{sec:GIDgraph}



%\spacing{1.5}   



%\nts{$ \ig{G} = H$.  For fuck sake, $G$ is the seed, $H$ is the $i$-graph.}

%================================== SECTION: INTRO  =============================	
%\section{Introduction} \label{sec:GIDgraph}

Having examined in Chapter \ref{ch:slater} several parameters $\pi$ with the property that every graph is a $\pi$-graph of some graph, we turn our attention now to a much more challenging variant: the $i$-graph. 


The \emph{$i$-graph} of a graph $G$, denoted $\ig{G}=(V(\ig{G}),E(\ig{G}))$, is the graph with vertices representing the minimum independent-dominating sets of $G$ (that is, the \emph{$i$-sets} of $G$).  As with the graphs in Chapter \ref{ch:slater}, adjacency in $\ig{G}$ follows a slide model where $u,v\in V(\ig{G})$, corresponding to the $i$-sets  $S_u$ and $S_v$, respectively, of $G$,  are adjacent in $\ig{G}$ if and only if there exists  $xy \in E(G)$ such that $S_u = (S_v-x)\cup\{y\}$.  We say $H$ is an $i$-graph (or is $i$-\emph{graph realizable}) if there exists some graph $G$ such that $\ig{G}\cong H$. Moreover, we refer to $G$ as the \emph{seed graph} of the $i$-graph $H$.  Going forward, we mildly abuse notation to denote both the $i$-set $X$ of $G$ and its corresponding vertex in $H$ as $X$, so that $X \subseteq V(G)$ and $X \in V(H)$.  





This version of a reconfiguration problem (and indeed, all of those discussed in Chapter \ref{ch:slater}) is also known as a \emph{token-sliding model}, where each $i$-set of $G$ can be imagined as a configuration of tokens lying on the vertices of a graph (see \cite{HIMNOST16,IDHPSUU11, MN20, SMN16}).  Two configurations are adjacent in $\ig{G}$ if and only if a single token can be slid along an edge of $G$ to transform one configuration into another.  Notice that the \emph{token-jump model} of reconfiguration for independent domination is identical to the token-slide model.  On a graph $G$ a token may only ``jump'' from a vertex $v$ in the $i$-set $S_1$ to another vertex $w$ (to form the $i$-set $S_2$) if $w$ is dominated only by $v$ in $S_1$.  Otherwise,  if $w$ is dominated by some other $u \neq v$ in $S_1$, then $(S_1-{u}) \cup \{w\}$ is not an independent set as it contains the adjacent vertices $u$ and  $w$.  A token is said to be \emph{frozen} (in any reconfiguration model) if there are no available vertices to which it may be  slid/jumped.


In acknowledgment of the slide-action in $i$-graphs, given $i$-sets  $X = \{x_1,x_2,\dots,x_k\}$ and $Y=\{y_1,x_2,\dots x_k\}$ of $G$ with $x_1y_1 \in E(G)$, we denote the adjacency of $X$ and $Y$ in $\ig{G}$ as $\edge{X,x_1,y_1,Y}$, where we imagine transforming the $i$-set $X$ into $Y$ by sliding the token at $x_1$ along an edge to $y_1$.  When discussing several graphs, we use the notation $\edgeG{X,x_1,y_1,Y,G}$ to specify that the relationship is on $G$.  
More generally, we use $x \sim y$ to denote the adjacency of vertices $x$ and $y$ (and $x\not \sim y$ to denote non-adjacency); this is used in the context of both the seed graph and the target graph.


Although the focus of this chapter is on the $i$-graph, for later comparison, we now also include the definition of the related \emph{$\agraph$-graph} of a graph $G$, denoted  $\ag{G}$.  The $\agraph$-graph is the slide reconfiguration graph with vertices representing the maximum independent sets of $G$ (that is, the $\alpha$-sets), and where adjacency is defined the same as in the $i$-graph.   In Chapter \ref{ch:comp}, we present several constructions for $i$-graphs that are also constructions for $\agraph$-graphs.


As the reader can likely surmise by noting that three chapters of this dissertation are dedicated to  $i$-graphs, there is no such  tidy theorem like those of Chapter \ref{ch:slater} for $i$-graphs; as we see later in this chapter, not every graph is an $i$-graph and determining which classes are (or are not) $i$-graphs has proven to be an interesting challenge.  

We begin our investigation into $i$-graph realizability in Section \ref{sec:i:obs} by composing a series of observations and technical lemmas concerning the adjacency of vertices in an $i$-graph and the structure of their associated $i$-sets in the seed graph.    In Section \ref{sec:i:Real}, we present the three smallest graphs which are not $i$-graphs,  and then in Section \ref{sec:i:basicGraphs}, we show that several common graph classes, like trees and cycles, are $i$-graphs.  Section \ref{sec:i:tools} concludes this chapter by considering $i$-graphs from the opposing view: when given a graph $G$ from a specific class, what is the resulting $i$-graph of $G$?


%================================== SECTION: Observations  =============================	
\section{Observations} \label{sec:i:obs}


To begin, we propose several observations about the structure of $i$-sets within given $i$-graphs, which we then use to construct a series of useful lemmas.

%>>>S Obs {obs:i:edge}
\begin{obs} \label{obs:i:edge}
	Let $G$ be a graph and $H=\ig{G}$.  A vertex $X \in V(H)$ has $\deg_H(X)\geq 1$ if and only if for some $v \in X \subseteq V(G)$, there exists $u\in epn(v,X)$ such that $u$ dominates $pn(v,X)$.  
\end{obs}
%<<<E Obs{obs:i:edge}

\noindent From a token-sliding perspective, Observation \ref{obs:i:edge} shows that a token on an $i$-set vertex $v$ is frozen if and only if $epn(v) = \varnothing$ or $G[epn(v,X)]$ has no dominating vertex.


For some path $X_1,X_2,\dots,X_k$ in $H$, at most one vertex of the $i$-set is changed at each step, and so $X_1$ and $X_k$ differ on at most $k$ vertices.  This is yields the following immediate observation.  

%>>>S Obs {obs:i:dist}
\begin{obs} \label{obs:i:dist}
	Let $G$ be a graph and $H = \ig{G}$.  Then for any $i$-sets $X$ and $Y$ of $G$, the distance $d_H(X,Y) \geq |X-Y|$.  
\end{obs}

%<<<E obs {obs:i:dist}



%>>>S  Lemma {lem:i:claw}
\begin{lemma} \label{lem:i:claw}
	Let $G$ be a graph with $H = \ig{G}$.  Suppose $XY$ and $YZ$ are edges in $H$ with $\edge{X,x,y_1,Y}$ and $\edge{Y,y_2,z,Z}$, with $X \neq Z$.  Then $XZ$ is an edge of $H$ if and only if $y_1=y_2$.
\end{lemma}

\begin{proof}
	Let $X=\{x,v_2,v_3\dots,v_k\}$ and $Y=\{y_1,v_2,,v_3\dots,v_k\}$ so that $\edge{X,x,y_1,Y}$.  	
	To begin, suppose $y_1=y_2$.  Then  $\edge{Y,y_1,z,Z}$ and $Z=\{z,v_2,,v_3\dots,v_k\}$, and $|X-Z|  = 1$.   Since $X$ is dominating, $z$ is adjacent to a vertex in $\{x,v_2,v_3\dots,v_k\}$; moreover, since $Z$ is independent, $z$ is not adjacent to any of $\{v_2,v_3,\dots v_k\}$.  Thus $z$ is adjacent to $x$ in $G$ and $\edge{X,x,z,Z}$, so that $XZ \in E(H)$.  
	
	Conversely, suppose $y_1\neq y_2$.  Then, without loss of generality, say $y_2=v_2$ and so $X=\{x,y_2,v_3\dots,v_k\}$, $Y=\{y_1,y_2,v_3\dots,v_k\}$, and $Z=\{y_1,z,v_3\dots,v_k\}$.  Notice that $x \neq z$ since $x \sim y_1$ and $z \not\sim y_1$.  Thus  $|X-Z| = 2$, and it follows that $XZ \notin E(H)$.
\end{proof}
%<<<E  Lemma {lem:i:claw}


\noindent Combining the results from Lemma \ref{lem:i:claw} with Observation \ref{obs:i:dist}, yields the following observation for vertices of $i$-graphs at distance two. 

%>>>S Obs {obs:i:d2}
\begin{obs} \label{obs:i:d2}
	Let $G$ be a graph and $H = \ig{G}$.  Then for any $i$-sets $X$ and $Y$ of $G$, if $d_H(X,Y) = 2$, then $|X-Y|=2$.  
\end{obs}
%<<<E Obs {obs:i:d2}




%>>>S: Lemma {lem:i:K1m}
\begin{lemma} \label{lem:i:K1m}  Let $G$ be a graph and  $H = \ig{G}$.  Suppose $H$ contains an induced $K_{1,m}$ with vertex set $\{X,Y_1,Y_2, \dots, Y_m\}$ and $\deg_H(X)=m$.  Let $i \neq j$.  Then in $G$:  
	\begin{enumerate}[itemsep=1pt, label=(\roman*)]
		\item $(X-Y_i) \neq (X-Y_j)$, \label{lem:K1m:a}
		\item  $|Y_i \cap Y_j| = i(G)-2$, and  \label{lem:K1m:b}
		\item $m \leq i(G)$. \label{lem:K1m:c}
	\end{enumerate}
\end{lemma}

\begin{proof}
	Suppose $\edge{X,x_i,y_i,Y_i}$ and $\edge{X,x_j,y_j,Y_j}$.  Then, $(X - Y_i) = \{x_i\}$ and $(X-Y_j) = \{x_j\}$.    From Lemma \ref{lem:i:claw}, since $Y_i \not\sim Y_j$, we have that $x_i \neq x_j$, which establishes Statement \ref{lem:K1m:a}.  Moreover, $Y_i \cap Y_j = X - \{x_i,x_j\}$, and so as these are $i$-sets, Statement \ref{lem:K1m:b} also follows.  Finally, for Statement \ref{lem:K1m:c},  again apply Lemma \ref{lem:i:claw}, $|\bigcap_{1\leq i \leq m} Y_i| = |X|-m = i(G)-m \geq 0$.
	\null \hfill
\end{proof}
% <<< E: Lemma {lem:i:K1m}




% >>>S:  Prop  {prop:i:C4struct}
\begin{prop} \label{prop:i:C4struct}
	Let $G$ be a graph and $H=\ig{G}$.  Suppose $H$ has an induced $C_4$ subgraph with vertices $X,A,B,Y$, where $XY, AB \notin E(H)$.   Then, without loss of generality, the set composition of $X,A,B,Y$ in $G$, and the edge labelling  of  the induced $C_4$ in $H$, are as in Figure \ref{fig:i:C4struct}.
\end{prop}

%~~~~~~~~~~~~FIG START~~~~~~~~~~~
\begin{figure}[H]
	\centering
	\begin{tikzpicture}[scale=0.8]
		\scriptsize
		\node[std,label={270:$Y=\{y_1,y_2,v_3,\dots,v_k\}$}] (y) at (0,0) {};
		\node[std,label={180:$A=\{y_1,x_2,v_3,\dots,v_k\}$}] (a) at (-2,2) {};
		\node[std,label={0:$B=\{x_1,y_2,v_3,\dots,v_k\}$}] (b) at (2,2) {};
		\node[std,label={90:$X=\{x_1,x_2,v_3,\dots,v_k\}$}] (x) at (0,4) {};
		
		\draw[thick] (x)--(a) node[midway,left=10pt,fill=white]{$\edge{X,x_1,y_1,A}$};
		\draw[thick] (x)--(b) node[midway,right=10pt,fill=white]{$\edge{X,x_2,y_2,B}$};
		\draw[thick] (a)--(y) node[midway,left=10pt,fill=white]{$\edge{A,x_2,y_2,Y}$};
		\draw[thick] (b)--(y) node[midway,right=10pt,fill=white]{$\edge{B,x_1,y_1,Y}$};
	\end{tikzpicture}			
	\caption{Reconfiguration structure of an induced $C_4$ subgraph from Proposition \ref{prop:i:C4struct}.}
	\label{fig:i:C4struct}%
\end{figure}
%~~~~~~~~~~~~~FIG END~~~~~~~~~~~~~

\begin{proof}
	Suppose that the $i$-set $X$ of $G$ has $X=\{x_1,x_2,v_3,\dots,v_k\}$. 
	Then by Lemma \ref{lem:i:claw}, without loss of generality, the edge from $X$ to $A$ can be labelled as $\edge{X,x_1,y_1,A}$ for some $y_1 \in V(G) - X$, so that $A = \{y_1,x_2,v_3,\dots,v_k\}$, while the edge from $X$ to $B$ can be labelled $\edge{X,x_2,y_2,B}$ for some $y_2$ and $B=\{x_1,y_2,v_3,\dots,v_k\}$.  
	
	Consider now the edge $AY \in E(H)$ labelled $\edge{A,a,y^*,Y}$.  From Lemma \ref{lem:i:claw}, since  $XY \notin E(G)$, $a \neq y_1$.  If, say, $a=v_3$, then $Y=\{y_1,x_2,y^*,\dots,v_k\}$.  However, neither $y_1$ nor $x_2$ is in $B$, so $|Y-B| \geq 2$, a contradiction of Observation \ref{obs:i:dist}.  	
	Thus, $a \neq v_i$ for any $3 \leq i \leq k$.  This leaves $a=x_2$, and $Y=\{y_1,y^*,v_3\dots,v_k\}$.  Since $|Y-B|=1$, $y^*=y_2$ and $Y=\{y_1,y_2,v_3,\dots,v_k\}$   as required.
\end{proof}
% <<< E:  Prop  {prop:i:C4struct}


Finally, given an $i$-graph $G$ with $i$-sets $X$ and $Y$, and vertices $x_1 \in X$ and $y_1 \in Y$, we define a relation $\mathcal{R}_i$ on the ordered pairs $(X,x_1)$ and $(Y,y_1)$ so that $(X,x_1)\mathcal{R}_i (Y,y_1)$ if and only if $(X,x_1)=(Y,y_1)$, $\edge{X,x_1,y_1,Y}$. First notice that $\mathcal{R}_i$ is symmetric: if  $\edge{X,x_1,y_1,Y}$, the slide of the token previously at $x_1$ to $y_1$ can be reversed, so that   $\edge{Y,y_1,x_1,X}$.  Moreover, Lemma \ref{lem:i:claw} confirms that $\mathcal{R}_i$ is also transitive.  Since reflexivity is embedded in the definition, the following observation is immediate.

\begin{obs}\label{obs:i:equiv}
	The relation $\mathcal{R}_i$ is an equivalence relation.  The equivalence classes correspond to the components of the resulting $i$-graph.
\end{obs}

%Moreover, the equivalence classes correspond to the components of the $i$-graph.


%================================== SECTION: REALIZABILITY  =============================	
\section{Realizability of $i$-Graphs} \label{sec:i:Real}
%----------------------SUBSEC: NON REALIZABILITY  ----------------------------------------------------

Having now established  a series of observations and lemmas about the structures of $i$-graphs and the composition of their associate $i$-sets, we demonstrate that not all graphs are $i$-graphs by presenting three counterexamples: the diamond graph $\Dia$, $K_{2,3}$ and $\kappa$, as pictured in Figure \ref{fig:3nonReal}.


%~~~~~~~~~~~~~~~~~~~~~~~~~FIG START~~~~~~~~~~~~~~~~~~~~~~
\begin{figure}[H]
	\centering
	\begin{figure}[H]
		\centering
		\begin{tikzpicture}%[line width=0.3mm,scale=1]			
			
			%---------- REF-------------------
			\node(cent) at (0,0) {};			
			\path (cent) ++(180:35 mm) node(lcent)  {};	
			
			\path (lcent) ++(90:10 mm) node[std](x)  {};	
			\path (x) ++(90: 4mm) node (xL)  {$X$};
			\path (lcent) ++(-90:10 mm) node[std](y)  {};
			\path (y) ++(-90: 4mm) node (zL)  {$Y$};
			\path (lcent) ++(180:8 mm) node[std](a)  {};
			\path (a) ++(180: 4mm) node (aL)  {$A$};
			\path (lcent) ++(0:8 mm) node[std](b)  {};
			\path (b) ++(0: 4mm) node (bL)  {$B$};
			
			\draw(x)--(y)--(a)--(x);
			\draw(x)--(b)--(y);
			
			\path (lcent) ++(-90: 24mm) node (GL)  {$\Dia=K_4-e$};	
			
			%---------- REF-------------------
			
			\path (cent) ++(90:10mm) node[std](x)  {};
			\path (x) ++(90: 4mm) node (xL)  {$X$};
			\path (cent) ++(-90:10 mm) node[std](y)  {};
			\path (y) ++(-90: 4mm) node (yL)  {$Y$};
			\path (cent) ++(180:8 mm) node[std](a)  {};
			\path (a) ++(180: 4mm) node (aL)  {$A$};
			\path (cent) ++(0:8 mm) node[std](c)  {};
			\path (c) ++(0: 4mm) node (cL)  {$C$};
			\path (cent) ++(0:0 mm) node[std](b)  {};
			\path (b) ++(0: 4mm) node (bL)  {$B$};
			
			\draw(x)--(a)--(y)--(c)--(x)--(b)--(y);
			
			\path (cent) ++(-90: 24mm) node (GL)  {$K_{2,3}$};			
			
			%---------- REF-------------------
			
			\path (cent) ++(0:35 mm) node[std](brcent)  {};	
			\path (brcent) ++(0: 4mm) node (bL)  {$B$};			
			
			\path (brcent) ++(90:10mm) node[std](x)  {};	
			\path (x) ++(90: 4mm) node (xL)  {$X$};
			\path (brcent) ++(-90:10 mm) node[std](y)  {};
			\path (y) ++(-90: 4mm) node (yL)  {$Y$};
			\path (brcent) ++(180:8 mm) node[std](a)  {};
			\path (a) ++(180: 4mm) node (aL)  {$A$};
			\path (brcent) ++(0:8 mm) node (b)  {};
			
			\path (b) ++(90:4 mm) node[std](b1)  {};
			\path (b1) ++(0: 4mm) node (bL)  {$C_1$};
			\path (b) ++(-90:4 mm) node[std](b2)  {};
			\path (b2) ++(0: 4mm) node (bL)  {$C_2$};
			
			\draw(x)--(y)--(a)--(x);
			\draw(x)--(b1)--(b2)--(y);
			
			
			\begin{comment}
				\path (cent) ++(0:35mm) node(rcent)  {};
				\path (rcent) ++(90:8mm) node[std](x)  {};
				\path (x) ++(0:8 mm) node[std](x1)  {};
				\path (x) ++(180:8mm) node[std](x2)  {};
				
				\path (rcent) ++(270:8 mm) node(mid)  {};
				\path (mid) ++(0:6 mm) node[std](y1)  {};
				\path (mid) ++(180:6 mm) node[std](y2)  {};
				\path (rcent) ++(180:7mm) node[std](z)  {};
				
				\draw(y2)--(x)--(y1);
				\draw(y2)--(x1)--(y1);
				\draw(y2)--(x2)--(y1);
			\end{comment}
			
			\path (brcent) ++(-90: 24mm) node (GL)  {$\kappa: K_{2,3}$ with an};
			\path (brcent) ++(-90: 30mm) node (GL)  {edge subdivision};
		\end{tikzpicture}	
	\end{figure}			
	\caption{Three graphs not realizable as $i$-graphs.}
	\label{fig:3nonReal}%
\end{figure}
%~~~~~~~~~~~~~~~~~~~~~~~~~FIG END~~~~~~~~~~~~~~~~~~~~~~


%>>>S: Prop {prop:i:diamond}
\begin{prop} \label{prop:i:diamond}
	The diamond graph $\Dia = K_4-e$ is not $i$-graph realizable.
\end{prop}

\begin{proof}
	Suppose to the contrary there is some graph $G$ with $\ig{G}=\Dia$.  Let $V(\Dia)=\{X,A,B,Y\}$ where $AB \notin E(\Dia)$.   Say $\edge{X,x,y,Y}$.  Then by Lemma \ref{lem:i:claw}, without loss of generality, the incident edges with $A$ can be labelled as $\edge{X,x,a,A}$ and $\edge{A, a,y,Y}$.  Likewise, $\edge{X,x,b,B}$ and $\edge{B, b,y,Y}$ (see Figure \ref{fig:3nonReal}).  However,  since $\edge{B, b,x,X}$ and $\edge{X,x,a,A}$, Lemma \ref{lem:i:claw} implies that $AB\in E(\Dia)$, a contradiction.	  
\end{proof}
% <<< E: Prop {prop:i:diamond}


%>>>S: Prop {prop:i:K23}
\begin{prop} \label{prop:i:K23}
	The graph $K_{2,3}$ is not $i$-graph realizable.
\end{prop}

\begin{proof}
	Suppose $K_{2,3} = \ig{G}$ for some graph $G$.  Let  $ \{\{X,Y\},\{A,B,C\}\}$ be the bipartition of $K_{2,3}$. 
	To begin, apply the exact labelling from Proposition \ref{prop:i:C4struct} and Figure \ref{fig:i:C4struct} to the $i$-sets and edges of  $X,A,B,$ and $Y$.  We attempt to extend the labelling to $C$.  By Lemma \ref{lem:i:claw}, since $C$ is adjacent to $X$, but not $A$ nor $B$,  without loss of generality, $\edge{X, v_3,c,C}$ and $C=\{x_1,x_2,c,v_4,\dots,v_k\}$.  As $A$ is an $i$-set, $y_1v_3\notin E(G)$.   Since $v_3c\in E(G)$, $c \neq y_1$.  Similarly, $c \neq y_2$.  
	Now $|C-Y| =3$ and $d(C,Y)=1$, contradicting Observation \ref{obs:i:dist}.   	
\end{proof}

% <<< E: Prop {prop:i:K23}


% >>> S: Prop {prop:i:kappa}
\begin{prop} \label{prop:i:kappa}
	The graph $\kappa$ is not $i$-graph realizable.
\end{prop}


\begin{proof}
	Suppose $\kappa = \ig{G}$ for some graph $G$ and let $V(\kappa) = \{X,A,B,C_1,C_2,Y\}$ as in  Figure  \ref{fig:3nonReal}, and to the subgraph induced by $X,A,B,Y$, apply the labelling of Proposition \ref{prop:i:C4struct} and Figure \ref{fig:i:C4struct}.  Through additional applications of Proposition \ref{prop:i:C4struct}, we can as in the proof of Proposition \ref{prop:i:K23}, without loss of generality, assume $\edge{X,x_3,y_3,C_1}$.  However, $d(C_1,Y)=2$ but $|Y-C_1|=3$, contradicting Observation \ref{obs:i:dist}.  It follows that no such $G$ exists and $\kappa$ is not an $i$-graph.
\end{proof}




% <<< E: Prop {prop:i:kappa}

The observant reader will have undoubtedly noticed the common structure between the graphs in the previous three propositions; they are all members of the class of \emph{theta graphs} \label{i:pg:theta} (see \cite {B72}), graphs that are the union of three internally disjoint paths with the same two distinct end vertices (not to be confused with the Theta graph, or $\Theta$-graph, of computation geometry introduced by Clarkson \cite{clarkson87}).  The graph $\thet{j,k,\ell}$ with $j \leq k \leq \ell$, is the theta graph with paths of lengths $j$, $k$,  and $\ell$.  In this notation, our three non $i$-graph realizable examples are $\Dia \cong \thet{1,2,2}$, $K_{2,3}\cong\thet{2,2,2}$, and $\kappa \cong \thet{2,2,3}$.


Further rumination on the similarity in structure suggests that additional subdivisions of the central path in $\kappa$ could yield more graphs that are not $i$-graphs.  However, the proof technique used for $\kappa$ no longer applies when the central path between the starting and ending vertices is longer than four vertices.  In Chapter \ref{ch:comp}, we explore an alternative method for determining the $i$-realizability of theta graphs.




%---------------------------------------SECTION: REALIZABILITY ----------------

\section{Some Classes of $i$-Graphs}
\label{sec:i:basicGraphs}


Having studied several graphs that are not $i$-graphs, we now examine the problem of $i$-graph realizability from the positive direction.  To begin, it is easy to see that complete graphs are $i$-graphs; moreover, as with $\gamma$-graphs, complete graphs are their own $i$-graphs with $\ig{K_n} \cong K_n$.  

\begin{prop} \label{prop:comp} 
	Complete graphs are $i$-graph realizable. 
\end{prop}



\noindent  Hypercubes $Q_n$ (the Cartesian product of $K_2$ taken with itself $n$ times) are also straightforward to construct as $i$-graphs, with $\ig{nK_2} \cong Q_n$.  Each $K_2$ pair can be viewed as a $0-1$ switch, with the vertex of the $i$-set in each component sliding between the two states.

\begin{prop} \label{prop:hCube} 
	Hypercubes are $i$-graph realizable. 
\end{prop}


\noindent  Hypercubes are a special case of the following result regarding Cartesian products of $i$-graphs.

% >>> S: Prop {prop:i:cart}
\begin{prop} \label{prop:i:cart}
	If $\ig{G_1} \cong H_1$ and $\ig{G_2} \cong H_2$, then $\ig{G_1 \cup G_2} \cong H_1 \boksie H_2$
\end{prop}

\begin{proof}
	Let $\{X_1, X_2, \dots, X_k\}$ be the $i$-sets of $G_1$ and let $\{Y_1, Y_2, \dots, Y_{\ell}\}$ be the $i$-sets of $G_2$.  Then, the $i$-sets of $G_1 \cup G_2$ are of the form $X_i \cup Y_j$.  Clearly $\edgeG{X_i\cup Y_j,,,X^*_{i^*}\cup Y^*_{j^*},G_1 \cup G_2}$ if and only if $\edgeG{X_i,,,X^*_i,G}$ and $Y_j = Y_j^*$, or $\edgeG{Y_j,,,Y_j^*,G_2}$ and $X_i=X_i^*$.		This gives a natural isomorphism to $H_1 \boksie H_2$, where $X_i \cup Y_j$ is the vertex $(X_i,Y_j)$.
\end{proof}	




\noindent Moving to cycles, the constructions become markedly more difficult.  

% >>> S: Prop {prop:i:cycle}
\begin{prop} \label{prop:i:cycle} 
	Cycles are $i$-graph realizable. 
\end{prop}


\begin{proof}	
	The constructions for each cycle  $C_k$ for $k \geq 3$ are as described below.	
	\begin{enumerate}[itemsep=1pt, label=\bf (\roman*)]
		\item  $\ig{C_3} \cong C_3$ \\
		From Proposition \ref{prop:comp}.
		
		\item  $\ig{2K_2} \cong C_4$\\			
		From Proposition \ref{prop:hCube}. 
		
		
		\item $\ig{C_5} \cong C_5$\\		
		Recall that $i(C_5)=2$.  A labelled $C_5$ and the resulting $i$-graph with $\ig{C_5}\cong C_5$ are given in Figure \ref{fig:i:C5C5} below.
		
		%~~~~~~~~~~~~~~~~~~~~~~~~~FIG START~~~~~~~~~~~~~~~~~~~~~~
		\begin{figure}[H]
			\centering
			\begin{tikzpicture}	
				
				%---------- REF-------------------
				%	\fill[lgray, dashed] (0,0) circle (1.7cm);
				\node (cent) at (0,0) {};
	
				% ---------- C5 - LEFT--------
				\path (cent) ++(0:0 mm) node (C1)  {};		
				
				\foreach \i/\c in {1/90/, 5/162, 4/234, 3/306, 2/378} {
					\path (C1) ++(\c:10 mm) node[std] (v\i)  {};
					\path (v\i) ++(\c:5 mm) node (vL\i) {$x_{\i}$};  
					
				}			
				
				\draw (v1)--(v2)--(v3)--(v4)--(v5) --(v1);	
				
				% ---------- C5 --------
				\path (cent) ++(0:60 mm) node (C2)  {};		
				
				\foreach \i/\c/\x/\y in {1/90/1/4, 2/162/1/3, 3/234/3/5, 4/306/2/5, 5/378/2/4} {
					\path (C2) ++(\c:10 mm) node[std] (u\i)  {};
					\path (u\i) ++(\c:8 mm) node (uL\i) {$\{x_{\x},x_{\y}\}$};  
					
				}
				
				\draw (u1)--(u2)--(u3)--(u4)--(u5) --(u1);	
				
				
			\end{tikzpicture}			
			\caption{ $C_5$ and $\ig{C_5}\cong C_5$.}
			\label{fig:i:C5C5}%
		\end{figure}
		%~~~~~~~~~~~~~~~~~~~~~~~~~FIG END~~~~~~~~~~~~~~~~~~~~~~
		
		\newpage
		
		\item  $\ig{K_2 \boksie K_3} \cong C_6$		
		
		\noindent	Let $V(K_2 \boksie K_3) = \{x_1, x_2,x_3, y_1,y_2,y_3\}$, where the $x_i$'s and $y_i$'s form the $K_3$'s and $x_iy_i \in E(K_2 \boksie K_3)$ for each $1 \leq i \leq 3$.  The set $\{x_i,y_j\}$ is an $i$-set of $K_2 \boksie K_3$ if and only if $i \neq j$, so that $|V(\ig{K_2 \boksie K_3})| = 6$, and adjacencies are as in Figure \ref{fig:i:C6} below. 
		
		%~~~~~~~~~~~~~~~~~~~~~~~~~FIG START~~~~~~~~~~~~~~~~~~~~~~
		\begin{figure}[H]
			\centering
			\begin{tikzpicture}	
				
				%---------- REF-------------------
				%	\fill[lgray, dashed] (0,0) circle (1.7cm);
				\node (cent) at (0,0) {};
				%	\node [std](mid) at (cent)[label=above:$*$] {};	
				%\draw[gray, dashed] (0,0) circle (1.7cm);
				%\node (H) at (0,-1.4) [color=gray](L){$G$};	
				
				%---------- K2 K3 ------------------			
				\foreach \i/\c in {3/-10,2/-20,1/-30} {
					\path (cent) ++(\c mm, -5 mm) node[std] (x\i)  {};
					\path (x\i) ++(270:5 mm) node (xL\i) {$x_{\i}$};
					\path (cent) ++(\c mm, 5 mm) node[std] (y\i) {};
					\path (y\i) ++(90:5 mm) node (yL\i) {$y_{\i}$};
					\draw (x\i)--(y\i);				
				}
				
				\draw(x1)--(x3);
				\draw(y1)--(y3);
				
				\draw(x1) to [out=-20,in=200](x3);
				\draw(y1) to [out=20,in=160](y3);				
				
				% ---------- C6 --------
				\path (cent) ++(0:40 mm) node (C2)  {};		
				
				\foreach \i/\c/\x/\y in {1/90/1/2, 2/150/1/3, 3/210/2/3, 4/270/2/1, 5/330/3/1, 6/30/3/2} {
					\path (C2) ++(\c:10 mm) node[std] (u\i)  {};
					\path (u\i) ++(\c:8 mm) node (uL\i) {$\{x_{\x},y_{\y}\}$};  
					
				}
				
				\draw (u1)--(u2)--(u3)--(u4)--(u5)--(u6)--(u1);	
				
				
			\end{tikzpicture}			
			\caption{ $K_2 \; {\scriptstyle\square} \; K_3$ and $\ig{K_2 \; {\scriptstyle\square} \; K_3} \cong C_6$.}
			\label{fig:i:C6}%
		\end{figure}
		%~~~~~~~~~~~~~~~~~~~~~~~~~FIG END~~~~~~~~~~~~~~~~~~~~~~
		
		
		%	\item $\ig{C_k} \cong C_k$ for $k \equiv 1,2 \Mod 3$, $k \geq 5(?)$.  			
		
		\item \emph{For any $k \geq 7$, construct the graph $H$ with $V(H) = \{v_0,v_1, \dots,v_{k-1}\}$, and $v_iv_j \in E(H)$ if and only if $j \not\equiv i-2, i-1,i,i+1,i+2 \Mod k$.  Then $\ig{H} \cong C_k$.} 		
		
		
		For convenience, we assume that all subscripts are given modulo $k$.  Thus in $H$, for all $0 \leq i \leq k-1$, we have the following:
		\begin{enumerate}[label=(\Roman*)]
			\item $N[v_i] \backslash N[v_{i+1}] = \{v_i,v_{i+3}\}$ \label{prop:i:cycle:k:1}
			\item $N[v_{i+1}] \backslash N[v_i] = \{v_{i-2}, v_{i+1}\}$. \label{prop:i:cycle:k:2}
		\end{enumerate}
		
		 Since $H$ is vertex-transitive, suppose that $v_i$ is in some $i$-set $S$.  Then $v_{i-2},v_{i-1},v_{i+1},$ and $v_{i+2}$ are not dominated by $v_i$.  To dominate $v_{i+1}$, either $v_{i+1}$ or $v_{i-2}$ is in $S$, because all other vertices in $N[v_{i+1}]$ are also adjacent to $v_i$, as in \ref{prop:i:cycle:k:2}.  Begin by assuming that $v_{i+1} \in S$.  Now since $\{v_i,v_{i+1}\}$ dominates all of $H$ except $v_{i+2}$ and $v_{i-1}$, and $N({v_{i+2},v_{i-1}}) \subseteq N(v_i,v_{i+1})$, either $v_{i+2}$ or $v_{i-1}$ is in $S$.  Thus $S = \{v_i,v_{i+1},v_{i+2}\}$ or $S = \{v_{i-1},v_i,v_{i+1} \}$.
		
		Suppose now instead that $v_{i-2} \in S$.     Now, only $v_{i-1}$ is not dominated by $\{v_i, v_{i-2}\}$; moreover, since $N(v_{i-1}) \subseteq N(\{v_{i-2}, v_{i}\})$, we have that $v_{i-1} \in S$, and so  $S = \{v_{i-2}, v_{i-1}, v_i\}$.
		Combining the above two cases yields that $i(H) =3$ and that all $i$-sets of $H$ have the form $S_i=\{v_i, v_{i+1}, v_{i+2}\}$, for each $ 0  \leq i \leq k-1$.  Moreover, as there are $k$ unique such sets, it follows that $|V(\ig{H})| = k$.  
		
		
		We now consider the adjacencies of $\ig{H}$.  From our set definitions,  $\edge{S_i, v_{i-1}, v_{i+2}, S_{i+1}}$, and $\edge{S_i, v_{i+1}, v_{i-2}, S_{i-1}}$.  To see that $S_i$ is not adjacent to any other $i$-set in $H$, notice that the token at $v_i$ is frozen; $N(v_i)) \subseteq (N(v_{i-1}) \cup N(v_{i+1}))$.  Moreover, by \ref{prop:i:cycle:k:2}, the token at $v_{i+1}$ can only slide to $v_{i-2}$, and likewise, the token at $v_{i-1}$ can only slide to $v_{i+2}$.  Thus $\adjL{S_i,S_{i+1},S_{i-1},S_{i}}$, and so $\ig{H} \cong C_k$ as required.	
	\end{enumerate}		
	This completes the $i$-graph constructions for all cycles.
\end{proof}

%\vspace{-1cm}
	

% <<< E: Prop {prop:i:cycle}

The constructions presented in Proposition \ref{prop:i:cycle} are, of course, not unique.  Later in this chapter, we show that for $k \geq 5$ and $k \equiv 2 \Mod 3$, $\ig{C_k} \cong C_k$.  Moreover, in Chapter \ref{ch:comp}, we  demonstrate how graph complements can be used to construct graphs with $i$-graphs that are cycles.   

We now present three lemmas with the eventual goal of demonstrating that all forests are $i$-graphs.  When considering the  $i$-graph of some graph  $H$, if a vertex $v$ of some $i$-set $S$ of $H$ has no external private neighbours, then the token at $v$ is frozen.  In the first of the three lemmas,  Lemma \ref{lem:epnAdd}, we construct a new seed graph for a given target graph, where each vertex of the seed graph's $i$-set has a non-empty private neighbourhood.  Ironically, although the addition of external private neighbours initially unfreezes tokens in the seed graph, we later use this lemma in a construction to force tokens into a certain configuration.


%>>> S: Lemma {lem:epnAdd}
\begin{lemma} \label{lem:epnAdd}
	For any graph $H$, there exists a graph $G$ ($G \not\cong H$) such that $\ig{G} \cong \ig{H}$ and for any $i$-set $S$ of $G$, all $v\in S$ have $epn(v,S) \neq \varnothing$.
\end{lemma}


\begin{proof}
	Suppose $S$ is such an $i$-set of $H$ having some $v \in S$ with $epn(v,S) = \varnothing$.  Construct the graph $G_1$ from $H$ by joining new vertices $a$ and $b$ to each vertex of $N[v]$.  
	
	To begin, we show that the $i$-sets of $G_1$ are exactly the $i$-sets of $H$.  Let $R$ be some $i$-set of $H$ and say that $v$ is dominated by $u\in R$.  Then $u \in N[v]$, so $u$ also dominates $a$ and $b$ in $G_1$; therefore, $R$ is independent and dominating in $G_1$, and so $i(G_1) \leq i(H)$.  Conversely, suppose that $Q$ is an $i$-set of $G_1$.  If neither $a$ nor $b$ is in $Q$, then $Q$ is an independent dominating  set of $H$, and so $i(H) \leq i(G_1)$.  Hence, suppose instead that $a \in Q$.  Notice that since $Q$ is independent and $a$ is adjacent to each vertex in $N(v)$, $N_H[v] \cap Q = \varnothing$.  Some vertex in $Q$ dominates $b$; however, since $N_H(a) = N_H(b)$ and $Q$ is independent, it follows that $b$ is self-dominating and so $b\in Q$.  	
	However, since $N_{G_1}[\{a,b\}] = N_{G_1}[v]$, the set $Q' = (Q - \{a,b\}) \cup \{v\}$ is an independent dominating set of $G_1$ such that $|Q'| < |Q|$, a contradiction.  Thus, $i(G_1) = i(H)$ and the $i$-sets of $H$ and $G_1$ are identical.  In particular, $S$  is an $i$-set of $G_1$, and moreover, $epn_{G_1}(v,S) = \{a,b\}$.	
	
	By repeating the above process for each $i$-set of $G_i$, $i\geq 1$, containing a vertex $v$ with $epn(v,S) = \varnothing$, we eventually obtain a graph $G=G_k$ such that for each $i$-set of $S$ of $G$ and each vertex $v \in S$, $epn_G(v,S) \neq \varnothing$.  Since the $i$-sets of $H$ and $G$ are identical and $H$ is a subgraph of $G$, $\ig{G} = \ig{H}$ as required.  	
\end{proof}
% <<< E: Lemma  {lem:epnAdd}


Next on our way to constructing forests, we demonstrate that given an $i$-graph, the resultant graph obtained by adding any number of isolated vertices is also an $i$-graph.  



%\nts{G and H backwards}

%>>> S: Lemma {lem:vAdd}
\begin{lemma} \label{lem:vAdd}
	%If $G$ is the $i$-graph of some graph $H$, then there exists some graph $H^*$ such that $\ig{H^*} = G \cup \{v\}$. 
	If $H$ is the $i$-graph of some graph $G$, then there exists some graph $G^*$ such that $\ig{G^*} = H \cup \{v\}$.  
\end{lemma}

%\nts{NEEDS A PROOF HERE}

%\nts{PROOF SUMMARY:}  Take $H \vee W$ (the join) where $W$ is a new vertex set of size $i$.
%** be careful, this only works if original $i \geq 2$.  


\begin{proof}
	First, assume that $i(G) \geq 2$.  Let $V(G) = \{v_1, v_2, \dots, v_n\}$ and let $W$ be an independent set of size $i(G)=k$ disjoint from $V(G)$, say $W=\{w_1, w_2, \dots, w_k \}$.  Construct a new graph $G^*$ by taking the join of $G$ with the vertices of $W$, so that $G^* = G \vee W$.  
	
	
	%	\nts{Add figure?}
	
	Notice that $W$ is independent and dominating in $G^*$.  Moreover, if an $i$-set $S$ of $G^*$ contains any vertex $w_i$ of $W$, since $W$ is independent and each vertex of $W$ is adjacent to all of $\{v_1, v_2, \dots, v_n\}$, it follows that $S$ contains all of $W$, and so, $S=W$.  That is, if an $i$-set of $G^*$ contains any vertex of $W$, it contains all of $W$.  Thus, $i(G) = i(G^*)$. 
	Furthermore, any $i$-set of $G$ is also an $i$-set of $G^*$, and so the $i$-sets of $G^*$ comprise of $W$ and the $i$-sets of $G$.  That is, $V(\ig{G^*}) = V(\ig{G}) \cup \{W\} = V(H) \cup \{W\}$.
	
	If $S$ is an $i$-set of $G$, $S \cap W = \varnothing$.  Thus, $W$ is not adjacent to any other $i$-set $\ig{G^*}$.  	 Relabelling the vertex representing the $i$-set $W$ in $G^*$ as $v$ in $\ig{G^*}$ yields  $\ig{G^* } = H \cup \{v\}$ as required.
	
	%	Let $S$ be an $i$-set of $G$, then $S$ is independent and dominating in $G^*$, and so, $i(G^*) \leq i(G)$.    
	%On the other hand, suppose that $S$ is an $i$-set of $G^*$ such that $S \cap W \neq \varnothing$; say, $w_i\in S \cap W$.  Then since $W$ is independent and $w_i$ is adjacent to all of $\{v_1, v_2, \dots, v_n\}$, in order for $W - \{w_i\}$ to the be dominated in $S$, we have that $W \subseteq S$.  Since $W$ is independent and dominating, $S=W$, and so $i(G^*) = k = i(G)$.
	
	% Notice that since $W$ is independent, if any vertex of $W$ is in $S$, then to dominate $W$, all of $W$ is in $S$; that is $W \subseteq S$.  
	
	%	This the $i$-sets of $G^*$ are the $i$-sets of $G$ and the set $W$.  
	
	
	%	 If $S \cap W \neq \varnothing $, say $w_i \in S \cap W$,  then since $w_i$ is adjacent to all of  $ \{v_1, v_2, \dots, v_n\}$, it follows that $S \cap \{v_1, v_2, \dots, v_n\} = \varnothing$.  Then, since  $W$ is independent, in order to dominate $W$, $W \subseteq S$.  In particular, $W = S$.  
	
	
	%	Since each vertex of $W$ is adjacent to each of $\{v_1,v_2,\dots, v_n\}$, $i(G^*) = i(G)$, and each $S$ that is an $i$-set of $G$, is also an $i$-set of $G^*$. 
	
	
	%	Note that $W$ is an $i$-set of $G^*$.
	
	%	Moreover, $\ig{G^* } = H \cup \{v\}$ as required.  
	
	If $i(G)=1$, then $G$ has a dominating vertex; begin with $G \cup K_1$, which has $\ig{G} = \ig{G \cup K_1}$ and $i(G\cup K_1)=2$, and then proceed as above.	 
\end{proof}

% <<< E: Lemma {lem:vAdd}


As a final lemma before demonstrating the $i$-graph realizability of forests, we show  that a pendant vertex can be added to any $i$-graph to create a new $i$-graph.  The proof proceeds similarly to the construction for trees as $\gamma$-graphs by Fricke et al. in \cite{FHHH11}.



\begin{lemma} \label{lem:leafAdd}
	If $H$ is the $i$-graph of some graph $G$, and $H_u$ is the graph $H$ with some pendant vertex $u$ added, then there exists some graph $G_u$ such that $\ig{G_u} = H_u$.  
\end{lemma}

%>>>START proof
\begin{proof}
	By Lemma \ref{lem:epnAdd} we may assume that for any $i$-set $S$ of $G$, $epn(v,S)\neq \varnothing$ for all $v \in S$.
	
	To construct $G_u$, begin with a copy of $G$.  If $w$ is the stem of $u$ in $H_u$, then consider the $i$-set $W=\{v_1,v_2,\dots,v_k\}$ in $G$ corresponding to $w$.  To each $v_i\in W$, attach a new vertex $x_i$ for all $1 \leq i \leq k$.  Then join each $x_i$ to a new vertex $y$, and then to $y$, add a final pendant vertex $z$.  Thus $V(G_u) = V(G) \cup \{x_1,x_2,\dots, x_k,y,z\}$ as in Figure \ref{fig:pendAdd}.
	
	
	
	%~~~~~~~~~~~~~~~~~~~~~~~~~FIG START~~~~~~~~~~~~~~~~~~~~~~
	\begin{figure}[H]
		\centering
		\begin{tikzpicture}					
			%---------- REF-------------------
			\node(cent) at (0,0) {};
			%\path (cent) ++(0:30 mm) node (Zcent)  {};
			\path (cent) ++(0:20 mm) node (Wcent)  {};			
			\path (cent) ++(0:0 mm) node (Gcent)  {};	
			\path (cent) ++(0:40 mm) node (Xcent)  {};	
			\path (cent) ++(0:60 mm) node (Ycent)  {};
			
			%---------- W References ------------------			
			\foreach \label/\rad in {1/0,2/1,3/2,4/3}
			{\path (Wcent) ++(90:\label*6 mm) node[std] (w\label)  {};				
				\path (w\label) ++(30: 4mm) node (wL\label)  {$v_{\label}$};
				
			}
			
			%---------- X References ------------------			
			\foreach \label/\rad in {1/0,2/1,3/2,4/3}
			{
				\path (w\label) ++(0: 20mm) node[std] (x\label)  {};	
				\draw[thick] (w\label)--(x\label);
				
				\path (x\label) ++(150: 4mm) node (xL\label)  {$x_{\label}$};
			}
			
			%---------- X=N(K) 1  - not adj to Z References ----------------			
			\foreach \label/\rad in {1/0,2/1,3/2}
			{
				\path (Gcent) ++(90:4+6*\label mm) node[std] (g\label)  {};
				
			}
			
			%---------- Y and Z ----------------			
			\path (Ycent) ++(90: 15mm) node[std] (y)  {};	
			\path (y) ++(90: 5mm) node (yL)  {$y$};
			
			\foreach \label/\rad in {1/0,2/1,3/2,4/3}
			{
				\draw[thick] (y)--(x\label);
			}
			
			\path (y) ++(0: 15mm) node[std] (z)  {};	
			\path (z) ++(90: 5mm) node (zL)  {$z$};		
			\draw[thick](z)--(y);	
			
			%------------ BLOBS --------------
			\begin{pgfonlayer}{blob}			
				\draw[draw=mgray,  fill=white, dashed] \convexpath{w1,w4}{6mm};
				\path (w1) ++(-90: 8mm) node (WL)  {$W$};
				
				\draw[draw=mgray,  fill=white, dashed] \convexpath{g1,g3}{5mm};
				\path (g1) ++(-90: 6mm) node (GL)  {$G-W$};	
				
			\end{pgfonlayer}
			
			%------------ bEDGES --------------
			\begin{pgfonlayer}{bedge}		
				
				
				\draw[draw=gray,  fill=lgray] \convexpath{w4,w1,g1,g3}{10mm};
				
			\end{pgfonlayer}
			
			
			
			%----------Lines ------------------		
			\begin{pgfonlayer}{bedge}	
				\foreach \i in {1,2,3}
				\path (g\i) ++(0:5 mm) coordinate (gh\i)  {};
				%\path(h\i) ++(90:2mm) node(hm\i) [std]{};	
				\foreach \i in {1,2,3,4}	
				\path (w\i) ++(0:-5 mm) coordinate (wh\i)  {};	
				
				
				\foreach \i in {1,2,3}			
				{
					\foreach \j in {1,2,3,4}	
					\draw[dashed, mgray] (gh\i)--(wh\j);
				}
			\end{pgfonlayer}
			
			\path (cent) ++(0:9 mm) coordinate (GLcent)  {};	
			\path (GLcent) ++(90:28 mm) node (GLcent)  {$G$};	
			
			
		\end{tikzpicture}			
		\caption{The construction of $G_u$ from $G$  in Lemma \ref{lem:leafAdd}.}
		\label{fig:pendAdd}%
	\end{figure}
	%~~~~~~~~~~~~~~~~~~~~~~~~~FIG END~~~~~~~~~~~~~~~~~~~~~~
	
	It is easy to see that if $S$ is an $i$-set of $G$, then $S_y=S\cup\{y\}$ is an independent dominating set of $G_u$.  The set $W_z = W \cup \{z\}$ is also an independent dominating set of $G_u$.  Thus,  $i(G_u) \leq i(G)+1$.  It remains only to show that these are $i$-sets and the only $i$-sets of $G_u$.
	
	
	We claim that no $x_i$ in $X = \{x_1,x_2,\dots, x_k\}$ is in any $i$-set of $G_u$.  To show this, suppose to the contrary that $S^*$ is an $i$-set with $S^* \cap X = \{x_1,x_2,\dots, x_{\ell}\}$ for some $1 \leq \ell \leq k$.  Then, $y \notin S^*$; that is, $\{y,z\} \cap S^* = \{z\}$.  To dominate the remaining $\{x_{\ell+1},x_{\ell+2},\dots, x_k\}$, we have that $S^*=\{x_1,x_2,\dots,x_{\ell}\}\cup \{v_{\ell+1},v_{\ell+2},\dots, v_k\} \cup \{z\}$.  Recall from our initial assumption on $G$ that there exists some $v_1^* \in epn_G(v_1,W)$.  Thus, $v_1^* \notin (N_{H_u}[\{v_{\ell+1},v_{\ell+2},\dots, v_k\}] \cap V(G))$, and so $v_1^*$ is undominated by $S^*$, which implies that $S^*$ is not an $i$-set.   
	
	Thus in every $i$-set of $G_u$, $y$ is dominated either by itself or by $z$.  If $y$ is not in a given $i$-set $S$ (and so $z\in S$), then to dominate $X$, $W\subseteq S$, and so $S = W \cup \{z\}$.  Conversely, if $y\in S$ (and $z\notin S$), then since the vertices of $G$ can only be dominated internally, $S$ is an $i$-set of $G_u$ if and only if $S-\{y\}$ is an $i$-set of $G$, which completes the proof of our claim.
	
	If  $u^*$ and $w^*$ are the vertices in $\ig{G_u}$ associated with $W_z$ and $W_y = W\cup \{y\}$ respectively, then clearly $\ig{G_u} - \{u^*\} \cong \ig{G}$.  Furthermore, since  $W_y$ is the only $i$-set  with $|W_y - W_z| = 1$ and $yz\in E(G_u)$, it follows that $\deg(u^*)=1$ and $u^*w^* \in E(\ig{G_u})$, and we conclude that $\ig{G_u} \cong H_u$.
\end{proof}
%<<< END proof








\begin{comment}  **** SAFETY BACK-UP  before G-H SWAP
	\nts{G and H backwards}
	\begin{lemma} \label{lem:leafAdd}
		If $G$ is the $i$-graph of some graph $H$, and $G_u$ is the graph $G$ with some pendant vertex $u$ added, then there exists some graph $H_u$ such that $\ig{H_u} = G_u$.  
	\end{lemma}
	
	%>>>START proof
	\begin{proof}
		By Lemma \ref{lem:epnAdd} we may assume that for any $i$-set $S$ of $H$, $epn(v,S)\neq \varnothing$ for all $v \in S$.
		
		To construct $H_u$, begin with a copy of $H$.  If $w$ is the stem of $u$ in $G_u$, then consider the $i$-set $W=\{v_1,v_2,\dots,v_k\}$ in $H$ corresponding to $w$.  To each $v_i\in W$, attach a new vertex $x_i$ for all $1 \leq i \leq k$.  Then join each $x_i$ to a new vertex $y$, and then to $y$, add a final pendant vertex $z$.  Thus $V(H_u) = V(H) \cup \{x_1,x_2,\dots, x_k,y,z\}$ as in Figure \ref{fig:pendAdd}.
		
		It is easy to see that if $S$ is an $i$-set of $H$, then $S_y=S\cup\{y\}$ is an $i$-set of $H_u$.  The set $W_z = W \cup \{z\}$ is also an $i$-set of $H_u$.  It remains only to show that these are the only $i$-sets of $H_u$.
		
		
		We claim that no $x_i$ in $X = \{x_1,x_2,\dots, x_k\}$ is in any $i$-set of $H_u$.  To show this, suppose to the contrary that $S^*$ is an $i$-set with $S^* \cap X = \{x_1,x_2,\dots, x_{\ell}\}$ for some $1 \leq \ell \leq k$.  Then, $y \notin S^*$.  To dominate the remaining $\{x_{\ell+1},x_{\ell+2},\dots, x_k\}$, we have that $W \cap S^*=\{v_{\ell+1},v_{\ell+2},\dots, v_k\}$.  Recall from our initial assumption on $H$ that there exists some $v_1^* \in epn_H(v_1,W)$.  Thus, $v_1^* \notin (N[\{v_{\ell+1},v_{\ell+2},\dots, v_k\}] \cap V(H))$, and so $v_1^*$ is undominated in $S^*$, and $S^*$ is not an $i$-set.   
		
		Thus in every $i$-set of $H_u$, $y$ is dominated either by itself or by $z$.  If $y$ is not in a given $i$-set $S$ (and so $z\in S$), then to dominated $X$, $W\subseteq S$, and so $S = W \cup \{z\}$.  Conversely, if $y\in S$ (and $z\notin S$), then since the vertices of $H$ can only be dominated internally, $S$ is an $i$-set of $H_u$ if and only if $S-\{y\}$ is an $i$-set of $H$, which completes the proof of our claim.
		
		If  $u^*$ and $w^*$ are the vertices in $\ig{H_u}$ associated with $W_z$ and $W_y = W\cup \{y\}$ respectively, then clearly $\ig{H_u} - \{u^*\} \cong \ig{H}$.  Furthermore, since  $W_y$ is the only $i$-set  with $|W_y \cap W_z| = 1$ and $yz\in E(H_u)$, it follows that $deg(u^*)=1$ and $u^*w^* \in E(\ig{H_u})$, and we conclude that $\ig{H_u} \cong G_u$.
	\end{proof}
	%<<< END proof
\end{comment}






\noindent Finally, we amalgamate the previous lemmas on adding isolated and pendant vertices to $i$-graphs to demonstrate that forests are $i$-graphs.

%>>>S: Theorem {thm:i:forests}
\begin{theorem} \label{thm:i:forests}
	All forests are  $i$-graph  realizable.
\end{theorem}

%>>>START proof
\begin{proof}
	We show by induction on the number of  vertices that if $F$ is a forest with $m$ components, then $F$ is $i$-graph realizable.  For a base, note that $\ig{\overline{K_2}} = K_1$.  Construct the graph  $\overline{K_m}$ by repeatedly applying Lemma \ref{lem:vAdd}.  Suppose  that all forests on $m$ components on at most $n$ vertices are $i$-graph realizable.  Let $F$ be some forest with  $|V(F)| = n+1$ and components $T_1,T_2,\dots, T_m$.   If all  vertices of $F$ are isolated, we are done, so assume there is some leaf $v$ with stem $w$ in component $T_1$.  Let $F^* =  F-\{v\}$.  By induction there exists some graph $G^*$ with $\ig{G^*} \cong F^*$.  Applying Lemma \ref{lem:leafAdd} to $G^*$ at $w$ constructs a graph $G$ with $\ig{G} \cong F$.
\end{proof}
%<<< END proof
%<<< END Theorem {thm:i:forests}



\noindent Moreover, by adding Proposition \ref{prop:i:cycle} to the previous results, we obtain the following immediate corollary.  

\begin{coro} \label{coro:unicyclic}
	Unicyclic graphs are $i$-graph realizable.
\end{coro}



With the completion of the constructions of forests and unicyclic graphs as $i$-graphs, we have now determined the $i$-graph realizability of many collections of small graphs.  In particular, we draw the reader's attention to the  following observation.  

\begin{obs} \label{obs:i:4v}  
	Every graph on at most four vertices except $\Dia$ is an $i$-graph.
\end{obs}






%================================== SECTION: BUILDING TOOLS  =============================	
\section{Building $i$-Graphs} \label{sec:i:tools}

In this section, we examine how new $i$-graphs can be constructed from known ones.  To begin, we present three very useful tools for constructing new $i$-graphs: the \textbf{Max Clique Replacement Lemma}, the \textbf{Deletion Lemma}, and the \textbf{Inflation Lemma}.  The first among these shows that maximal cliques in $i$-graphs can  be replaced by arbitrarily larger maximal cliques.


%>>>S: Lemma {lem:i:cliqueRep}
\begin{lemma} \textbf{(Max Clique Replacement Lemma)} \label{lem:i:cliqueRep}
	Let $H$ be an $i$-graph with a maximal $m$-vertex clique, $\mathcal{K}_m$.  Then, the graph $H_w$ formed by adding a new vertex $w^*$ adjacent to all of $\mathcal{K}_m$ is also an $i$-graph.	
\end{lemma}


\begin{proof}	
	Suppose $G$ is a graph such that $\ig{G}=H$ and $i(G)=k+1$ where $k\geq 1$, and let $\mathcal{K}_m=\{V_1, V_2, \dots, V_m\}$ be a maximal clique in $H$.  From Lemma \ref{lem:i:claw}, the corresponding $i$-sets $V_1, V_2, \dots, V_m$ of $G$ differ on exactly one vertex, so for each $1\leq i \leq m$, let $V_i = \{v_i, z_1,z_2,\dots,z_{k}\} \subseteq V(G)$, so that $Z=\{z_1,z_2,\dots,z_{k}\} = \bigcap_{1 \leq i \leq m} V_i$.  Notice also from Lemma \ref{lem:i:claw}, for each $1 \leq i  < j \leq m$, $v_iv_j \in E(G)$, and so $Q_m=\{v_1,v_2,\dots,v_m\}$ is a (not necessarily maximal) clique of size $m$ in $G$. 
	
	In addition to ${Q_m}$ and $Z$ defined above, we further weakly partition (i.e. some of the sets of the partition may be empty) the vertices of $G$ as:
	\begin{enumerate}[itemsep=0pt, label=]
		\item $X= N(Q_m) \backslash N(Z)$, the vertices dominated by $Q_m$ but not $Z$.
		\item $Y = N(Q_m) \cap N(Z)$, the vertices dominated by both $Q_m$ and $Z$.
		\item $A= N(Z) \backslash N(Q_m)$, the vertices dominated by $Z$ but not $Q_m$.
	\end{enumerate}
	
	
	
	\noindent This partition (as well as the later defined construction of $G_w$) is illustrated in Figure \ref{fig:i:cliqueRep}.  Before proceeding with the construction, we state the following series of claims regarding the set $X$:
	\begin{enumerate}[itemsep=5pt, label=]
		\item \textbf{Claim 1:} \emph{Each  $x \in X$ is dominated by every vertex of $Q_m$.  }\\
		Otherwise, if some $x \in X$ is not adjacent to some $v_j \in Q_m$, then $x$ is undominated in the the $i$-set $V_j = \{v_j\} \cup Z$.
		
		
		\item \textbf{Claim 2:} \emph{$|X| \neq 1$}.\\ %\emph{ Either $X = \varnothing$ or $|X| \geq 2$.}\\
		If $X=1$, say $X = \{x\}$, then $X^*= \{x\}\cup Z$ is independent, dominating, and has $|X^*| = i(G)$; that is, $X^*$ is an $i$-set of $G$.  However, since $x$ is adjacent to all of $Q_m$ in $G$, $\edge{X^*,x,v_j,V_j}$ for each $1 \leq j \leq m$, contradicting the maximality of the clique $\mathcal{K}_m$ in $H$.
		
		\item \textbf{Claim 3:} \emph{No $x \in X$ dominates all of $X$}. \\ %\emph{$X$ is not a clique}.
		If $x \in X$ dominates $X$, then $\{x\} \cup Z$ is an $i$-set of $G$. Following a similar argument  of  Claim 2, this contradicts the maximality of $\mathcal{K}_m$ in $H$.
		
		
		\item \textbf{Claim 4:} \emph{For any $v \in (X \cup Y  \cup A)$, $\{v\} \cup Z$ is not an $i$-set}.\\
		Combining Claims 2 and 3, if $v \in X$, then there exists some $x_i\in X$ such that $v\not\sim x_i$, and thus $\{v\} \cup Z$ does not dominate $x_i$.
		If $v \in (Y\cup A)$, then $v\in N(Z)$,  and so $\{v\} \cup Z$ is not independent.  		
		
	\end{enumerate}	
	
	We construct a new graph $G_w$ from $G$ by joining a new vertex $w$ to each vertex in $V(G)-Z$, as in Figure \ref{fig:i:cliqueRep}.  We claim that $\ig{G_w} \cong H_w$.  %To demonstrate the result, we proceed with an additional series of claims, noting first that the previous two claims also apply to $G_w$.
	
	
	\begin{figure}[H]
		\centering
		\begin{tikzpicture}	
			
			%---------- REF-------------------
			\node(cent) at (0,0) {};
			\path (cent) ++(0:30 mm) node (Zcent)  {};
			\path (cent) ++(180:30 mm) node (Kcent)  {};
			
			\path (cent) ++(90:40 mm) node (Wcent)  {};
			
			\path (cent) ++(90: 0mm) node (Ycent)  {};		
			\path (cent) ++(180:60 mm) node (Xcent)  {};
			\path (cent) ++(0:70 mm) node (Vcent)  {};		
			
			%---------- K References ------------------			
			\foreach \label/\rad in {1/6,2/2,3/-2,4/-6}
			\path (Kcent) ++(90:\rad mm) node[std] (k\label)  {};	
			
			\draw(k1)--(k4);
			\draw[black] (k1) to [out=225,in=135](k3);	
			\draw[black] (k2) to [out=225,in=135](k4);
			\draw[black] (k1) to [out=215,in=145](k4);		
			
			
			%---------- X=N(K) 1  - not adj to Z References ----------------			
			\foreach \label/\rad in {1/6,2/0,3/-6}
			\path (Xcent) ++(90:\rad mm) node[std] (x\label)  {};
			
			%---------- Y= N(K) 2 - ajd to Z References ------------------			
			\foreach \label/\rad in {1/6,2/-6}
			\path (Ycent) ++(90:\rad mm) node[std] (y\label)  {};
			
			%---------- Z References ------------------			
			\foreach \label/\rad in {1/0,2/-4,3/-8}
			\path (Zcent) ++(90:\rad mm) node[std] (z\label)  {};	
			
			%---------- V References ------------------			
			\foreach \label/\rad in {1/6,2/2,3/-2, 4/-6}
			\path (Vcent) ++(90:\rad mm) node (v\label)[std]  {};	
			
			%---------- W References ------------------			
			\path (cent) ++(120:30 mm) node (w)[regRed]  {};	
			\path (w) ++(90: 6mm) node (WL)  {$w$};	
			
			%--------- Extra Internal Edges for Style -----
			\draw[ll](x1)--(x2);
			\draw[ll](v1)--(v2)--(v3);	
			
			%------------ BLOBS --------------
			\begin{pgfonlayer}{blob}			
				\draw[draw=gray,  fill=lgray] \convexpath{k1,k4}{5mm};
				\path (k4) ++(-90: 15mm) node (KL)  {$Q_m$};
				
				\draw[draw=gray,  fill=lgray] \convexpath{x1,x3}{5mm};
				\path (x3) ++(-90: 15mm) node (XL)  {$X$};	
				
				\draw[draw=gray, thick, fill=lgray] \convexpath{z1,z3}{5mm};
				\path (z3) ++(-90: 13mm) node (ZL)  {$Z$};	
				
				\draw[draw=gray, thick, fill=lgray] \convexpath{y1,y2}{5mm};
				\path (y2) ++(-90: 15mm) node (YL)  {$Y$};	
				
				\draw[draw=gray, thick, fill=lgray] \convexpath{v1,v4}{5mm};
				\path (v4) ++(-90: 15mm) node (VL)  {$A$};				
				
			\end{pgfonlayer}
			
			%------------ bEDGES --------------
			%\begin{pgfonlayer}{bedge}				
			
			\foreach \i in {1,2,3}
			{
				\foreach \j in {1,2,3,4}
				\draw[ll](x\i)--(k\j);
			}		
			
			\draw[ll](y1)--(k2);
			\draw[ll](y2)--(k4);
			\draw[ll](y1)--(k1);
			
			
			\draw[ll](z1)--(y1)--(z2);
			\draw[ll](y2)--(z2);
			
			
			\draw[ll](z1)--(v1);
			\draw[ll](z2)--(v2);
			\draw[ll](z2)--(v3);
			\draw[ll](z2)--(v4);
			\draw[ll](z3)--(v4);
			
			\draw[ll] (x3) to [out=-30,in=210](y2);	
			
			\draw[ll] (y2) to [out=-30,in=210](v4);	
			\draw[ll] (y2) to [out=-30,in=210](v3);	
			
			
			%\draw[ll] (x1) to [out=15,in=165](v1);	
			
			%\end{pgfonlayer}	
			
			
			%------------ bEDGES --------------
			%	\begin{pgfonlayer}{bedge}	
				\foreach \i in {1,2,3}
				\draw[red] (w)--(x\i);
				
				\foreach \i in {1,2,3,4}		
				{	\draw[red] (w)--(k\i);	
					\draw[red] (w)--(v\i);
				}
				
				\draw[red] (y1)--(w)--(y2);
				%	\end{pgfonlayer}		
			
		\end{tikzpicture}
		\caption{Construction of $G_w$ from $G$ in Lemma  \ref{lem:i:cliqueRep}.}
		\label{fig:i:cliqueRep}
	\end{figure}	
	
	Let $S$ be some $i$-set of $G_w$.  If $w \notin S$, then $S \subseteq V(G)$ and so $S$ is also independent dominating in $G$, implying $|S| = i(G)= k+1$.  However, if $w\in S$, then since $w$ is adjacent to all of $V(G)-Z$ and $Z$ is independent, we have that $S = \{w\} \cup Z$.  It follows that $i(G_w) = i(G)$.  Moreover, any $i$-set of $G$ is also an $i$-set of $G_w$, and so $W:=\{w\} \cup Z$ is the only new $i$-set generated in $G_w$.  Thus $V(\ig{G_w}) = V(\ig{G}) \cup \{W\}$.
	
	Consider now the edges of $\ig{G_w}$.  Since $w$ is adjacent to all of $Q_m$ in $G_w$,  $\edge{W,w,v_j,V_j}$ for each $1 \leq j \leq m$, and thus $\mathcal{K}_m \cup W$ is a clique in $\ig{G_w}$. 
	
	Finally, we demonstrate that $W$ is adjacent only to the $i$-sets of $\mathcal{K}_m$.  Consider some $i$-set $S \notin \mathcal{K}_m$, and suppose to the contrary that $\onlyedge{W,S}$.  	
	As $W$ is the only $i$-set containing $w$, we have that $w\notin S$, and hence $\edge{W,w,u,S}$ for some vertex $u$.
	Since $w \sim u$,   $u \notin Z$.  Moreover, since $W$ and $S$ differ at exactly one vertex and $Z \subseteq W$, it  follows that $Z \subseteq S$; that is, $S = \{u\} \cup Z$.  If $ u\in Q_m$ then $S \in \mathcal{K}_m$, a contradiction.  If $u \in (X \cup Y \cup A)$, then by Claim 4, $S$ is not an $i$-set, which is again a contraction.  We conclude that $W \not\sim S$ for any $i$-set $S \notin \mathcal{K}_m$, and therefore $E(\ig{G_w}) = E(\ig{G}) \cup \left( \bigcup_{v_i\in Q_m} wv_i\right)$.  If follows that $\ig{G_w} \cong H_w$.		
\end{proof}
%<<<< E: Lemma {lem:i:cliqueRep}



%\nts{Scrap this and the following OP, given updated max clique?}


%\noindent Part \ref{lem:i:cliqueRepB} leads to the natural question of whether a vertex of degree $r-1$ is necessary to construct $H^*_m$.  At this time, we have no insights into the matter and leave it as an open problem.

%\begin{open}  	Let $H$ be an $i$-graph with a maximal $K_r$ clique such that for all $v\in K_r$, $\deg(v) \geq r$.  Given any $m\geq r+1$, is the graph $H_m$ formed by adding $m-r$ vertices to $H$, each adjacent to one another and to all of $K_r$,  also an $i$-graph?
%\end{open}

%Notice that the maximality of the clique in $H$ is required.  Otherwise, for example, if an edge of the $i$-realizable $K_3$ is replaced with another $K_3$, the non $i$-realizable Diamond graph $\Dia$ results.
%%%% No longer true with the new neighbourhood requirement?


Our next result, the Deletion Lemma, shows that the class of $i$-graphs is closed under vertex deletion. It is unique among our other constructions; unlike most of our results  which demonstrate how to build larger $i$-graphs from smaller ones, the Deletion Lemma instead shows that every induced subgraph of an $i$-graph is also an $i$-graph.  


%>>> START Theorem {lem:i:inducedI}
\begin{lemma} \label{lem:i:inducedI} \textbf{(The Deletion Lemma)}
	If $H$ is a nontrivial $i$-graph, then any induced subgraph of $H$ is also an $i$-graph.
\end{lemma}

\begin{proof}  
	Let $G$ be a graph such that $H= \ig{G}$ and $i(G)=k$.   To prove this result, we show that for any $X \in V(H)$, there exists some graph $G_X$ such that $\ig{G_X} = H-X$.
	
	To construct $G_X$, take a copy of $G$ and add to it a vertex $z$ so that $z$ is adjacent to each vertex of $G-X$ (see Figure \ref{fig:i:Gx}).  	
	Observe first that since $H$ is nontrivial, there exists an $i$-set $S \neq X$ of $G$.  Then, $S$ is also an independent dominating set of $G_X$, and so $i(G_X) \leq k$.    		
	Consider now some $i$-set $S_X$ of $G_X$.   Clearly $S_X \neq X$ because $X$ does not dominate $z$.  	 
	If $z\in S_X$, then as $S_X$ is independent, no vertex of $G-X$ is in $S_X$.  
	Moreover, since $X$ is also independent and its vertices have all of their neighbors in $G-X$, this leaves each vertex of $X$ to dominate itself.  That is, $X \subseteq S_X$, implying that $S_X = X \cup \{z\}$ and  $|S_X| = k + 1$.  This contradicts that $i(G_X) \leq k$, and thus we conclude that $z$ is not in any $i$-set of $G_X$.  	  
	It follows that each $i$-set of $G_X$ is composed only of vertices from $G$ and so $i(G_X) = k$.  Thus, $S_X \neq X$ is an $i$-set of $G_X$ if and only if it is an $i$-set of $G$.   	 Given that $V(\ig{G_X}) = V(\ig{G}) - \{X\} = V(H) - \{X\}$, we have that $\ig{G_X} = H - X$ as required.  \null \hfill
\end{proof}



%\noindent \underline{Construction of $G_X$:}  Begin with a copy of $G$,  with vertices partitioned into $X$ and $G-X$.  Add a vertex $u$ and join edges between $u$ and each vertex of $G-X$.  Now add a copy of the start $K_{1,m}$, with leaves labelled as $\{w,z_1,z_2,\dots,z_m\}$ and centre $z$.  To complete the construction, join $u$ and $w$ with an edge.  See Figure \ref{fig:i:Gx}.  


%~~~~~~~~~~~~~~~~~~~~~~~~~FIG START~~~~~~~~~~~~~~~~~~~~~~
\begin{figure}[H]
	\centering
	\begin{tikzpicture}					
		
		%---------- REF-------------------
		\node(cent) at (0,0) {};
		
		%---------- X References ------------------			
		\foreach \label/\rad in {1/0,2/5,3/10,4/15}
		\path (cent) ++(90:\rad mm) node (x\label)  {};		
		
		% ---------- Y References --------
		\path (cent) ++(0:30 mm) node (yM)  {};					
		
		\foreach \label/\rad in {1/-5,2/0,3/5,4/10,5/15,6/20}
		\path (yM) ++(90:\rad mm) node (y\label) [std]  {};		
		
		%----------Lines ------------------		
		
		\foreach \i in {1,2,3,4}
		\path (x\i) ++(0:4 mm) node (h\i)  {};
		%\path(h\i) ++(90:2mm) node(hm\i) [std]{};	
		\foreach \i in {1,2,3,4,5,6}	
		\path (y\i) ++(0:-4 mm) node (j\i)  {};	
		
		\draw[dashed, mgray] (h1)--(j2);
		\draw[dashed, mgray] (h2)--(j4);
		%	\draw[gray] (h2)--(j3);
		\draw[dashed, mgray] (h4)--(j5);
		\draw[dashed, mgray] (h4)--(j4);
		%	\draw[gray] (h3)--(j4);
		\draw[dashed, mgray] (h3)--(j3);
		\draw[dashed, mgray] (h1)--(j3);	
		\draw[dashed, mgray] (h1)--(j1);	
		\draw[dashed, mgray] (h4)--(j6);	
		
		\draw[draw=mgray, fill=lgray, dashed] \convexpath{x1,x4}{5mm};	
		
		\foreach \i in {1,2,3,4}
		\node [std](xD\i) at (x\i) {};	
		
		\path (x1) ++(-90: 15mm) node (XL)  {$X$};		
		
		%----------G- X and z ------------------	
		\draw[draw=mgray,fill=lgray, dashed] \convexpath{y1,y6}{5mm};		
		
		\path (y3) ++(90:5 mm) node (y35)  {};	
		\path (y35) ++(0:20 mm) node (z) [std] {};
		\path (z) ++(0:4 mm) node (zL) {$z$};
		
		\foreach \i in {1,2,3,4,5,6}{
			\node [std](yD\i) at (y\i) {};		
			\draw(z)--(yD\i);
		}
		
		\path (y1) ++(-90: 10mm) node (GL)  {$G-X$};	
		
	\end{tikzpicture}			
	\caption{Construction of $G_X$ in Lemma \ref{lem:i:inducedI}.}
	\label{fig:i:Gx}%
\end{figure}
%~~~~~~~~~~~~~~~~~~~~~~~~~FIG END~~~~~~~~~~~~~~~~~~~~~~


%<<< END Theorem {lem:i:inducedI}



\noindent The following corollary is immediate as the contrapositive of Lemma \ref{lem:i:inducedI}.  

%>>> START Coro {coro:i:notInduced}
\begin{coro} \label{coro:i:notInduced}
	If $H$ is not an $i$-graph, then any graph containing an induced copy of $H$ is also not an $i$-graph.
\end{coro}
%<<< END  Coro {coro:i:notInduced}


\noindent  
This corollary, although simple in statement and proof, immediately removes many families of graphs from $i$-graph realizability.  For example, all wheels, 2-trees, and maximal planar graphs on at least five vertices contain an induced copy of  the Diamond graph $\Dia$, which was shown in Proposition \ref{prop:i:diamond} to not be an $i$-graph.
Moreover, given that $i$-graph realizability is an inherited property, this suggests that there may be a finite-family forbidden subgraph characterization for $i$-graph realizability. 



We now alter course to examine how one may construct new $i$-graphs by combining several known $i$-graphs.  Understandably, an immediate obstruction to combining the constructions of $i$-graphs of, say, $\ig{G_1} = H_1$ and $\ig{G_2}=H_2$ is that it is possible (and indeed, likely) that $i(G_1) \neq i(G_2)$.  

Two solutions to this quandary are presented in the following  lemmas. In the first, Lemma \ref{lem:i:infFam},  given a graph $G$, we  progressively construct an infinite family of seed graphs $\mathcal{G}$ with the same number of components as $G$, and such that $\ig{G} = \ig{G_i}$ for each $G_i \in \mathcal{G}$.    The second, Lemma \ref{lem:i:anySize} or the \textbf{Inflation Lemma}, offers a more direct solution: given an $i$-graph $H$, we demonstrate how to ``inflate" a seed graph $G$ to produce a new graph $G^*$ such that $\ig{G^*} = \ig{G}$ and the $i$-sets of $G^*$ are arbitrarily larger than the $i$-sets of $G$.

%A solution to this quandary is presented in the following Lemma \ref{lem:i:anySize} or the ``Inflation Lemma":  given an $i$-graph $H$, we demonstrate how to ``inflate" a seed graph $G$ to produce a new graph $G^*$ such that $\ig{G^*} = \ig{G}$ and the $i$-sets of $G^*$ are arbitrarily larger than the $i$-sets of $G$.


%>>>S: Lemma {lem:i:infFam}
\begin{lemma} \label{lem:i:infFam}
	If $G$ is a graph with $\ig{G}\cong H$, then there exists an infinite family of graphs $\mathcal{G}$ such that $\ig{G_i}\cong H$ for each $G_i \in \mathcal{G}$. 
	Moreover, the number of components of $G_i \in \mathcal{G}$ is the same as $G$ ($k(G) = k(G_i)$).
	
	% Moreover, if $G$ is a connected, there exists an infinite family of such connected graphs.
\end{lemma}

\begin{proof}
	Suppose $v \in V(G)$, and let $G^*$ be the graph  obtained by attaching a copy of the star $K_{1,3}$ with $V(K_{1,3})=\{x,y_1,y_2,y_3\}$ ($\deg(x)=3$) by joining $v$ to $y_1$.   As $y_2$ and $y_3$ are pendant vertices, $i(G^*) \geq i(G)+1$.  If $S$ is an $i$-set of $G$, then $S^*=S \cup \{x\}$ is dominating and independent, and so $i(G^*) =  i(G)+1$.  Thus, $x$ is in every $i$-set of $G^*$, and we can conclude that $S^*$ is an $i$-set of $G^*$ if and only if $S^*-\{x\}$ is an $i$-set of $G$.		It follows that $\ig{G^*} \cong  \ig{G}$ as required.  		
	Attaching additional copies of $K_{1,3}$ as above at any vertex of $H$ similarly creates the other graphs of $\mathcal{G}$.		
\end{proof}
% <<< E: Lemma {lem:i:infFam}





%>>>S: Lemma {lem:i:anySize}
\begin{lemma} \label{lem:i:anySize} \textbf{(The Inflation Lemma)}
	If $H$ is the $i$-graph of some graph $G$, then for any $k \geq i(G)$ there exists a graph $G^*$ such that $i(G^*) =k$ and $\ig{G^*}\cong H$.  		
\end{lemma}

\begin{proof}
	Begin with a copy of $G$ and add to it $\ell = k - i(G)$ isolated vertices, $S=\{v_1,v_2,\dots,v_{\ell}\}$.   Immediately, $X$ is an $i$-set of $G$ if and only if $X\cup S$ is an $i$-set of $G^*$.  Moreover, if $X$ and $Y$ are $i$-sets of $G$ such that $\adjG{X,Y,G}$ in $H$, then $\adjG{( X\cup S), (Y\cup S), G^*}$, and so $\ig{G^*} \cong H$.  
\end{proof}
% <<< E: Lemma {lem:i:anySize}

Now, when attempting to combine the constructions of $\ig{G_1} = H_1$ and $\ig{G_2}=H_2$ and $i(G_1) < i(G_2)$, we need only inflate $G_1$ until its $i$-sets are the same size as those in $G_2$.  A powerful construction tool, the Inflation Lemma is used repeatedly in almost all of the following results of this section; in the first of these, we show how two $i$-graphs may be connected by an edge between any two vertices to produce a new $i$-graph.  


%>>>S: Prop {prop:i:brg}	
\begin{prop}\label{prop:i:brg}
	Let $H_1$ and $H_2$ be disjoint $i$-graphs.  Then the graph $H$, formed by connecting  $H_1$ to $H_2$ by an edge between any $x\in V(H_1)$ and any $y \in V(H_2)$, is also an $i$-graph.			
\end{prop}


%\begin{comment}
%~~~~~~~~~~~~~~~~~~~~~~~~~FIG START~~~~~~~~~~~~~~~~~~~~~~
{\begin{figure}[H]
		\centering
		\begin{tikzpicture}					
			
			%---------- REF-------------------
			%	\fill[lgray, dashed] (0,0) circle (1.7cm);
			\node(cent) at (0,0) {};
			\path (cent) ++(90:35 mm) node (Zcent)  {};
			\path (cent) ++(180:30 mm) node (Xcent)  {};
			\path (cent) ++(0:30 mm) node (Ycent)  {};
			%	\node [std](mid) at (cent)[label=above:$*$] {};	
			%\draw[gray, dashed] (0,0) circle (1.7cm);
			%\node (H) at (0,-1.4) [color=gray](L){$G$};	
			
			%---------- Z References ------------------			
			\foreach \label/\rad/\i in {1/10/90,2/5/90,3/0/0,4/5/-90,5/10/-90}
			\path (Zcent) ++(\i:\rad mm) node (z\label)  {};	
			
			%---------- X References ------------------			
			\foreach \label/\rad in {1/20,2/15,3/10,4/5,5/0}
			\path (Xcent) ++(180:\rad mm) node (x\label)  {};		
			
			\path (z5) ++(210:15 mm) node [std](xk)  {};
			\path (z5) ++(210:10 mm) node (xHull)  {};
			
			\path (x1) ++(180: 15mm) node (G1L)  {$G_1- X$};	
			
			%---------- Y References ------------------			
			\foreach \label/\rad in {1/20,2/15,3/10,4/5,5/0}
			\path (Ycent) ++(0:\rad mm) node (y\label)  {};		
			
			\path (z5) ++(-30:15 mm) node [std](yk)  {};
			\path (z5) ++(-30:10 mm) node (yHull)  {};
			
			\path (y1) ++(0: 15mm) node (G2L)  {$G_2- Y$};
			
			%----------Lines ------------------					
			
			\foreach \i in {1,2,3,4,5}
			{\path (x\i) ++(270:2 mm) node (h\i)  {};
				\path (x\i) ++(90:2 mm) node (a\i) {};	
				\path (y\i) ++(270:2 mm) node (j\i)  {};
				\path (y\i) ++(90:2 mm) node (b\i) {};	
			}
			
			\foreach \i in {1,2,3,4,5}
			{						
				\foreach \j in {1,2,3,4,5}
				{
					\draw[black] (h\i) to [out=-30,in=210](j\j);
				}
				
				\draw[black] (xk)--(b\i);
				\draw[black] (yk)--(a\i);				
				
				\draw[gray,dashed] (a\i) to [out=90,in=190](z\i);
				\draw[gray,dashed] (b\i) to [out=90,in=-10](z\i);
			}
			
			\draw[gray] (yk)--(xk);				
			
			%------------ BLOBS --------------
			
			\draw[draw=gray, thick, fill=lgray] \convexpath{z1,z5}{6mm};
			\path (z1) ++(90: 12mm) node (ZL)  {$Z$};
			
			\draw[draw=blue, thick] \convexpath{z1,z5,xk}{7mm};
			\path (z1) ++(35: 12mm) node[red] (YL)  {$Y$};
			\draw[draw=red,thick] \convexpath{yk,z5,z1}{8mm};
			\path (z1) ++(145: 12mm) node[blue] (YL)  {$X$};
			
			\draw[draw=gray,thick, fill=lgray] \convexpath{x1,x5}{3mm};
			\draw[draw=gray,thick, fill=lgray] \convexpath{y1,y5}{3mm};
			
			%------------ NODE PRINTS --------------
			\foreach \i in {1,2,3,5}
			\node [std](zD\i) at (z\i) {};
			\path (z1) ++ (0:4mm) node (zL1) {$z_{1}$};
			\path (z2) ++ (0:4mm) node (zL2) {$z_{2}$};
			\path (z3) ++ (0:4mm) node (zL3) {$z_{3}$};
			\node (zD3) at (z3) {$\vdots$};
			\node (zD4) at (z4) {$\vdots$};
			%\path (z4) ++ (0:6mm) node (zL4) {$z_{k-1}$};
			\path (z5) ++ (0:4mm) node (zL5) {$z_{k}$};
			
			\foreach \i in {1,2,3,4,5}
			\node [std](yD\i) at (y\i) {};
			
			\foreach \i in {1,2,3,4,5}
			\node [std](xD\i) at (x\i) {};
			
			\node [std](xDk) at (xk) {};
			\path (xk) ++ (90:3mm) node (xkL) {$x_{k+1}$};
			\node [std](yDk) at (yk) {};
			\path (yk) ++ (90:3mm) node (ykL) {$y_{k+1}$};
			
		\end{tikzpicture}			
		\caption{Construction of $G$ in Proposition  \ref{prop:i:brg}.}
		\label{fig:i:brg}%
\end{figure}}
%~~~~~~~~~~~~~~~~~~~~~~~~~FIG END~~~~~~~~~~~~~~~~~~~~~~
%\end{comment}




\begin{proof}
	Suppose that $G_1^*$ and $G_2^*$ are graphs such that $\ig{G_1^*} = H_1$ and $\ig{G_2^*} = H_2$.  Without loss of generality, let $k= i(G_1^*) \geq i(G_2^*)$.  Applying  the Inflation Lemma (Lemma \ref{lem:i:anySize}), create graphs $G_1$ and $G_2$ with $\ig{G_1} = H_1$, $\ig{G_2} = H_2$, and $i(G_1)=i(G_2) = k+1$, by adding isolated vertices to $G_1^*$ and $G_2^*$.  In particular, let $x_{k+1}$ be one of the added isolated vertices in $G_1$, and likewise $y_{k+1}$ in $G_2$.  Then $x_{k+1}$ (respectively, $y_{k+1}$) is in every $i$-set of $G_1$ (respectively, $G_2$).
	
	Now suppose that the $i$-set $X=\{x_1,x_2,\dots,x_{k+1}\}$ of $G_1$ corresponds to the vertex $x\in V(H_1)$, and the $i$-set $Y=\{y_1,y_2,\dots,y_{k+1}\}$ of $G_2$  corresponds to $y\in V(H_2)$.  Construct the graph $G$ by identifying $x_i \in V(G_1)$  with $y_i \in V(G_2)$ for all $ 1\leq i \leq k$, and renaming the identified vertex $z_i$.  Let $Z = \{z_1, z_2, \dots, z_k\}$.  Then, join each 
	%$x' \in V(G_1) \backslash (X-\{x_{k+1}\})$ to each $y' \in V(G_2) \backslash (Y-\{y_{k+1}\})$.
	$x' \in V(G_1) \backslash Z$ to each $y' \in V(G_2) \backslash Z$.
	We claim that $\ig{G} = H$.  Through this proof (and those that follow), we mildly abuse notation by referring to both the seed graph used to build $G$, and the vertices of $G$ corresponding to that graph as $G_1$ (and similarly with $G_2$).
	
	Notice that $Z$  does not dominate $x_{k+1}$ nor $y_{k+1}$, and so $Z$ is not itself an $i$-set of $G$.  Suppose $S^*$ is some $i$-set of $G$; clearly, $S^*$ is not a subset of $Z$. Since all vertices of $G_1-Z$ are adjacent to all vertices of $G_2 - Z$,   either $S^* \subseteq G_1$ or $S^* \subseteq G_2$.  Without loss of generality, say $S^* \subseteq G_1$.   Then to  dominate $G_1$, $|S^*| \geq k+1$.
	Now consider any $i$-set $S$ of $G_1$.  Since $x_{k+1} \in S$, $S$ dominates $G_2$ and is therefore an independent dominating set of $G$.  Thus $i(G) \leq k +1$, and so $i(G)=k+1$, and  all $i$-sets of $G_1$ and $G_2$ are also $i$-sets of $G$. Moreover, since all $i$-sets of $G$ are subsets of $G_1$ or $G_2$, we  conclude that $S$ is an $i$-set of $G$ if and only if it is an $i$-set of $G_1$ or $G_2$.  
	
	If $\adjG{X_1,X_2,G_1}$, then clearly $\adjG{X_1,X_2,G}$, and likewise for some $\adjG{Y_1,Y_2,G_2}$.   Thus the subgraph of $\ig{G}$ induced by the $i$-sets of $G_1$ (likewise, $G_2$) is $H_1$ ($H_2$).    Moreover, from their definitions, $\edgeG{X,x_{k+1},y_{k+1},Y,G}$ in $\ig{G}$.
	
	Now suppose that $Y^*\neq Y$ is some $i$-set of $G_2$.  Since every $i$-set of $G_2$ contains $y_{k+1}$, $Y$ and $Y^*$ differ at some other vertex: say, $y^* \in Y^* - Y$ and without loss of generality, $z_1 \in Y- Y^*$.  Then $|X - Y^*| \geq 2$, and so $X$ is not adjacent to $Y^*$ in $\ig{G}$, as required. Similar arguments show that there are no other edges between the $i$-sets of $G_1$ and $G_2$, except between $X$ and $Y$.   
	Thus the only edge between $H_1$ and $H_2$ in $\ig{G}$ is $xy$.	We concluded that $\ig{G} = H$.	  
\end{proof}	
	






The following Corollary \ref{coro:i:brg} provides a way to connect two $i$-graphs with a clique, rather than a bridge.  Notice that the same result is obtainable by applying the Max Clique Replacement Lemma (Lemma \ref{lem:i:cliqueRep}) to Proposition \ref{prop:i:brg}, but we include the following alternative construction and proof below for completeness.

%>>>S: Coro {coro:i:brg}	
\begin{coro}\label{coro:i:brg}
	Let $H_1$ and $H_2$ be $i$-graphs, and let $H$ be the graph formed from them as in Proposition \ref{prop:i:brg} by creating a bridge $xy$ between them.  Then the graph $H_m$  formed by replacing $xy$ with a $K_m$ for $m\geq 2$ is also an $i$-graph.
\end{coro}


%\begin{comment}
%~~~~~~~~~~~~~~~~~~~~~~~~~FIG START~~~~~~~~~~~~~~~~~~~~~~
{\begin{figure}[H]
		\centering
		\begin{tikzpicture}					
			
			%---------- REF-------------------
			%	\fill[lgray, dashed] (0,0) circle (1.7cm);
			\node(cent) at (0,0) {};
			\path (cent) ++(90:35 mm) node (Zcent)  {};
			\path (cent) ++(180:40 mm) node (Xcent)  {};
			\path (cent) ++(0:40 mm) node (Ycent)  {};
			\path (cent) ++(0:0 mm) node (Wcent)  {};
			%	\node [std](mid) at (cent)[label=above:$*$] {};	
			
			%---------- Z References ------------------			
			\foreach \label/\rad/\i in {1/10/90,2/5/90,3/0/0,4/5/-90,5/10/-90}
			\path (Zcent) ++(\i:\rad mm) node (z\label)  {};	
			
			%---------- X References ------------------			
			\foreach \label/\rad in {1/20,2/15,3/10,4/5,5/0}
			\path (Xcent) ++(180:\rad mm) node (x\label)  {};		
			
			\path (z5) ++(210:15 mm) node [std](xk)  {};
			
			\path (x1) ++(180: 15mm) node (G1L)  {$G_1- X$};
			
			%---------- W References ------------------			
			\foreach \label/\rad in {1/10,2/5,3/0,4/-5,5/-10}
			\path (Wcent) ++(180:\rad mm) node (w\label)  {};					
			
			%---------- Y References ------------------			
			\foreach \label/\rad in {1/20,2/15,3/10,4/5,5/0}
			\path (Ycent) ++(0:\rad mm) node (y\label)  {};		
			
			\path (z5) ++(-30:15 mm) node [std](yk)  {};	
			\path (y1) ++(0: 15mm) node (G2L)  {$G_2- Y$};
			
			%----------Lines ------------------					
			
			\foreach \i in {1,2,3,4,5}
			{	\path (x\i) ++(270:2 mm) node (h\i)  {};
				\path (x\i) ++(90:2 mm) node (a\i) {};	
				\path (y\i) ++(270:2 mm) node (j\i)  {};
				\path (y\i) ++(90:2 mm) node (b\i) {};
				\path (w\i) ++(90:4 mm) node (wA\i)  {};
			}
			
			\foreach \i in {1,2,3,4,5}
			{
				
				\foreach \j in {1,2,3,4,5}
				{
					\draw[black] (h\i) to [out=-30,in=210](j\j);
				}
				
				\draw[black] (xk)--(b\i);
				\draw[black] (yk)--(a\i);
				\draw[black] (xk)--(wA\i);
				\draw[black] (yk)--(wA\i);
				
				\draw[gray,dashed] (a\i) to [out=90,in=190](z\i);
				\draw[gray,dashed] (b\i) to [out=90,in=-10](z\i);
			}
			
			
			\draw[gray] (yk)--(xk);		
			
			\path(w1)++(180:6mm) node (wLft){};
			\path(w5)++(0:6mm) node (wRt){};		
			
			%-----------  Edges between W and X  
			\foreach \j in {65,285}
			\path (x5)++(\j:2mm) node (xr\j) {};
			\path (x5)++(0:0mm) node (xr0) {};	
			
			\foreach \i in {130,180,220} 
			{	\foreach \j in {0,65,285}
				{\path (w2) ++(\i:4 mm) node (l\i)  {};									
					\draw(l\i)--(xr\j);
				}
			}
			
			%-----------  Edges between W and Y
			\foreach \j in {115,245}
			\path (y5)++(\j:2mm) node (yr\j) {};
			\path (y5)++(0:0mm) node (yr0) {};	
			
			\foreach \i in {130,180,220} 
			{	\foreach \j in {0,115,245}
				{\path (w5) ++(\i:4 mm) node (l\i)  {};									
					\draw(l\i)--(yr\j);
				}
			}	
			
			%------------ BLOBS --------------
			
			\draw[draw=gray, thick, fill=lgray] \convexpath{z1,z5}{6mm};
			\path (z1) ++(90: 12mm) node (ZL)  {$Z$};
			
			\draw[draw=blue, thick] \convexpath{z1,z5,xk}{7mm};
			\path (z1) ++(35: 12mm) node[red] (YL)  {$Y$};
			\draw[draw=red,thick] \convexpath{yk,z5,z1}{8mm};
			\path (z1) ++(145: 12mm) node[blue] (YL)  {$X$};
			
			
			\draw[draw=gray, thick, fill=lgray] \convexpath{w1,w5}{6mm};
			\path (w3) ++(270: 10mm) node (WL)  {$W$};
			
			\draw[draw=gray,thick, fill=lgray] \convexpath{x1,x5}{3mm};
			\draw[draw=gray,thick, fill=lgray] \convexpath{y1,y5}{3mm};
			
			%------------ NODE PRINTS --------------
			\foreach \i in {1,2,3,5}
			\node [std](zD\i) at (z\i) {};
			\path (z1) ++ (0:4mm) node (zL1) {$z_{1}$};
			\path (z2) ++ (0:4mm) node (zL2) {$z_{2}$};
			\path (z3) ++ (0:4mm) node (zL3) {$z_{3}$};
			\node (zD3) at (z3) {$\vdots$};
			\node (zD4) at (z4) {$\vdots$};
			%\path (z4) ++ (0:6mm) node (zL4) {$z_{k-1}$};
			\path (z5) ++ (0:4mm) node (zL5) {$z_{k}$};
			
			%Y prints
			\foreach \i in {1,2,3,4,5}
			\node [std](yD\i) at (y\i) {};
			
			%X Prints
			\foreach \i in {1,2,3,4,5}
			\node [std](xD\i) at (x\i) {};
			
			%W Prints
			\foreach \i in {1,2,3,5}
			\node [std](wD\i) at (w\i) {};
			\foreach \i in {1,2,3}
			%\path (w\i) ++ (270:4mm) node (wL\i) {$w_{\i}$};
			\node (wD4) at (w4) {$\cdots$};
			%\path (w5) ++ (250:4mm) node (wL5) {$w_{m-2}$};
			
			%W Clique Edges
			\foreach \i in {2,3,5}
			\draw[black] (wD1) to [out=-45,in=-130](wD\i);
			\foreach \i in {3,5}
			\draw[black] (wD2) to [out=-45,in=-130](wD\i);
			\draw[black] (wD3) to [out=-45,in=-130](wD5);
			
			\node [std](xDk) at (xk) {};
			\path (xk) ++ (90:3mm) node (xkL) {$x_{k+1}$};
			\node [std](yDk) at (yk) {};
			\path (yk) ++ (90:3mm) node (ykL) {$y_{k+1}$};	
			
		\end{tikzpicture}			
		\caption{Construction of $G$ in Corollary  \ref{coro:i:brg}.}
		\label{fig:i:cor:brg}%
\end{figure}}
%~~~~~~~~~~~~~~~~~~~~~~~~~FIG END~~~~~~~~~~~~~~~~~~~~~~
%\end{comment}

\begin{proof}
	We proceed by fashioning a graph $G_m$ and then demonstrating that $\ig{G_m} = H_m$.
	Begin by constructing $G$ from $G_1$ and $G_2$ as in the proof of Proposition \ref{prop:i:brg}; as before, identify $k$ vertices of the $i$-set $X$, with $k$ vertices of the $i$-set $Y$, and label them as $Z=\{z_1,z_2,\dots,z_k\}$, so that $X=Z \cup \{x_{k+1}\}$ and $Y=Z \cup \{y_{k+1}\}$.  In particular, recall that $i(G) = k+1$.  Then, to construct $G_m$, add $m-2$ additional vertices $W= \{w_1,w_2,\dots, w_{m-2}\}$ to $G$, making each $w_i$ adjacent to every vertex in  $G\backslash Z$ and to each other (i.e.  $W=K_{m-2}$).   
	
	Suppose $S$ is an $i$-set of $G$.  Since the vertices of $W$ form a clique, $|S \cap W| \leq 1$.  Consider first the case  where $|S \cap W| = 1$, so that, without loss of generality, $w_1 \in S$.  The vertices of $Z$ are not dominated by $w_1$.
	However, since $w_1$ is adjacent to everything in $G_m\backslash Z$ and $Z$ is independent, the vertices of $Z$ are therefore self-dominating in $S$.  Thus, $W_1 = Z\cup\{w_1\} \subseteq S$, and since $W_1$ is dominating, we have that $W_1=S$ with $|W_1| = k+1$.  
	On the other hand, if $S \cap W  = \varnothing$, then as in Proposition \ref{prop:i:brg}, $S$ is a subset of either  $V(G_1)$ or $V(G_2)$, and using similar arguments, $|S| = k+1$.  Thus,   we conclude that 
	$i(G_m) = k+1$.  
	
	From the above, the $i$-sets of $G_m$ are precisely the $i$-sets of $G_1$ and $G_2$, as well as the sets of the form $W_i=Z \cup \{w_i\}$ for each $ i \in \{1,2,\dots,m-2\}$.  Since $W \cup \{x_{k+1}, y_{k+1}\}$ is a clique, clearly $\edgeG{W_i,w_i,x_{k+1},X,G_m}$, $\edgeG{W_i,w_i,y_{k+1},Y,G_m}$, and $\edgeG{W_i,w_i,w_j,W_j,G_m}$,   for each $1 \leq i < j \leq m-2$.  Therefore, in $\ig{G_m}$, the vertex set $\{W_1,W_2,\dots, W_{m-2}, X, Y\}$  is an induced clique.  	
	
	Now consider an $i$-set $X^* \neq X$ of $G_1$ and the $i$-set $W_i$ for some $1 \leq i \leq m-2$.   Using the same arguments that were applied to $X$ and $Y$ in Proposition \ref{prop:i:brg},  we see that $X^*$ and $W_i$ are non-adjacent in $\ig{G_m}$.  Likewise for some $i$-set $Y^*\neq Y$ and $W_i$, and then again for $X^*$ and $Y^*$.  It follows that $\ig{G_m} = H_m$.  
\end{proof}
% <<< E: Coro {coro:i:brg}	


Next, Proposition \ref{prop:i:disjointU} provides a method for combining two $i$-graphs without connecting them by an edge. 

%>>>S: Prop {prop:i:disjointU}
\begin{prop} \label{prop:i:disjointU}
	If $H_1$ and $H_2$ are $i$-graphs, then $H_1 \cup H_2$ is an $i$-graph.		
\end{prop}


\begin{proof}
	Suppose $G_1$ and $G_2$ are graphs such that $\ig{G_1}=H_1$ and $\ig{G_2} = H_2$.  We assume that  $i(G_1) = i(G_2) \geq 2$.  Otherwise, apply the Inflation Lemma (Lemma \ref{lem:i:anySize}) to obtain graphs with $i$-sets of equal size at least 2.  Let $G=G_1 \vee G_2$, the join of $G_1$ and $G_2$. We claim that $\ig{G} = H_1 \cup H_2$.   
	
	We proceed similarly to the proof of Proposition \ref{prop:i:brg}; namely, if $S$ is an $i$-set of $G_1$, of $G_2$, then $S$ is an independent dominating set of $G$.  Likewise, we observe that any $i$-set of $G$ is a subset of $G_1$ or $G_2$, and so, $S$ is a $i$-set of $G$ if and only if it is an $i$-set of $G_1$ or $G_2$.  
	
	Suppose $\edgeG{X,x,y,Y,G_1}$.  Then in $G$, sets $X$ and $Y$ are still $i$-sets, and likewise, vertices $X$ and $Y$ are still adjacent, and so $\edgeG{X,x,y,Y,G}$.  Now suppose instead that $X$ is an $i$-set of $G_1$ and $Y$ is an $i$-set of $G_2$.  Within $G$, $X \cap Y = \varnothing$ and $|X|=|Y| \geq 2$, so $X$ and $Y$ are not adjacent in $\ig{G}$.  Therefore, $\adjG{X,Y,G}$ if and only if $\adjG{X,Y,G_1}$ or $\adjG{X,Y,G_2}$.  It follows that $\ig{G}= \ig{G_1} \cup \ig{G_2} = H_1\cup H_2$ as required.	
\end{proof}
% <<< E: Prop {prop:i:disjointU}


Applying these new tools in combination yields some unexpected results.  For example, the following corollary, which makes use of the previous Proposition \ref{prop:i:disjointU} in partnership with the Deletion Lemma (a construction for combining $i$-graphs and a construction for vertex deletions) gives our first result on $i$-graph edge deletions.


%>>>S: Coro {coro:i:cutBridge}	
\begin{coro}\label{coro:i:cutBridge}	
	Let $H$ be an $i$-graph with a bridge $e$, such that the deletion of $e$ separates $H$ into components $H_1$ and $H_2$.  Then,
	\begin{enumerate}[itemsep=1pt, label=(\roman*)]	
		\item \label{coro:i:cutBridge:1} $H_1$ and $H_2$ are $i$-graphs, and
		\item \label{coro:i:cutBridge:2} the  graph $H^*=H-e$ is an $i$-graph. 	
	\end{enumerate}
\end{coro}

\begin{proof}
	Result \ref{coro:i:cutBridge:1} follows immediately from Lemma \ref{lem:i:inducedI}.  
	For \ref{coro:i:cutBridge:2}, by result \ref{coro:i:cutBridge:1}, $H_1$ and $H_2$ are $i$-graphs.  Then, from Proposition \ref{prop:i:disjointU}, the graph $H_1 \cup H_2 = H-e$ is also an $i$-graph. \\ \null \hfill
\end{proof}
% <<< E: Coro {coro:i:cutBridge}	


In the next result, we show that given $i$-graphs $H_1$ and $H_2$, a new $i$-graph can be formed by identifying any two vertices in $H_1$ and $H_2$.  This result provides an alternative proof for Theorem \ref{thm:i:forests}.


%>>>S: Prop {prop:i:cutV}	
\begin{prop}\label{prop:i:cutV}	
	Let $H_1$ and $H_2$ be $i$-graphs.  Then the graph $H$, formed by identifying a vertex $x$ of $H_1$ with a vertex $y$ of $H_2$, is also an $i$-graph.		
\end{prop}



%\begin{comment}
%~~~~~~~~~~~~~~~~~~~~~~~~~FIG START~~~~~~~~~~~~~~~~~~~~~~
\begin{figure}[H]
	\centering
	\begin{tikzpicture}					
		
		%---------- REF-------------------
		\node(cent) at (0,0) {};
		\path (cent) ++(180:25mm) node (Xcent)  {};	
		\path (cent) ++(0: 25mm) node (Ycent)  {};
		\path (Xcent)  ++(180:25mm) node (Acent)  {};
		\path (Ycent)  ++(0:25mm) node (Bcent)  {};	
		
		%---------- X References ------------------			
		\foreach \label/\i  in {1/90,2/270}
		\path (Xcent) ++(\i:7 mm) node (x\label)  {};		
		
		% ---------- Y References --------
		\foreach \label/\i  in {1/90,2/270}
		\path (Ycent) ++(\i:7 mm) node (y\label)  {};
		
		
		% ---------- Z References --------
		\path (cent) ++(90:25 mm) node [std](z11cent)  {};
		\path (z11cent) ++(90:4 mm) node [std](z11U)  {};
		\path (z11cent) ++(90:-4 mm) node [std](z11D)  {};
		\path (cent) ++(-90:15 mm) node [std](z22cent)  {};
		\path (z22cent) ++(90:4 mm) node [std](z22U)  {};
		\path (z22cent) ++(90:-4 mm) node [std](z22D)  {};
		\path (x1) ++(0:15 mm) node [std](z12cent)  {};
		\path (z12cent) ++(90:4 mm) node [std](z12U)  {};
		\path (z12cent) ++(90:-4 mm) node [std](z12D)  {};			
		\path (y1) ++(180:15 mm) node [std](z21cent)  {};
		\path (z21cent) ++(90:4 mm) node [std](z21U)  {};
		\path (z21cent) ++(90:-4 mm) node [std](z21D)  {};		
		
		% ---------- A = G1-X References --------
		\foreach \label/\i  in {1/10,2/5, 3/0, 4/-5, 5/-10}
		\path (Acent) ++(90:\i mm) node (a\label)  {};
		
		% A-B Bridge references
		\foreach \label/\i  in {1/10,2/63, 3/116,4/170 }
		\path (a1) ++ (\i:3 mm) node (aa\label)  {};
		
		% ---------- B = G2-Y References --------
		\foreach \label/\i  in {1/10,2/5, 3/0, 4/-5, 5/-10}
		\path (Bcent) ++(90:\i mm) node (b\label)  {};	
		
		% B-A Bridge references
		\foreach \label/\i  in{1/10,2/63, 3/116,4/170 }
		\path (b1) ++ (\i:3 mm) node (bb\label)  {};	
		
		
		% B-A Bridge references - C
		\foreach \label/\i  in{1/10,2/12, 3/14,4/16, 5/18 }
		\path (z11U) ++ (90:\i mm) node (c\label)  {};	
		
		%---------- Grey Lines ------------------			
		\foreach \i/\j in {1/-45,2/45}
		{\path (x\i) ++(180:6 mm) node (h\i)  {};
			\path (x\i) ++(\j:6 mm) node (hd\i)  {};
			\path (y\i) ++(0:-6 mm) node (j\i)  {};
			\path (y\i) ++(\j:-6 mm) node (jd\i)  {};
		}
		
		\foreach \i in {1,2}
		\foreach \j  in {1,3,5}
		{
			\draw [draw=gray, dashed] (x\i)--(a\j);
			\draw [draw=gray, dashed] (y\i)--(b\j);
		}
		
		%A-B Bridge Lines
		\foreach \i in {1,2,3,4}
		{
			
			\foreach \j in {1,2,3,4}
			{
				\draw[black] (aa\i) to [out=90,in=90](bb\j);
			}
			
		}
		
		\foreach \i in {1,2,3,4,5}
		{
			
			\foreach \j in {1,2,3,4,5}
			{
				%		\draw[black] (a\i) to [out=180,in=180](c\j);
				%		\draw[black] (b\i) to [out=0,in=0](c\j);
			}
			
		}
		
		
		
		%---------- BLOBS ------------------		
		\draw[draw=gray, fill=lgray] \convexpath{x1,x2}{6mm};	
		\draw[draw=gray, fill=lgray] \convexpath{y1,y2}{6mm};
		\draw[draw=gray, fill=lgray] \convexpath{a1,a5}{5mm};
		\draw[draw=gray, fill=lgray] \convexpath{b1,b5}{5mm};
		\draw[draw=gray, fill=lgray] \convexpath{z11U,z21U,z21D,z22D,z12D,z12U}{3mm};
		
		%----------PRINTS ------------------		
		\foreach \i in {1,2}
		{	\node [std](xD\i) at (x\i) {};	
			\path (x\i) ++(180: 3mm) node (xL\i)  {$x_{\i}$};	
			\node [std](yD\i) at (y\i) {};
			\path (y\i) ++(0: 3mm) node (yL\i)  {$y_{\i}$};
		}
		
		\foreach \i in {1,2,3,4,5}
		{	\node [std](aD\i) at (a\i) {};	
			\node [std](bD\i) at (b\i) {};
		}
		
		\foreach \j in {1,2} \foreach \k in {1,2} \foreach \i  in {cent,U,D}
		{
			\draw(xD\j)--(z\j\k\i)--(yD\k);
		}
		
		\foreach \i in {1,2} \foreach \j in {1,2} \foreach \k in {U,D,cent}
		{
			\node [std] (zD\i\j\k) at (z\i\j\k) {};
		}			
		
		
		\path (x2) ++(-90: 10mm) node (XL)  {$X$};		
		\path (y2) ++(-90: 10mm) node (YL)  {$Y$};		
		\path (a5) ++(-90: 10mm) node (GXL)  {$G_1-X$};	
		\path (b5) ++(-90: 10mm) node (GYL)  {$G_2-Y$};
		\path (z22D) ++(-90: 10mm) node (ZL)  {$Z$};	
		
	\end{tikzpicture}			
	\caption{Construction of $G$ in Proposition \ref{prop:i:cutV}.}
	\label{fig:i:cutV}	
\end{figure}
%~~~~~~~~~~~~~~~~~~~~~~~~~FIG END~~~~~~~~~~~~~~~~~~~~~~
%\end{comment}




\begin{proof}
	Suppose $G_1$ and $G_2$ are graphs such that $\ig{G_1}=H_1$ and $\ig{G_2} = H_2$.  As before, we assume  $i(G_1) = i(G_2)=k \geq 2$ via the Inflation Lemma.  Let $X=\{x_1,x_2,\dots,x_k\}$ and $Y = \{y_1,y_2,\dots,y_k\}$ be the $i$-sets corresponding to $x$ and $y$, respectively.  Construct the graph $G$ by adding $3k^2$ vertices to $G_1 \cup G_2$, labelled as $z_{i,j,\ell}$ for all $i,j\in\{1,2,\dots,k\}$ and $\ell \in \{1,2,3\}$, so that $z_{i,j,\ell}$ is adjacent to $x_i$ and $y_j$ for all $1 \leq \ell \leq 3$.  Let $Z$ be the set of these $z_{i,j,\ell}$ and note that $Z$ is an independent set.
	%$\displaystyle{Z = \bigcup_{\substack{1 \leq i,j \leq k \\ 1 \leq \ell \leq 3}} \{ z_{i,j,\ell}\}}$ 
	Finally, add edges between all vertices of $G_1\backslash X$ to all vertices of $G_2 \backslash Y$.
	We claim that $i(G)=2k$ and $\ig{G} = H$.
	
	First, observe that $X\cup Y$ is an independent dominating set of $G$, and so $i(G) \leq 2k$.  Let $S$ be some $i$-set of $G$. To show that $S \cap Z=\varnothing$, suppose to the contrary that some vertex of $Z$ is in $S$, say $z_{1,1,1} \in S$.  Then, for independence, neither $x_1$ nor $y_1$ is in $S$, and so both $z_{1,1,2}$ and $z_{1,1,3}$ are self-dominating  in $S$.   Since $x_1 \notin S$, for any $1 \leq j \leq k$, to dominate $Z_{1,j}=\{z_{1,j,1},z_{1,j,2},z_{1,j,3}\}$  requires either $Z_{1,j} \subseteq S$ or $y_j \in S$.  Likewise, since $y_1 \notin S$, for all $1 \leq i \leq k$, either $Z_{i,1} \subseteq S$ or $x_i \in S$.  Thus, $|S| \geq 3 + 2(k-1) = 2k+1$.  However, we have already established that $i(G) \leq 2k$, and  so, we conclude that $S \cap Z=\varnothing$.   
	
	Now, suppose that some for some $1 \leq i,j \leq k$,  $x_i \notin S$ and $y_j \notin S$.  Then, since $Z \cap S = \varnothing$, the vertices of $\{z_{i,j,1}, z_{i,j,2},z_{i,j,3}\}$ are undominated, contradicting that $S$ is an $i$-set.  Thus, any $i$-set of $G$ has either $X$ or $Y$ as a subset.  Suppose, without loss of generality, that $X \subseteq S$.  Then, all of $G_1\backslash X$ and $Z$ are dominated by $X$ (and none of $G_2$).  Now, since $N_G[G_2] \cap X = \varnothing$, the vertices of $G_2$ are internally dominated; thus $Y^*$ is an $i$-set of $G_2$ if and only if $X \cup Y^*$ is an $i$-set of $G$.	 Similarly, $X^*$ is an $i$-set of $G_1$ if and only if $Y \cup X^*$ is an $i$-set of $G$, and so $i(G)=2k$. 
	
	%As in the previous results, if $S \cap (G_1\backslash X) \neq \varnothing$ then $S \cap (G_2\backslash Y) = \varnothing$, and vice versa. 
	
	For adjacency, clearly $\edgeG{X_i, x_i, x_j, X_j,G_1}$ if and only if $\edgeG{(X_i\cup Y), x_i, x_j, (X_j\cup Y),G}$.  Similarly, $\edgeG{Y_i, y_i, y_j, Y_j,G_2}$ if and only if $\edgeG{(X\cup Y_i), y_i, y_j, (X\cup Y_j),G}$.  Consider some $i$-sets $X^*\neq X$ of $G_1$ and $Y^* \neq Y$ of $G_2$ and their corresponding $i$-sets in $G$: $(X^* \cup Y)$ and $(X \cup Y^*)$, respectively.  
	
	Since $|X \cap X^*| \geq 1$ and $|Y \cap Y^*| \geq 1$,   $|(X^* \cup Y) \cap (X \cup Y^*)| \geq 2$,  and so $(X^* \cup Y)$ and $(X \cup Y^*)$ are nonadjacent in $\ig{G}$.   Therefore, in $\ig{G}$, there are no edges between the subgraphs induced by $\ig{G_1}$ and $\ig{G_2}$.  Therefore,  $(X\cup Y)$ is a cut vertex, and we  conclude that $\ig{G} = H$.		
\end{proof}
% <<< E: Prop {prop:i:cutV}	

An alternative proof of Proposition \ref{prop:i:cutV} can be realized by utilizing Proposition \ref{prop:i:cart}.  Consider $i$-graphs $H_1$ and $H_2$, with equal sized $i$-set seed graphs $G_1$ and $G_2$, respectively.  From Proposition \ref{prop:i:cart}, there is some graph $G$ such that $\ig{G} = H_1 \boksie H_2$.  Since the graph $H$ described in the statement of Proposition \ref{prop:i:cutV} is an induced subgraph of  $H_1 \boksie H_2$,  applying Lemma \ref{lem:i:inducedI}, delete all other vertices of $H_1 \boksie H_2$ until only $H$ remains.



Combining the results of Proposition \ref{prop:i:cutV}	with Proposition \ref{prop:i:brg} and Corollary \ref{coro:i:cutBridge}, yields the following main result.

%>>>S: Theorem {thm:i:iffBlock}	
\begin{theorem}\label{thm:i:iffBlock}
	A graph $G$ is an $i$-graph if and only if all of its blocks are $i$-graphs.
\end{theorem}
% <<< E: Theorem  {thm:i:iffBlock}	



\noindent As observed in Corollary \ref{coro:i:notInduced}, graphs with an induced $\Dia$ subgraph are not $i$-realizable.  If we consider the family of connected chordal graphs excluding those with an induced copy of  $\Dia$, we are left with the family of block graphs (also called clique trees): graphs where each block is a clique.  As cliques are their own $i$-graph, the following is immediate.


%>>>S: Prop {prop:i:block}	
\begin{prop} \label{prop:i:block}
	Block graphs are $i$-graph realizable.  
\end{prop}
%<<<E: Prop {prop:i:block}	

Cacti are  graphs whose blocks are cycles or edges.  Thus, we have the following immediate corollary.


%Cacti are $i$-graphs (take cycles, join together at vertex, add leaves).  Alternatively, cacti have a single forbidden minor (ie, the Diamond graph $\Dia$)), so obviously $i$-graphs.

%>>>S: Coro {coro:i:cacti}	
\begin{coro} \label{coro:i:cacti}	
	Cactus graphs are $i$-graph realizable.  
\end{coro}
%<<<E: Coro {coro:i:cacti}	

While the proof of Proposition \ref{prop:i:cutV} does provide a method for building block graphs, it is laborious to do so on a graph with many blocks, as the construction is iterative, with each block being appended one at a time; moreover, when the edges between $G_1-X$ and $G_2-Y$  (as in Figure \ref{fig:i:cutV}) are added at each iteration, the resultant seed graph is often a confusing mess to behold.   
However, when we consider that the blocks of block graphs are complete graphs, and that complete graphs are their own $i$-graphs (and thus arguably the easiest to construct $i$-graphs), it is logical that there is a simpler construction.  We offer one such construction below that uses similar gadgets to the proof of Proposition \ref{prop:i:cutV}, but ultimately yields a cleaner and more illuminating seed graph.  An example of this process is illustrated in Figure \ref{fig:i:block}.


%>>> S: Construction {cons:i:block} 	
\begin{cons} \label{cons:i:block} Let $H$ be a block graph with $V(H) = \{v_1,v_2,\dots, v_n\}$ and let  $\mathcal{B}_H = \{B_1, B_2, \dots, B_m\}$ be the collection of maximal cliques of $H$.  	To construct a graph $G$ such that $\ig{G}=H$:
	
	\begin{enumerate}[itemsep=1pt, label=(\roman*)]	
		\item Begin with a copy of each of the maximal cliques of $H$, labelled $A_1, A_2, \dots, A_m$ in $G$, where $A_i$ of $G$ corresponds to $B_i$ of $H$ for each $1 \leq i \leq m$, and the $A_i$ are pairwise disjoint. Notice that each cut vertex of $H$ has multiple corresponding vertices in $G$.
		
		\item \label{item:cons:i:block:cutV} Let $v \in V(H)$ be a cut vertex and $\mathcal{B}_v$ be the collection of blocks containing $v$ in $H$; for notational ease, say  $\mathcal{B}_v= \{B_1,B_2,\dots,B_k\}$, and suppose that $W=\{w_1, w_2,\dots, w_k\} \subseteq V(G)$ are the $k$ vertices corresponding to $v$, where $w_i \in A_i$ for all $1 \leq i \leq k$.  
		
		For each distinct pair $w_i$ and $w_j$ of $W$, add to $G$ three internally disjoint paths of length two between $w_i$ and $w_j$.  Since $v$ is in $k$ blocks of $H$, $3\binom{k}{2}$ vertices are added in this process.  These additions are represented as the green vertices in Figure \ref{fig:i:block}.	
		
		\item Repeat Step \ref{item:cons:i:block:cutV} for each cut vertex of $H$.
	\end{enumerate}	
\end{cons}	
% <<< E: Construction {cons:i:block} 	




%~~~~~~~~~~~~~~~~~~~~~~~~~FIG START~~~~~~~~~~~~~~~~~~~~~~

\begin{figure}[H]
	\begin{minipage}{0.1\textwidth}
		(a)
	\end{minipage}	
	\begin{minipage}{0.8\textwidth} \centering
		\begin{tikzpicture}[line width=0.3mm,scale=1.3]			
			
			%---------- REF-------------------
			\node(cent) at (0,0) {};	
			
			\path (cent) ++(0:10 mm) node (centR)  {};
			\path (cent) ++(0:-10 mm) node (centL)  {};
			
			\path (centL) ++(0:-10 mm) node (centA)  {};
			\path (centL) ++(0: 0 mm) node (centB)  {};
			\path (centL) ++(0: 0 mm) node (centD)  {};
			\path (cent) ++(0: 0 mm) node (centE)  {};
			\path (centR) ++(0: 0 mm) node (centF)  {};
			
			%---------- A-------------------
			\foreach \label/\j in {2/90,3/180, 4/270}
			{	\path (centA) ++(\j:5 mm) node[std](a\label)  {};	
				%\draw(x)--(x\label);	
			}
			\path (centL) ++(0:0 mm) node[std](a1)  {};	
			\draw(a1)--(a2)--(a3)--(a4)--(a1)--(a3);
			\draw(a2)--(a4);
			
			%---------- B-------------------
			\foreach \label/\j in {1/0,2/8}
			{	\path (centB) ++(270:\j mm) node[std](b\label)  {};	
				%\draw(x)--(x\label);	
			}
			\draw(b1)--(b2);			
			
			%---------- D-------------------
			\foreach \label/\j in {1/0,2/8}
			{	\path (centD) ++(250:\j mm) node[std](d\label)  {};	
				%\draw(x)--(x\label);	
			}
			\draw(d1)--(d2);	
			
			%---------- E-------------------
			\foreach \label/\j/\k in {2/90/5, 4/240/10, 5/300/10}
			{	\path (centE) ++(\j:\k mm) node[std](e\label)  {};	
				%\draw(x)--(x\label);	
			}
			
			\path (centL) ++(0:0 mm) node[std](e3)  {};	
			\path (e3) ++(90:4 mm) node (el3)  {\color{red}$X_H$};	
			\path (centR) ++(0:0 mm) node[std](e1)  {};	
			
			\draw(e1)--(e2)--(e3)--(e4)--(e5)--(e1)--(e3)--(e5)--(e2)--(e4)--(e1);	
			
			%---------- F-------------------
			\foreach \label/\j in {2/45,3/-45}
			{	\path (centF) ++(\j:8 mm) node[std](f\label)  {};	
				%\draw(x)--(x\label);	
			}
			\path (centR) ++(0:0 mm) node[std](f1)  {};	
			\draw(f1)--(f2)--(f3)--(f1);	
			
			%\uncover<2->
			{
				\draw[ltteal, line width=1mm](f1)--(f2)--(f3)--(f1);
				\draw[medOrch, line width=1mm](e1)--(e2)--(e3)--(e4)--(e5)--(e1)--(e3)--(e5)--(e2)--(e4)--(e1);	
				\draw[forGreen, line width=1mm](d1)--(d2);
				\draw[brown, line width=1mm](b1)--(b2);
				\draw[orange, line width=1mm](a1)--(a2)--(a3)--(a4)--(a1)--(a3);
				\draw[orange, line width=1mm](a2)--(a4);
				
			}		
			
			%\uncover<5->
			{
				\node[byellow](s1) at (e2) {};	
			}
		\end{tikzpicture}			
	\end{minipage}	
%\end{figure}
%~~~~~~~~~~~~~ Split

\vspace{5mm}

%\begin{figure}[H]
	\begin{minipage}{0.1\textwidth}
		(b)
	\end{minipage}	
	\begin{minipage}{0.9\textwidth} \centering
		\begin{tikzpicture}[line width=0.3mm,scale=1.3]			
			
			%---------- REF-------------------
			\node(cent) at (0,0) {};	
			
			\path (cent) ++(0:10 mm) node (centR)  {};
			\path (cent) ++(0:-10 mm) node (centL)  {};
			
			\path (centL) ++(0:-55 mm) node (centA)  {};
			\path (centL) ++(0: -15 mm) node (centB)  {};
			\path (centL) ++(0: -15 mm) node (centD)  {};
			\path (cent) ++(0: 0 mm) node (centE)  {};
			\path (centR) ++(0: 0 mm) node (centF)  {};
			
			
			%	\uncover<3->
			{	
				%---------- A - ORANGE -------------------
				\foreach \label/\j in {2/90,3/180, 4/270, 1/0}
				{	\path (centA) ++(\j:5 mm) node[std](a\label)  {};	
					%\draw(x)--(x\label);	
				}
				%\path (centL) ++(0: mm) node[std](a1)  {};	
				\draw(a1)--(a2)--(a3)--(a4)--(a1)--(a3);
				\draw(a2)--(a4);
				
				%---------- B - BROWN -------------------
				\foreach \label/\j in {1/15,2/23}
				{	\path (centB) ++(90:\j mm) node[std](b\label)  {};	
					%\draw(x)--(x\label);	
				}
				\draw(b1)--(b2);
				
				
				%----------  D - GREEN -------------------
				\foreach \label/\j in {1/15,2/23}
				{	\path (centD) ++(270:\j mm) node[std](d\label)  {};	
					%\draw(x)--(x\label);	
				}
				\draw(d1)--(d2);	
				
				%---------- E - PURPLE -------------------
				\foreach \label/\j/\k in {2/90, 3/162, 4/234, 5/306, 1/18}
				{	\path (centE) ++(\j:8 mm) node[std](e\label)  {};	
					%\draw(x)--(x\label);	
				}
				
				\path (e3) ++(90:4 mm) node (el3)  {\color{red}$x_G$};	
				
				%\path (centL) ++(0:0 mm) node[std](e3)  {};	
				%\path (centR) ++(0:0 mm) node[std](e1)  {};	
				
				\draw(e1)--(e2)--(e3)--(e4)--(e5)--(e1)--(e3)--(e5)--(e2)--(e4)--(e1);	
				
				%---------- F - LTTEAL -------------------
				\path (centR) ++(0:10 mm) node[std](f1)  {};	
				
				\foreach \label/\j in {2/45,3/-45}
				{	\path (f1) ++(\j:8 mm) node[std](f\label)  {};	
					%\draw(x)--(x\label);	
				}
				
				\draw(f1)--(f2)--(f3)--(f1);	
				
				\draw[ltteal, line width=1mm](f1)--(f2)--(f3)--(f1);
				\draw[medOrch, line width=1mm](e1)--(e2)--(e3)--(e4)--(e5)--(e1)--(e3)--(e5)--(e2)--(e4)--(e1);	
				\draw[forGreen, line width=1mm](d1)--(d2);
				\draw[brown, line width=1mm](b1)--(b2);
				\draw[orange, line width=1mm](a1)--(a2)--(a3)--(a4)--(a1)--(a3);
				\draw[orange, line width=1mm](a2)--(a4);				
			}		
			
			%	\uncover<4->
			{
				%--------EF
				\node[regG] (ef) at ($(f1)!0.5!(e1)$) {};
				%	\path (e1) ++(-5: 9mm) node[regG](ef)  {};	
				\draw(e1)--(ef)--(f1);
				\foreach \label/\j in {1/90,2/-90}
				{
					\path (ef) ++(\j:3 mm) node[regG](ef\label)  {};
					\draw(e1)--(ef\label)--(f1);
				}
				
				%--------AB
				\node[regG] (ab) at ($(a1)!0.5!(b1)$) {};
				
				\draw(a1)--(ab)--(b1);
				\foreach \label/\j in {1/90,2/-90}
				{
					\path (ab) ++(\j:3 mm) node[regG](ab\label)  {};
					\draw(a1)--(ab\label)--(b1);
				} 	
				
				%--------AD
				\node[regG] (ad) at ($(a1)!0.5!(d1)$) {};
				
				\draw(a1)--(ad)--(d1);
				\foreach \label/\j in {1/90,2/-90}
				{
					\path (ad) ++(\j:3 mm) node[regG](ad\label)  {};
					\draw(a1)--(ad\label)--(d1);
				} 			 		
				
				%--------AE
				\node[regG] (ae) at ($(a1)!0.5!(e3)$) {};
				
				\draw(a1)--(ae)--(e3);
				\foreach \label/\j in {1/90,2/-90}
				{
					\path (ae) ++(\j:3 mm) node[regG](ae\label)  {};
					\draw(a1)--(ae\label)--(e3);
				} 		
				
				%--------DE
				\node[regG] (de) at ($(d1)!0.5!(e3)$) {};
				
				\draw(d1)--(de)--(e3);
				\foreach \label/\j in {1/90,2/-90}
				{
					\path (de) ++(\j:3 mm) node[regG](de\label)  {};
					\draw(d1)--(de\label)--(e3);
				} 	
				%--------DE
				\node[regG] (be) at ($(b1)!0.5!(e3)$) {};
				
				\draw(b1)--(be)--(e3);
				\foreach \label/\j in {1/90,2/-90}
				{
					\path (be) ++(\j:3 mm) node[regG](be\label)  {};
					\draw(b1)--(be\label)--(e3);
				} 		
				
				%--------DB
				
				\node[regG] (bd) at ($(b1)!0.7!(d1)$) {};
				\draw(b1)--(bd)--(d1);
				\foreach \label/\j in {1/0,2/180}
				{
					\path (bd) ++(\j:3 mm) node[regG](bd\label)  {};
					\draw(b1)--(bd\label)--(d1);
				} 					
				
			}
			
			%	\uncover<6->
			{
				\node[byellow] (se) at (e2){};
				\node[byellow] (sa) at (a1){};
				\node[byellow] (sb) at (b1){};
				\node[byellow] (sd) at (d1){};
				\node[byellow] (sf) at (f1){};
				
			}	  
		\end{tikzpicture}		
	\end{minipage}		
	\caption{The construction of $G$ from $H$  in the proof of Proposition \ref{prop:i:block}.}
	\label{fig:i:block}%
\end{figure}
%~~~~~~~~~~~~~~~~~~~~~~~~~FIG END~~~~~~~~~~~~~~~~~~~~~~




%>>>START inf proof
To see that the graph $G$ from Construction \ref{cons:i:block}  does indeed have $\ig{G}=H$, notice that $i(G)=m$, where $m$ is the number of blocks in $H$; if $X$ is an $i$-set of $G$, then $|X \cap A_i|$=1 for each $A_i \in \{A_1, A_2, \dots A_m\}$.  Moreover, no $i$-set of $G$ has vertices in the added green vertices, because, as with the proof of Proposition \ref{prop:i:cutV}, the inclusion of any one of these green vertices in an independent dominating set necessitates the addition of them all. 

In Figure \ref{fig:i:block}(b), the five yellow vertices form the $i$-set corresponding to the yellow vertex of $G$ in Figure \ref{fig:i:block}(a).  Only the token on the purple $K_5$ can move in $G$; the other four tokens remain frozen, thereby generating the corresponding purple $K_5$ of $H$.  It is only when the token on the purple $K_5$ is moved to the vertex $x_G$ that the tokens on the orange $K_4$, and the brown and green $K_2$'s, unfreeze one clique at a time.  This corresponds to the cut vertex $i$-set $X_H$ of $H$.  The freedom of movement now transfers from the purple  $K_5$ to any of the three other cliques, allowing for the generation of their associated blocks in  $G$ as required.
%<<< END inf proof



% <<< E:  Prop {prop:i:block}	


Finally, before we depart from block graphs, as chordal graphs are among the most well-studied families of graphs, we offer one additional reframing of this block graph result from the chordal graph perspective.   

%>>>S: Coro {coro:i:chordal}	
\begin{coro} A chordal graph $G$ is $i$-graph realizable if and only if $G$ is $\Dia$-free.
\end{coro}
% <<< E: Coro {coro:i:chordal}	

With the addition of Proposition \ref{prop:i:block} to the results used to build Observation \ref{obs:i:4v}, this leaves only the House graph (see Figure \ref{fig:i:houseConstruct}(b)) as unsettled with regard to its $i$-graph realizability among the 34 non-isomorphic graphs on five vertices.  Although not strictly a result concerning the construction of larger $i$-graphs from known results, we include the following short proposition here for the sake of completeness.


%>>>S: Prop {prop:i:house}
\begin{prop}\label{prop:i:house}
	The House graph $\house$ is an $i$-graph.
\end{prop}


To demonstrate Proposition \ref{prop:i:house}, we provide an exact seed graph for the $i$-graph:  the graph $G$ in Figure  \ref{fig:i:houseConstruct}(a) ($K_3$ with a $P_3$ tail) has  $\ig{G} =\house$.  The $i$-sets of $G$ and their adjacency are overlaid on $\mathcal{H}$ in Figure  \ref{fig:i:houseConstruct}(b).


%~~~~~~~~~~~~~~~~~~~~~~~~~FIG START~~~~~~~~~~~~~~~~~~~~~~
\begin{figure}[H]
	\centering	
	\begin{subfigure}{.4\textwidth}  \centering
		\begin{tikzpicture}			
			%---------- REF-------------------
			\coordinate (cent) at (0,0) {};
			
			%----- PAW -----
			\foreach \i / \j in {a/1,b/2,c/3}
			{
				\path(cent) ++(0: \j*10mm) node[std,label={ 90:${\i}$}]  (\i) {};
			}
			\draw[thick] (a)--(c);	
			
			\foreach \i / \j in {d/45,e/-45}
			{
				\path(c) ++(\j: 15 mm) node[std,label={ 2*\j:${\i}$}]  (\i) {};
			}
			
			\draw[thick](c)--(d)--(e)--(c);	
			
			\path (cent) ++ (90:30mm) coordinate (vfil) {};
			
			% ----- HOUSE -----
			
			%	\path(cent) ++(0: 70mm) coordinate (rcent) {};
			
			%	\path(rcent) ++(0: 10mm) node[std,label={ 90:$a$}]  (x) {};	
		\end{tikzpicture}
		\caption{A graph $G$ such that $\ig{G} = \mathcal{H}$.}
		\label{fig:i:houseConstruct:a}%
	\end{subfigure}	\hspace{1cm}
	\begin{subfigure}{.5\textwidth} \centering
		\begin{tikzpicture}			
			%---------- REF-------------------
			\coordinate (cent) at (0,0) {};
			
			%----- PAW -----
			\foreach \i / \j / \k in {1/a/e, 2/a/d, 3/b/d, 4/b/e}
			{
				\path(cent) ++(\i*90-45: 13mm) node[std,label={\i*90-45:$\{\j,\k\}$}]  (v\i) {};
			}
			\draw[thick] (v1)--(v2)--(v3)--(v4)--(v1);
			
			\path(cent) ++(90: 20mm) node[std,label={ 90:$\{a,c\}$}]  (v5) {};	
			
			\draw[thick] (v1)--(v5)--(v2);
			
		\end{tikzpicture}
		\caption{The House graph $\mathcal{H}$ with $i$-sets of $G$.}
		\label{fig:i:houseConstruct:b}%	
	\end{subfigure}		
	\caption{The graph $G$ for Proposition \ref{prop:i:house} with $\ig{G}=\mathcal{H}$.}
	\label{fig:i:houseConstruct}%
\end{figure}
%~~~~~~~~~~~~~~~~~~~~~~~~~FIG END~~~~~~~~~~~~~~~~~~~~~~

%<<< END proof

% <<< E: Prop {prop:i:house}


The observant reader will have noted that $\house$ is a theta graph, namely $\house = \thet{1,2,3}$.  Thus, an alternative confirmation that $\house$ is an $i$-graph is given with the other theta graph results in  Chapter \ref{ch:comp} (see Lemma \ref{lem:c:thet12k}).

Having established the foundation for constructing new $i$-graphs from known $i$-graphs, in the following Chapter \ref{ch:pathcycles}, we take a detour from $i$-graph realizability back to structural results to examine the properties of the $i$-graphs of paths and cycles.  The realizability of $i$-graphs returns in Chapter \ref{ch:comp}, where we characterize which theta graphs are $i$-graphs.



==> thetasM.tex <==
\chapter{Constructions of $i$-Graphs Using Complements}

\label{ch:comp}




	
When visualizing the connections between the $i$-sets of a graph $G$, it is sometimes advantageous to consider its complement, $\cp{G}$, instead. 
From a human perspective, it is curiously easier see to which vertices a vertex $v$ is adjacent, rather than to which vertices $v$ is nonadjacent.
This is especially true when $i(G) = 2$ or $3$, when we may interpret the adjacency of $i$-sets of $G$ as the adjacencies of edges and triangles (i.e. $K_3$), respectively, in $\cp{G}$.  

In the following sections, we examine how the use of graph complements can be exploited to construct the $i$-graph seeds for certain classes of line graphs, theta graphs, and maximal planar graphs.   In Sections \ref{sec:c:thetaComp} and \ref{sec:c:nonthetas} we further confirm that these theta graph constructions complete the full characterization of theta graphs that are $i$-graphs, by proving that each of the remaining theta graphs are not   realizable as $i$-graphs.



%---------------------------------------SECTION: Line Graphs----------------
\section{Line Graphs and Claw-free Graphs}	\label{sec:c:line}


To begin, consider a graph $G$ with $i(G)=2$ and where $X = \{u,v\}$ is an $i$-set of $G$.  In $\cp{G}$, $u$ and $v$ are adjacent, so $X$ is represented as the edge $uv$.  Moreover, no other vertex $w$ is adjacent to both vertices of $X$ in $\cp{G}$; otherwise, $\{u,v,w\}$ is independent in $G$, contrary to $X$ being an $i$-set.   %That is, if $uv\not\in E(G)$, then $uv$ does not belong to any triangles in $\cp{G}$.





Consider now the line graph of $\cp{G}$, $L(\cp{G})$.  If $X=\{u,v\}$ is an $i$-set of $G$, then $e=uv$ is an edge of $\cp{G}$ and hence $e$ is a vertex of $L(\cp{G})$.  Thus, the $i$-sets of $G$ correspond to a subset of the vertices of $L(\cp{G})$. In the case where $\cp{G}$ is triangle-free (that is, $G$ has no independent sets of cardinality three or more,  i.e. $G$  is well-covered), these  $i$-sets of $G$ are exactly the vertices of $L(\cp{G})$.
Now suppose $Y$ is an $i$-set of $G$ adjacent to $X$; say, $\edge{X,u,w,Y}$, so that $Y=\{v,w\}$.  Then, in $\cp{G}$, $f=vw$ is an edge, and so in $L(\cp{G})$, $f \in V(L(\cp{G}))$.  Since $e$ and $f$ are both incident with $v$ in $\cp{G}$, $ef \in E(L(\cp{G}))$.
That is, for $i$-sets $X$ and $Y$ of a well-covered graph $G$, $X \sim Y$ if and only if $X$ and $Y$ correspond to adjacent vertices in $L(\cp{G})$.   Thus $\ig{G} \cong L(\cp{G})$ for well-covered  graphs $G$ with $i(G) = \alpha(G)=2$.

In the example illustrated in Figure \ref{fig:c:compEx} below, $\mathcal{H}$ is the house graph, where $X=\{a,c\}$ and $Y=\{c,e\}$ are $i$-sets with $\edge{X,a,e,Y}$.  In $L(\cp{\mathcal{H}})$, the two vertices in each of these $i$-sets are likewise adjacent.   


%~~~~~~~~~~~~FIG START~~~~~~~~~~~
\begin{figure}[H]
	\centering
	\begin{tikzpicture}%[line width=0.3mm,scale=1]			
		
		%---------- REF-------------------
		\node(cent) at (0,0) {};			
		\path (cent) ++(0:50 mm) node(mcent)  {};	
		\path (cent) ++(0:100 mm) node(rcent)  {};
		
		%----- box ----------	
		\foreach \i/\c in {a/-135,b/135,d/45, e/-45} {				
			\path (cent) ++(\c:10 mm) node [std] (v\i) {};
			\path (v\i) ++(\c:5 mm) node (Lv\i) {${\i}$};
		}
		
		\draw[thick] (va)--(vb)--(vd)--(ve)--(va)--cycle;
		
		\path (cent) ++(90:15 mm) node [std] (vc) {};
		\path (vc) ++(90:5 mm) node (Lvc) {${c}$};
		
		\draw[thick] (vb)--(vc)--(vd);	
		
		\path (cent) ++(-90: 20mm) node (HL)  {$\mathcal{H}$};
		
		
		%----- mid obj ----------	
		\foreach \i/\c in {a/-135,b/135,d/45, e/-45} {				
			\path (mcent) ++(\c:10 mm) node [std] (m\i) {};
			\path (m\i) ++(\c:5 mm) node (Lm\i) {${\i}$};
		}
		
		\path (mcent) ++(90:15 mm) node [std] (mc) {};
		\path (mc) ++(90:5 mm) node (Lmc) {${c}$};
		
		\draw[thick] (mb)--(me)--(mc)--(ma)--(md);
		
		\path (mcent) ++(-90: 20mm) node (HcL)  {$\cp{\mathcal{H}}$};
		
		%----- far obj ---------
		\foreach \i/\j/\c in {c/e/-135,b/e/135,a/d/45, a/c/-45} {				
			\path (rcent) ++(\c:10 mm) node [std] (r\i\j) {};
			\path (r\i\j) ++(\c:8 mm) node (Lr\i\j) {$\{\i,\j\}$};
		}
		
		\draw[thick] (rbe)--(rce)--(rac)--(rad);
		\path (rcent) ++(-90: 20mm) node (HiL)  {$L(\cp{\mathcal{H}}) \cong \ig{\mathcal{H}}$};
		
	\end{tikzpicture}				
	\caption{The complement and line graphs complement of the well-covered house graph $\mathcal{H}$.}
	\label{fig:c:compEx}
\end{figure}
%~~~~~~~~~~~~~FIG END~~~~~~~~~~~~~


Before continuing with the theme of $i$-graph realizability, we make the following observation on the order of $\ig{G}$ when $i(G)=2$.	


%>>> START Prop {prop:c:numb2isets}
\begin{prop} 
	\label{prop:c:numb2isets}
	Let $G$ be a graph of order $n$ with $i(G)=2$.  Then $G$ has at most $ \frac{1}{2}n(n-1) - \frac{1}{2}\sum_{v\in V(G)} deg(v)$ distinct $i$-sets.  That is, $|V(\ig{G})| \leq  \frac{1}{2}n(n-1) - \frac{1}{2}\sum_{v\in V(G)} \deg(v)$.
\end{prop}

\begin{proof}
	Since $i(G)=2$, each $i$-set of $G$ corresponds to an edge of $\cp{G}$.  So, $|V(\ig{G})| \leq  |E(\cp{G})|=\binom{n}{2} - |E(G)| =  \frac{1}{2}n(n-1) - \frac{1}{2}\sum_{v\in V(G)} \deg(v)$.
\end{proof}
% <<< END: Prop {prop:c:numb2ise`ts}

This connection between graphs with $i(G)=2$ and line graphs helps us not only understand the structure of $\ig{G}$, but also lends itself towards some interesting realizability results.  
We follow this thread for the remainder of this section, and build towards determining the $i$-graph realizability of line graphs and claw-free graphs.

%>>> START Lemma {lem:c:lineK3}
\begin{lemma}
	\label{lem:c:lineK3}
	%The line graphs of a connected graph $G$ contains $\Dia$ as an induced subgraph if and only if $G$ is not $K_3$ and $G$ contains a triangle.
	
	%\ft{OR:} 
	The line graph of a connected graph $G$ of order at least four contains $\Dia$ as an induced subgraph if and only if $G$ contains a triangle. 
\end{lemma}

\begin{proof}
	Suppose $G$ contains a triangle with vertices $a,b,$ and $c$, and let $d\notin \{a,b,c\}$ be a vertex adjacent to (say) $a$.  Then $\{ab, ac, ad\}$ and $\{ab,ac,bc\}$ are triangles in $L(G)$.  Since $\{b,c\} \cap \{a,d\} = \varnothing$ in $G$, $bc$ is nonadjacent to $ad$ in $L(G)$.  That is,  $\Dia$ is an induced subgraph of $L(G)$.
	
	Conversely, suppose $L(G)$ contains $\Dia$ as an induced subgraph.  Then, $G$ has at least four edges, and hence $G \not\cong K_3$.  
	Since the graph $H$ in Figure \ref{fig:c:paw} (i.e. ``the paw" or the ``3-pan") has $L(H) \cong \Dia$, it follows from the uniqueness of line graphs  (see \cite{W32})
	% in \cite{Hara}) 
	that $G$ contains $H$ as a subgraph.
\end{proof}
% <<< END: Lemma {lem:c:lineK3}



\begin{figure}[H] \centering	
	\begin{tikzpicture}			
		%---------- REF-------------------
		\node(cent) at (0,0) {};
		\path (cent) ++(0,0 mm) node(lcent)  {};			
		\path (cent) ++(0:50 mm) node(mcent)  {};	
		
		%----- paw ----------	
		\node[std,label={0:$a$}]  at (lcent) (va) {}; 
		
		%-d
		\path (lcent) ++(90:10 mm) node [std] (vd) {};
		\path (vd) ++(90:5 mm) node (Lvd) {${d}$};
		%-c
		\path (lcent) ++(180:10 mm) coordinate (hc1) {};	
		\path (hc1) ++(-90:10 mm) node [std] (vc) {};
		\path (vc) ++(-90:5 mm) node (Lvc) {${c}$};	
		
		%-b
		\path (vc) ++(0:20 mm) node [std] (vb) {};
		\path (vb) ++(-90:5 mm) node (Lvb) {${b}$};	
		
		\draw[thick](va)--(vb)--(vc)--(va)--cycle;
		\draw[thick](va)--(vd);	
		
		\path (cent) ++(-90: 22mm) node (HL)  {$H$};		
		
		%----- mid obj ----------	
		\foreach \i/\c in {ad/0,ac/90,bc/180, ab/-90} {				
			\path (mcent) ++(\c:10 mm) node [std] (m\i) {};
			\path (m\i) ++(\c:5 mm) node (Lm\i) {${\i}$};
		}
		
		\draw[thick] (mad)--(mac)--(mbc)--(mab)--(mad) -- cycle;
		\draw[thick] (mac)--(mab);
		
		\path (mcent) ++(-90: 22mm) node (HcL)  {$L(H) \cong \Dia$};		
	\end{tikzpicture}
	\caption{The ``paw'' $H$ with $L(H) \cong \Dia$.}
	\label{fig:c:paw}		
\end{figure}


%*REFREF* Harary Textbook Theorem 8.3 - H. Whitney, Congruent Graph and Connectivity of Graphs, Amer J Math. 54 1932 150-169


%>>> START Theorem {thm:c:line}
\begin{theorem}
	\label{thm:c:line}  Let $H$ be a connected line graph.  Then $H$ is an $i$-graph if and only if $H$ is $\Dia$-free.	
\end{theorem}

\begin{proof}  Suppose $H$ is an $i$-graph.  By Proposition \ref{prop:i:diamond} 
	%($\Dia$ result)
	and Corollary \ref{coro:i:notInduced},  
	%(induced subgraphs result), 
	$H$ is $\Dia$-free.
	
	Conversely, suppose that $H$ is $\Dia$-free.  If $H$ is complete, then $H$ is the $i$-graph of itself.  So, assume that $H$ is not complete.  Say $H$ is the line graph of some graph $F$, where we may assume $F$ has no isolated vertices (as isolated vertices do not affect line graphs).  Since $H$ is $\Dia$-free and connected, $F$ has no triangles by Lemma  \ref{lem:c:lineK3}.  Since $F$ has edges (which it does since $H$ exists), $
	\alpha(\cp{F}) \leq 2$.  Moreover, as $F$ is connected, $\cp{F}$ has no universal vertices, and so $i(\cp{F})\geq 2$.   Thus, $i(\cp{F}) = \alpha(\cp{F})$ and $\cp{F}$ is well-covered. It follows that every edge of $F$ corresponds to an $i$-set of $\cp{F}$.  Since $H$ is the line graph of $F$, it is the $i$-graph of $\cp{F}$.  
\end{proof}
% <<< END: Theorem {thm:c:line}

Finally, if we examine Beineke's forbidden subgraph characterization for line graphs (see \cite{B70}), it is interesting to note that eight of the nine minimal non-line graphs contain an induced $\Dia$, and are therefore not $i$-graphs.  The ninth minimal non-line graph is the claw, $K_{1,3}$.  Thus, claw-free graphs without an induced $\Dia$ are $\Dia$-free line graphs, and therefore are $i$-graphs. 

%>>> START  Coro {coro:c:clawfree} 
\begin{coro}	\label{coro:c:clawfree}  
	Let $H$ be a connected claw-free graph.  Then $H$ is an $i$-graph if and only if $H$ is $\Dia$-free.	
\end{coro}

\begin{proof}
	If $H$ is $i$-graph realizable, it is $\Dia$-free.
	Conversely, suppose that $H$ is $\Dia$-free.  Then by the forbidden subgraph characterization of line graphs \cite{B70}, $H$ is a line graph.  From Theorem \ref{thm:c:line}, $H$ is a $\Dia$-free line graphs and thus an $i$-graph.
\end{proof}
% <<< END: Coro {coro:c:clawfree} 

While Theorem \ref{thm:c:line} and Corollary \ref{coro:c:clawfree} reveal the $i$-graph realizability of many famous graph families (including another construction for cycles, which are connected, claw-free, and $\Dia$-free), the realizability problem for graphs containing claws remains unresolved.  Moreover, among clawed graphs are the theta graphs which we first alluded to in Section \ref{sec:i:Real} as containing three of the small known non-$i$-graphs.  In the next section we apply similar techniques with graph complements to construct all theta graphs that are realizable as $i$-graphs.    


%---------------------------------------SECTION: Graph Complements ----------------
\section{Theta Graphs From Graph Complements} \label{sec:c:thetaComp}

Consider now a graph $G$ with $i(G)=3$.  Each $i$-set of $G$ is represented as a triangle (i.e., an induced $K_3$) in $\cp{G}$.  
%We adhere to the convention that all triangles are \emph{maximal} $K_3$ cliques; that is, if the vertices $\{u,v,w,x\}$ form a clique, then $\{u,v,w\}$ is not considered to be a triangle.  
If $X$ and $Y$ are two $i$-sets of $G$ with $\edge{X,u,v,Y}$, then $\cp{G}[X]$ and $\cp{G}[Y]$ are triangles in $\cp{G}$, and have $|X \cap Y| =2$.  Although it is technically the induced subgraphs $\cp{G}[X]$ and $\cp{G}[X]$ that are the triangles of $\cp{G}$,  for notational simplicity going forward, we refer to $X$ and $Y$ as triangles.  In $\cp{G}$, the triangle $X$ can be transformed into the triangle $Y$ by removing the vertex $u$ and adding in the vertex $v$  (where $u\not\sim_{\cp{G}} v$).  Thus, we say that two triangles are \emph{adjacent} if they share exactly one edge (two vertices).  Moreover, since two $i$-sets of a graph $G$ with $i(G)=3$ are adjacent if and only if their associated triangles in $\cp{G}$ are adjacent, we use the same notation for $i$-set adjacency in $G$  as triangle adjacency in $\cp{G}$; that is, the notation $X \sim Y$ represents both $i$-sets $X$ and $Y$ of $G$ being adjacent, and triangles $X$ and $Y$ of $\cp{G}$ being adjacent.

In the following section,  we use triangle adjacency to construct \emph{complement seed graphs} for the $i$-graphs of theta graphs; that is, a graph $\cp{G}$ such that $\ig{G}$ is isomorphic to some desired theta graph. Before proceeding with these constructions, we note some observations which will help us with this process.


\begin{obs}\label{obs:c:cutEdge}
	If a graph $\cp{G}$ has a bridge, then $i(G) \leq 2$.   
\end{obs}


\begin{obs}\label{obs:c:i3}
	A graph  $G$ has $i(G)=2$ if and only if  $\cp{G}$ is nonempty and has an edge that does not lie on a triangle.
\end{obs}

\noindent If $\cp{G}$ has an edge $uv$ that does not lie on a triangle, then every other vertex is  adjacent to at least one of $u$ or $v$ in $G$.  That is, $\{u,v\}$ is independent and dominating in $G$, and so $i(G) \leq 2$.  When building our various seed graphs with $i(G)=3$, it is therefore necessary to ensure that every edge of the complement $\cp{G}$ belongs to a triangle.

%Similarly, if $G$ is a graph with $i(G)=3$, then $\cp{G}$ contains at least one maximal $K_3$ clique (and no cut-edges).  If the vertices $\{u,v,w,x\}$ form a (possibly non-maximal) clique in $\cp{G}$, then we can disregard the triangle formed by any three vertices of the set as it does not represent an $i$-set of $G$.  For example, although $\{u,v,w\}$ forms a triangle in $\cp{G}$, $x$ is not dominated by $\{u,v,w\}$.  

\begin{obs}
	Let $G$ be a graph with $i(G)=3$.  If  $S$ with $|S| \geq 4$ is a (possibly non-maximal) clique in $\cp{G}$, then no three-vertex subset of $S$ is  an $i$-set of $G$.
\end{obs}


\noindent Suppose that $S=\{u,v,w,x\}$ is such a clique of $\cp{G}$.  Then, for example, $x$ is undominated by $\{u,v,w\}$ in $G$, and so $\{u,v,w\}$ is not an $i$-set of $G$.  
Conversely, suppose that $\{u,v,w\}$ is a triangle in a graph $\cp{G}$ with $i(G)=3$.  By attaching a new vertex $x$ to all of $\{u,v,w\}$ in $\cp{G}$, we remove $\{u,v,w\}$ as an $i$-set of $G$, while keeping all other $i$-sets of $G$.  This observation proves to be very useful in the constructions  in the following section: we now have a technique to eliminate any unwanted triangles in $\cp{G}$ (and hence $i$-sets of $G$) that may arise.  Notice that this technique is an application of the Deletion Lemma (Lemma \ref{lem:i:inducedI}) in $\cp{G}$, instead of the usual $G$.

%\begin{obs}
%	Let $G$ be a graph on at least two vertices.   If for each $uv\in E(\cp{G})$, there exists some vertex $w$ such that $uw$ and $vw \in E(\cp{G})$, then $i(G) =3$. 
%\end{obs}


The use of triangle adjacency in a graph $\cp{G}$ to determine $i$-set adjacency in $G$ provides a key technique to finally resolve a question posed in Chapter \ref{ch:igraphs}: which theta graphs are $i$-graphs?  In the following Theorem \ref{thm:c:thetas}, we show that all theta graphs except the seven listed exceptions are $i$-graphs.  The proofs of the lemmas for the affirmative cases make up most of the remainder of Section \ref{sec:c:thetaComp}, and  almost all use this method of complement triangles.  The proofs of  the lemmas for the seven negative cases are given in Section \ref{sec:c:nonthetas}.  

\begin{theorem}\label{thm:c:thetas}
	%All theta graphs except the seven listed in Table \ref{tab:c:thetaLong} are $i$-graphs.
	
	A theta graph is an $i$-graph if and only if it is not one of the seven exceptions listed below: 
	
	\begin{tabular}{lllll}  \centering
		$\thet{1,2,2}$, 	&&&&	\\
		$\thet{2,2,2}$,	\	&		$\thet{2,2,3}$,	\	&		$\thet{2,2,4}$,  \  &	$\thet{2,3,3}$, \ 	&		$\thet{2,3,4}$, \ 	\\
		$\thet{3,3,3}.$ &&&& \\
	\end{tabular}
	
	
\end{theorem}

%\nts{Is the list of 7 above good as is?  Or would it be better with all 7 on a single line?}


\noindent Table \ref{tab:c:thetaLong} summarizes the cases used to establish Theorem \ref{thm:c:thetas} and their associated results.   





\begin{table}[H] \centering
	\begin{tabular}{|l|l|l|}  \hline
		$\thet{j,k,\ell}$	&	Realizability	&	Result	\\	\hline
	%	&		&		\\	
		$\thet{1,2,2}$	&	non-$i$-graph	&	$\Dia$.  Proposition \ref {prop:i:diamond}	\\	
		$\thet{1,2,\ell}$, $\ell \geq 3$ 	&	$i$-graph	&	Lemma \ref{lem:i:cliqueRep}	\\	
		$\thet{1,k,\ell}$, $3 \leq k \leq \ell$ 	&	$i$-graph	&	Lemma \ref{lem:c:thet1kl}	\\	
		&		&		\\	
		$\thet{2,2,2}$	&	non-$i$-graph	&	$K_{2,3}$.  Proposition \ref{prop:i:K23}	\\	
		$\thet{2,2,3}$	&	non-$i$-graph	&	$\kappa$.  Proposition \ref{prop:i:kappa}	\\	
		$\thet{2,2,4}$	&	non-$i$-graph	&	Proposition \ref{prop:c:thet224}	\\	
		$\thet{2,2,\ell}$, $\ell\geq 5$	&	$i$-graph	&	Lemma \ref{lem:c:thet22l}	\\	
		$\thet{2,3,3}$	&	non-$i$-graph	&	Proposition \ref{prop:c:thet233}	\\	
		$\thet{2,3,4}$	&	non-$i$-graph	&	Proposition \ref{prop:c:thet234}	\\	
		$\thet{2,3,\ell}$, $\ell\geq 5 $	&	$i$-graph	&	Lemma \ref{lem:c:thet23k}	\\	
		$\thet{2,4,4}$	&	$i$-graph	&	Lemma \ref {lem:c:thet244}	\\	
		$\thet{2,k,5}$, $4 \leq k \leq 5$	&	$i$-graph	&	Lemma \ref{lem:c:thet2k5}	\\	
		$\thet{2,k,\ell}$, $k \geq 4$, $\ell \geq 6$, $\ell \geq k$	&	$i$-graph	&	 Lemma \ref{lem:c:thet2kl}	\\	
		&		&		\\	
		$\thet{3,3,3}$	&	non-$i$-graph	&	 Proposition \ref{prop:c:thet333}	\\	
		$\thet{3,3,4}$	&	$i$-graph	&	Lemma \ref{lem:c:thet334}	\\	
		$\thet{3,3,5}$	&	$i$-graph	&	Lemma \ref {lem:c:thet335}	\\	
		$\thet{3,3,\ell}$, $\ell\geq 6$	&	$i$-graph	&	Lemma \ref {lem:c:thet33k}	\\	
		$\thet{3,4,4}$	&	$i$-graph	&	Lemma \ref{lem:c:thet344}	\\	
		$\thet{3,4,\ell}$, $\ell\geq 5$	&	$i$-graph	&	Lemma \ref{lem:c:thet34k}	\\	
		$\thet{3,5,5}$	&	$i$-graph	&	Lemma \ref{lem:c:thet355}	\\	
		&		&		\\	
		$\thet{4,4,4}$	&	$i$-graph	&	Lemma \ref{lem:c:thet444}	\\	
		$\thet{j,k,5}$, $4 \leq j \leq k \leq 5 $.	&	$i$-graph	&	Lemma \ref{lem:c:thetjk5}	\\	
		$\thet{j,k,\ell}$, $3 \leq j \leq k \leq \ell$, and $\ell \geq 6$.	&	$i$-graph	&	Lemma \ref{lem:c:thetjkl}	\\	\hline
	\end{tabular} \caption{$i$-graph realizability of theta graphs.} \label{tab:c:thetaLong}
\end{table}



\begin{comment}
	
	\begin{table}[H] \centering
		\begin{tabular}{|l|l|l|}  \hline
			$\thet{j,k,\ell}$	&	Realizability	&	Note	\\ \hline
			&		&		\\
			$\thet{1,2,2}$	&	non-$i$-graph	&	$\Dia$.  Proposition \ref {prop:i:diamond}	\\
			$\thet{1,2,\ell}$, $\ell \geq 3$ 	&	$i$-graph	&	Lemma \ref{lem:i:cliqueRep}	\\
			$\thet{1,k,\ell}$, $3 \leq k \leq \ell$ 	&	$i$-graph	&	Lemma \ref{lem:i:t(1kl)}	\\
			&		&		\\
			$\thet{2,2,2}$	&	non-$i$-graph	&	$K_{2,3}$.  Proposition \ref{prop:i:K23}	\\
			$\thet{2,2,3}$	&	non-$i$-graph	&	$\kappa$.  Proposition \ref{prop:i:kappa}	\\
			$\thet{2,2,4}$	&	non-$i$-graph	&	Proposition \ref{prop:c:thet224}	\\
			$\thet{2,2,\ell}$, $\ell\geq 5$	&	$i$-graph	&	K1: Lemma 3	\\
			$\thet{2,3,3}$	&	non-$i$-graph	&	Proposition \ref{prop:c:thet233}	\\
			$\thet{2,3,4}$	&	non-$i$-graph	&	Proposition \ref{prop:c:thet234}	\\
			$\thet{2,3,\ell}$, $\ell\geq 5$	&	$i$-graph	&	K1: Lemma 4	\\
			$\thet{2,4,4}$	&	$i$-graph	&	K1: Lemma 5	\\
			$\thet{2,k,\ell}$, $k\geq 4$, $\ell \geq 5$	&	$i$-graph	&	K1: Lemma 4	\\
			&		&		\\
			$\thet{3,3,3}$	&	non-$i$-graph	& Proposition \ref{prop:c:thet333}	\\
			$\thet{3,3,4}$	&	$i$-graph	&	K1: Lemma 6	\\
			$\thet{3,3,\ell}$, $\ell\geq 5$	&	$i$-graph	&	K1: Lemma 7	\\
			$\thet{3,4,4}$	&	$i$-graph	&	K1: Lemma 6	\\
			$\thet{3,4,\ell}$, $\ell\geq 5$	&	$i$-graph	&	K1: Lemma 7	\\
			$\thet{3,k,\ell}$, $5\leq k \leq \ell$	&	$i$-graph	&	K1: Lemma 7	\\
			&		&		\\
			$\thet{j,k,\ell}$, $4 \leq j \leq k \leq \ell$.	& $i$-graph	&	No reference!	\\	
			\hline
		\end{tabular} \caption{$i$-graph realizability of theta graphs.} \label{tab:c:thetaLong}
	\end{table}
	
\end{comment}

%......................  SUB SECTION:  theta (1,k,l) .........................
\subsection{$\thet{1,k,\ell}$}  \label{subsec:c:1kl}



We have already seen that the diamond graph $\Dia = \thet{1,2,2}$ is not an $i$-graph  (Proposition \ref{prop:i:diamond}) and that the House graph $\mathcal{H} = \thet{1,2,3}$ is an $i$-graph (Proposition \ref{prop:i:house}).  Indeed, we can further exploit previous results to see that all graphs $\thet{1,2,\ell}$ for $\ell \geq 3$ are $i$-graphs by taking a cycle $C_n$ with $n \geq 4$, and replacing one of its maximal cliques (i.e. an edge) with a $K_3$.  By the Max Clique Replacement Lemma (Lemma \ref{lem:i:cliqueRep}), the resultant $\thet{1,2,n-1}$ is also $i$-graph.
Notice that when we likewise attempt to replace an edge of a $C_3$ with a $K_3$, the result no longer holds; a single edge in a $C_3$ is not  a maximal clique.   For reference, we explicitly state this result as a lemma below.

\begin{lemma} \label{lem:c:thet12k}  
	For $\ell \geq 3$, the theta graphs $\thet{1,2,\ell}$ are $i$-graphs.
\end{lemma}



%In the following sections, we determine the $i$-graph realizability of all theta graphs, dividing our results into subsections by the length of the theta graph's shortest path.  




%______________________  SUBSUB SECTION:  theta (1,k,l) ______________________
\subsubsection{Construction of $\cp{G}$ for $\thet{1,k,\ell}$, $3 \leq k \leq \ell$}  \label{subsubsec:c:1kl+}




In Figure \ref{fig:c:thet145} below, we provide a first example of the technique we employ repeatedly throughout this section to construct our theta graphs.  To the left is a graph $\cp{G}$, where each of its nine triangles corresponds to an $i$-set of its complement $G$.  The resultant $i$-graph of $G$, $\ig{G} = \thet{1,4,5}$, is presented on the right.  For consistency, we use $X$ and $Y$ to denote the triangles corresponding to the degree 3 vertices in the theta graphs in this example, as well as all constructions to follow.



%>>>S: Figure {fig:c:thet145}	
\begin{figure}[H] \centering	
	\begin{tikzpicture}	
		
		%---------- REF-------------------
		\node (cent) at (0,0) {};
		\path (cent) ++(0:40 mm) node (rcent) {};	
		
		%----- W0 - Left Wheel ----------
		\node [std] at (cent) (w0) {};
		\path (w0) ++(40:4 mm) node (w0L) {$w_0$};
		
		\foreach \i/\c in {1/90,3/270,4/210, 5/150} {				
			\path (w0) ++(\c:20 mm) node [std] (w\i) {};
			\path (w\i) ++(\c:5 mm) node (Lw\i) {$w_{\i}$};
			\draw [thick] (w0)--(w\i);
		}
		
		%Node W2
		\path (w0) ++(0:20 mm) node [std] (w2) {};
		\path (w2) ++(90:5 mm) node (Lw2) {$w_{2}$};
		\draw [thick] (w0)--(w2);	
		
		\draw  [thick] (w1)--(w2)--(w3)--(w4)--(w5)--(w1);		
		
		%----- Right Path ----------
		\foreach \i/\c in {1/15,2/0,3/-15} {				
			\path (rcent) ++(90:\c mm) node [bblue] (v\i) {};
			\path (v\i) ++(0:5 mm) node [color=blue] (Lv\i) {$v_{\i}$};
			\draw[bline] (w2)--(v\i);
		}
		\draw[bline] (w1)--(v1)--(v2)--(v3)--(w3);	
		
		%-- X and Y
		\path (w0) ++(45:10 mm) node  [color=red] (LX) {$X$};
		\path (w0) ++(-45:10 mm) node  [color=red] (LY) {$Y$};
		
		%-- D's	
		\foreach \i/\c in {1/120,2/180,3/240} {				
			\path (w0) ++(\c:12 mm) node [color=red] (A\i) {$A_{\i}$};	
		}		
		
		%-- B's	
		\foreach \i/\c in {1/90, 2/18, 3/-18, 4/-90} {				
			\path (w2) ++(\c:12 mm) node [color=red] (B\i) {$B_{\i}$};	
		}	
		\node[broadArrow,fill=white, draw=black, ultra thick, text width=6mm] at (5.8cm,0){};
	\end{tikzpicture}
	\begin{tikzpicture}		
		%---------- REF-------------------	
		\node (cent) at (0,0) {};
		\node  at (cent) (w0) {};
		\path (w0) ++(0:20 mm) node (w2) {};	
		
		%-- X and Y
		\path (w0) ++(45:10 mm) node [bred] (X) {};
		\path (X) ++(90:5 mm) node [color=red] (LX) {$X$};
		
		\path (w0) ++(-45:10 mm) node [bred] (Y) {};
		\path (Y) ++(-90:5 mm) node [color=red] (LY) {$Y$};
		
		\draw [rline] (X)--(Y);	
		
		%-- A's	
		\foreach \i/\c in {1/120,2/180,3/240} {			
			\path (w0) ++(\c:12 mm) node [bred] (A\i) {};		
			\path (A\i) ++(\c:5 mm) node [color=red] (LA\i) {$A_{\i}$};	
		}		
		\draw [rline] (X)--(A1)--(A2)--(A3)--(Y);
		
		%-- B's	
		\foreach \i/\c in {1/90, 2/22, 3/-22, 4/-90} {				
			\path (w2) ++(\c:15 mm) node [bred] (B\i) {};
			\path (B\i) ++(\c:5 mm) node [color=red] (LB\i) {$B_{\i}$};	
		}	
		\draw [rline] (X)--(B1)--(B2)--(B3)--(B4)--(Y);	
		
		%--- Force vertical spacing
		\path (Y) ++(-90: 20mm) node (S) {};		
		
	\end{tikzpicture}
	\caption{A graph $\cp{G}$ (left) such that $\ig{G} = \thet{1,4,5}$ (right).}
	\label{fig:c:thet145}	
\end{figure}						
% <<< E: Figure {fig:c:thet145}

We proceed now to the general construction of a graph $\cp{G}$ with $\ig{G}=\thet{1,k,\ell}$ for $3 \leq k \leq \ell$.   As it is our first construction using this triangle technique, we provide the construction and proof for Lemma \ref{lem:c:thet1kl} with an abundance of detail.   




\begin{cons} \label{cons:c:thet1kl} (See Figure \ref{fig:c:thet1kl})  
	Let $\overline{H}\cong W_{k+2}=C_{k+1}\vee K_{1}$, where
	$C_{k+1}=(w_{1},...,w_{k+1},w_{1})$ and $w_{0}$ 
	is the central hub, that is, the vertex with degree $k+1$.  Add a path $P_{\ell-2}%
	:(v_{1},...,v_{\ell-2})$, joining each $v_{i},\ i=1,...,\ell-2$, to $w_{2}$.
	Also join $v_{1}$ to $w_{1}$ and $v_{\ell-2}$ to $w_{3}$. (If $\ell=3$, then
	$v_{1}=v_{\ell-2}$, hence $v_{1}$ is adjacent to $w_{1},w_{2}$ and $w_{3}$.)
	This is the (planar) graph $\overline{G}$.
\end{cons}




%>>>S: Lemma {lem:c:thet1kl}	
\begin{lemma} \label {lem:c:thet1kl}	
	If $\cp{G}$ is the graph constructed by Construction \ref{cons:c:thet1kl}, then $\ig{G} = \ag{G} = \thet{1,k,\ell}$, $ 3 \leq k \leq \ell$.
\end{lemma}





%>>>S: Figure {fig:c:thet1kl}	
\begin{figure}[H] \centering	
	\begin{tikzpicture}	
		
		%---------- REF-------------------
		\node (cent) at (0,0) {};
		\path (cent) ++(0:45 mm) node (rcent) {};	
		
		%----- W0 - Left Wheel ----------
		\node [std] at (cent) (w0) {};
		\path (w0) ++(15:6 mm) node (w0L) {$w_0$};
		
		%	\foreach \i/\c /\l in {1/90/1,3/270/3,4/210/4, 5/150/{k}} {		
			\foreach \i/\c /\l in {1/45/1,3/-45/3,4/-90/4, 5/-135/{5}, 6/135/{k}, 7/90/{k+1}} {						
				\path (w0) ++(\c:20mm) node [std] (w\i) {};
				\path (w\i) ++(\c:5 mm) node (Lw\i) {$w_{\l}$};
				\draw[thick] (w0)--(w\i);
			}
			
			%Node W2
			\path (w0) ++(0:20 mm) node [std] (w2) {};
			\path (w2) ++(80:5 mm) node (Lw2) {$w_{2}$};
			\draw[thick]  (w0)--(w2);	
			
			\draw[thick]  (w1)--(w2)--(w3)--(w4)--(w5);
			\draw[thick]  (w6)--(w7)--(w1);		
			
			\path (w0) ++(165:20mm) coordinate (z1) {};
			\path (w0) ++(195:20mm)coordinate (z2) {};
			
			\draw[thick] (w5)--(z2)--(z1)--(w6);
			
			\draw [dashed,thick] (z2)--(w0);
			\draw [dashed,thick] (z1)--(w0);
			
			%---- V-Path	
			\foreach \i / \j  / \k in {1/2.2/1, 2/1/2, 3/-1/{\ell-3}, 4/-2.2/{\ell-2}}
			{	
				\path (rcent) ++(90:\j cm) node [bblue] (v\i) {};
				\path (v\i) ++(0:5 mm) node (Lv\i) {\color{blue} $v_{\k}$};
				
				\draw[bline] (w2)--(v\i);
			}
			
			\draw[bline] (v1)--(v2);
			\draw[bline] (v3)--(v4);
			
			\draw[bline] (v2)--(v3);
			
			\draw[bline] (v1)--(w1);
			\draw[bline] (v4)--(w3);	
			
			\coordinate  (q1) at ($(v2)!0.33!(v3)$) {};
			\coordinate  (q2) at ($(v2)!0.66!(v3)$) {};
			
			\draw [dashed,bline] (q2)--(w2);
			\draw [dashed,bline] (q1)--(w2);		
			
			%-- X and Y
			\path (w0) ++(22:14 mm) node  [color=red] (LX) {$X$};
			\path (w0) ++(-22:14 mm) node  [color=red] (LY) {$Y$};		
			
			%-- A's	
			\foreach \i/\c / \l in {1/67/1,2/112/2,3/-112/{k-2}, 4/-67/{k-1}} 			
			\path (w0) ++(\c:14 mm) node [color=red] (A\i) {$A_{\l}$};				
			
			%-- B's	
			\foreach \i/\c /\l in {1/80/1,  4/-80/{\ell-1}} 				
			\path (w2) ++(\c:10 mm) node [color=red] (B\i) {$B_{\l}$};	
			\foreach \i/\c /\l in { 2/32/2, 3/-30/{\ell-2}} 			
			\path (w2) ++(\c:20 mm) node [color=red] (B\i) {$B_{\l}$};	
			
		\end{tikzpicture} \hspace{5mm}	
		\caption{The graph $\cp{G}$ from Construction \ref{cons:c:thet1kl} such that $\ig{G} = \thet{1,k,\ell}$ for $3 \leq k \leq \ell$.}
		\label{fig:c:thet1kl}	
	\end{figure}						
	% <<< E: Figure {fig:c:thet1kl}
	
	
	\begin{proof}
		To begin, notice that since in $\cp{G}$, the vertices $\mathcal{W}=\{w_0,w_1,\dots,w_{k},w_{k+1}\}$ form a wheel on at least five vertices, $\cp{H} \ncong K_4$.  Likewise, the graph induced by $\{w_0, w_1, w_2, w_3, v_1, v_2,$ $\dots, v_{\ell-2}\}$ in $\cp{G}$ is also a wheel on $\ell +2$ vertices, where $w_2$ is the central hub, and so it too contains no $K_4$.  Therefore, $\cp{G}$ is $K_4$-free. Moreover, since the triangles of $\cp{G}$ are its smallest maximal cliques, these triangles are precisely the maximal cliques of $\cp{G}$, and so $\omega(\cp{G}) = i(G) = \alpha(G) = 3$.  Since the $i$-sets of $G$ are identical to its $\alpha$-sets, $\ig{G}=\ag{G}$, and so for ease of notation, we will refer only to  $\ig{G}$ throughout the remainder of this proof.
		
		We label the triangles as in Figure \ref{fig:c:thet1kl} by dividing them into two collections.  The first are the triangles composed only of the vertices from $\mathcal{W}$ and each containing $w_0$: let $X = \{w_0,w_1,w_2\}$, $Y = \{w_0, w_2,w_3\}$, $A_1 =\{w_0,w_{k+1},w_1\} $, $A_2=\{w_0, w_{k}, w_{k+1}\}$, $\dots$ $A_{k-2} = \{w_0, w_{4}, w_{5}\}$,  $A_{k-1} = \{w_0, w_3, w_4\}$.
		%$A_3 = \{w_0, w_3,w_4\}$, $\dots$, and $A_{k+1}  = \{w_0, w_{k+1}, w_1\}$.  
		The remainder are the triangles with vertex sets not fully contained in $\cp{H}$: $B_1 = \{w_2,w_1,v_1\}$, $B_2 = \{w_2, v_1, v_2\}$, $B_3 = \{w_2, v_2, v_3\}$, $\dots$, $B_{\ell-2} = \{w_2, v_{\ell-3}, v_{\ell-2}\}$,  and $B_{\ell-1} = \{w_2, v_{\ell-2},w_3\}$.  We refer to these collections as $\mathcal{S} = \{X, Y\}$,  $\mathcal{A}=\{A_1,A_2,\dots,A_{k-1}\}$, and $\mathcal{B} = \{B_1, B_2, \dots, B_{\ell-1}\}$, and claim that these are the only triangles of $\cp{G}$.  
		
		To demonstrate this, we show that each vertex $v_i$ on the path $P_{\ell-2}$ is incident with exactly two of the triangles defined above.  
		
		Consider first a vertex $v_i$ for $2 \leq i \leq \ell-3$ on $P_{\ell-1}$ (in $\cp{G}$).  From the above definitions, $v_i$ is already on the triangles $B_i$ and $B_{i+1}$.  Since $\cp{G}$ is a planar graph, and $\deg(v_i)=3$, there is at most one more triangle incident with $v_i$.   The triangle $B_{i}$ is incident with edges $v_{i-1}v_i$ and $v_iw_2$, and $B_{i+1}$  is incident with edges $v_iv_{i+1}$ and $v_iw_2$.  Thus, a third triangle incident with $v_i$ would make use of edges $v_iv_{i-1}$ and $v_iv_{i+1}$.  However, since $v_{i-1}v_{i+1} \notin  E(\cp{G})$, no such third triangle exists; $v_i$ is incident only with $B_{i-1}$ and  $B_i$.  
		In the special case where $i=1$, the vertex $v_1$ is incident with triangles $B_1$ and $B_2$.  Since $w_1v_2 \notin E(\cp{G})$, these are the only two such triangles.  Similarly, for $i=\ell-3$, $v_{\ell-3}$ is incident only to $B_{\ell-2}$ and $B_{\ell-1}$, since $w_3v_{\ell-3} \notin E(\cp{G})$.  Thus, we conclude that for $1 \leq i \leq \ell-2$, the vertex $v_i$ is incident to the triangles $B_i$ and  $B_{i+1}$, and no others.
		
		Now, since all triangles incident with $v_i$ have already been considered, any unaccounted for triangles would be composed only of vertices from $\mathcal{W}$.  However, clearly the vertices of $\mathcal{W}$ form a wheel, for which we have  already accounted for all its $2+(k-1)=k+1$ triangles.
		We conclude that the only triangles of $\cp{G}$ are the $2+(k-1)+(\ell-1)=k+\ell$ such ones defined above.  It follows that these $k+\ell$ triangles represent all the $i$-sets of $G$, and so  $V(\ig{G})=\{X,Y, A_1,A_2,\dots,A_{k-1}, B_1,B_2,\dots,B_{\ell-1}\}$.
		
		Having determined all triangles of $\cp{G}$ (and thus $V(\ig{G})$), we now show that the required adjacencies hold.  		
		From the original construction of $\cp{G}$, the following are immediate for $\ig{G}$:
		
		\newpage
		
		\begin{enumerate}[itemsep=0pt, label=(\roman*)]
			\item \label{it:c:thet1kl:1}  $\edge{X, w_1, w_3,Y}$, 
			
			\item \label{it:c:thet1kl:j} $\edge{X, w_0,  v_1,B_1}  \adedge{w_1,v_2,B_2} \adedge{v_1,v_3,B_3} \dots \edge{B_{\ell-2}, v_{\ell-3},  w_3,B_{\ell-1}} \adedge{v_{\ell-2},w_0,Y}$, 
			
			\item \label{it:c:thet1kl:k}  $\edge{X, w_2,  w_{k+1}, A_1}  \adedge{w_1,w_k,A_2} \dots \edge{A_{k-2}, w_{5},  w_3, A_{k-1}} \adedge{w_{4},w_2,Y}$. 
		\end{enumerate}
		
		\noindent Hence, we need only show that there are no additional unwanted edges generated in the construction of $\ig{G}$.  	
		
		Since $\cp{G}$ is a planar graph and all of its triangles are facial (that is, the edges of the $K_3$ form a face in the planar embedding of the graph shown in Figure \ref{fig:c:thet1kl}), each triangle is adjacent to at most three others.  From \ref{it:c:thet1kl:1}-\ref{it:c:thet1kl:k}  above, triangles $X$ and $Y$ are both adjacent to the maximum three (and hence $\deg_{\ig{G}}(X)=\deg_{\ig{G}}(Y)=3$).  
		
		Recall that to be adjacent, two triangles share exactly two vertices.  Notice that the triangles of $\mathcal{A}$ are composed entirely of vertices from $\mathcal{W}-\{w_2\}$, and that for $2\leq i \leq \ell-2$, $B_i\cap\mathcal{W}=\{w_2\}$; furthermore, $B_1\cap\mathcal{W}=\{w_1,w_2\}$ and $B_{\ell-2}\cap\mathcal{W}=\{w_2,w_3\}$.  We conclude that no triangle of $\mathcal{B}$ is adjacent to any triangle of $\mathcal{A}$.
		
		It remains only to show that there are no additional unwanted adjacencies between two triangles of $\mathcal{A}$ or two triangles of $\mathcal{B}$.
		Clearly from the definitions, there is no triangle of $\mathcal{A}$ aside from $A_1$ that contains both the vertices $w_1$ and $w_{k+1}$.  For $2 \leq i \leq k-2$, consider a triangle $A_i$.  From \ref{it:c:thet1kl:k}, we have already shown that $A_i$ is adjacent to two other triangles: one sharing the vertex pair $\{w_0,w_{(k+2)-i}\}$ and the other sharing the vertices $\{w_0,w_{(k+3)-i}\}$.  From their definitions, we see that there is no triangle $A_j$ with $i\neq j$ sharing the third vertex pair with $A_i$.  That is, there is no $A_j$ such that $\{w_{(k+2)-i},w_{(k+3)-i} \} \subseteq A_j$.  Hence, for all $A_i\in \mathcal{A}$, $A_i$ is adjacent to exactly two other triangles, and so $\deg_{\ig{G}}(A_i)=2$.
		
		Applying arguments very similar to those from $\mathcal{A}$ to the triangles of $\mathcal{B}$ shows that no  additional unwanted edges are generated in the construction of the $i$-graph.  		
		This completes the exhaustive examination of the triangles of $\cp{G}$.  We conclude that the graph $\cp{G}$ generated by Construction \ref{cons:c:thet1kl} yields $\ig{G} =\ag{G}= \thet{1,k,\ell}$.
	\end{proof}
	% <<< E: Lemma {lem:c:thet1kl}
	
	
	
	%--------------------------------------------
	%\subsubsection{The $i$-graphs of the Complements of Wheels Are Cycles}  \label{subsubsec:c:wheel}
	\subsection{The $i$-graphs of the Complements of Wheels Are Cycles}  \label{subsec:c:wheel}
	
	
	Before we proceed with the remainder of the theta graph constructions, let us return to Figure \ref{fig:c:thet1kl} to notice the prominence of the wheel subgraph in the complement seed graph $\cp{G}$.  In the constructions throughout this chapter, this wheel subgraph will appear repeatedly; indeed, all of the complement seed graphs for the $i$-graphs of theta graphs have a similar basic form: begin with a wheel, add a path of some length, and then add some collection of edges between them.   Lemma \ref{lem:c:wheel} below demonstrates that a wheel in a triangle-based complement seed graph $\cp{G}$ corresponds to a cycle in the $i$-graph of $G$.  Using this result, in our later constructions with a wheel subgraph, we already have two of the three paths of a theta graph formed.  Hence, we need only confirm that whatever unique additions are present in a given construction form the third path in the $i$-graph.
	
	
	Notice that when $k=3$, the wheel $W_4$ is isomorphic to the complete graph $K_4$, the complement of which has only a single $i$-set, namely, the set including all vertices.  Hence, $\ig{\cp{W_4}} = \ig{\cp{K_4}} =  K_1$.
	
	
	
	%>>>S: Lemma {lem:c:wheel}	
	\begin{lemma}\label{lem:c:wheel}
		For $k\geq 4$, let $H_{k}$ be the wheel $W_{k+1} =C_{k} \vee K_1$.  Then $\ig{\cp{H_{k}}} \cong \ag{\cp{H_{k}}} \cong C_k$.
	\end{lemma}
	
	

	
	%>>>S: Figure {fig:c:wheel}
	\begin{figure}[H] \centering	
		\begin{tikzpicture}	
			%---------- REF-------------------
			\node (cent) at (0,0) {};
			
			%----Left Wheel
			\node[std,label={0:$w_0$}] (w0) at (cent) {};
			
			\foreach \i/\j in {1/1,2/2,3/3,4/4,5/5,6/k}
			{
				\node[std,label={150-\i*60: $w_{\j}$}] (w\i) at (150-\i*60:2.5cm) {}; 
				\draw[thick] (w0)--(w\i);        
			}
			
			\draw[thick] (w1)--(w2)--(w3)--(w4)--(w5);
			\draw[thick] (w6)--(w1);
			\draw[thick] (w5)--(w6);
			
			\coordinate  (v1) at ($(w5)!0.33!(w6)$) {};
			\coordinate  (v2) at ($(w5)!0.66!(w6)$) {};
			
			\draw [dashed] (v2)--(w0);
			\draw [dashed] (v1)--(w0);	
			
			%\path (w0) ++(170:25mm) coordinate (t1) {};
			%\path (w0) ++(190:25mm)coordinate (t2) {};
			%\draw[thick] (w5)--(t2)--(t1)--(w6);
			
			%\draw [dashed,thick] (t2)--(w0);
			%\draw [dashed,thick] (t1)--(w0);
			
			%----- Internal Red Nodes	
			\foreach \i/\j in {1/1,2/2,3/3,4/4,6/k}
			\node[dred,label={120-\i*60: \color{red}$A_{\j}$}] (a\i) at (120-\i*60:12mm) {}; 
			
			\draw[thick,red, densely dashdotted](a6)--(a1)--(a2)--(a3)--(a4);
			
			\foreach \i/\j in {5/195,6/180,7/165}
			\coordinate (b\i) at (\j:12mm) {}; 		
			
			\draw[dashed,red] (a4)--(b5)--(b6)--(b7)--(a6);
			
		\end{tikzpicture} 
		\caption{The wheel  $H_k=W_{k+1}$, with the $i$-graph of its complement, $\ig{\cp{H_k}} \cong \ag{\cp{H_k}} \cong  C_k$, embedded in red.}
		\label{fig:c:wheel}
	\end{figure}		
	% <<< E: Figure {fig:c:wheel}
	
	\begin{proof}
		Let $H_k$ be the wheel graph $W_{k+1}$ for $k \geq 4$.  We apply the standard vertex labelling used throughout this section, where the degree 3 vertices are labelled $w_1,w_2,\dots, w_k$, and the central degree $k$ vertex is  $w_0$. 
		
		Since $H_k$ is $K_4$-free and each vertex of $H_k$ lies on a triangle, $i(\cp{H_k}) = 3$; moreover, each triangle of $H_k$ represents an $i$-set of $\cp{H_k}$.   %Likewise, since there are no induced $K_4$'s in $H_k$, 
		For the same reasons, we have that $\alpha(\cp{H_k})=3$ and the triangles represent also the $\alpha$-sets of $\cp{H_k}$.
		
		We label these triangles as  $A_i = \{w_0, w_i, w_{i+1}\}$ for $1 \leq i \leq k-1$ and $A_k=\{w_0,w_k,w_1\}$.  
		
		To check that there are no other unaccounted for triangles in $H_k$, consider one of the exterior wheel vertices of $H_k$, say $w_i$ with, for ease of notation, $2 \leq i \leq k-1$ (similar arguments with worse notation hold for $i=1$ and $i=k$).  Since $deg(w_i) = 3$, $w_i$ is on at most $\binom{3}{2}=3$  triangles, of which we have already accounted for two: $A_{i-1}=\{w_0,w_{i-1},w_i\}$ (using edges  $w_0w_i$ and $w_0w_{i-1}$) and $A_i =\{w_0, w_i, w_{i+1}\}$  (using edges  $w_0w_i$ and $w_0w_{i+1}$).  The final potential triangle would make use  of the edges $w_iw_{i+1}$ and $w_{i-1}w_i$; however, since $w_{i-1}w_{i+1} \notin E(H_k)$, this does not form a triangle.  Thus, $w_i$ (and hence all of the exterior wheel vertices) is (are) on exactly two triangles. We have accounted for all triangles of $H_k$ and therefore all $i$-sets of $\cp{H_k}$, and so $V(\ig{\cp{H_k}}) = \{A_1,A_2,\dots,A_k\}$.
		
		Now, since $H_k$ is planar, and each triangle $A_1,A_2,\dots,A_k$ is a facial triangle, each triangle is  adjacent to at most three other triangles.  Clearly, for $2 \leq i \leq k-1$, $A_{i-1} \sim A_i \sim A_{i+1}$, which makes use of the shared edges $w_0w_i$ and $w_0w_{i+1}$ of $A_i$.  As observed before, the third edge, $w_iw_{i+1}$, is only on $A_i$, and so $A_i$ is adjacent only to $A_{i-1}$ and $A_{i+1}$.   Similar arguments follow for $A_1$ and $A_k$.  Thus, $\deg_{\ig{\cp{H_k}}}(A_i)=2$ for all $1 \leq i \leq k$ and since $A_1 \sim  A_2  \sim \dots \sim A_k \sim A_1$, it follows that $\ig{\cp{H_{k}}} \cong \ag{\cp{H_{k}}} \cong C_k$.	
	\end{proof}
	% <<< E: Lemma {lem:c:wheel}
	
	We note the following analogous  - although less frequently applied - result for fans of the form $K_1+P_k$.
	The proof proceeds similarly to the previous result for wheels, and is omitted.
	
	
	%>>>S: Lemma {lem:c:wheel}	
	\begin{lemma}\label{lem:c:fan}
		For $k\geq 2$, let $H_{k}$ be the $k$-fan $K_1 \vee P_{k}$.  Then $\ig{\cp{H_{k}}} \cong \ag{\cp{H_k}} \cong P_{k-1}$.
	\end{lemma}
	
	
	
	%>>>S: Figure {fig:c:fan}
	
	\begin{figure}[H] \centering	
		\begin{tikzpicture}	
			%---------- REF-------------------
			\node (cent) at (0,0) {};
			\path (cent) ++(0:40 mm) node (rcent) {};	
			
			%----Right Path
			\node[std,label={180:$v_0$}] (w0) at (cent) {};
			
			\foreach \i/\d/\j in {1/1/1,2/2/2,3/3/3,4/4/4,5/6/{k-1},6/7/{k}}
			{
				\path (rcent) ++(90:40mm-\d*10mm) node[std,label={0: $v_{\j}$}] (w\i) {};
				\draw[thick] (w0)--(w\i);        
			}
			
			\draw[thick] (w1)--(w2)--(w3)--(w4);
			\draw[thick] (w5)--(w6);
			\draw[dashed] (w4)--(w5);
			
			\coordinate  (v1) at ($(w4)!0.33!(w5)$) {};
			\coordinate  (v2) at ($(w4)!0.66!(w5)$) {};
			
			\draw [dashed] (v2)--(w0);
			\draw [dashed] (v1)--(w0);	
			
			%----- Internal Red Nodes		
			\foreach \i/\d /\r /\j in {1/1/25/1,2/2/10/2,3/3/0/3,5/6/-25/{k-1}}
			{
				\path (rcent) ++(90:35mm-\d*10mm) coordinate  (z\i) {};	
				\coordinate  (y\i) at ($(z\i)!0.25!(w0)$) {};
				\node[dred] (a\i) at (y\i) {};	
				\path (a\i) ++(\r:5mm) node  (AL\i) { \color{red}$A_{\j}$};	
			}
			
			%----- Lines	
			\path (a3) ++(270:5mm) coordinate (d3) {};	
			\path (a5) ++(90:5mm) coordinate (d5) {};	
			
			\draw[thick,red](a1)--(a2)--(a3);
			\draw[thick,red](a3)--(d3);
			\draw[thick,red](a5)--(d5);
			
			\draw[dashed,thick, red, densely dashdotted] (d3)--(d5);
		\end{tikzpicture} 	
		\caption{The  fan  $H_k=K_1 \vee P_k$, with the $i$-graph of its complement, $\ig{\cp{H_k}} \cong \ag{\cp{H_k}} \cong P_{k-1}$, embedded in red.}
		\label{fig:c:fan}	
	\end{figure}
	% <<< E: Figure {fig:c:fan}
	
	
	
	
	
	
	
	%......................  SUB SECTION:  theta (2,k,l) .........................
	\subsection{$\thet{2,k,\ell}$  for $2  \leq k  \leq \ell$ }  \label{subsec:c:2kl}
	
	
	%______________________  SUBSUB SECTION:  theta (2,2,\ell) ______________________
	\subsubsection{Construction of $\cp{G}$ for $\thet{2,2,\ell}$, $\ell \geq 5$}  \label{subsubsec:c:22l}
	
	
	In Chapter \ref{ch:igraphs}, we saw that $K_{2,3} \cong \thet{2,2,2}$  (Proposition \ref{prop:i:K23})  and $\kappa \cong \thet{2,2,3}$ (Proposition \ref{prop:i:kappa}) are not $i$-graphs.   Extending these results, we find that the length of the third path in $\thet{2,2,\ell}$ has a transition point between $\ell=4$ and $\ell=5$; while $\ell=4$ is still too short to form an $i$-graph (see Lemma \ref{prop:c:thet224}), for  $\ell \geq 5$, $\thet{2,2,\ell}$ is $i$-graph realizable.
	
	
	%In the following constructions, we build our graphs around the graph $\cp{H} \cong W_5 = C_4 \vee K_1$, labelling the degree 3 vertices as $w_1,w_2,w_3,w_4$ and the central degree 4 vertex as $w_0$.
	
	
	%>>> S:CONS {con:c:thet22k}
	\begin{cons} \label{con:c:thet22k}
		Refer to Figures \ref{fig:c:thet22k} and \ref{fig:c:thet225}.	Begin with a copy of the graph $\cp{H} \cong W_5 = C_4 \vee K_1$, labelling the degree 3 vertices as $w_1,w_2,w_3,w_4$ and the central degree 4 vertex as $w_0$.
		
		
		\begin{enumerate}[itemsep=0pt, label=(\alph*)]
			\item \label{con:c:thet22k:ell}
			If $\ell \geq 6$ (as in Figure \ref{fig:c:thet22k}), attach to $\cp{H}$ a path  $P_{\ell -3}: (v_1, v_2,\dots,v_{\ell-3})$ by joining $w_1$ to $v_1, v_2, \dots, v_{\ell-4}$.  Join $v_{\ell-5}$ to $v_{\ell-3}$.  Next, join $w_2$ to $v_1$, and $w_3$ to $v_{\ell-3}$.  Then, join $w_4$ to $v_{\ell-4}$ and $v_{\ell-3}$.  Add a new vertex $z$, joined to $w_1, w_4,$ and $v_{\ell-4}$.
			
			
			\item \label{con:c:thet22k:5} If $\ell = 5$ (as in Figure \ref{fig:c:thet225}), attach to $\cp{H}$ a path of $P_{2}: (v_1, v_2)$, by joining $w_1$ to $v_1$, and $w_2$ to $v_1$ and $v_2$.  Then join $w_3$ to $v_2$, and $w_4$ to both $v_1$ and $v_2$.  Add two new vertices, $z_1$ and $z_2$, joining $z_1$ to $v_1, w_1$, and $w_4$, and $z_2$ to $v_2, w_2$ and $w_3$.
			
		\end{enumerate}
		
		We label the resultant (planar) graph $\cp{G}$.	
	\end{cons}
	% <<< E: Cons {con:c:thet22k}
	
	
	
	%>>> S: Figure {fig:c:thet22k}		
	\begin{figure}[H] \centering	
		\begin{tikzpicture}	
			%---------- REF-------------------
			\node (cent) at (0,0) {};
			\path (cent) ++(0:45 mm) node (rcent) {};	
			
			%----Left Wheel
			\node[std,label={10:$w_0$}] (w0) at (cent) {};
			
			\foreach \i in {1,2,3,4}
			{
				\node[std,label={180-\i*90: $w_{\i}$}] (w\i) at (180-\i*90:2cm) {}; 
				\draw[thick] (w0)--(w\i);        
			}
			\draw[thick] (w1)--(w2)--(w3)--(w4)--(w1);
			
			%---- V-Path	
			\foreach \i / \j  / \k in {1/3/1, 2/2/2, 3/-1/{\ell-5}, 4/-2.2/{\ell-4}, 5/-3.4/{\ell-3}}
			{	
				\path (rcent) ++(90:\j cm) node [bblue] (v\i) {};
			}
			
			\path (v1) ++(0:4 mm) node (Lv1) {\color{blue} $v_{1}$};
			\path (v2) ++(0:4 mm) node (Lv2) {\color{blue} $v_{2}$};
			\path (v3) ++(-10:5 mm) node (Lv3) {\color{blue} $v_{\ell-5}$};
			\path (v4) ++(15:8 mm) node (Lv4) {\color{blue} $v_{\ell-4}$};
			\path (v5) ++(260:4 mm) node (Lv5) {\color{blue} $v_{\ell-3}$};		
			
			\draw[bline] (v1)--(v2);
			\draw[bline] (v3)--(v4)--(v5);
			
			\draw[bline,dashed] (v2)--(v3);
			
			%---- Zs
			\path (v4) ++(0:15 mm) node [bzed, label={[zelim2]0:$\boldsymbol{z}$}] (z) {};
			
			\path (v4) ++(270:3cm) coordinate  (c1) {};
			\draw[zline] (z) to[out=-40, in=20]  (c1) to [out=200,in=250] (w4); 
			
			\path (v1) ++(90:2cm) coordinate  (c2) {};
			%\draw[rline] (z) to[out=0, in=20]  (c2) to [out=200,in=45] (w1); 
			\draw[zline] (w1) to[out=50, in=170]  (35:6.9cm) to [out=350,in=40]  (z); 
			
			\draw[zline] (v4)--(z);		
			
			%---- V3 to V5 
			\path (v4) ++(180:1.3 cm) coordinate  (c1) {};
			\draw[bline] (v3) to[out=190, in=90]  (c1) to [out=270,in=170] (v5);  
			
			%---- V1 to W1 W2
			\draw[bline] (w1)--(v1)--(w2);	
			
			%-- V5 to W4
			\draw[bline] (v5) to[out=180,in=-90] (w4);  
			
			%-- V5 to W3
			\draw[bline] (v5) to[out=170,in=-30] (w3);  
			
			%-- V4 to W4
			\draw[bline] (v4) to[out=-35, in=25]  (4.6cm,-4.2cm) to [out=205,in=260] (w4);  	
			%	\node[std] at (4.6cm,-4.2cm) {};
			
			%-- W1 to V2  
			\draw[bline] (w1) to[out=20, in=170]  (35:6.1cm) to [out=350,in=45]  (v2); 
			%	\node[std] at (35:6.2cm)  {};
			
			%-- W1 to  V3 
			\draw[bline] (w1) to[out=38, in=170]  (35:6.4cm) to [out=350,in=45]  (v3); 
			%\node[std] at (30:5.8cm) {};
			
			%-- W1 to V4
			\draw[bline] (w1) to[out=46, in=170]  (35:6.6cm) to [out=350,in=40]  (v4); 
			%\node[std] at (30:5.8cm) {};
			
			%-- W1 to Dashed T1 T2
			\path (rcent) ++(90:1 cm) coordinate  (t1) {};
			\draw[bline, dashed] (w1) to[out=28, in=170]   (35:6.2cm)  to [out=350,in=45]  (t1); 
			
			\path (rcent) ++(90:0 cm) coordinate  (t2) {};
			\draw[bline, dashed] (w1) to[out=34, in=170]  (35:6.3cm) to [out=350,in=45]  (t2); 
			
			%----- Internal Red Labellings	
			\path (w0) ++(45:9 mm) node [color=red] (X) {$X$};			
			\path (w0) ++(45:-9 mm) node [color=red] (Y) {$Y$};
			
			%-- A's
			\path (w0) ++(-45:8 mm) node [color=red] (A1) {$A$};	
			
			%-- B's	
			\path (w0) ++(135:8 mm) node [color=red] (B1) {$B$};			
			
			%-- D's
			\path (w2) ++(90:15 mm) node [color=red] (D1) {$D_1$};	
			\path (v1) ++(170:9 mm) node [color=red] (D2) {$D_2$};	
			\path (v4) ++(160:7 mm) node [color=red] (D3) {$D_{\ell-3}$};
			\path (v5) ++(195:20mm) node [color=red] (D4) {$D_{\ell-2}$};
			\path (w4) ++(-55:20 mm) node [color=red] (D5) {$D_{\ell-1}$};			
			
		\end{tikzpicture} 
		\caption{The graph $\cp{G}$ from Construction \ref{con:c:thet22k} such that $\ig{G} = \thet{2,2,\ell}$ for $\ell \geq 6$.}
		\label{fig:c:thet22k}
	\end{figure}	
	% <<< E: Figure {fig:c:thet22k}
	
	
	
	
	%>>> S: Figure {fig:c:thet225}	
	\begin{figure}[H] \centering	
		\begin{tikzpicture}	
			
			%---------- REF-------------------
			\node (cent) at (0,0) {};
			\path (cent) ++(0:45 mm) node (rcent) {};	
			
			%----Left Wheel
			\node[std] (w0) at (cent) {};
			\path (w0) ++(30: 4 mm) node (Lw0) {${w_0}$};	
			
			\foreach \i in {1,2,3,4}
			{
				\node[std,label={180-\i*90: $w_{\i}$}] (w\i) at (180-\i*90:2.5cm) {}; 
				\draw[thick] (w0)--(w\i);        
			}
			\draw[thick] (w1)--(w2)--(w3)--(w4)--(w1);
			
			%---- V-Path	
			\foreach \i / \j in {1/1.5,2/-1.5}
			{	
				\path (rcent) ++(90:\j cm) node [std] (v\i) {};
				\path (v\i) ++(0:4 mm) node (Lv\i) {$v_{\i}$};
				%\node[bblue,label={0: $v_\i$}] (v\i) at (4,2-\i) {};
			}
			\draw[thick] (w1)--(v1)--(v2)--(w3);
			\draw[thick] (v2)--(w2)--(v1);	
			
			%---- Zs
			\path (w2) ++(270:1 cm) node [bzed, label={[zelim]15:$ \boldsymbol{z_2}$}] (z2) {};
			\draw[zline] (w2)--(z2)--(w3);
			\draw[zline] (z2)--(v2);
			
			\path (w1) ++(125:1.2 cm) node [bzed, label={[zelim]14:$\boldsymbol{z_1}$}] (z1) {};
			\draw[zline] (w4)--(z1)--(w1);
			\draw[zline] (z1)--(v1);
			
			%--- V2 to W4 
			\draw[thick] (v2) to[out=230, in=-5]  (270:3.3cm) to [out=170,in=280] (w4);
			
			%--- V1 to W4
			\draw[thick] (v1) to[out=130, in=0]  (90:4.3cm) to [out=180,in=90] (w4);	
			
			%------------ THETA
			
			%---- INNER Cycle	
			\foreach \i / \j  in {1/X,2/B,3/Y,4/A}
			{	
				\node[dred] (t\i) at (-45+\i*90:1.0cm) {}; 
				\path (t\i) ++(-45+\i*90: 4 mm) node (Lt\i) {\color{red}${\j}$};				
			}
			
			\path (w2) ++(90: 7mm) node [dred] (d1) {};
			\path (d1) ++(90: 4 mm) node (Ld1) {\color{red}${D_1}$};
			
			\path (w2) ++(0: 15mm) node [dred] (d2) {};
			\path (d2) ++(90: 4 mm) node (Ld2) {\color{red}${D_2}$};	
			
			\path (v2) ++(-45: 10mm) node [dred] (d3) {};
			\path (d3) ++(0: 4 mm) node (Ld3) {\color{red}${D_3}$};	
			
			\path (t3) ++(260: 15mm) node [dred] (d4) {};
			\path (d4) ++(170: 4 mm) node (Ld4) {\color{red}${D_4}$};					
			
			\draw[rlinemb](t1)--(t2)--(t3)--(t4)--(t1);
			\draw[rlinemb](t1)--(d1)--(d2);	
			\draw[rlinemb](t3)--(d4);
			
			%--- D2 to D3 
			\draw[rlinemb] (d2) to [out=-45,in=90] (d3);
			
			%--- D3 to D4
			\draw[rlinemb] (d3) to [out=230,in=300] (d4);
			
		\end{tikzpicture} 
		
		\caption{The graph $\cp{G}$ from Construction \ref{con:c:thet22k} such that $\ig{G} = \thet{2,2,5}$, with $\thet{2,2,5}$ overlaid in red.}
		\label{fig:c:thet225}
	\end{figure}	
	% <<< E: Figure {fig:c:thet225}
	
	
	
	
	
	
	
	% <<< E: Figure {fig:c:thet22l}
	
	
	As with our other constructions, the triangles of $\cp{G}$ are its smallest maximal cliques, and so $i(G)=3$. As before, we use these triangle faces to visualize the movements of tokens between the $i$-set reconfigurations; however, we now employ a technique of adding vertices to create $K_4$'s through $\cp{G}$ and eliminate any ``unwanted" triangles that might arise in our construction.  In  \ref{con:c:thet22k:ell}, the addition of $z$  prevents $\{w_1,w_4,v_{\ell-3}\}$ from being a maximal clique of $\cp{G}$ and hence an $i$-set of $G$. Similarly, in \ref{con:c:thet22k:5}, $z_1$  and $z_2$  eliminate triangles $\{w_1,w_4,v_1\}$ and $\{w_2,w_3,v_2\}$, respectively.  
	The unfortunate trade-off in this triangle-elimination technique is that the remaining triangles are no longer $\alpha$-sets; the constructions work only for $i$-graphs, not $\alpha$-graphs. 
	
	
	%>>>S: Lemma {lem:c:thet22l}	
	\begin{lemma} \label{lem:c:thet22l}
		If $\cp{G}$ is the graph constructed by Construction \ref{con:c:thet22k}, then $\ig{G} = \thet{2,2,\ell}$, for $\ell \geq 5.$
	\end{lemma}
	
	
	\begin{proof}		
		We prove the two constructions separately, beginning with the more general case.
		
		\begin{enumerate}[itemsep=0pt,label=(\alph*)]
			
			% ``````````````````````````````````  THET (2,2,l) ``````````````````````````````

\newpage
			
			\item $\mathbf{\thet{2,2,\ell}, \ell \geq 6}$.	\label{lem:c:thet22lpf} 
			
			As in the previous constructions, since each edge of $\cp{G}$ belongs to a triangle and some triangles are not contained in $K_4$'s, these maximal triangles of $\cp{G}$ form the smallest maximal cliques of $\cp{G}$ and, hence, the $i$-sets of $G$.  We label these triangles as in Figure \ref{fig:c:thet22k}; in particular,	
			
			\begin{center}	
				\begin{tabular}{rlcrl}
					$X$ & $=\{w_0,w_1,w_2\},$  & \null \hspace{20mm} \null &  	$D_1$ & $= \{w_1,w_2,v_1\},$ \\
					$Y$ & $= \{w_0,w_3,w_4\},$ &&   	$D_i$ & $= \{w_1,v_{i-1},v_i\}$  for $  2 \leq i \leq \ell-4,$\\
					$A$ & $=\{w_0,w_2,w_3\},$  &&		$D_{\ell-3}$ & $= \{v_{\ell-5}, v_{\ell-4}, v_{\ell-3} \},$ \\
					$B$ & $=\{w_0,w_1,w_4\},$  &&   	$D_{\ell-2}$ & $= \{w_{4}, v_{\ell-4}, v_{\ell-3} \},$ \\
					& && 							$D_{\ell-1}$ & $= \{w_3,w_4,v_{\ell-3}\}.$
				\end{tabular}
			\end{center}
			
			We further partition the vertices of $\cp{G}$ into two sets: the wheel vertices \linebreak  $W = \{w_0,w_1,\dots,w_4\}$ and the path vertices $Q=\{v_1,v_2,\dots, v_{\ell-3}\}$.  
			
			We first show that the only induced $K_4$ in $\cp{G}$ is $Z=\{z, w_1,w_4,v_{\ell-4}\}$, and hence each of the above listed $\ell+3$ sets is an $i$-set of $G$.  
			The vertices of $Q$ induce a path of length $\ell-2$, with an extra edge between $v_{\ell-3}$ and $v_{\ell-5}$, so no $K_4$ is contained entirely in $Q$.  There is likewise no $K_4$ with three vertices in $Q$, since the only set of three mutually adjacent vertices from $Q$ is $\{v_{\ell-5}, v_{\ell-4}, v_{\ell-3}\}$,  but $v_{\ell-5}$ and  $v_{\ell-3}$ have no common neighbours outside of $Q$ in $\cp{G}$.   Moreover, there is also no $K_4$ using exactly two vertices of $Q$; notice that $w_2$ and $w_3$ both have only a single edge  to $Q$, and so any $K_4$ with two vertices on $Q$ would necessarily contain $w_1$ and $w_4$. Since $N_{\cp{G}}(\{w_1,w_4\})\cap Q=\{v_{\ell-4}\}$, the only $K_4$ containing two vertices from $\mathcal{W}$ is $Z$, as required.
			
				
			%=========== NO EXTRA TRIANGLES ==========
			Next, we show that there are no additional $i$-sets in $G$ beyond the $\ell+3$ labelled maximal clique triangle faces of $\cp{G}$ listed above. As all of the neighbours of $z$ lie on a $K_4$, we can divide any potential unaccounted for $i$-sets into two categories: those with at least two vertices on the wheel $W$, and those with at least two vertices on the path $Q$.
			
			In the first case, $N_{\cp{G}}(w_0) = \{w_1,w_2,w_3,w_4\}$, so every triangle containing $w_0$ has already been accounted for (on the faces of the wheel), including those with three vertices on $W$.  As  noted above, the open neighbourhoods of $w_3$ and $w_4$ share only $v_{\ell-3}$ on $Q$, and we have already labelled $D_{\ell-1}  = \{w_3, w_4, v_{\ell-3}\}$.  The only neighbour of $w_2$ on $Q$ is $v_1$, which is not adjacent to $w_3$, so there are no triangles containing both $w_2$ and $w_3$, aside from $A$.  The only other wheel vertex adjacent to $v_1$ is $w_1$, but we have again already accounted for $D_1 = \{w_1,w_2,v_1\}$.  Finally, $\left( N_{\cp{G}}(w_1) \cap N_{\cp{G}}(w_4) \right) \cap Q = \{v_{\ell-4}\}$, and since $\{w_1,w_4,v_{\ell-4}\}$ is a part of the clique  $Z$, it is not an $i$-set of $G$.
			
			We now show that there are no additional triangles of $\cp{G}$ with at least two vertices on $Q$ that are $i$-sets of $G$.  For a vertex $v_i \in Q$ with $ 2 \leq i \leq {\ell-6}$, we have that $N(v_i) \cap Q = \{v_{i-1}, v_{i+1}\}$ and, furthermore, $\left(N_{\cp{G}}(v_i) \cap N_{\cp{G}}(v_{i+1}) \right) \cap W = \{w_1\}$.  Each such triangle $D_{i+1} = \{w_i,v_{i},v_{i+1}\}$ has already been accounted for.  With the vertices of  $Q$ along  the middle of the path now checked, we consider special cases present in the end vertices.  The only triangle entirely contained in $Q$ is $D_{\ell-3} = \{v_{\ell-5}, v_{\ell-4}, v_{\ell-3} \}$, which has already been considered.  
			For $v_1$, $N_{\cp{G}}(v_{1}) \cap Q = \{v_2\}$, and as before, since $N_{\cp{G}}(v_1) \cap N_{\cp{G}}(v_{2}) = \{w_1\}$, we have already listed the triangle $D_2 = \{v_1,v_2,w_2\}$ as an $i$-set of ${G}$.  
			Once again,  $N_{\cp{G}}(v_{\ell-4}) \cap N_{\cp{G}}(v_{\ell-5}) = \{w_1, v_{\ell-3}\}$, so $v_{\ell-4}$ and $v_{\ell-5}$ are on only the previously considered triangles $D_{\ell-3}$ and $D_{\ell-4}$.  Finally, 
			$N_{\cp{G}}(v_{\ell-3}) \cap N_{\cp{G}}(v_{\ell-4}) = \{w_4\}$, which is once more associated only with the previously labelled triangle $	D_{\ell-1}  = \{w_3,w_4,v_{\ell-3}\}$.  This concludes all possible cases where a triangle of $\cp{G}$ could be an $i$-set of $G$;  the $i$-sets of $G$, and hence the vertices of $\ig{G}$, are exactly the $\ell+3$ sets listed above.
			
	
			Moving to the edges of $\ig{G}$, the following adjacencies are clear from Figure \ref{fig:c:thet22k}.
			%=========== EDGES =====================
			\begin{enumerate}[itemsep=0pt, label=(\roman*)]
				\item \label{lem:c:thet22l:i}  $\edge{X, w_1, w_3,A} \adedge{w_2,w_4,Y}$, 
				
				\item \label{lem:c:thet22l:j} $\edge{X, w_2, w_4,B} \adedge{w_1,w_3,Y}$, 
				
				\item \label{lem:c:thet22l:k} $\edge{X, w_0,  v_1,D_1}  \adedge{w_2,v_2,D_2} \adedge{v_1,v_3,D_3} \dots \edge{D_{\ell-3}, w_1,  v_{\ell-2},D_{\ell-2}} \adedge{v_{\ell-4},w_4,D_{\ell-1}}  \adedge{v_{\ell-2},w_0,Y}$. 
			\end{enumerate}
			% =========== NO EXTRA EDGES =============
			
			We need only show that there are no additional adjacencies in $\ig{G}$ not listed above.
			Since $\cp{G}$ is planar, and an $i$-set triangle is adjacent to another $i$-set triangle if and only if they share exactly one edge if $\cp{G}$, each $i$-set of $G$ is adjacent to at most three others.  
			In our lists above, $X$ and $Y$ are each adjacent to three other $i$-sets, and thus no others.  The $i$-set $A$ is adjacent to both $X$ and $Y$ in the list, and from the above, no other triangles of $\cp{G}$ contain both $w_2$ and $w_3$, and so there is no triangle adjacent to $A$ sharing the edge $w_2w_3$.  
			Similarly, the $i$-set $B$ is listed above as being adjacent to both $X$ and $Y$.  While $\{w_1,w_4,z\}$ is a triangle adjacent to $B$, it is part of the $K_4$, $Z$, and so not an $i$-set.
			
			
			All that remains is to show that each $D_i \in \ig{V(G)}$ has $\deg_{\ig{G}}(D_i)=2$ for all $i=1,2, \dots \ell-1$.  Suppose that some $D_i$ had  $\deg_{\ig{G}}(D_i)\geq 3$.  We have already established that $D_i$ is not adjacent to $A$ nor to $B$, and   unless $i=1$ or $ \ell-1$, $D_i$ is not adjacent to any of $X$ or $Y$ either.  
			%So say that $D_i$ is adjacent to some  $D_j$ (without loss of generality, $i  < j$), where $j-i \geq 2$. 
			If $ 1 \leq i \leq \ell-5$, then because $\deg_{\cp{G}} (v_i) =3$, the triangle $D_i$  is adjacent only to $D_{i-1}$ and $D_{i+1}$ as in the lists above.	
			The triangle $D_{\ell-4}$ is adjacent to both $D_{\ell-3}$ and $D_{\ell-5}$, and while it does share the edge $w_1v_4$ with the triangle $\{w_1,v_4,z\} \subseteq Z$, the triangle is not an $i$-set of $G$.	
			The triangle $D_{\ell-3}$ is adjacent to both $D_{\ell-2}$ and $D_{\ell-4}$, and no other triangles contain the edge $v_{\ell-5}v_{\ell-3}$.
			Similarly to $D_{\ell-4}$, the triangle $D_{\ell-2}$ does share the edge $w_4v_4$ with the triangle $\{w_4,v_4,z\} \subseteq Z$, which is not an $i$-set of $G$.	
			The triangle $D_{\ell-1}$ is adjacent to both $Y$ and $D_{\ell-2}$, and no other triangles contain the edge $w_3v_{\ell-3}$.  This completes the exhaustive verification that $\deg_{\ig{G}}(D_i) =2$ for all $1 \leq i \leq  \ell-1$. Moreover, we have confirmed that no additional edges are  present in the $i$-graph of $G$ beyond those given in $(i)-(iii)$.  We conclude that $\ig{G} = \thet{2,2,\ell}$.
			
			
			% ``````````````````````````````````  THET (2,2,l) ``````````````````````````````	
			
			\item $\mathbf{\thet{2,2,5}}$	\label{lem:c:thet225pf}
			
			As in part (a), we begin by listing the triangle sets:
			
			%=========== TRIANGLES =====================
			\begin{center}	
				\begin{tabular}{rlcrl}
					$X$ & $=\{w_0,w_1,w_2\},$  & \null \hspace{20mm} \null &  	$D_1$ & $= \{w_1,w_2,v_1\},$ \\
					$Y$ & $= \{w_0,w_3,w_4\},$ &&   	$D_2$ & $= \{w_2,v_{1},v_2\},$  \\
					$A$ & $=\{w_0,w_2,w_3\},$  &&		$D_{3}$ & $= \{ w_4,v_1,v_2 \},$ \\
					$B$ & $=\{w_0,w_1,w_4\},$  &&   	$D_4$ & $= \{ w_3,w_4,v_2 \}.$ \\
				\end{tabular}
			\end{center}
			
			\noindent Using this labelling of the vertices and triangles of $\cp{G}$ (and as in Figure \ref{fig:c:thet225}), we see that many of the arguments for this case proceed similarly to those in (a).  
			In particular, the triangles of $\cp{G}$ correspond to the $i$-sets of $G$, and so the triangles $A, B, X$ and $Y$, which form a wheel in $\cp{G}$, are an induced $C_4$ in $\ig{G}$.  We need only confirm that a third disjoint path in $\ig{G}$ is formed between $X$ and $Y$ (and nothing else).   Explicitly, the three pathways are:
			
			%=========== EDGES =====================
			\begin{enumerate}[itemsep=0pt, label=(\roman*)]
				\item \label{lem:c:thet225:i}  $\edge{X, w_1, w_3,A} \adedge{w_2,w_4,Y}$, 
				
				\item \label{lem:c:thet225:j} $\edge{X, w_2, w_4,B} \adedge{w_1,w_3,Y}$, 
				
				\item \label{lem:c:thet225:k} $\edge{X, w_0,  v_1,D_1}  \adedge{w_1,v_2,D_2} 
				\adedge{w_2,w_4,D_3} 
				\adedge{v_1,w_3,D_4} 
				\adedge{v_2,w_0,Y}$.		
			\end{enumerate}
			
			
			To see that there are no additional  $i$-sets of $G$ beyond those corresponding to the eight labelled triangles of Figure \ref{fig:c:thet225}, notice first that neither $z_1$ nor $z_2$ are in any $i$-sets as each of their closed neighbourhoods forms a $K_4$.  The vertices of the wheel $\{w_0,w_1,\dots,w_4\}$ form a $C_4$ in $\ig{G}$ by Lemma \ref{lem:c:wheel}, so any potential additional triangles contain at least one of $v_1$ or $v_2$.  Since $\cp{G}$ is planar, each vertex $v_i$ is in at most $\deg_{\cp{G}}(v_i)$ triangles of $\cp{G}$ and hence at $\deg_{\cp{G}}(v)$ $i$-sets of $G$.  For $v_1$, since $z_1\in N_{\cp{G}}(v_1)$ and $z_1$ is not any $i$-sets, $v_1$ is in at most $\deg_{\cp{G}}(v_1)-2 = 5-2=3$ $i$-sets, of which we have already accounted for all three ($D_1, D_2$, and $D_3$).   Similar arguments for $v_2$ follow.  Thus, the eight $i$-sets listed above are the only $i$-sets of $G$.
			
			Again, since $\cp{G}$ is planar and all triangles are facial, each $i$-set of $G$ is adjacent to at most three others in $\ig{G}$. 
			For $D_1$, notice that the edge $w_1v_1$ in $\cp{G}$ is part of a $K_4$ with $z_1$, and hence not adjacent to another triangle over that shared edge, and so $\deg_{\ig{G}}(D_1)=2$.    Similarly, each $D_i$  for $i\in \{2,3,4\}$ also has at least one shared edge with a $K_4$ in $\cp{G}$, containing either $z_1$ or $z_2$, so that $\deg_{\ig{G}}(D_i)=2$ for all $1 \leq i \leq 4$; there are no additional edges in $\ig{G}$ than those listed above.  We can therefore conclude that $X,D_1, D_2, D_3, D_4, Y$  forms the third disjoint path of length five  of a theta graph in $\ig{G}$, as required.
		\end{enumerate}	
	\end{proof}
	
	
	% <<< E: Lemma {lem:c:thet22l}
	
	
	
	
	
	
	
	%______________________  SUBSUB SECTION:  theta (2,3,ell) ______________________
	
	\subsubsection{Construction of $\cp{G}$ for $\thet{2,3,\ell}$ for $\ell \geq 5$}  \label{subsubsec:c:23k}
	
	
	For many of the results going forward, we apply small modifications to previous constructions.  In the first of these, we begin with the graphs from Construction \ref{con:c:thet22k}, which were used to find $i$-graphs for $\thet{2,2,5}$ and $\thet{2,2,\ell}$ for $\ell \geq 6$,  and expand the central wheel used in there  to build $i$-graphs for $\thet{2,3,5}$ and $\thet{2,3,\ell}$ for $\ell \geq 6$. 
	
	
	%>>> S:CONS {con:c:thet23k}
	\begin{cons} \label{con:c:thet23k}  Refer to Figures \ref{fig:c:thet23k} and \ref{fig:c:thet235}.	
		
		\begin{enumerate}[itemsep=0pt, label=(\alph*)]
			\item \label{con:c:thet23k:ell}
			If $\ell \geq 6$, begin with a copy of the graph $\cp{G}$ from Construction \ref{con:c:thet22k}.  Subdivide the edge $w_1w_4$, adding the new vertex $w_5$.  Join $w_5$ to $w_0$, so that $w_0,w_1,\dots,w_5$ forms a wheel.  Delete the vertex $z$.
			
			
			\item \label{con:c:thet23k:5} If $\ell=5$,	begin with a copy of the graph $\cp{G}$ from Construction \ref{con:c:thet22k}.  Subdivide the edge $w_1w_4$, adding the new vertex $w_5$.  Join $w_5$ to $w_0$, so that $w_0,w_1,\dots,w_5$ forms a wheel.  Delete the vertex $z_1$.
		\end{enumerate}
		
		We rename the resultant (planar) graph $\cp{G_{2,3,\ell}}$ for $\ell \geq 5$.	
	\end{cons}
	% <<< E: Cons {con:c:thet23k}
	
	
	
	%\nts{For any of the modified constructions, be careful that $\cp{G^*}$ is being used, not just $\cp{G}$}.
	
	
	%>>> S: Figure {fig:c:thet23k}		
	\begin{figure}[H] \centering	
		\begin{tikzpicture}	
			%---------- REF-------------------
			\node (cent) at (0,0) {};
			\path (cent) ++(0:45 mm) node (rcent) {};	
			
			%----Left Wheel
			\node[std,label={10:$w_0$}] (w0) at (cent) {};
			
			\foreach \i in {1,2,3,4}
			{
				\node[std,label={180-\i*90: $w_{\i}$}] (w\i) at (180-\i*90:2cm) {}; 
				\draw[thick] (w0)--(w\i);        
			}
			\draw[thick] (w1)--(w2)--(w3)--(w4);
			
			
			%---- Wheel Division
			
			\node[std,label={135: $w_5$}] (w5) at (135:2cm) {}; 
			\draw[thick] (w0)--(w5); 
			\draw[thick] (w4)--(w5)--(w1);
			
			
			%---- V-Path	
			\foreach \i / \j  / \k in {1/3/1, 2/2/2, 3/-1/{\ell-5}, 4/-2.2/{\ell-4}, 5/-3.4/{\ell-3}}
			{	
				\path (rcent) ++(90:\j cm) node [bblue] (v\i) {};
			}
			
			\path (v1) ++(0:4 mm) node (Lv1) {\color{blue} $v_{1}$};
			\path (v2) ++(0:4 mm) node (Lv2) {\color{blue} $v_{2}$};
			\path (v3) ++(-10:5 mm) node (Lv3) {\color{blue} $v_{\ell-5}$};
			\path (v4) ++(15:8 mm) node (Lv4) {\color{blue} $v_{\ell-4}$};
			\path (v5) ++(260:4 mm) node (Lv5) {\color{blue} $v_{\ell-3}$};		
			
			\draw[bline] (v1)--(v2);
			\draw[bline] (v3)--(v4)--(v5);
			
			\draw[bline,dashed] (v2)--(v3);
							
			%---- V3 to V5 
			\path (v4) ++(180:1.3 cm) coordinate  (c1) {};
			\draw[bline] (v3) to[out=190, in=90]  (c1) to [out=270,in=170] (v5);  
			
			%---- V1 to W1 W2
			\draw[bline] (w1)--(v1)--(w2);	
			
			%-- V5 to W4
			\draw[bline] (v5) to[out=180,in=-90] (w4);  
			
			%-- V5 to W3
			\draw[bline] (v5) to[out=170,in=-30] (w3);  
			
			%-- V4 to W4
			\draw[bline] (v4) to[out=-35, in=25]  (4.6cm,-4.2cm) to [out=205,in=260] (w4);  	
			%	\node[std] at (4.6cm,-4.2cm) {};
			
			%-- W1 to V2  
			\draw[bline] (w1) to[out=20, in=170]  (35:6.1cm) to [out=350,in=45]  (v2); 
			%	\node[std] at (35:6.2cm)  {};
			
			%-- W1 to  V3 
			\draw[bline] (w1) to[out=38, in=170]  (35:6.4cm) to [out=350,in=45]  (v3); 
			%\node[std] at (30:5.8cm) {};
			
			%-- W1 to V4
			\draw[bline] (w1) to[out=46, in=170]  (35:6.6cm) to [out=350,in=40]  (v4); 
			%\node[std] at (30:5.8cm) {};
			
			%-- W1 to Dashed T1 T2
			\path (rcent) ++(90:1 cm) coordinate  (t1) {};
			\draw[bline, dashed] (w1) to[out=28, in=170]   (35:6.2cm)  to [out=350,in=45]  (t1); 
			
			\path (rcent) ++(90:0 cm) coordinate  (t2) {};
			\draw[bline, dashed] (w1) to[out=34, in=170]  (35:6.3cm) to [out=350,in=45]  (t2); 
			
			%----- Internal Red Labellings	
			\path (w0) ++(45:9 mm) node [color=red] (X) {$X$};			
			\path (w0) ++(45:-9 mm) node [color=red] (Y) {$Y$};
			
			%-- A's
			\path (w0) ++(-45:8 mm) node [color=red] (A1) {$A$};	
			
			%-- B's	
			%\path (w0) ++(135:8 mm) node [color=red] (B1) {$B$};		
			\path (w0) ++(113:12 mm) node [color=red] (B1) {$B_1$};	
			\path (w0) ++(158:12 mm) node [color=red] (B2) {$B_2$};	
			
			%-- D's
			\path (w2) ++(90:15 mm) node [color=red] (D1) {$D_1$};	
			\path (v1) ++(170:9 mm) node [color=red] (D2) {$D_2$};	
			\path (v4) ++(160:7 mm) node [color=red] (D3) {$D_{\ell-3}$};
			\path (v5) ++(195:20mm) node [color=red] (D4) {$D_{\ell-2}$};
			\path (w4) ++(-55:20 mm) node [color=red] (D5) {$D_{\ell-1}$};			
			
		\end{tikzpicture} 
		\caption{The graph $\cp{G_{2,3,\ell}}$ from Construction \ref{con:c:thet23k} \ref{con:c:thet23k:ell} such that $\ig{G_{2,3,\ell}} = \ag{G_{2,3,\ell}} =  \thet{2,3,\ell}$ for $\ell \geq 6$.}
		\label{fig:c:thet23k}
	\end{figure}	
	% <<< E: Figure {fig:c:thet23k}
	
	
	
	
	
	%>>> S: Figure {fig:c:thet235}	
	\begin{figure}[H] \centering	
		\begin{tikzpicture}				
			%---------- REF-------------------
			\node (cent) at (0,0) {};
			\path (cent) ++(0:45 mm) node (rcent) {};	
			
			%----Left Wheel
			\node[std] (w0) at (cent) {};
			\path (w0) ++(30: 4 mm) node (Lw0) {${w_0}$};	
			
			\foreach \i in {1,2,3,4}
			{
				\node[std,label={180-\i*90: $w_{\i}$}] (w\i) at (180-\i*90:2.5cm) {}; 
				\draw[thick] (w0)--(w\i);        
			}
			\draw[thick] (w1)--(w2)--(w3)--(w4);
			
			%---- Wheel Division
			\node[std,label={90: $w_5$}] (w5) at (135:2.2cm) {}; 
			\draw[thick] (w0)--(w5); 
			\draw[thick] (w4)--(w5)--(w1);				
			
			%---- V-Path	
			\foreach \i / \j in {1/1.5,2/-1.5}
			{	
				\path (rcent) ++(90:\j cm) node [std] (v\i) {};
				\path (v\i) ++(0:4 mm) node (Lv\i) {$v_{\i}$};
				%\node[bblue,label={0: $v_\i$}] (v\i) at (4,2-\i) {};
			}
			\draw[thick] (w1)--(v1)--(v2)--(w3);
			\draw[thick] (v2)--(w2)--(v1);	
			
			%---- Zs
			\path (w2) ++(270:1 cm) node [bzed, label={[zelim]15:$\boldsymbol{z_2}$}] (z2) {};
			\draw[zline] (w2)--(z2)--(w3);
			\draw[zline] (z2)--(v2);			
					
			%--- V2 to W4 
			\draw[thick] (v2) to[out=230, in=-5]  (270:3.3cm) to [out=170,in=280] (w4);
			
			%--- V1 to W4
			\draw[thick] (v1) to[out=130, in=5]  (90:3.3cm) to [out=190,in=80] (w4);	
			
			%------------ THETA--------------------			
			%---- INNER Cycle	
			\foreach \i / \j  in {1/X,3/Y,4/A}
			{	
				\node[dred] (t\i) at (-45+\i*90:1.0cm) {}; 
				\path (t\i) ++(-45+\i*90: 4 mm) node (Lt\i) {\color{red}${\j}$};
				
			}
			
			%-- Modified B
			\path (w0) ++(113:10 mm) node [dred, label={[red]113: $B_1$}] (t2a) {};	
			\path (w0) ++(158:10 mm) node [dred, label={[red]158: $B_2$}] (t2b) {};			
			
			%---- D- Path
			\path (w2) ++(90: 7mm) node [dred] (d1) {};
			\path (d1) ++(90: 4 mm) node (Ld1) {\color{red}${D_1}$};
			
			\path (w2) ++(0: 15mm) node [dred] (d2) {};
			\path (d2) ++(90: 4 mm) node (Ld2) {\color{red}${D_2}$};	
			
			\path (v2) ++(-45: 10mm) node [dred] (d3) {};
			\path (d3) ++(0: 4 mm) node (Ld3) {\color{red}${D_3}$};	
			
			\path (t3) ++(260: 15mm) node [dred] (d4) {};
			\path (d4) ++(170: 4 mm) node (Ld4) {\color{red}${D_4}$};					
			
			\draw[rlinemb](t1)--(t2a)--(t2b)--(t3)--(t4)--(t1);
			\draw[rlinemb](t1)--(d1)--(d2);	
			\draw[rlinemb](t3)--(d4);
			
			%--- D2 to D3 
			\draw[rlinemb] (d2) to [out=-45,in=90] (d3);
			
			%--- D3 to D4
			\draw[rlinemb] (d3) to [out=230,in=300] (d4);
			
		\end{tikzpicture} 
		
		\caption{The graph $\cp{G_{2,3,5}}$ from Construction \ref{con:c:thet23k} \ref{con:c:thet23k:5} such that $\ig{G_{2,3,5}} = \thet{2,3,5}$, with $\ig{G_{2,3,5}}$ overlaid in red.}
		\label{fig:c:thet235}
	\end{figure}	
	% <<< E: Figure {fig:c:thet235}
	
	
	
	In Construction \ref{con:c:thet23k} \ref{con:c:thet23k:ell}, notice that the vertex $z$ is deleted from $\cp{G}$.    In the original Construction \ref{con:c:thet22k} for a graph $\cp{G}$ with $\ig{G} = \thet{2,2,\ell}$ for $\ell \geq 6$, $z$ served to eliminate the unwanted triangle formed by $\{w_1,w_4, v_{\ell-4}\}$.   Now with the expanded wheel including $w_5$, $\{w_1,w_4, v_{\ell-4}\}$ is not a triangle in $\cp{G_{2,3,\ell}}$ ($\ell \geq 6$), and $z$ is not needed.  Indeed, as $\cp{G_{2,3,\ell}}$ now has $\alpha({G_{2,3,\ell}}) = 3$, its triangles are also $\alpha$-sets in $G$, and so we can immediately extend the construction from $i$-graphs to $\alpha$-graphs.
	
	The extension, however, does not apply to  Construction \ref{con:c:thet23k} \ref{con:c:thet23k:5} for the graph $\cp{G_{2,3,5}}$.  Here, we no longer require  $z_1$ (which served to eliminate the unwanted triangle formed by $\{w_1,w_4, v_1\}$), but $z_2$ remains and forms the clique $\{w_2,w_3,z_2,v_2\}$; thus, $\alpha({G_{2,3,5}}) = 4$.  
	
	%In Construction \ref{con:c:thet23k} \ref{con:c:thet23k:5}, notice the vertex $z_1$ is deleted from $\cp{G}$.    In the original Construction \ref{con:c:thet22k} for a graph $\cp{G}$ with $\ig{G} = \thet{2,2,5}$, $z_1$ served to eliminate the unwanted triangle formed by $\{w_1,w_4, v_1\}$.   Now with the expanded wheel including $w_5$, $\{w_1,w_4, v_1\}$ is not a triangle in $\cp{G^*}$, and $z_1$ is not needed.  The proof for the  following Lemma \ref{lem:c:thet23k} is otherwise very similar to the proof of Lemma \ref{lem:c:thet22l}, and so is omitted.
	
	The proof for the  following Lemma \ref{lem:c:thet23k} is otherwise very similar to the proof of Lemma \ref{lem:c:thet22l}, and so is omitted.
	
	
	%>>>S: Lemma {lem:c:thet23k}
	
	\begin{lemma}\label{lem:c:thet23k}
		If $\cp{G_{2,3,5}}$ is the graph constructed in Construction \ref{con:c:thet23k} \ref{con:c:thet23k:5}, then $\ig{G_{2,3,5}} = \thet{2,3,5}$.  
		For $\ell \geq 6$, if $\cp{G_{2,3,\ell}}$  is the graph constructed in Construction \ref{con:c:thet23k} \ref{con:c:thet23k:ell}, then $\ig{G_{2,3,\ell}} = \ag{G_{2,3,\ell}} = \thet{2,3,\ell}$ for $\ell \geq 6$.  	
	\end{lemma}
	
	% <<< E: Lemma {lem:c:thet23k}
	
	
	
	%Given the similarly between Constructions \ref{con:c:thet22k} and \ref{con:c:thet23k}, the proof for Lemma \ref{lem:c:thet23k} 
	
	
	%______________________  SUBSUB SECTION:  theta (2,4,4) ______________________
	
	\subsubsection{Construction of $\cp{G}$ for $\thet{2,4,4}$}  \label{subsubsec:c:244}
	
	
	In the following construction for a graph $\cp{G}$ with $\ig{G} = \thet{2,4,4}$, we again apply the technique of  adding vertices to eliminate unwanted triangles.
	
	%>>>S: Figure {fig:c:thet244}
	\begin{figure}[H] \centering	
		\begin{tikzpicture}		
			%---------- REF-------------------
			\node (cent) at (0,0) {};
			\path (cent) ++(0:50mm) node (rcent) {};	
			
			%----Left Wheel
			\node[std,label={0:$w_0$}] (w0) at (cent) {};
			
			\foreach \i in {1,2,3,4,5,6}
			{
				\node[std,label={150-\i*60: $w_{\i}$}] (w\i) at (150-\i*60:2cm) {}; 
				\draw[thick] (w0)--(w\i);        
			}
			\draw[thick] (w1)--(w2)--(w3)--(w4)--(w5)--(w6)--(w1);
			
			%---- V-Path
			\path (rcent) ++(90:0 cm) node [bblue] (v) {};
			\path (v) ++(0:4 mm) node (Lv) {\color{blue} $v$};	
			
			\foreach \i / \j in {2,3}
			\draw[bline] (v)--(w\i);	
			
			%--- W1 to V
			\draw[bline] (w1)   to[out=0,in=100] (v); 	
			%--- W4 to V
			\draw[bline] (w4)   to[out=0,in=-100] (v); 
			%--- W4 to W1
			\draw[bline] (w4) to[out=-15, in=270]  (0:6.5cm)  to[out=90,in=15] (w1); 		
			
			%---- Zs
			\path (w0) ++(0:3.5 cm) node [bzed, label={[zelim]180:$\boldsymbol{z}$}] (z) {};
			\draw[zline] (w2)--(z)--(w3);
			\draw[zline] (z)--(v);
			
			%\path (w0) ++(60:-3 cm) node [bred, label={[red]180:$z'$}] (z1) {};
			\path (w0) ++(180:4 cm) node [bzed, label={[zelim]180:$\boldsymbol{z'}$}] (z1) {};
			%	\draw[rline] (z1)--(w0);
			\draw[zline] (w0)   to[out=165,in=15] (z1); 
			\draw[zline] (w1)   to[out=180,in=80] (z1); 		
			\draw[zline] (w4)   to[out=180,in=-80] (z1); 	
			
			%----- Internal Red Labellings	
			\path (w0) ++(60:12 mm) node [color=red] (X) {$X$};	
			\path (w0) ++(0:12 mm) node [color=red] (A) {$A$};	
			\path (w0) ++(-60:12 mm) node [color=red] (Y) {$Y$};	
			
			%-- B's	
			\foreach \i/\c in {1/120,2/180,3/240} {				
				\path (w0) ++(\c:12 mm) node [color=red] (B\i) {$B_{\i}$};	
			}
			
			%-- D's
			\path (w2) ++(05:15 mm) node [color=red] (D1) {$D_1$};	
			\path (v) ++(60:8 mm) node [color=red] (D2) {$D_2$};	
			\path (w3) ++(-05:15 mm) node [color=red] (D3) {$D_3$};
			
		\end{tikzpicture} 
		\caption{A graph $\cp{G}$ such that $\ig{G} = \thet{2,4,4}$.}
		\label{fig:c:thet244}
	\end{figure}	
	% <<< E: Figure {fig:c:thet244}
	
	
	\begin{cons} \label{con:c:thet244}
		Refer to Figure \ref{fig:c:thet244}.	Begin with a copy of the graph $\cp{H} \cong W_7 = C_6 \vee K_1$, labelling the degree 3 vertices as $w_1,w_2,\dots, w_6$ and the central degree 6 vertex as $w_0$.  Join $w_1$ to $w_4$.    Add a new vertex $v$ to $\cp{H}$, joining $v$ to $w_1, \dots, w_4$.    Then, add the new vertex $z$, joined to $v$, $w_2$ and $w_3$, and the new vertex $z'$, joined to $w_0, w_1$, and $w_4$.  We label the resultant (non-planar) graph $\cp{G}$.	
	\end{cons}
	
	
	%>>>S: Lemma {lem:c:thet244}	
	\begin{lemma}\label{lem:c:thet244}
		If $\cp{G}$ is the graph constructed by Construction \ref{con:c:thet244}, then $\ig{G} = \thet{2,4,4}$.
	\end{lemma}
	
	
	\begin{proof}	
		Once again, the triangles of $\cp{G}$ form the smallest maximal cliques of $\cp{G}$, and are therefore the $i$-sets of $G$.  As in Figure \ref{fig:c:thet244}, we label them as follows:	
		
		%=========== VERTICES  ==========		
		\begin{center}	
			\begin{tabular}{rlcrlcrl}
				$X$ & $=\{w_0,w_1,w_2\},$  & \null \hspace{1mm} \null &  	$B_1$ & $= \{w_0,w_1,w_6\},$ & \null \hspace{1mm} \null &  	$D_1$ & $= \{w_1,w_2,v\},$ \\
				$Y$ & $= \{w_0,w_3,w_4\},$ &&   	$B_2$ & $= \{w_0,w_5,w_6\}$,  & \null \hspace{1mm} \null &  	$D_2$ & $= \{w_1,w_4,v\},$ \\
				$A$ & $=\{w_0,w_2,w_3\},$  &&		$B_3$ & $= \{w_0,w_4,w_5 \},$ & \null \hspace{1mm} \null &  	$D_3$ & $= \{w_3,w_4,v\}.$ \		
			\end{tabular}
		\end{center}
		
		%=========== NO EXTRA TRIANGLES ==========	
		Similarly to the construction for $\thet{2,2,5}$  in the proof of Lemma \ref{lem:c:thet22l}, the vertices $z$ and $z'$ are added to ensure that $\{v,w_2,w_3\}$ and $\{w_0,w_1,w_4\}$, respectively, are not maximal cliques in  $\cp{G}$, and hence are not $i$-sets of $G$.
		
		To see that there are no other triangles in $\cp{G}$ beyond the nine listed above (and thus, no unaccounted for $i$-sets in $G$), consider how one such unaccounted for triangle might be constructed.  Since $N[z]$ forms a maximal clique, $z$ (and likewise $z'$) is not on any such triangle.  Moreover, all triangles comprised entirely of vertices from the wheel $W_7 = \{w_0,w_1,\dots,w_6\}$ have already been considered.  This leaves only triangles potentially formed by two adjacent wheel vertices and $v$.  However, $\deg(v)=4$, so it is incident with at most $\binom{4}{2}=6$ triangles, three of which have already been accounted for in $D_1, D_2, D_3$, and one that has been eliminated by the clique $\{v,w_2,w_3,z\}$.  For the remaining two edge combinations, $vw_3$ and $vw_1$ are not on a triangle as $w_1w_2 \notin E(\cp{G})$, and likewise, $vw_2$ and $vw_4$ are not on a triangle as $w_2w_4 \notin E(\cp{G})$. We therefore conclude that the collection of triangles of $G$ are exactly the nine sets listed above; moreover, these nine sets are the $i$-sets of $G$ and hence form $V(\ig{G})$.
		
		
		From Figure \ref{fig:c:thet244}, the following triangle adjacencies are immediate:
		%=========== EDGES =====================		
		\begin{enumerate}[itemsep=0pt, label=(\roman*)]
			\item \label{lem:c:thet244:i}  $\edge{X, w_1, w_3,A} \adedge{w_2,w_4,Y}$, 
			
			\item \label{lem:c:thet244:j} $\edge{X, w_2, w_6,B_1} \adedge{w_1,w_5,B_2} \adedge{w_6,w_4,B_3} \adedge{w_5,w_3,Y} $, 
			
			\item \label{lem:c:thet244:k} $\edge{X, w_0,  v,D_1}  \adedge{w_2,w_4,D_2} \adedge{w_1,w_3,D_3}  \adedge{v,w_0,Y}$. 
		\end{enumerate}
		
		
		% =========== NO EXTRA EDGES =============	
		
		Lemma \ref{lem:c:wheel} ensures that there are no additional adjacencies between two triangles on the wheel $\cp{H}$. Thus, we need only check that there are no unaccounted for edges between the triangles of the collection $\mathcal{D} =\{D_1,D_2,D_3\}$, either among themselves, or with triangles from the wheel.  The former is easily removed by observing from Figure \ref{fig:c:thet244} that $D_1$ and $D_3$ share no edges and are therefore not adjacent.   For the latter, notice that each wheel triangle contains the vertex $w_0$, which  is not a part of any of $\mathcal{D}$.  Thus only triangles of $\mathcal{D}$ containing two consecutively numbered wheel vertices (i.e. $w_iw_{i+1}$ or $w_6w_1$) are adjacent to wheel triangles.  From the figure, this occurs exactly twice: $w_1w_2$ in $D_1$ and $w_3w_4$ in $D_3$, and has already been accounted for in the adjacencies $\edge{X, w_0,  v,D_1} $ and $\edge{Y,w_0,v,D_3}$.  This ensures that there are no additional edges in $\ig{G}$ than the ten outlined in the list above, and so  we conclude that $\ig{G} = \thet{2,4,4}$ as required.
	\end{proof}
	% <<< E:  Lemma {lem:c:thet244}	
	
	
	
	
	Notice that Construction \ref{con:c:thet244}  is our first theta graph construction that is not planar.  In particular, the constructed graph $\cp{G}$ has a $K_{3,3}$ minor, as illustrated in Figure \ref{fig:c:thet244nonPlanar}.  Indeed, with the exception of the constructions that are based upon Construction \ref{con:c:thet244}, all of our $i$-graph constructions use planar complement seed graphs.   
	
	
	%>>> S: Figure {fig:c:thet244nonPlanar}	
	\begin{figure}[H] \centering	
		\begin{tikzpicture}	
			
			%---------- REF-------------------
			\node (cent) at (0,0) {};
			\coordinate(arrowLeft) at (2.7cm,0){};
			\coordinate(arrowRight) at (4.5cm,0){};
			
			
			%----Left Wheel
			\node[std,label={0:$w_0$}] (w0) at (cent) {};
			
			\foreach \i in {1,2,3,4,5,6}
			{
				\node[std,label={150-\i*60: $w_{\i}$}] (w\i) at (150-\i*60:2cm) {}; 
				\draw[thick] (w0)--(w\i);        
			}
			\draw[thick] (w1)--(w2)--(w3)--(w4)--(w5)--(w6)--(w1);
			
			%---- Zs
			\path (w0) ++(180:3.6 cm) node [std, label={[red]180:$z'$}] (z1) {};
			\draw[thick] (w0)   to[out=165,in=15] (z1); 
			\draw[thick] (w1)   to[out=180,in=80] (z1); 		
			\draw[thick] (w4)   to[out=180,in=-80] (z1); 
			
			
			%---- Arrow
			\node[broadArrow,fill=white, draw=black, ultra thick, text width=1cm] at (3.5cm,0){};
			
		\end{tikzpicture} 	
		\begin{tikzpicture}	
			
			%---------- REF-------------------
			\node (cent) at (0,0) {};
			
			%----Left Wheel
			\node[bblue,label={0:$w_0$}] (w0) at (cent) {};
			
			\foreach \i in {1,2,3,4,5,6}
			\coordinate (w\i) at (150-\i*60:2cm) {}; 
			
			\draw[thick] (w1)--(w2)--(w3)--(w4)--(w5)--(w6)--(w1);
			
			\foreach \i in {2,6}
			\node[regRed,label={150-\i*60: $w_{\i}$}] (nw\i) at (w\i) {}; 
			
			\foreach \i in {1,4}
			\node[bblue,label={150-\i*60: $w_{\i}$}] (nw\i) at (w\i) {}; 
			
			\draw[thick] (nw6)--(w0)--(nw2);
			
			%---- Zs
			\path (w0) ++(180:3.6 cm) node [regRed, label={[red]180:$z'$}] (z1) {};
			\draw[thick] (w0)   to[out=165,in=15] (z1); 
			\draw[thick] (nw1)   to[out=180,in=80] (z1); 		
			\draw[thick] (nw4)   to[out=180,in=-80] (z1); 
			
		\end{tikzpicture} 
		\caption{A $K_{3,3}$ minor in a subgraph of $\cp{G}$ from Figure \ref{fig:c:thet244}.}
		\label{fig:c:thet244nonPlanar}
	\end{figure}	
	% <<< E: Figure {fig:c:thet244nonPlanar}
	
	
	\begin{problem}	\null 	
		\begin{enumerate}[label=(\roman*)]
			\item Find a planar graph-complement construction for $\thet{2,4,4}$.  
			
			\item 	 Do all $i$-graphs with largest induced stars of $K_{1,3}$, always have a planar graph-complement construction?
			
			\emph{A large target graph requires a large seed graph in order to generate a sufficient number of unique $i$-sets.   Can a target graph become too dense to allow for a planar graph-complement construction?}	
		\end{enumerate}
		
	\end{problem}
	
	
	
	
	%~~~~~~~~~~~~~~~~~~~~
	Moving forward, we will no longer explicitly check that there are no additional unaccounted for triangles in our constructions.  Should the construction indeed result in triangles of $\cp{G}$ that produce extraneous vertices in $\ig{G}$, we can easily remove them using the Deletion Lemma (Lemma \ref{lem:i:inducedI}).   In fact, in the previous results like in Construction \ref{con:c:thet244}, the addition of the vertices $z$ and $z'$ were exactly such applications.  Recall that in the Deletion Lemma, when removing a vertex $X$ from the $i$-graph, a new vertex $z$ is added to the seed graph and joined to every vertex \emph{except} those of $X$.  In the complement seed graph $\cp{G}$, this amounts to adding $z$ and joining to everything in $X$ (and nothing else), exactly as we did in Construction \ref{con:c:thet244}.
	
	Although we are quite certain that the graphs presented in the following constructions are the exact ones that build the given theta graphs, it is of no actual consequence to the existence of the theta graph as an $i$-graph if they are not; by the Deletion Lemma, it is enough to present the graph $\cp{G}$ with the knowledge that its complement produces  an $i$-graph that contains the desired theta graph as an induced subgraph.
	
	
	
	
	
	
	
	%______________________  SUBSUB SECTION:  theta (2,4,5) ______________________
	
	\subsubsection{Constructions of $\cp{G}$ for $\thet{2,4,5}$ and $\thet{2,5,5}$}  \label{subsubsec:c:245}
	
	%	\nts{Subdivision of 235 on B-Line once and twice, resp}
	
	%	\nts{Check construction environment}
	
	
	\begin{cons} \label{cons:c:thet2k5}	  Refer to Figure  \ref{fig:c:thet255}.
		\begin{enumerate}[itemsep=0pt, label=(\alph*)]
			\item \label{con:c:thet245:a}
			Begin with a copy of the graph $\cp{G_{2,3,5}}$ from Construction \ref{con:c:thet23k} \ref{con:c:thet23k:5} for $\thet{2,3,5}$.  Subdivide the edge $w_1w_5$, adding the new vertex $w_6$.  Join $w_6$ to $w_0$, so that $w_0,w_1,\dots,w_6$ forms a wheel.  Call this graph $\cp{G_{2,4,5}}$. 
			
			
			\item \label{con:c:thet255:b} Begin with a copy of the graph $\cp{G_{2,4,5}}$  from  Construction \ref{cons:c:thet2k5} \ref{con:c:thet245:a}.  Subdivide the edge $w_1w_6$, adding the new vertex $w_7$.  Join $w_7$ to $w_0$, so that $w_0,w_1,\dots,w_7$ forms a wheel.  Call this graph $\cp{G_{2,5,5}}$.  
		\end{enumerate}
	\end{cons}
	
	
	%>>> S: Figure {fig:c:thet255}	
	\begin{figure}[H] \centering	
		\begin{tikzpicture}	
			
			%---------- REF-------------------
			\node (cent) at (0,0) {};
			\path (cent) ++(0:45 mm) node (rcent) {};	
			
			%----Left Wheel
			\node[std] (w0) at (cent) {};
			\path (w0) ++(30: 4 mm) node (Lw0) {${w_0}$};	
			
			\foreach \i in {1,2,3,4}
			{
				\node[std,label={180-\i*90: $w_{\i}$}] (w\i) at (180-\i*90:2.5cm) {}; 
				\draw[thick] (w0)--(w\i);        
			}
			\draw[thick] (w1)--(w2)--(w3)--(w4);
			
			%---- Wheel Division
			%	\node[std,label={92: $w_5$}] (w5) at (157.5:2.5cm) {}; 
			\node[std] (w5) at (157.5:2.5cm) {}; 
			\path (w5) ++(94: 5 mm) node (Lw5) {${w_5}$};	
			\draw[thick] (w0)--(w5); 
			
			\node[std,label={90: $w_6$}] (w6) at (135:2.5cm) {}; 
			\draw[thick] (w0)--(w6); 
			
			\node[std,label={90: $w_7$}] (w7) at (112.5:2.5cm) {}; 
			\draw[thick] (w0)--(w7); 
			\draw[thick] (w4)--(w5)--(w6)--(w7)--(w1);		
			
			
			%---- V-Path	
			\foreach \i / \j in {1/1.5,2/-1.5}
			{	
				\path (rcent) ++(90:\j cm) node [std] (v\i) {};
				\path (v\i) ++(0:4 mm) node (Lv\i) {$v_{\i}$};
				%\node[bblue,label={0: $v_\i$}] (v\i) at (4,2-\i) {};
			}
			\draw[thick] (w1)--(v1)--(v2)--(w3);
			\draw[thick] (v2)--(w2)--(v1);	
			
			%---- Zs
			\path (w2) ++(270:1 cm) node [bzed, label={[zelim]15:$\boldsymbol{z_2}$}] (z2) {};
			\draw[zline] (w2)--(z2)--(w3);
			\draw[zline] (z2)--(v2);	
			
			%--- V2 to W4 
			\draw[thick] (v2) to[out=230, in=-5]  (270:3.3cm) to [out=170,in=280] (w4);
			
			%--- V1 to W4
			\draw[thick] (v1) to[out=130, in=5]  (110:3.5cm) to [out=195,in=110] (w4);	
			
			%	\node[std] (t1) at (110:3.3cm) {};
			
			
			%------------ THETA--------------------
			
			%---- INNER Cycle	
			\foreach \i / \j  in {1/X,3/Y,4/A}
			{	
				\node[dred] (t\i) at (-45+\i*90:1.0cm) {}; 
				\path (t\i) ++(-45+\i*90: 4 mm) node (Lt\i) {\color{red}${\j}$};
				
			}
			
			%-- Modified B
			%\path (w0) ++(101.25:10 mm) node [bred, label={[red]101.25: $B_1$}] (t2a) {};
			\path (w0) ++(101.25:10 mm) node [dred] (t2a) {};	
			\path (t2a) ++(101.25: 4 mm) node (Lt2a) {\color{red}${B_1}$};		
			\path (w0) ++(123.75:10 mm) node [dred] (t2b) {};
			\path (t2b) ++(123.75: 4 mm) node (Lt2b) {\color{red}${B_2}$};	
			\path (w0) ++(146.25:10 mm) node [dred] (t2c) {};	
			\path (t2c) ++(146.25: 4 mm) node (Lt2c) {\color{red}${B_3}$};	
			\path (w0) ++(168.75:10 mm) node [dred] (t2d) {};	
			\path (t2d) ++(168.75: 4 mm) node (Lt2d) {\color{red}${B_4}$};	
			
			
			%---- D- Path
			\path (w2) ++(90: 7mm) node [dred] (d1) {};
			\path (d1) ++(90: 4 mm) node (Ld1) {\color{red}${D_1}$};
			
			\path (w2) ++(0: 15mm) node [dred] (d2) {};
			\path (d2) ++(90: 4 mm) node (Ld2) {\color{red}${D_2}$};	
			
			\path (v2) ++(-45: 10mm) node [dred] (d3) {};
			\path (d3) ++(0: 4 mm) node (Ld3) {\color{red}${D_3}$};	
			
			\path (t3) ++(260: 15mm) node [dred] (d4) {};
			\path (d4) ++(170: 4 mm) node (Ld4) {\color{red}${D_4}$};			
			
			
			\draw[rlinemb](t1)--(t2a)--(t2b)--(t2c)--(t2d)--(t3)--(t4)--(t1);
			\draw[rlinemb](t1)--(d1)--(d2);	
			\draw[rlinemb](t3)--(d4);
			
			%--- D2 to D3 
			\draw[rlinemb] (d2) to [out=-45,in=90] (d3);
			
			%--- D3 to D4
			\draw[rlinemb] (d3) to [out=230,in=300] (d4);
			
		\end{tikzpicture} 
		
		\caption{The graph $\cp{G_{2,5,5}}$ from Construction \ref{cons:c:thet2k5}	 such that $\ig{G} = \thet{2,5,5}$, with $\ig{G}$ overlaid in red.}
		\label{fig:c:thet255}
	\end{figure}	
	% <<< E: Figure {fig:c:thet255}
	
	
	%>>>S: Lemma {lem:c:thet2k5}	
	\begin{lemma} \label{lem:c:thet2k5}	
		If $\cp{G_{2,k,5}}$ is the graph constructed by Construction \ref{cons:c:thet2k5}, then $\ig{G_{2,k,5}} = \thet{2,k,5}$, for $4 \leq k \leq 5$.
	\end{lemma}
	% <<< E: Lemma {lem:c:thet2k5}	
	
	
	\noindent The proof for Lemma \ref{lem:c:thet2k5} is similar to that of Lemma \ref{lem:c:thet22l}\ref{lem:c:thet225pf} and is omitted.
	
	%______________________  SUBSUB SECTION:  theta (2,4,4) ______________________
	
	\subsubsection{Construction of $\cp{G}$ for $\thet{2,k,\ell}$ for $\ell \geq k \geq 4$ and $\ell \geq 6$}  \label{subsubsec:c:2kl}
	
	
	
	%	\nts{Subdivision of 23L on B-Line (and D line)}
	
	\begin{cons}\label{cons:c:thet2kl} 
		See Figure \ref{fig:c:thet2kl}.   Begin with a copy of the graph $\cp{G_{2,3,\ell}}$ from Construction \ref{con:c:thet23k} \ref{con:c:thet23k:ell} for $\ell\geq 5$.  Subdivide the edge $w_1w_5$ $k-3$ times (for $k \leq \ell$), adding the new vertices $w_6$, $w_7, \dots, w_{k+2}$.  Join $w_6, w_7, \dots, w_{k+2}$ to $w_0$, so that $w_0,w_1,\dots,w_{k+2}$ forms a wheel.  Call this graph $\cp{G_{2,k,\ell}}$.		
	\end{cons}
	
	
	
	
	%>>> S: Figure {fig:c:thet2kl}	
	\begin{figure}[H] \centering	
		\begin{tikzpicture}	
			%---------- REF-------------------
			\node (cent) at (0,0) {};
			\path (cent) ++(0:45 mm) node (rcent) {};	
			
			%----Left Wheel
			\node[std,label={10:$w_0$}] (w0) at (cent) {};
			
			\foreach \i in {1,2,3,4}
			{
				\node[std,label={180-\i*90: $w_{\i}$}] (w\i) at (180-\i*90:2cm) {}; 
				\draw[thick] (w0)--(w\i);        
			}
			\draw[thick] (w1)--(w2)--(w3)--(w4);
			
			
			
			
			\node[std] (w5) at (157.5:2cm) {}; 
			\path (w5) ++(157: 5 mm) node (Lw5) {${w_5}$};	
			\draw[thick] (w0)--(w5); 
			
			
			\node[std,label={112: $w_{k-3}$}] (w7) at (112.5:2cm) {}; 
			\draw[thick] (w0)--(w7); 
			\draw[thick] (w4)--(w5);
			\draw[thick] (w7)--(w1);	
			\draw[dashed](w5)--(w7);	
			
			
			\coordinate  (c1) at ($(w5)!0.33!(w7)$) {};
			\coordinate  (c2) at ($(w5)!0.66!(w7)$) {};
			
			\draw [dashed] (c2)--(w0);
			\draw [dashed] (c1)--(w0);		
			
			
			
			%---- V-Path	
			\foreach \i / \j  / \k in {1/3/1, 2/2/2, 3/-1/{\ell-5}, 4/-2.2/{\ell-4}, 5/-3.4/{\ell-3}}
			{	
				\path (rcent) ++(90:\j cm) node [bblue] (v\i) {};
			}
			
			\path (v1) ++(0:4 mm) node (Lv1) {\color{blue} $v_{1}$};
			\path (v2) ++(0:4 mm) node (Lv2) {\color{blue} $v_{2}$};
			\path (v3) ++(-10:5 mm) node (Lv3) {\color{blue} $v_{\ell-5}$};
			\path (v4) ++(15:8 mm) node (Lv4) {\color{blue} $v_{\ell-4}$};
			\path (v5) ++(260:4 mm) node (Lv5) {\color{blue} $v_{\ell-3}$};		
			
			\draw[bline] (v1)--(v2);
			\draw[bline] (v3)--(v4)--(v5);
			
			\draw[bline,dashed] (v2)--(v3);
			
			
			%---- V3 to V5 
			\path (v4) ++(180:1.3 cm) coordinate  (c1) {};
			\draw[bline] (v3) to[out=190, in=90]  (c1) to [out=270,in=170] (v5);  
			
			%---- V1 to W1 W2
			\draw[bline] (w1)--(v1)--(w2);	
			
			%-- V5 to W4
			\draw[bline] (v5) to[out=180,in=-90] (w4);  
			
			%-- V5 to W3
			\draw[bline] (v5) to[out=170,in=-30] (w3);  
			
			%-- V4 to W4
			\draw[bline] (v4) to[out=-35, in=25]  (4.6cm,-4.2cm) to [out=205,in=260] (w4);  	
			%	\node[std] at (4.6cm,-4.2cm) {};
			
			%-- W1 to V2  
			\draw[bline] (w1) to[out=20, in=170]  (35:6.1cm) to [out=350,in=45]  (v2); 
			%	\node[std] at (35:6.2cm)  {};
			
			%-- W1 to  V3 
			\draw[bline] (w1) to[out=38, in=170]  (35:6.4cm) to [out=350,in=45]  (v3); 
			%\node[std] at (30:5.8cm) {};
			
			%-- W1 to V4
			\draw[bline] (w1) to[out=46, in=170]  (35:6.6cm) to [out=350,in=40]  (v4); 
			%\node[std] at (30:5.8cm) {};
			
			%-- W1 to Dashed T1 T2
			\path (rcent) ++(90:1 cm) coordinate  (t1) {};
			\draw[bline, dashed] (w1) to[out=28, in=170]   (35:6.2cm)  to [out=350,in=45]  (t1); 
			
			\path (rcent) ++(90:0 cm) coordinate  (t2) {};
			\draw[bline, dashed] (w1) to[out=34, in=170]  (35:6.3cm) to [out=350,in=45]  (t2); 
			
			%----- Internal Red Labellings	
			\path (w0) ++(45:9 mm) node [color=red] (X) {$X$};			
			\path (w0) ++(45:-9 mm) node [color=red] (Y) {$Y$};
			
			%-- A's
			\path (w0) ++(-45:8 mm) node [color=red] (A1) {$A$};	
			
			
			%-- B's	
			\path (w0) ++(100:14 mm) node [color=red] (B1) {$B_1$};	
			\path (w0) ++(170:14 mm) node [color=red] (B2) {$B_{k-1}$};
			
			
			%-- D's
			\path (w2) ++(90:15 mm) node [color=red] (D1) {$D_1$};	
			\path (v1) ++(170:9 mm) node [color=red] (D2) {$D_2$};	
			\path (v4) ++(160:7 mm) node [color=red] (D3) {$D_{\ell-3}$};
			\path (v5) ++(195:20mm) node [color=red] (D4) {$D_{\ell-2}$};
			\path (w4) ++(-55:20 mm) node [color=red] (D5) {$D_{\ell-1}$};			
			
		\end{tikzpicture} 
		\caption{The graph $\cp{G_{2,k,\ell}}$ from Construction \ref{cons:c:thet2kl} such that $\ig{\cp{G_{2,k,\ell}}} = \thet{2,k,\ell}$ for $\ell \geq k \geq 4$ and $\ell \geq 6$.}
		\label {fig:c:thet2kl}
	\end{figure}	
	% <<< E: Figure {fig:c:thet2kl}
	
	
	
	
	
	\noindent The proof for Lemma \ref{lem:c:thet2kl} again proceed similarly to the proof of Lemma \ref{lem:c:thet22l}\ref{lem:c:thet22lpf} and is also omitted.
	
	%>>>S: Lemma {lem:c:thet2kl}	
	\begin{lemma} \label{lem:c:thet2kl}
		If $\cp{G_{2,k,\ell}}$ is the graph constructed by Construction \ref{cons:c:thet2kl}, then $\ig{G_{2,k,\ell}} = \ag{G_{2,k,\ell}} = \thet{2,k,\ell}$, for $\ell \geq k \geq 4$ and $\ell \geq 6$.
	\end{lemma}
	% <<< E: Lemma {lem:c:thet2kl}
	
	
	
	%......................  SUB SECTION:  theta (3,k,l) .........................
	\subsection{$\thet{3,k,\ell}$}  \label{subsec:c:3kl}
	
	
	
	%.______________________ SUBSUB SECTION:  theta (3,3,4) ______________________
	
	\subsubsection{Construction of $\cp{G}$ for $\thet{3,3,4}$}  \label{subsubsec:c:334}
	
	When initially exploring the $i$-graph realizability of $\thet{3,3,4}$, we encountered difficulties in trying to use a similar method as above utilizing graph complements to create a graph $\cp{G}$ such that $\ig{G} = \thet{3,3,4}$.  Through trial and error, we instead found the graph $G$ in Figure \ref{fig:c:thet334}  which  has $\ig{G} = \thet{3,3,4}$.  Although the following Lemma \ref{lem:c:thet334} does not use graph complements, we include it here for the completeness of determining the $i$-graph realizability of theta graphs.
	
	
	%>>> START Prop {lem:c:thet334}
	\begin{lemma} \label{lem:c:thet334}
		$\thet{3,3,4}$ is an $i$-graph.
	\end{lemma}
	
	
	\begin{proof}		
		Consider the graph $G$ in Figure \ref{fig:c:thet334}.	We claim that $\ig{G}= \thet{3,3,4}$, with corresponding $i$-sets as illustrated in Figure \ref{fig:c:thet334Sets}.
		
		%>>>S: Figure {fig:c:thet334}
		\begin{figure}[H]\centering
			\begin{tikzpicture}	
				
				%---------- REF-------------------
				\node (cent) at (0,0) {};
				
				%----- W0 - Left Wheel ----------
				
				\node [std] at (cent) (v0) {};
				\path (v0) ++(90:4 mm) node (v0L) {$v_0$};		
				
				\foreach \i/\c in {1/25,2/155,3/-155, 4/-25} {				
					\path (v0) ++(\c:20 mm) node [std] (v\i) {};
					\path (v\i) ++(\c:5 mm) node (Lv\i) {$v_{\i}$};
					\draw[thick] (v0)--(v\i);
				}
				
				\draw[thick] (v1)--(v2)--(v3)--(v4)--(v1);
				
				\foreach \i/\c/\j /\d in {5/90/90/15,6/-90/-90/15,7/0/45/30} {				
					\path (v0) ++(\c:\d mm) node [std] (v\i) {};
					\path (v\i) ++(\j:5 mm) node (Lv\i) {$v_{\i}$};
				}	
				
				\draw[thick] (v1)--(v5)--(v2);
				\draw[thick] (v3)--(v6)--(v4);
				
				\draw[thick] (v1)--(v7)--(v4);
				\draw[thick] (v0)--(v7);
				
				\path (v0) ++(0:45 mm) node [std] (v8) {};
				\path (v8) ++(0:5 mm) node (Lv8) {$v_{8}$};
				\draw[thick] (v7)--(v8);
				
			\end{tikzpicture}
			\caption{A graph $G$ such that $\ig{G} = \thet{3,3,4}$.}
			\label{fig:c:thet334}	
		\end{figure}						
		% <<< E: Figure {fig:c:thet334}
		
		
		
		%>>>S: Figure {fig:c:thet334Sets}
		\begin{figure}[H]\centering
			\begin{tikzpicture}	
				
				%---------- REF-------------------
				\node (cent) at (0,0) {};
				\path (cent) ++(0:30 mm) node (rcent) {};	
				\path (cent) ++(180:10 mm) node (lcent) {};	
				
				%----- cent path ----------
				
				\foreach \i/\c in {1/20,2/5,3/-5, 4/-20} {				
					\path (cent) ++(90:\c mm) node [std] (v\i) {};
				}
				
				\draw[thick] (v1)--(v2)--(v3)--(v4);
				
				% --- left path ---
				\foreach \i/\c in {5/5,6/-5} {				
					\path (lcent) ++(90:\c mm) node [std] (v\i) {};		
				}	
				
				\draw[thick] (v1)--(v5)--(v6)--(v4);
				
				% --- right path ---
				\foreach \i/\c in {7/10,8/0,9/-10} {				
					\path (rcent) ++(90:\c mm) node [std] (v\i) {};
				}	
				
				\draw[thick] (v1)--(v7)--(v8)--(v9)--(v4);		
				
				% ---Set Coding ---	
				\foreach \i/\j/\k /\l / \a in {1/2/6/8/15,2/2/4/8/0,3/4/5/8/0,4/3/5/8/-15}
				\path (v\i) ++(\a:12 mm) node (Ls\i) {$\{v_{\j},v_{\k},v_{\l}\}$};
				
				\foreach \i/\j/\k /\l in {5/1/6/8,6/1/3/8}
				\path (v\i) ++(180:12 mm) node (Ls\i) {$\{v_{\j},v_{\k},v_{\l}\}$};
				
				\foreach \i/\j/\k /\l in {7/2/6/7,8/5/6/7,9/3/5/7}
				\path (v\i) ++(0:12 mm) node (Ls\i) {$\{v_{\j},v_{\k},v_{\l}\}$};		
				
			\end{tikzpicture}
			\caption{The $i$-graph of $G$ from Figure \ref{fig:c:thet334}.}
			\label{fig:c:thet334Sets}	
		\end{figure}						
		% <<< E: Figure {fig:c:thet334Sets}
		
		Notice that  at least one vertex of $T_1=\{v_1,v_2,v_5\}$, $T_2=\{v_3,v_4,v_6\}$ and $\{v_7,v_8\}$ is in each $i$-set of $G$, and hence $i(G)=3$.  It is straight-forward to confirm that each set illustrated in Figure \ref{fig:c:thet334} is an $i$-set of $G$, and that the $i$-set adjacencies (and edges of $\ig{G}$) are as drawn.
		
		Thus, we need only confirm that $G$ has only the nine $i$-sets listed there, and that none are unaccounted for in Figure \ref{fig:c:thet334}.  To do so, we proceed with a counting argument.
		If $v_8 \in S$, then there are three options for each of $T_1$ and $T_2$, except for the cases where the selected vertices of each triangle are adjacent to each other: $\{v_2,v_3\}$, $\{v_1,v_4\}$, and the case where $v_0$ is left undominated, $\{v_5,v_6\}$.  Thus there are $(3)(3) -3 = 6$ $i$-sets containing $v_8$.  If an $i$-set contains $v_7$, then $v_1$ and $v_4$ are not in the $i$-set, so exactly one each of $T_1-\{v_1\} = \{v_2,v_5\}$ and $T_2 - \{v_4\} = \{v_3,v_6\}$ are in the $i$-set.  We again must exclude the case where both adjacent $v_2$ and $v_3$ are present; since $v_7$ dominates $v_0$, we no longer exclude the case where both $v_5$ and $v_6$ are present.    Thus, there are $(2)(2)-1=3$ $i$-sets containing $v_7$.  This accounts for all nine of the $i$-sets required to construct $\thet{3,3,4}$.
	\end{proof}
	
	
	
	For completeness, in Figure \ref{fig:c:thet334comp} we include a sketch of the complement of the graph $G$ given in Figure \ref{fig:c:thet334}, using a layout more familiar to the format we saw in the previous constructions, but with the same vertex labellings as in Figure \ref{fig:c:thet334}.  Although very similar, it is one of only two the constructions (along with Construction \ref{con:c:thet244}) that require an additional edge between two of the wheel vertices (i.e. $v_5$ and $v_6$).   Moreover, this representation of $\cp{G}$ -  and the set $D_2$ in particular - highlights how easily triangles of $\cp{G}$ can be overlooked when they are non-facial triangles.  We also note that this construction joins $\thet{2,4,4}$ among those currently lacking a planar graph complement construction.
	
	
	\begin{figure}[H] \centering	
		\begin{tikzpicture}	
			%---------- REF-------------------
			\node (cent) at (0,0) {};
			\path (cent) ++(0:40 mm) node (rcent) {};	
			
			%----Left Wheel
			\node[std,label={0:$w_0$}] (w0) at (cent) {};
			
			\foreach \i / \j in {1/2,2/6,3/1,4/3,5/5,6/4}
			{
				\node[std,label={150-\i*60: $v_{\j}$}] (w\i) at (150-\i*60:2cm) {}; 
				\draw[thick] (w0)--(w\i);        
			}
			\draw[thick] (w1)--(w2)--(w3)--(w4)--(w5)--(w6)--(w1);
			
			%---- V-Path	
			\path (rcent) ++(90:-0.5 cm) node [bblue,label={[blue]0: $v_7$}] (v) {};	
			
			%---- W2 to V
			\draw[bline] (v)--(w2);
			
			%---- V to W1-Path
			\draw[bline] (v) to[out=90,in=0] (w1);  	
			
			
			%---- V2 to W4-Path
			\draw[bline] (v) to[out=230,in=0] (w4);  	
			
			%-- V to W5
			\draw[bline] (v) to [out=260,in=15]  (-60:3.5cm) to [out=195,in=270] (w5);  
			
			%--- W2 to W5	
			\draw[bline] (w2) to [out=90, in=20]  (120:3cm) to[out=200,in=160] (w5); 
			
			%------ Z 
			\path (w0) ++(120:5 mm) node [bzed, label={[zelim]90:$\boldsymbol{v_0}$}] (z) {};
			\draw[zline] (z)--(w0);
			\draw[zline] (w5)--(z)--(w2);
			
			
			%----- Internal Red Labellings	
			\path (w0) ++(60:12 mm) node [color=red] (X) {$X$};			
			\path (w0) ++(60:-12 mm) node [color=red] (Y) {$Y$};
			
			%-- A's
			\path (w0) ++(0:12 mm) node [color=red] (A1) {$A_1$};	
			\path (w0) ++(-60:12 mm) node [color=red] (A2) {$A_2$};
			
			%-- B's	
			\path (w0) ++(-60:-14 mm) node [color=red] (B1) {$B_1$};	
			\path (w0) ++(180:13 mm) node [color=red] (B2) {$B_2$};
			
			%-- D's
			\path (w2) ++(-10:15mm) node [color=red] (D1) {$D_1$};	
			\path (v) ++(280:10 mm) node [color=red] (D2) {$D_2$};
			\path (w4) ++(-25:15 mm) node [color=red] (D3) {$D_3$};
			
		\end{tikzpicture} 
		\caption{The complement of the graph $G$ from Figure  \ref{fig:c:thet334}: a graph $\cp{G}$ such that $\ig{G} = \thet{3,3,4}$.}
		\label{fig:c:thet334comp}
	\end{figure}		
	
	
	%______________________  SUBSUB SECTION:  theta (3,3,5) ______________________
	\subsubsection{Construction of $\cp{G}$ for $\thet{3,3,5}$}  \label{subsubsec:c:335}
	
	
	%>>> S: Cons {con:c:thet335}
	\begin{cons} \label{con:c:thet335}
		Refer to  Figure \ref{fig:c:thet335}.	Begin with a copy of the graph $\cp{H} \cong W_7 = C_6 \vee K_1$, labelling the degree 3 vertices as $w_1,w_2,\dots, w_6$ and the central degree 6 vertex as $w_0$.     Add new vertices $v_1$ and $v_2$ to $\cp{H}$, joined to each other.  Then, join $v_1$ to each of $\{w_1,w_2,w_5\}$, and $v_2$ to each of $\{w_2, w_4,w_5\}$.  Call this graph $\cp{G_{3,3,5}}$.
	\end{cons}
	% <<< E: Cons {con:c:thet335}
	
	
	%>>> S: Figure {fig:c:thet335}	
	\begin{figure}[H] \centering	
		\begin{tikzpicture}	
			%---------- REF-------------------
			\node (cent) at (0,0) {};
			\path (cent) ++(0:40 mm) node (rcent) {};	
			
			%----Left Wheel
			\node[std,label={0:$w_0$}] (w0) at (cent) {};
			
			\foreach \i in {1,2,3,4,5,6}
			{
				\node[std,label={150-\i*60: $w_{\i}$}] (w\i) at (150-\i*60:2cm) {}; 
				\draw[thick] (w0)--(w\i);        
			}
			\draw[thick] (w1)--(w2)--(w3)--(w4)--(w5)--(w6)--(w1);
			
			%---- V-Path	
			%\foreach \i in {1,2}
			\foreach \i/\j in {1/1.7, 2/-0.5}
			{
				%\node[bblue,label={[blue]0: $v_\i$}] (v\i) at (4,3.5-2*\i) {};
				\path (rcent) ++(90:\j cm) node [bblue,label={[blue]0: $v_\i$}] (v\i) {};
				%\path (v\i) ++(0:4 mm) node (Lv\i) {\color{blue} $v_{\i}$};		
			}	
			
			\draw[bline] (w1)--(v1)--(v2)--(w2)--(v1);
			
			%---- V2 to W4-Path
			\draw[bline] (v2) to[out=230,in=0] (w4);  	
			
			%-- V2 to W5
			%\node[std] (v2w5A) at (-60:3.5cm) {};
			%\node[std] (v2w5B) at  (-60:4cm){};
			\draw[bline] (v2) to [out=260,in=15]  (-60:3.5cm) to [out=195,in=270] (w5);  
			
			%--- V1 to W5		
			%\node[std] (v1w5A) at (-15:5cm){};
			%\node[std] (v1w5B) at  (-60:4cm){};
			\draw[bline] (v1) to [out=-45, in=70]  (-15:5cm) to [out=250,in=15]  (-60:4cm) to[out=195,in=260] (w5); 
			
			%----- Internal Red Labellings	
			\path (w0) ++(60:12 mm) node [color=red] (X) {$X$};			
			\path (w0) ++(60:-12 mm) node [color=red] (Y) {$Y$};
			
			%-- A's
			\path (w0) ++(0:12 mm) node [color=red] (A1) {$A_1$};	
			\path (w0) ++(-60:12 mm) node [color=red] (A2) {$A_2$};
			
			%-- B's	
			\path (w0) ++(-60:-12 mm) node [color=red] (B1) {$B_1$};	
			\path (w0) ++(180:12 mm) node [color=red] (B2) {$B_2$};
			
			%-- D's
			\path (w2) ++(100:5 mm) node [color=red] (D1) {$D_1$};	
			\path (w2) ++(-10:15mm) node [color=red] (D2) {$D_2$};	
			\path (v2) ++(280:10 mm) node [color=red] (D3) {$D_3$};
			\path (w4) ++(-25:15 mm) node [color=red] (D4) {$D_4$};	
			
		\end{tikzpicture} 
		\caption{A graph $\cp{G_{3,3,5}}$ from Construction \ref{con:c:thet335} such that $\ig{G_{3,3,5}} =$ $\thet{3,3,5}$.}
		\label{fig:c:thet335}
	\end{figure}		
	% <<< E: Figure {fig:c:thet335}
	
	
	\newpage
	
	%>>>S: Lemma {lem:c:thet335}
	\begin{lemma}\label{lem:c:thet335}
		If $\cp{G_{3,3,5}}$ is the graph constructed by Construction \ref{con:c:thet335}, then $\ig{G_{3,3,5}} = \ag{G_{3,3,5}} = \thet{3,3,5}$.
	\end{lemma}
	
	
	\begin{proof}	
		From Lemma \ref{lem:c:wheel}, the wheel $\mathcal{W} = \{w_0,w_1,\dots,w_6\}$ in $\cp{G}$ forms a cycle $C_6$ with vertices $\{X,A_1,A_2,Y,B_1,B_2\}$  in $\ig{G}$.	We need only check that in $\ig{G}$, $\mathcal{D}=\{D_1,D_2,D_3,D_4\}$ (where each $D_i$ is defined as in Figure \ref{fig:c:thet335}) forms the necessary third disjoint path between $X$ and $Y$.  As discussed above, we need not concern ourselves over whether there are additional triangles of $\cp{G}$ (and hence vertices of $\ig{G}$)  present beyond the ten labelled in red in Figure \ref{fig:c:thet335}: they can easily be removed via the Deletion Lemma if needed. 
		
		From Figure \ref{fig:c:thet335}, we have that
		\begin{align*}
			\edge{X, w_0,  v_1,D_1}  \adedge{w_1,v_2,D_2} \adedge{w_2,w_5,D_3}   \adedge{v_1,w_4,D_4}  \adedge{v_2,w_0,Y},
		\end{align*}
		which forms the additional path between $X$ and $Y$ in $\ig{G}$.  Since $D_2$ and $D_3$ both contain $v_1$ and $v_2$, of the four triangles in $\mathcal{D}$, only $D_1$ and $D_4$ contain at least two of the wheel vertices from $\mathcal{W}$.  Thus, only $D_1$ and $D_2$ are adjacent to wheel triangles, namely $X$ and $Y$, respectively.  It follows that there are no additional edges between the vertices of $\mathcal{D}$ in $\ig{G}$.  
		We conclude that $\ig{\cp{G}}= \thet{3,3,5}$. 		
	\end{proof}
	% <<< E: Lemma {lem:c:thet335}
	
	
	
	
	
	
	
	
	%______________________  SUBSUB SECTION:  theta (3,3,k) ______________________
	
	\subsubsection{Construction of $\cp{G}$ for $\thet{3,3,\ell}$ for $\ell \geq 6$}  \label{subsubsec:c:33k}
	
	
	
	%>>> S: Cons {con:c:thet33k}
	\begin{cons} \label{con:c:thet33k}
		Refer to Figure \ref{fig:c:thet33k}.	Begin with a copy of the graph $\cp{H} \cong W_7 = C_6 \vee K_1$, labelling the degree 3 vertices as $w_1,w_2,\dots, w_6$ and the central degree 4 vertex as $w_0$.     For $\ell \geq 6$, add to $\cp{H}$  a new path of $\ell-3$ vertices labelled as $v_1$, $v_2, \dots, v_{\ell-3}$.  Then, join $w_1$ to each of $\{v_1,v_2,\dots, v_{\ell-4}\}$, $w_4$ to $v_{\ell-3}$, and $w_5$ to $v_{\ell-4}$ and $v_{\ell-3}$.  Finally, join $v_{\ell-5}$ to $v_{\ell-3}$, so that $\{v_{\ell-5}, v_{\ell-4}, v_{\ell-3}\}$ form a  $K_3$.  
		Call this graph $\cp{G_{3,3,\ell}}$ for $\ell \geq 6$.
	\end{cons}
	% <<< E: Cons {con:c:thet33k}
	
	
	Although the general construction still applies for the case when $\ell=6$, we include a separate figure for the construction of $\thet{3,3,6}$ for reference below, because of the additional complication that now $v_1 = v_{\ell-5}$, and so the single vertex now has dual roles in the construction.
	
	
	%>>> S: Figure {fig:c:thet336}	
	\begin{figure}[H] \centering	
		\begin{tikzpicture}	
			
			%---------- REF-------------------
			\node (cent) at (0,0) {};
			\path (cent) ++(0:40 mm) node (rcent) {};	
			
			%----Left Wheel
			\node[std,label={0:$w_0$}] (w0) at (cent) {};
			
			\foreach \i in {1,2,3,4,5,6}
			{
				\node[std,label={150-\i*60: $w_{\i}$}] (w\i) at (150-\i*60:2cm) {}; 
				\draw[thick] (w0)--(w\i);        
			}
			\draw[thick] (w1)--(w2)--(w3)--(w4)--(w5)--(w6)--(w1);
			
			%---- V-Path	
			\foreach \i / \j in {1/1.5,2/0,3/-1.5}
			{	
				\path (rcent) ++(90:\j cm) node [bblue] (v\i) {};
				\path (v\i) ++(0:4 mm) node (Lv\i) {\color{blue} $v_{\i}$};
				%\node[bblue,label={0: $v_\i$}] (v\i) at (4,2-\i) {};
			}
			\draw[bline] (w1)--(v1)--(v2)--(v3)--(w4);
			\draw[bline] (w2)--(v1);
			
			%---- V1 to V3 
			\draw[bline] (v1) to[out=210,in=150] (v3);  	
			
			%-- V3 to W5
			\draw[bline] (v3) to[out=230,in=290] (w5);  
			
			%--- V2 to W5 and W1
			\draw[bline] (v2) to[out=-45, in=90]  (-15:4.9cm) to [out=270,in=0]  (-60:3.5cm) to[out=180,in=260] (w5); 
			\draw[bline] (v2) to[out=45, in=-90]  (15:4.9cm) to [out=-270,in=0]  (45:3.5cm) to[out=-180,in=20] (w1);	
			
			%----- Internal Red Labellings	
			\path (w0) ++(60:12 mm) node [color=red] (X) {$X$};			
			\path (w0) ++(60:-12 mm) node [color=red] (Y) {$Y$};
			
			%-- A's
			\path (w0) ++(0:12 mm) node [color=red] (A1) {$A_1$};	
			\path (w0) ++(-60:12 mm) node [color=red] (A2) {$A_2$};
			
			%-- B's	
			\path (w0) ++(-60:-12 mm) node [color=red] (B1) {$B_1$};	
			\path (w0) ++(180:12 mm) node [color=red] (B2) {$B_2$};
			
			%-- D's
			\path (w2) ++(100:5 mm) node [color=red] (D1) {$D_1$};	
			\path (v1) ++(140:9 mm) node [color=red] (D2) {$D_2$};	
			\path (v2) ++(180:5 mm) node [color=red] (D3) {$D_3$};
			\path (v3) ++(270:6 mm) node [color=red] (D4) {$D_4$};
			\path (w4) ++(-10:15 mm) node [color=red] (D5) {$D_5$};		
			
		\end{tikzpicture} 
		\caption{The graph $\cp{G_{3,3,6}}$ from Construction \ref{con:c:thet33k} such that $\ig{G_{3,3,6}} =  \ag{G_{3,3,6}}= \thet{3,3,6}$.}
		\label{fig:c:thet336}
	\end{figure}	
	% <<< E: Figure {fig:c:thet336}
	
	
	
	
	%>>> S: Figure {fig:c:thet33k}	
	%$\thet{3,3,k}$
	\begin{figure}[H] \centering	
		\begin{tikzpicture}	
			%---------- REF-------------------
			\node (cent) at (0,0) {};
			\path (cent) ++(0:45 mm) node (rcent) {};	
			
			%----Left Wheel
			\node[std,label={0:$w_0$}] (w0) at (cent) {};
			
			\foreach \i in {1,3,4,5,6}
			{
				\node[std,label={150-\i*60: $w_{\i}$}] (w\i) at (150-\i*60:2cm) {}; 
				\draw[thick] (w0)--(w\i);        
			}
			\node[std,label={0: $w_{2}$}] (w2) at (30:2cm) {}; 
			\draw[thick] (w0)--(w2);        
			
			\draw[thick] (w1)--(w2)--(w3)--(w4)--(w5)--(w6)--(w1);
			
			%---- V-Path	
			\foreach \i / \j  / \k in {1/3/1, 2/2/2, 3/-1/{\ell-5}, 4/-2.2/{\ell-4}, 5/-3.4/{\ell-3}}
			{	
				\path (rcent) ++(90:\j cm) node [bblue] (v\i) {};
				\path (v\i) ++(0:5 mm) node (Lv\i) {\color{blue} $v_{\k}$};
				%\node[bblue,label={0: $v_\i$}] (v\i) at (4,2-\i) {};
			}
			
			\draw[bline] (v1)--(v2);
			\draw[bline] (v3)--(v4)--(v5);
			
			\draw[bline,dashed] (v2)--(v3);
			
			%---- V3 to V5 
			\path (v4) ++(180:1.3 cm) coordinate  (c1) {};
			\draw[bline] (v3) to[out=190, in=90]  (c1) to [out=270,in=170] (v5);  
			
			%---- V1 to W1 W2
			\draw[bline] (w1)--(v1)--(w2);	
			
			%-- V5 to W4
			\draw[bline] (v5) to[out=180,in=-45] (w4);  
			
			%-- V5 to W5
			\draw[bline] (v5) to[out=200,in=290] (w5);  
			
			%-- V4 to W5
			\draw[bline] (v4) to[out=-35, in=25]  (4.6cm,-4.2cm) to [out=205,in=270] (w5);  	
			%	\node[std] at (4.6cm,-4.2cm) {};
			
			%-- W1 to V2  
			\draw[bline] (w1) to[out=30, in=170]  (35:6.1cm) to [out=350,in=45]  (v2); 
			%	\node[std] at (35:6.2cm)  {};
			
			%-- W1 to  V3 
			\draw[bline] (w1) to[out=38, in=170]  (35:6.4cm) to [out=350,in=45]  (v3); 
			%\node[std] at (30:5.8cm) {};
			
			%-- W1 to V4
			\draw[bline] (w1) to[out=46, in=170]  (35:6.6cm) to [out=350,in=40]  (v4); 
			%\node[std] at (30:5.8cm) {};
			
			%-- W1 to Dashed T1 T2
			\path (rcent) ++(90:1 cm) coordinate  (t1) {};
			\draw[bline, dashed] (w1) to[out=32, in=170]   (35:6.2cm)  to [out=350,in=45]  (t1); 
			
			\path (rcent) ++(90:0 cm) coordinate  (t2) {};
			\draw[bline, dashed] (w1) to[out=34, in=170]  (35:6.3cm) to [out=350,in=45]  (t2); 
			
			%----- Internal Red Labellings	
			\path (w0) ++(60:12 mm) node [color=red] (X) {$X$};			
			\path (w0) ++(60:-12 mm) node [color=red] (Y) {$Y$};
			
			%-- A's
			\path (w0) ++(0:12 mm) node [color=red] (A1) {$A_1$};	
			\path (w0) ++(-60:12 mm) node [color=red] (A2) {$A_2$};
			
			%-- B's	
			\path (w0) ++(-60:-12 mm) node [color=red] (B1) {$B_1$};	
			\path (w0) ++(180:12 mm) node [color=red] (B2) {$B_2$};
			
			%-- D's
			\path (w2) ++(105:8 mm) node [color=red] (D1) {$D_1$};	
			\path (v1) ++(170:9 mm) node [color=red] (D2) {$D_2$};	
			\path (v4) ++(160:7 mm) node [color=red] (D3) {$D_{\ell-3}$};
			\path (w4) ++(-55:25mm) node [color=red] (D4) {$D_{\ell-2}$};
			\path (w4) ++(-50:15 mm) node [color=red] (D5) {$D_{\ell-1}$};		
			
		\end{tikzpicture} 
		\caption{The graph $\cp{G_{3,3,\ell}}$ from Construction \ref{con:c:thet33k} such that $\ig{G} = \ag{G} = \thet{3,3,\ell}$ for $\ell \geq 6$.}
		\label{fig:c:thet33k}
	\end{figure}	
	% <<< E: Figure {fig:c:thet33k}
	
	
	
	
	%>>>S: Lemma {lem:c:thet33k}
	\begin{lemma}\label{lem:c:thet33k}
		If $\cp{G_{3,3,\ell}}$ is the graph constructed by Construction \ref{con:c:thet33k}, then $\ig{G_{3,3,\ell}} = \ag{G_{3,3,\ell}} = \thet{3,3,\ell}$ for $\ell \geq 6$.
	\end{lemma}
	
	
	\begin{proof}
		We proceed as in the proof of Lemma \ref{lem:c:thet335} for $\thet{3,3,5}$, labelling the triangles as in Figure \ref{fig:c:thet33k}, with the amendment that we now ensure that $\mathcal{D}=\{D_1,D_2,\dots,D_{\ell-1}\}$ forms the necessary third disjoint path between $X$ and $Y$ in $\ig{\cp{G}}$.
		
		Clearly from Figure \ref{fig:c:thet33k},
		\begin{align*}
			\edge{X, w_0,  v_1,D_1}  \adedge{w_2,v_2,D_2} \adedge{v_1,v_3,D_3}\onlyTilde{v_2,v_4} \dots
			\adedge{v_{\ell-6},v_{\ell-4},D_{\ell-4}} 
			\adedge{w_1,v_{\ell-3},D_{\ell-3}} 
			\adedge{v_{\ell-5},w_5,D_{\ell-2}}  
			\adedge{v_{\ell-4},w_4,D_{\ell-1}}
			\adedge{v_{\ell-3},w_0,Y},
		\end{align*}
		where $\edge{D_i, v_{i-1}, v_{i+1}, D_{i+1}}$ 	for $ 3 \leq i \leq \ell-5$.
		
		Similarly to  before, of the triangles in $\mathcal{D}$, only $D_1$ and $D_{\ell-1}$ contain at least two of the wheel vertices from $\mathcal{W}$, and so only $D_1$ and $D_{\ell-1}$  are adjacent to wheel triangles. 
		We may assume that each $i$-set of $\cp{G}$ corresponds to  a facial triangle of $G$; if this is not the case, then as previously observed, we can use the Deletion Lemma (Lemma \ref{lem:i:inducedI}) to remove any non-facial triangle $i$-sets from the construction.  Thus, a vertex of $\ig{G}$ corresponding to a triangle $D_i$ of $\cp{G}$  is adjacent to at most three others.
		
		For $i=2,3,\dots,\ell-5$, we have already seen that $\edge{D_{i-1},v_{i-2},v_i, D_i}\adedge{ v_{i-1}, v_{i+1}, D_{i+1}}$.  If $D_i$ were adjacent to a third facial triangle, it would be to a triangle sharing the edge  $v_{i-1}v_i \in E(\cp{G})$; however, $N_{\cp{G}}(\{v_{i-1},v_i\})	= \{w_1\}$ and since $D_i = \{w_1, v_{i-1},v_i\}$, no such third triangle exists.  Thus, we need only check that for $i\in\{1,\ell-4,\ell-3,\ell-2,\ell-1\}$,  $\deg_{\cp{G}}(D_i)=2$.  For these cases, it is not overly arduous to exhaustively check that the edges $v_1w_2$, $w_1v_{\ell-4}$, $v_{\ell-5}v_{\ell-3}$, $v_{\ell-4}w_5$, and $v_{\ell-3}w_4$, respectively, are incident with exactly one triangle in $\cp{G}$.
		It follows that in $\ig{G}$, $X,D_1, D_2, \dots, D_{\ell-2}, D_{\ell-1},Y$ forms a path of length $\ell$ from $X$ to $Y$, and hence that $\ig{G}=\thet{3,3,\ell}$.		
	\end{proof}
	
	
	% <<< E: Lemma {lem:c:thet33k}
	
	
	
	
	
	
	The proofs of the remaining lemmas in Section \ref{sec:c:thetaComp} are all similar to proofs of previous lemmas and are therefore omitted without further comments.
	
	
	
	
	
	
	%______________________  SUBSUB SECTION:  theta (3,4,4) ______________________
	\subsubsection{Construction of $\cp{G}$ for $\thet{3,4,4}$ }  \label{subsubsec:c:344}
	
	
	
	%\nts{PLACEHOLDER}
	%>>> S: Cons {con:c:thet344}
	\begin{cons}\label{con:c:thet344} See Figure \ref{fig:c:thet344}.	
		Begin with a copy of the graph $\cp{G}$ from Construction \ref{con:c:thet244}   for $\thet{2,4,4}$, which we rename here as $\cp{G_{2,4,4}}$.  Subdivide the edge $w_2w_3$, adding a new vertex $u_1$, and joining $u_1$ to $w_0$.  
		Delete the vertex $z$.   Call this graph $\cp{G_{3,4,4}}$.
		
		%Then, for each $3 \leq i \leq 6$,  relabel the vertices of the outter wheel from $w_i$ to $w_{i+1}$, and relabel $w^*$ as $w_3$.
		
		
		
	\end{cons}
	% <<< E: Cons {con:c:thet344}
	
	
	
	
	
	%>>> S: Figure {fig:c:thet344}	
	\begin{figure}[H] \centering	
		\begin{tikzpicture}	
			
			%---------- REF-------------------
			\node (cent) at (0,0) {};
			\path (cent) ++(0:50mm) node (rcent) {};	
			
			%----Left Wheel
			\node[std] (w0) at (cent) {};
			\path (w0) ++(55:6 mm) node (Lw0) {$w_0$};	
			
			\foreach \i in {1,2,3,4,5,6}
			{
				\node[std,label={150-\i*60: $w_{\i}$}] (w\i) at (150-\i*60:2cm) {}; 
				\draw[thick] (w0)--(w\i);        
			}
			
			\node[std,label={0: $u_1$}] (w) at (0:2cm) {}; 
			\draw[thick] (w0)--(w);
			
			\draw[thick] (w1)--(w2)--(w)--(w3)--(w4)--(w5)--(w6)--(w1);
			
			%---- V-Path
			
			\path (rcent) ++(90:0 cm) node [bblue] (v) {};
			\path (v) ++(0:4 mm) node (Lv) {\color{blue} $v$};	
			
			\foreach \i / \j in {2,3}
			\draw[bline] (v)--(w\i);	
			
			%--- W1 to V
			\draw[bline] (w1)   to[out=0,in=100] (v); 	
			%--- W4 to V
			\draw[bline] (w4)   to[out=0,in=-100] (v); 
			%--- W4 to W1
			\draw[bline] (w4) to[out=-15, in=270]  (0:6.5cm)  to[out=90,in=15] (w1); 	
			
			
			%\path (w0) ++(60:-3 cm) node [bred, label={[red]180:$z'$}] (z1) {};
			\path (w0) ++(180:4 cm) node [bzed, label={[zelim]180:$\boldsymbol{z'}$}] (z1) {};
			%	\draw[rline] (z1)--(w0);
			\draw[zline] (w0)   to[out=165,in=15] (z1); 
			\draw[zline] (w1)   to[out=180,in=80] (z1); 		
			\draw[zline] (w4)   to[out=180,in=-80] (z1); 
			
			
			%----- Internal Red Labellings	
			\path (w0) ++(60:12 mm) node [color=red] (X) {$X$};	
			\path (w0) ++(15:12 mm) node [color=red] (A1) {$A_1$};	
			\path (w0) ++(-15:12 mm) node [color=red] (A2) {$A_2$};	
			\path (w0) ++(-60:12 mm) node [color=red] (Y) {$Y$};	
			
			%-- B's	
			\foreach \i/\c in {1/120,2/180,3/240} {				
				\path (w0) ++(\c:12 mm) node [color=red] (B\i) {$B_{\i}$};	
			}
			
			%-- D's
			\path (w2) ++(05:15 mm) node [color=red] (D1) {$D_1$};	
			\path (v) ++(60:8 mm) node [color=red] (D2) {$D_2$};	
			\path (w3) ++(-05:15 mm) node [color=red] (D3) {$D_3$};
			
		\end{tikzpicture} 
		\caption{The   graph  \; $\cp{G_{3,4,4}}$ \;  from    Construction   \ref{con:c:thet344}    such    that    $\ig{G_{3,4,4}}$    $=$  $\thet{3,4,4}$.}
		\label{fig:c:thet344}
	\end{figure}		
	% <<< E: Figure {fig:c:thet344}
	
	
	
	%>>>S: Lemma {lem:c:thet344}
	\begin{lemma}\label{lem:c:thet344}
		If $\cp{G_{3,4,4}}$ is the graph constructed by Construction \ref{con:c:thet344}, then $\ig{G_{3,4,4}} = \thet{3,4,4}$.
	\end{lemma}
	%>>>E: Lemma {lem:c:thet344}
	
	
	%______________________  SUBSUB SECTION:  theta (3,4,l) ______________________
	\subsubsection{Construction of $\cp{G}$ for $\thet{3,4,\ell}$, $\ell \geq 5$}  \label{subsubsec:c:34l}
	
	
	%\nts{SUBDIVISION of 344 on B-line}
	
	
	
	%>>> S: Cons {con:c:thet34k}
	\begin{cons}\label{cons:c:thet34k} 
		Begin with a copy of the graph $\cp{G_{3,4,4}}$ from Construction \ref{con:c:thet344} for $\thet{3,4,4}$.  Subdivide the edge $w_1w_6$ $\ell-4$ times (for $\ell \geq 5$), adding the new vertices $w_7$, $w_8, \dots, w_{\ell+2}$.  Join $w_7, w_8, \dots, w_{\ell+2}$ to $w_0$, so that $w_0,w_1,\dots,w_{\ell+2}$ forms a wheel.  Call this graph $\cp{G_{3,4,\ell}}$. 
	\end{cons}
	% <<< E: Cons {con:c:thet34k}
	
	%>>>S: Lemma {lem:c:thet34k}
	\begin{lemma}\label{lem:c:thet34k}
		If $\cp{G_{3,4,\ell}}$ is the graph constructed by Construction \ref{cons:c:thet34k}, then $\ig{G_{3,4,\ell}} = \thet{3,4,\ell}$ for $\ell \geq 5$.
	\end{lemma}
	%>>>E: Lemma {lem:c:thet34k}
	
	%______________________  SUBSUB SECTION:  theta (3,5,5) ______________________
	\subsubsection{Construction of $\cp{G}$ for $\thet{3,5,5}$}  \label{subsubsec:c:355}
	
	
	%\nts{SUBDIVISION of 335 twice on B-line}
	
	
	
	%>>> S: Cons {con:c:thet355}
	\begin{cons} \label{con:c:thet355}
		Refer to  Figure \ref{fig:c:thet355}.	
		Begin with a copy of the graph $\cp{G_{3,3,5}}$ from  Construction \ref{con:c:thet335}.
		Subdivide the edge $w_1w_6$ twice, adding the new vertices $w_7$ and  $w_8$.  Join $w_7$ and $w_8$ to $w_0$, so that $w_0,w_1,\dots,w_{8}$ forms a wheel.  Call this graph $\cp{G_{3,5,5}}$.
	\end{cons}
	% <<< E: Cons {con:c:thet355}
	
	
	%>>> S: Figure {fig:c:thet355}	
	\begin{figure}[H] \centering	
		\begin{tikzpicture}	
			%---------- REF-------------------
			\node (cent) at (0,0) {};
			\path (cent) ++(0:40 mm) node (rcent) {};	
			
			%----Left Wheel
			\node[std,label={0:$w_0$}] (w0) at (cent) {};
			
			\foreach \i in {1,2,3,4,5}
			{
				\node[std,label={150-\i*60: $w_{\i}$}] (w\i) at (150-\i*60:2cm) {}; 
				\draw[thick] (w0)--(w\i);        
			}
			
			\foreach \i in {6,7,8}
			{
				\node[std,label={360-\i*30: $w_{\i}$}] (w\i) at (360-\i*30:2cm) {}; 
				\draw[thick] (w0)--(w\i);   
			}
			
			\draw[thick] (w1)--(w2)--(w3)--(w4)--(w5)--(w6)--(w7)--(w8)--(w1);
			
			%---- V-Path	
			%\foreach \i in {1,2}
			\foreach \i/\j in {1/1.7, 2/-0.5}
			{
				%\node[bblue,label={[blue]0: $v_\i$}] (v\i) at (4,3.5-2*\i) {};
				\path (rcent) ++(90:\j cm) node [bblue,label={[blue]0: $v_\i$}] (v\i) {};
				%\path (v\i) ++(0:4 mm) node (Lv\i) {\color{blue} $v_{\i}$};		
			}	
			
			\draw[bline] (w1)--(v1)--(v2)--(w2)--(v1);
			
			%---- V2 to W4-Path
			\draw[bline] (v2) to[out=230,in=0] (w4);  	
			
			%-- V2 to W5
			%\node[std] (v2w5A) at (-60:3.5cm) {};
			%\node[std] (v2w5B) at  (-60:4cm){};
			\draw[bline] (v2) to [out=260,in=15]  (-60:3.5cm) to [out=195,in=270] (w5);  
			
			%--- V1 to W5		
			%\node[std] (v1w5A) at (-15:5cm){};
			%\node[std] (v1w5B) at  (-60:4cm){};
			\draw[bline] (v1) to [out=-45, in=70]  (-15:5cm) to [out=250,in=15]  (-60:4cm) to[out=195,in=260] (w5); 
			
			%----- Internal Red Labellings	
			\path (w0) ++(60:12 mm) node [color=red] (X) {$X$};			
			\path (w0) ++(60:-12 mm) node [color=red] (Y) {$Y$};
			
			%-- A's
			\path (w0) ++(0:12 mm) node [color=red] (A1) {$A_1$};	
			\path (w0) ++(-60:12 mm) node [color=red] (A2) {$A_2$};
			
			%-- B's	
			\path (w0) ++(105:12 mm) node [color=red] (B1) {$B_1$};	
			\path (w0) ++(135:12 mm) node [color=red] (B2) {$B_2$};
			\path (w0) ++(165:12 mm) node [color=red] (B2) {$B_3$};
			\path (w0) ++(195:12 mm) node [color=red] (B2) {$B_4$};
			
			%-- D's
			\path (w2) ++(100:5 mm) node [color=red] (D1) {$D_1$};	
			\path (w2) ++(-10:15mm) node [color=red] (D2) {$D_2$};	
			\path (v2) ++(280:10 mm) node [color=red] (D3) {$D_3$};
			\path (w4) ++(-25:15 mm) node [color=red] (D4) {$D_4$};	
			
		\end{tikzpicture} 
		\caption{A graph $\cp{G_{3,5,5}}$ from Construction \ref{con:c:thet355} such that $\ig{G_{3,5,5}} = \thet{3,5,5}$.}
		\label{fig:c:thet355}
	\end{figure}		
	% <<< E: Figure {fig:c:thet355}
	
	
	%>>>S: Lemma {lem:c:thet355}
	\begin{lemma}\label{lem:c:thet355}
		If $\cp{G_{3,5,5}}$ is the graph constructed by Construction \ref{con:c:thet355}, then $\ig{G_{3,5,5}} = \ag{G_{3,5,5}} =\thet{3,5,5}$.
	\end{lemma}
	%>>>E: Lemma {lem:c:thet355}
	
	
	
	Notice that subdividing only once in Construction \ref{con:c:thet355} (adding only $w_7$ and not $w_8$) gives an alternative  (planar) construction for $\thet{3,4,5}$.
	
	
	
	
	
	
	
	
	
	
	
	
	
	
	
	
	
	%......................  SUB SECTION:  theta (j,k,l) .........................
	\subsection{$\thet{j,k,\ell}$ for $4 \leq j \leq k \leq \ell$ and $3 \leq j \leq k \leq \ell$, $\ell \geq 6$}  \label{subsec:c:jkl}
	
	
	
	
	%______________________  SUBSUB SECTION:  theta (4,k,l) ______________________
	\subsubsection{Construction of $\cp{G}$ for $\thet{j,k,\ell}$ for   $4 \leq j \leq k \leq \ell \leq 5$}  \label{subsubsec:c:4kl}
	
	
	
	
	%>>> S: Cons {con:c:thet444}
	\begin{cons} \label{con:c:thet444}
		Refer to  Figure \ref{fig:c:thet444}.	
		Begin with a copy of the graph $\cp{G_{3,4,4}}$ from  Construction \ref{con:c:thet344}.
		Subdivide the edge $u_1w_3$, adding the new vertex $u_2$.  Join $u_2$ to $w_0$, so that
		\begin{align*}
			w_0,w_1,w_2,u_1,u_2,w_3,\dots,w_{6}
		\end{align*}
		forms a wheel.  Call this graph $\cp{G_{4,4,4}}$.
	\end{cons}
	% <<< E: Cons {con:c:thet444}
	
	
	
	
	%>>> S: Figure {fig:c:thet444}
	\begin{figure}[H] \centering	
		\begin{tikzpicture}	
			
			%---------- REF-------------------
			\node (cent) at (0,0) {};
			\path (cent) ++(0:50mm) node (rcent) {};	
			
			%----Left Wheel
			\node[std] (w0) at (cent) {};
			\path (w0) ++(55:6 mm) node (Lw0) {$w_0$};	
			
			\foreach \i in {1,2,3,4,5,6}
			{
				\node[std,label={150-\i*60: $w_{\i}$}] (w\i) at (150-\i*60:2cm) {}; 
				\draw[thick] (w0)--(w\i);        
			}
			
			\node[std,label={0: $u_1$}] (u1) at (10:2cm) {}; 
			\draw[thick] (w0)--(u1);
			
			
			\node[std,label={0: $u_2$}] (u2) at (-10:2cm) {}; 
			\draw[thick] (w0)--(u2);
			
			
			\draw[thick] (w1)--(w2)--(u1)--(u2)--(w3)--(w4)--(w5)--(w6)--(w1);
			
			%---- V-Path
			
			\path (rcent) ++(90:0 cm) node [bblue] (v) {};
			\path (v) ++(0:4 mm) node (Lv) {\color{blue} $v$};	
			
			\foreach \i / \j in {2,3}
			\draw[bline] (v)--(w\i);	
			
			%--- W1 to V
			\draw[bline] (w1)   to[out=0,in=100] (v); 	
			%--- W4 to V
			\draw[bline] (w4)   to[out=0,in=-100] (v); 
			%--- W4 to W1
			\draw[bline] (w4) to[out=-15, in=270]  (0:6.5cm)  to[out=90,in=15] (w1); 	
			
			
			%\path (w0) ++(60:-3 cm) node [bred, label={[red]180:$z'$}] (z1) {};
			\path (w0) ++(180:4 cm) node [bzed, label={[zelim]180:$\boldsymbol{z'}$}] (z1) {};
			%	\draw[rline] (z1)--(w0);
			\draw[zline] (w0)   to[out=165,in=15] (z1); 
			\draw[zline] (w1)   to[out=180,in=80] (z1); 		
			\draw[zline] (w4)   to[out=180,in=-80] (z1); 
			
			
			%----- Internal Red Labellings	
			\path (w0) ++(60:12 mm) node [color=red] (X) {$X$};	
			\path (w0) ++(20:15 mm) node [color=red] (A1) {$A_1$};	
			\path (w0) ++(0:15 mm) node [color=red] (A2) {$A_2$};	
			\path (w0) ++(-20:15 mm) node [color=red] (A3) {$A_3$};	
			\path (w0) ++(-60:12 mm) node [color=red] (Y) {$Y$};	
			
			%-- B's	
			\foreach \i/\c in {1/120,2/180,3/240} {				
				\path (w0) ++(\c:12 mm) node [color=red] (B\i) {$B_{\i}$};	
			}
			
			%-- D's
			\path (w2) ++(05:15 mm) node [color=red] (D1) {$D_1$};	
			\path (v) ++(60:8 mm) node [color=red] (D2) {$D_2$};	
			\path (w3) ++(-05:15 mm) node [color=red] (D3) {$D_3$};
			
		\end{tikzpicture} 
		\caption{The graph \; $\cp{G_{4,4,4}}$ \; from Construction \ref{con:c:thet444} such that $\ig{G_{4,4,4}}$ $=$ $\thet{4,4,4}$.}
		\label{fig:c:thet444}
	\end{figure}		
	% <<< E: Figure {fig:c:thet444}
	
	
	%>>>S: Lemma {lem:c:thet444}
	\begin{lemma}\label{lem:c:thet444}
		If $\cp{G_{4,4,4}}$ is the graph constructed by Construction \ref{con:c:thet444}, then $\ig{G_{4,4,4}} = \thet{4,4,4}$.
	\end{lemma}
	%>>>E: Lemma {lem:c:thet444}
	
	
	
	
	
	
	%>>> S: Cons {con:c:thetjk5}
	\begin{cons} \label{con:c:thetjk5}
		%Refer to  Figure \ref{fig:c:thetjk5}
		Begin with a copy of the graph $\cp{G_{3,3,5}}$ from  Construction \ref{con:c:thet335}.
		For $k=4$ subdivide the edge $w_1w_6$ once, adding the vertex $w_7$; for $k=5$, subdivide a second time, adding the vertex $w_8$. 
		For $j=4$, subdivide the edge $w_2w_3$, adding the vertex $u_1$; for $j=5$ ($j \leq k$), subdivide a second time, adding the vertex $u_2$.  Connect all new vertices to $w_0$ to form a wheel.
		Call this graph $\cp{G_{j,k,5}}$ for $4 \leq j \leq k \leq 5$.
	\end{cons}
	% <<< E: Cons {con:c:thetjk5}
	
	An example of the construction of $\cp{G_{5,5,5}}$ is given in Figure \ref{fig:c:thet555} below.
	
	
	
	%>>> S: Figure {fig:c:thet555}	
	\begin{figure}[H] \centering	
		\begin{tikzpicture}	
			%---------- REF-------------------
			\node (cent) at (0,0) {};
			\path (cent) ++(0:40 mm) node (rcent) {};	
			
			%----Left Wheel
			\node[std,label={87:$w_0$}] (w0) at (cent) {};
			
			\foreach \i in {1,2,4,5}
			{
				\node[std,label={150-\i*60: $w_{\i}$}] (w\i) at (150-\i*60:2cm) {}; 
				\draw[thick] (w0)--(w\i);        
			}
			
			\foreach \i in {6,7,8}
			{
				\node[std,label={360-\i*30: $w_{\i}$}] (w\i) at (360-\i*30:2cm) {}; 
				\draw[thick] (w0)--(w\i);   
			}
			
			\foreach \i in {1,2}
			{
				\node[std,label={0: $u_{\i}$}] (u\i) at (30-\i*30:2cm) {}; 
				\draw[thick] (w0)--(u\i);   
			}		
			
			\node[std,label={0: $w_{3}$}] (w3) at (300:2cm) {}; 
			\draw[thick] (w0)--(w3);   
			
			
			\draw[thick] (w1)--(w2)--(u1)--(u2)--(w3)--(w4)--(w5)--(w6)--(w7)--(w8)--(w1);
			
			%---- V-Path	
			\foreach \i/\j in {1/1.7, 2/-0.5}
			{
				\path (rcent) ++(90:\j cm) node [bblue,label={[blue]0: $v_\i$}] (v\i) {};
			}	
			
			\draw[bline] (w1)--(v1)--(v2)--(w2)--(v1);
			
			%---- V2 to W4-Path
			\draw[bline] (v2) to[out=230,in=0] (w4);  	
			
			%-- V2 to W5	
			\draw[bline] (v2) to [out=260,in=15]  (-60:3.5cm) to [out=195,in=270] (w5);  
			
			%--- V1 to W5		
			\draw[bline] (v1) to [out=-45, in=70]  (-15:5cm) to [out=250,in=15]  (-60:4cm) to[out=195,in=260] (w5); 
			
			%----- Internal Red Labellings	
			\path (w0) ++(60:12 mm) node [color=red] (X) {$X$};			
			\path (w0) ++(60:-12 mm) node [color=red] (Y) {$Y$};
			
			%-- A's
			\path (w0) ++(15:15 mm) node [color=red] (A1) {$A_1$};	
			\path (w0) ++(-15:15 mm) node [color=red] (A2) {$A_2$};
			\path (w0) ++(-45:15 mm) node [color=red] (A1) {$A_3$};	
			\path (w0) ++(-75:15 mm) node [color=red] (A2) {$A_4$};
			
			%-- B's	
			\path (w0) ++(105:15 mm) node [color=red] (B1) {$B_1$};	
			\path (w0) ++(135:15 mm) node [color=red] (B2) {$B_2$};
			\path (w0) ++(165:15 mm) node [color=red] (B2) {$B_3$};
			\path (w0) ++(195:15 mm) node [color=red] (B2) {$B_4$};
			
			%-- D's
			\path (w2) ++(100:5 mm) node [color=red] (D1) {$D_1$};	
			\path (w2) ++(-10:15mm) node [color=red] (D2) {$D_2$};	
			\path (v2) ++(280:10 mm) node [color=red] (D3) {$D_3$};
			\path (w4) ++(-25:15 mm) node [color=red] (D4) {$D_4$};	
			
		\end{tikzpicture} 
		\caption{A graph $\cp{G_{5,5,5}}$ from Construction \ref{con:c:thet355} such that $\ig{G_{5,5,5}} = \thet{5,5,5}$.}
		\label{fig:c:thet555}
	\end{figure}		
	% <<< E: Figure {fig:c:thet555}
	
	
	
	
	%>>>S: Lemma {lem:c:thetjk5}
	\begin{lemma}\label{lem:c:thetjk5}
		If $\cp{G_{j,k,5}}$ is the graph constructed by Construction \ref{con:c:thetjk5}, then $\ig{G_{j,k,5}} = \ag{G_{j,k,5}} =\thet{j,k,5}$ for $4 \leq j \leq k \leq 5$.
	\end{lemma}
	%>>>E: Lemma {lem:c:thetjk5}
	
	
	
	
	
	
	
	
	
	
	
	
	%______________________  SUBSUB SECTION:  theta (j,k,l) ______________________
	\subsubsection{Construction of $\cp{G}$ for $\thet{j,k,\ell}$ for   $3 \leq j \leq k \leq \ell$, $\ell \geq 6$.}  \label{subsubsec:c:jkl}
	
	
	
	
	%>>> S: Cons {con:c:thetijk}
	\begin{cons} \label{con:c:thetijk}
		%Refer to  Figure \ref{fig:c:thetijk}.	
		Begin with a copy of the graph $\cp{G_{3,3,\ell}}$ from  Construction \ref{con:c:thet33k} for $\thet{3,5,\ell}$ for $\ell \geq 6$.
		For $3 \leq k \leq \ell$, subdivide the edge $w_1w_6$ $k-3$ times, adding the new vertices $w_7, w_8, \dots, w_{k+3}$.  Join each of  $w_7, w_8, \dots, w_{k+3}$  to $w_0$, so that $w_0,w_1,\dots,w_{k+3}$ forms a wheel. 
		Then, for  $3 \leq j \leq k$,  subdivide the edge $w_2w_3$ $j-3$ times, adding the new vertices $u_1, u_2, \dots, u_{j-3}$.  Again, join each  of $u_1, u_2, \dots, u_{j-3}$ to $w_0$ to form a wheel.
		Call this graph $\cp{G_{j,k,\ell}}$ for $3 \leq j \leq k \leq \ell$ and $\ell \geq 6$.
	\end{cons}
	% <<< E: Cons {con:c:thetijk}
	
	
	
	
	
	%>>> S: Figure {fig:c:thet33k}	
	%$\thet{i,k,k}$
	\begin{figure}[H] \centering	
		\begin{tikzpicture}	
			%---------- REF-------------------
			\node (cent) at (0,0) {};
			\path (cent) ++(0:45 mm) node (rcent) {};	
			
			%----Left Wheel
			\node[std,label={85:$w_0$}] (w0) at (cent) {};
			
			%	\foreach \i / \j in {1/1,  4/{k+1},5/{k+2}}
			\foreach \i / \j / \r in {1/1/2,  {4b}/{3}/7, 4/{4}/8, 5/{5}/10, {5b}/{6}/11, {6b}/{k+3}/13}
			{
				\node[std,label={150-\r*30: $w_{\j}$}] (w\i) at (150-\r*30:2cm) {}; 
				\draw[thick] (w0)--(w\i);        
			}
			\node[std,label={0: $w_{2}$}] (w2) at (30:2cm) {}; 
			\draw[thick] (w0)--(w2);       			
			
			%-- cycle insert nodes
			\node[std,label={0: $u_1$}] (w3) at (0:2cm) {}; 
			\draw[thick] (w0)--(w3);     
					
			\node[std,label={-15: $u_{2}$}] (u2) at (-15:2cm) {}; 
			\draw[dashed] (w0)--(u2);        
			
			\node[std,label={-45: $u_{j-3}$}] (uj) at (-45:2cm) {};
			\draw[dashed] (w0)--(uj); 
			
			
			\node[std,label={165: $w_{7}$}] (q1) at (165:2cm) {}; 
			\draw[dashed] (w0)--(q1);        
			
			\node[std,label={135: $w_{k+2}$}] (qk) at (135:2cm) {};
			\draw[dashed] (w0)--(qk); 
						
			
			\draw[thick] (w5)--(w5b)--(q1)--(qk)--(w6b)--(w1);
			
			\draw[thick] (w2)--(w3)--(u2)--(uj)--(w4b)--(w4);
			
			
			\draw[thick] (w1)--(w2);
			\draw[thick] (w4)--(w5);
			
			
			%\draw[thick] (w1)--(w2)--(w3)--(w4)--(w5)--(w6)--(w1);
			
			%---- V-Path	
			\foreach \i / \j  / \k in {1/3/1, 2/2/2, 3/-1/{\ell-5}, 4/-2.2/{\ell-4}, 5/-3.4/{\ell-3}}
			{	
				\path (rcent) ++(90:\j cm) node [bblue] (v\i) {};
				\path (v\i) ++(0:5 mm) node (Lv\i) {\color{blue} $v_{\k}$};
				%\node[bblue,label={0: $v_\i$}] (v\i) at (4,2-\i) {};
			}
			
			\draw[bline] (v1)--(v2);
			\draw[bline] (v3)--(v4)--(v5);
			
			\draw[bline,dashed] (v2)--(v3);
			
			%---- V3 to V5 
			\path (v4) ++(180:1.3 cm) coordinate  (c1) {};
			\draw[bline] (v3) to[out=190, in=90]  (c1) to [out=270,in=170] (v5);  
			
			%---- V1 to W1 W2
			\draw[bline] (w1)--(v1)--(w2);	
			
			%-- V5 to W4
			\draw[bline] (v5) to[out=180,in=-45] (w4);  
			
			%-- V5 to W5
			\draw[bline] (v5) to[out=200,in=290] (w5);  
			
			%-- V4 to W5
			\draw[bline] (v4) to[out=-35, in=25]  (4.6cm,-4.2cm) to [out=205,in=270] (w5);  	
			%	\node[std] at (4.6cm,-4.2cm) {};
			
			%-- W1 to V2  
			\draw[bline] (w1) to[out=30, in=170]  (35:6.1cm) to [out=350,in=45]  (v2); 
			%	\node[std] at (35:6.2cm)  {};
			
			%-- W1 to  V3 
			\draw[bline] (w1) to[out=38, in=170]  (35:6.4cm) to [out=350,in=45]  (v3); 
			%\node[std] at (30:5.8cm) {};
			
			%-- W1 to V4
			\draw[bline] (w1) to[out=46, in=170]  (35:6.6cm) to [out=350,in=40]  (v4); 
			%\node[std] at (30:5.8cm) {};
			
			%-- W1 to Dashed T1 T2
			\path (rcent) ++(90:1 cm) coordinate  (t1) {};
			\draw[bline, dashed] (w1) to[out=32, in=170]   (35:6.2cm)  to [out=350,in=45]  (t1); 
			
			\path (rcent) ++(90:0 cm) coordinate  (t2) {};
			\draw[bline, dashed] (w1) to[out=34, in=170]  (35:6.3cm) to [out=350,in=45]  (t2); 
			
			%----- Internal Red Labellings	
			\path (w0) ++(60:12 mm) node [color=red] (X) {$X$};			
			\path (w0) ++(60:-12 mm) node [color=red] (Y) {$Y$};
			
			%-- A's
			\path (w0) ++(15:12 mm) node [color=red] (A1) {$A_1$};	
			%\path (w0) ++(60:-12 mm) node [color=red] (Y) {$Y$};
			\path (w0) ++(-75:15 mm) node [color=red] (A2) {$A_{j-1}$};
			
			%-- B's	
			\path (w0) ++(-75:-12 mm) node [color=red] (B1) {$B_1$};	
			\path (w0) ++(195:14 mm) node [color=red] (B2) {$B_{k-1}$};
			
			
			%-- D's
			\path (w2) ++(105:8 mm) node [color=red] (D1) {$D_1$};	
			\path (v1) ++(170:9 mm) node [color=red] (D2) {$D_2$};	
			\path (v4) ++(160:7 mm) node [color=red] (D3) {$D_{\ell-3}$};
			\path (w4) ++(-55:25mm) node [color=red] (D4) {$D_{\ell-2}$};
			\path (w4) ++(-50:15 mm) node [color=red] (D5) {$D_{\ell-1}$};		
			
			
			%----- DASH SPLITS
			\coordinate  (c1) at ($(u2)!0.33!(uj)$) {};
			\coordinate  (c2) at ($(u2)!0.66!(uj)$) {};
			
			\draw [dashed] (c2)--(w0);
			\draw [dashed] (c1)--(w0);		
			
			%---	
			\coordinate  (d1) at ($(q1)!0.33!(qk)$) {};
			\coordinate  (d2) at ($(q1)!0.66!(qk)$) {};
			
			\draw [dashed] (d2)--(w0);
			\draw [dashed] (d1)--(w0);				
			
			
		\end{tikzpicture} 
		\caption{The graph $\cp{G_{j,k,\ell}}$ from Construction \ref{con:c:thetijk} such that $\ig{G_{j,k,\ell}} = \thet{j,k,\ell}$ for $3\leq j \leq k \leq \ell$ and $\ell \geq 6$.}
		\label{fig:c:thetijk}
	\end{figure}	
	% <<< E: Figure {fig:c:thetijk}
	
	
	
	%>>>S: Lemma {lem:c:thetjkl}
	\begin{lemma}\label{lem:c:thetjkl}
		If  $\cp{G_{j,k,\ell}}$ for $3 \leq j \leq k \leq \ell$ and $\ell \geq 6$ is the graph constructed by Construction \ref{con:c:thetijk}, then $\ig{G_{j,k,\ell}} = \ag{G_{j,k,\ell}} = \thet{j,k,\ell}$.
	\end{lemma}
	%>>>E: Lemma {lem:c:thetjkl}
	
	
	%\nts{Note here that having shown all of the above lemmas, then we have proven one direction of THeorem 8 (if it is one of these graphs, then it is an i-graph)}
	
	
	
	The lemmas above imply the sufficiency of Theorem \ref{thm:c:thetas}: if a theta graph is not one of seven exceptions listed, then it is an $i$-graph.  In the next section, we complete the proof by examining the exception cases.
	
	
	%From the Lemmas of Section \ref{sec:c:thetaComp}, we have shown one direction of the proof of Theorem \ref{thm:c:thetas}; that is, if a theta graph is one of those constructed in Section \ref{sec:c:thetaComp}, then it is and $i$-graph.  In the next section, we complete the proof by examining the exception case: the seven theta graphs that are not $i$-graphs.
	
	%@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@@ SPLIT TO NON IGRAPHS @@@@@@@@@@@@@@@@@@@@@@@
	
	
	
	
	
	
	
	
	
	
	
	
	
	%---------------------------------------SECTION: Graph Complements ----------------
	\section{Theta Graphs That Are Not $i$-Graphs} \label{sec:c:nonthetas}
	
	
	In this section we show that $\thet{2,2,4}$, $\thet{2,3,3}$, $\thet{2,3,4}$, and $\thet{3,3,3}$ are not $i$-graphs; together with Propositions \ref{prop:i:diamond},  \ref{prop:i:K23}, and \ref{prop:i:kappa}, this completes the proof of Theorem \ref{thm:c:thetas}.
	
	
	
	%______________________  SUBSUB SECTION:  theta (2,2,4) ______________________
	\subsubsection{$\thet{2,2,4}$ Is Not an $i$-Graph}  \label{subsubsec:c:224}
	
	%>>>S: Prop {prop:c:thet224}
	\begin{prop}	\label{prop:c:thet224}
		The graph $\thet{2,2,4}$ is not $i$-graph realizable.
	\end{prop}
	
	%~~~~~~~~~~~~FIG START~~~~~~~~~~~
	\begin{figure}[H]
		\centering
		\begin{tikzpicture}%[line width=0.3mm,le=1]			
			
			%---------- REF-------------------
			\node(cent) at (0,0) {};			
			\path (cent) ++(0:60 mm) node(rcent)  {};		
			
			%----- left C4 ----------	
			\foreach \i/\j/\c in {x/X/90,y/Y/-90} {				
				\path (cent) ++(\c:20 mm) node [std] (v\i) {};
				%\path (v\i) ++(\c:5 mm) node (Lv\i) {${\j}$};
			}
			
			\path (vx) ++(90:5 mm) node (Lvx) {$\color{blue}X=\{x_1,x_2,x_3,\dots, x_k\}$};
			\path (vy) ++(-90:5 mm) node (Lvy) {$\color{blue}Y=\{y_1,y_2,x_3,\dots, x_k\}$};
			
			\foreach \i/\j/\c in {a/A/180,b/B/0} {				
				\path (cent) ++(\c:8 mm) node [std] (v\i) {};
				%\path (v\i) ++(\c:5 mm) node (Lv\i) {${\j}$};
			}
			
			
			%\path (va) ++(180:25 mm) node (Lva) {$A=\{y_1,x_2,x_3,\dots, x_k\}$};
			\path (va) ++(175:20 mm) node (Lvau) {$\color{blue}A=$};
			\path (va) ++(185:20 mm) node (Lvad) {$\color{blue}\{y_1,x_2,x_3,\dots, x_k\}$};
			\path (vb) ++(0:25 mm) node (Lvb) {\color{blue}$B=\{x_1,y_2,x_3,\dots, x_k\}$};
			
			
			\draw[thick] (vx)--(va)--(vy)--(vb)--(vx)--cycle;				
			
			%----- right P4 ----------
			\foreach \i/\c in {1/15,2/0,3/-15} {				
				\path (rcent) ++(90:\c mm) node [std] (c\i) {};
				%\path (c\i) ++(0:5 mm) node (Lc\i) {$C_{\i}$};
			}
			
			\draw[thick] (vx)--(c1)--(c2)--(c3)--(vy);
			
			%\path (cent) ++(-90: 20mm) node (HL)  {$\mathcal{H}$};
			
			\path (c1) ++(0:25 mm) node (Lvc1) {\color{blue}$C_1=\{x_1,x_2,y_3,\dots, x_k\}$};
			%\path (c2) ++(0:25 mm) node (Lvc2) {\color{red}$C_2=\{x_1,x_2,y_3,\dots, x_k\}$};
			%\path (c3) ++(0:25 mm) node (Lvc3) {\color{red}$C_3=\{x_1,x_2,y_3,\dots, x_k\}$};
			\path (c2) ++(0:8 mm) node (Lvc2) {\color{red}$C_2=$};
			\path (Lvc2) ++(0:20 mm) node (Lvc2C) {\color{red} OR };
			\path (Lvc2C) ++(90:5 mm) node (Lvc2A) {\color{red} $\{y_1,x_2,y_3,\dots, x_k\}$};
			\path (Lvc2C) ++(-90:5 mm) node (Lvc2B) {\color{red} $\{x_1,y_2,y_3,\dots, x_k\}$};
			
			\path (c3) ++(0:5 mm) node (Lvc3) {\color{red}$C_3$};
			
			
		\end{tikzpicture}				
		\caption{$H=\thet{2,2,4}$ non-construction.}
		\label{fig:c:thet224}%
	\end{figure}
	
	
	\begin{proof}
		Suppose to the contrary that $\thet{2,2,4}$ is realizable as an $i$-graph, and  that $H = \thet{2,2,4} \cong \ig{G}$ for some graph $G$.  Label the vertices of $H$ as in Figure \ref{fig:c:thet224}.
		
		
		From Proposition \ref{fig:i:C4struct}, and similarly to the proofs of Propositions \ref{prop:i:K23} and \ref{prop:i:kappa}, the composition of the following $i$-sets of $G$ are immediate: 
		
		\begin{align*}
		X&=\{x_1,x_2,x_3,\dots,x_k\},& Y=\{y_1,y_2,x_3,\dots,x_k\}, \\
		A&=\{y_1,x_2,x_3,\dots,x_k\},& B=\{x_1,y_2,x_3,\dots,x_k\}, \\
		C_1&=\{x_1,x_2,y_3,\dots,x_k\} 
		\end{align*}
		
		\noindent
		where $k \geq 3$ and $y_1, y_2, y_3$ are three distinct vertices in $G-X$.  These sets are illustrated in blue in Figure \ref{fig:c:thet224}.  This leaves only the composition of $C_2$ and $C_3$ (in red) to be determined.  
		As we construct $C_2$, notice first that $y_3\in C_2$; otherwise, if say some other $z \in C_2$ so that $\edge{C_1,{y_3},z,C_2}$, then $\edge{X,x_3,z,C_2}$, and $XC_2 \in E(H)$.  Thus, a token on one of $\{x_1,x_2,x_4,\dots,x_k\}$ moves in the transition from $C_1$ to $C_2$.  We consider three cases.
		
		\textbf{Case 1:}  The token on $x_1$ moves.  If $\edge{C_1,{x_1},z,C_2}$ for some $z \notin \{y_1,y_2\}$, then $|C_2 \cap Y |=3$, contradicting the distance requirement between $i$-sets from Observation \ref{obs:i:dist}.    Moreover, from the composition of  $B$, $x_1 \not\sim y_2$, and so  $\edge{C_1,{x_1},y_1,C_2}$, so that $C_2 = \{y_1,x_2,y_3,\dots, x_k\}$.  However, since $x_3 \sim y_3$, we have that $\edge{A,x_3,y_3,C_2}$, so that $AC_2 \in E(G)$, a contradiction.
		
		%Again from the distance requirement, in the two-step transition from $C_2$ to $Y$, tokens are removed from $x_2$ and $y_3$, and tokens are moved to $y_2$ and $x_3$.  If $\edge{C_2,x_2,y_2,C_3}$ so that $C_3=\{y_1,y_2,y_3,\dots, x_k\}$,
		
		\textbf{Case 2:}  The token on $x_2$ moves.  An argument similar to Case 1 constructs $C_2 = \{x_1,y_2,y_3,\dots,x_k\}$, with $\edge{B,x_3,y_3,C_2}$, resulting in the contradiction $BC_2\in E(G)$.
		
		
		\textbf{Case 3:}  The token on $x_i$ for some $i\in \{4,5,\dots,k\}$ moves.	From the compositions of $X$ and $Y$, $x_i$ is not adjacent to any of $\{x_3,y_1,y_2\}$, so the token at $x_i$ moves to some other vertex, say $z$, so that $\edge{C_1,x_i,z,C_2}$ and $\{x_1,x_2,y_3,z\} \subseteq C_2$.  This again contradicts the distance requirement of Observation \ref{obs:i:dist} as $|C_2 \cap Y| = 4$.
		
		
		\noindent In all cases, we fail to construct a graph $G$ with $\ig{G} \cong \thet{2,2,4}$ and so conclude that no such graph exists.		
	\end{proof}
	
	% <<< E: Prop {prop:c:thet224}
	
	
	\newpage
	
	%______________________  SUBSUB SECTION:  theta (2,3,3) ______________________
	\subsubsection{ $\thet{2,3,3}$ Is Not an $i$-Graph} \label{subsubsec:c:233}
	
	
	
	
	%>>>S: Prop {prop:c:thet233}
	\begin{prop}	\label{prop:c:thet233}
		The graph $\thet{2,3,3}$ is not $i$-graph realizable.
	\end{prop}
	
	%~~~~~~~~~~~~FIG START~~~~~~~~~~~
	\begin{figure}[H]
		\centering
		\begin{tikzpicture}%[line width=0.3mm,scale=1]			
			
			%---------- REF-------------------
			\node(cent) at (0,0) {};			
			\path (cent) ++(0:60 mm) node(rcent)  {};		
			
			%----- left C4 ----------	
			\foreach \i/\j/\c in {x/X/90,y/Y/-90} {				
				\path (cent) ++(\c:20 mm) node [std] (v\i) {};
				%\path (v\i) ++(\c:5 mm) node (Lv\i) {${\j}$};
			}
			
			\path (vx) ++(90:5 mm) node (Lvx) {$\color{blue}X=\{x_1,x_2,x_3,\dots, x_k\}$};
			\path (vy) ++(-90:5 mm) node (Lvy) {$\color{red}Y$};
			%\path (vy) ++(-90:5 mm) node (Lvy) {$\color{blue}Y=\{y_1,y_2,x_3,\dots, x_k\}$};
			
			\path (cent) ++(180:8 mm) node [std] (va) {};	
			
			%\path (va) ++(180:25 mm) node (Lva) {$A=\{y_1,x_2,x_3,\dots, x_k\}$};
			\path (va) ++(175:20 mm) node (Lvau) {$\color{blue}A=$};
			\path (va) ++(185:20 mm) node (Lvad) {$\color{blue}\{y_1,x_2,x_3,\dots, x_k\}$};
			
			\draw[thick] (vx)--(va)--(vy);		
			
			
			%------------ B Pathway
			
			\path (cent) ++(0:8 mm) node (vb) {};
			
			\path (vb) ++(90:8 mm) node [std] (vb1) {};
			\path (vb1) ++(0:25 mm) node (Lvb) {\color{blue}$B_1=\{x_1,y_2,x_3,\dots, x_k\}$};
			
			\path (vb) ++(90:-8 mm) node [std] (vb2) {};
			\path (vb2) ++(0:5 mm) node (Lvb) {\color{red}$B_2$};	
			%  \path (vb2) ++(0:25 mm) node (Lvb) {\color{blue}$B_2=\{x_1,y_2,x_3,\dots, x_k\}$};	
			
			\draw[thick](vx)--(vb1)--(vb2)--(vy); 
			
			
			%----- right P4 ----------
			\foreach \i/\c in {1/14,2/-14} {				
				\path (rcent) ++(90:\c mm) node [std] (c\i) {};
				%\path (c\i) ++(0:5 mm) node (Lc\i) {$C_{\i}$};
			}
			
			\draw[thick] (vx)--(c1)--(c2)--(vy);
			
			%\path (cent) ++(-90: 20mm) node (HL)  {$\mathcal{H}$};
			
			\path (c1) ++(0:25 mm) node (Lvc1) {\color{blue}$C_1=\{x_1,x_2,y_3,\dots, x_k\}$};
			%\path (c2) ++(0:25 mm) node (Lvc2) {\color{red}$C_2=\{x_1,x_2,y_3,\dots, x_k\}$};
			%\path (c3) ++(0:25 mm) node (Lvc3) {\color{red}$C_3=\{x_1,x_2,y_3,\dots, x_k\}$};
			\path (c2) ++(0:5 mm) node (Lvc2) {\color{red}$C_2$};
			%	\path (Lvc2) ++(0:20 mm) node (Lvc2C) {\color{red} OR };
			%	\path (Lvc2C) ++(90:5 mm) node (Lvc2A) {\color{red} $\{y_1,x_2,y_3,\dots, x_k\}$};
			%	\path (Lvc2C) ++(-90:5 mm) node (Lvc2B) {\color{red} $\{x_1,y_2,y_3,\dots, x_k\}$};
			
			%	\path (c3) ++(0:5 mm) node (Lvc3) {\color{red}$C_3$};
			
			
		\end{tikzpicture}				
		\caption{$H=\thet{2,3,3}$ non-construction.}
		\label{fig:c:thet233}%
	\end{figure}
	
	
	\begin{proof}
		To begin, we proceed similarly to the proof of Proposition \ref{prop:c:thet224}: suppose to the contrary that $\thet{2,3,3}$ is realizable as an $i$-graph, and  that $H = \thet{2,3,3} \cong \ig{G}$ for some graph $G$.  Label the vertices of $H$ as in Figure \ref{fig:c:thet233}.  As before, the corresponding $i$-sets in blue are established from previous results, and those in red are yet to be determined.
		Moreover, from the composition of these four blue $i$-sets, we observe that for each $i\in \{1,2,3\}$, $x_i \sim y_j$ if and only if $i=j$. 
		
		
		
		Unlike the construction for $\thet{2,2,4}$, we no longer start with knowledge of the exact composition of $Y$.  	
		We proceed with a series of observations on the contents of the various $i$-sets:
		
		\begin{enumerate}[itemsep=1pt, label=(\roman*)]
			\item $y_1 \in Y$, $y_2\in B_2$, and $y_3 \in C_2$  by three applications of  Proposition \ref{prop:i:C4struct}.  \label{prop:c:thet233:a}
			
			\item $y_1 \not\in B_2$ and $y_1 \not\in C_2$.  If $y_1 \in B_2$, then $\edge{B_1,x_1,y_1,B_2}$ (because $A$ shows that $y_1$ is not adjacent to $x_3,\dots,x_k$) so that $B_2  = \{y_1,y_2,x_3,\dots,x_k\}$, and therefore $\edge{A,x_2,y_2,B_2}$, which is impossible.   Similarly, if $y_1 \in C_2$, then $\edge{A, x_3,y_3,C_2}$, which is also impossible.  \label{prop:c:thet233:b}
			
			\item $y_3 \notin B_2$.  Otherwise, $B_2 = \{x_1,y_2,y_3,x_4,\dots,x_k\}$ and so $\edge{C_1,x_2,y_2,B_2}$.  \label{prop:c:thet233:c}
			
			\item $y_2 \not\in Y$ and $y_3\notin Y$.  If $y_2 \in Y$, then  $Y=\{y_1,y_2,x_3,\dots,x_k\}$ and so $\edge{B_1,x_1,y_1,Y}$.	Likewise, if $y_3 \in Y$ then $\edge{C_1,x_1,y_1,Y}$.  \label{prop:c:thet233:d}
			
		\end{enumerate}
		
		
		
		From \ref{prop:c:thet233:a} and \ref{prop:c:thet233:b}, $y_1 \in Y$ but $y_1 \not\in B_2$, and similarly from \ref{prop:c:thet233:d} $y_2 \in B_2$ but $y_2 \not\in Y$; therefore,
		$\edge{B_2,y_2,y_1,Y}$.   Now, since $x_1 \sim y_1$, and $y_1 \in Y$, we have that $x_1 \not\in Y$. Thus, if $x_1$ were in $B_2$, its token would move in the transition from $B_2$ to $Y$.  However,  have already established that it is the token at $y_2$ that moves, and so $x_1 \not\in B_2$.  We conclude that $\edge{B_1,x_1,z,B_2}$ for some $z \not\in \{y_1,y_3\}$, so that $B_2 = \{z,y_2,x_3,\dots,x_k\}$.  Notice that since $B_2$ is independent, and $x_2 \sim y_2$, it follows that $z \neq x_2$.
		
		Using similar arguments, we determine that $\edge{C_2,y_3,y_1,Y}$, and that $\edge{C_1,x_1, w,C_2}$ for some $w\notin \{y_1,y_2,x_1\}$.  Moreover, $C_2=\{w,x_2,y_3,x_4,\dots,x_k\}$.  Again, note that since $x_3 \sim y_3$, $w \neq x_3$.
		
		From $\edge{B_2,y_2,y_1,Y}$, we have that $Y=\{y_1,z,x_3,x_4\dots,x_k\}$.  However, from $\edge{C_2,y_3,y_1,Y}$, we also have that $Y=\{y_1,x_2,w,x_4,\dots,x_k\}$.  As we have already established that $z \neq x_2$ and $w \neq x_3$, we arrive at two contradicting compositions of $Y$.
		Thus, no such graph $G$ exists, and we conclude that $\thet{2,3,3}$ is not an $i$-graph.
	\end{proof}
	
	% <<< E: Prop {prop:c:thet233}
	
	
	
	%______________________  SUBSUB SECTION:  theta (2,3,4) ______________________
	\subsubsection{ $\thet{2,3,4}$ Is Not an $i$-Graph} \label{subsubsec:c:234}
	
	
	
	
	%>>>S: Prop {prop:c:thet234}
	\begin{prop}	\label{prop:c:thet234}
		The graph $\thet{2,3,4}$ is not $i$-graph realizable.
	\end{prop}
	
	%~~~~~~~~~~~~FIG START~~~~~~~~~~~
	\begin{figure}[H]
		\centering
		\begin{tikzpicture}%[line width=0.3mm,scale=1]			
			
			%---------- REF-------------------
			\node(cent) at (0,0) {};			
			\path (cent) ++(0:60 mm) node(rcent)  {};		
			
			%----- left C4 ----------	
			\foreach \i/\j/\c in {x/X/90,y/Y/-90} {				
				\path (cent) ++(\c:20 mm) node [std] (v\i) {};
				%\path (v\i) ++(\c:5 mm) node (Lv\i) {${\j}$};
			}
			
			\path (vx) ++(90:5 mm) node (Lvx) {$\color{blue}X=\{x_1,x_2,x_3,\dots, x_k\}$};
			\path (vy) ++(-90:5 mm) node (Lvy) {$\color{red}Y = \{y_1,z,x_3,\dots, x_k\}$};
			%\path (vy) ++(-90:5 mm) node (Lvy) {$\color{blue}Y=\{y_1,y_2,x_3,\dots, x_k\}$};
			
			\path (cent) ++(180:8 mm) node [std] (va) {};	
			
			
			
			
			%\path (va) ++(180:25 mm) node (Lva) {$A=\{y_1,x_2,x_3,\dots, x_k\}$};
			\path (va) ++(175:20 mm) node (Lvau) {$\color{blue}A=$};
			\path (va) ++(185:20 mm) node (Lvad) {$\color{blue}\{y_1,x_2,x_3,\dots, x_k\}$};
			
			
			
			\draw[thick] (vx)--(va)--(vy);		
			
			
			%------------ B Pathway
			
			\path (cent) ++(0:8 mm) node (vb) {};
			
			\path (vb) ++(90:8 mm) node [std] (vb1) {};
			\path (vb1) ++(0:25 mm) node (Lvb) {\color{blue}$B_1=\{x_1,y_2,x_3,\dots, x_k\}$};
			
			\path (vb) ++(90:-8 mm) node [std] (vb2) {};
			\path (vb2) ++(0:25 mm) node (Lvb) {\color{red}$B_2=\{z, y_2,x_3,\dots, x_k\}$};	
			%  \path (vb2) ++(0:25 mm) node (Lvb) {\color{blue}$B_2=\{x_1,y_2,x_3,\dots, x_k\}$};	
			
			\draw[thick](vx)--(vb1)--(vb2)--(vy); 
			
			
			%----- right P4 ----------
			\foreach \i/\c in {1/15,2/0,3/-15} {				
				\path (rcent) ++(90:\c mm) node [std] (c\i) {};
				%\path (c\i) ++(0:5 mm) node (Lc\i) {$C_{\i}$};
			}
			
			\draw[thick] (vx)--(c1)--(c2)--(c3)--(vy);
			
			%\path (cent) ++(-90: 20mm) node (HL)  {$\mathcal{H}$};
			
			\path (c1) ++(0:25 mm) node (Lvc1) {\color{blue}$C_1=\{x_1,x_2,y_3,\dots, x_k\}$};
			%\path (c2) ++(0:25 mm) node (Lvc2) {\color{red}$C_2=\{x_1,x_2,y_3,\dots, x_k\}$};
			%\path (c3) ++(0:25 mm) node (Lvc3) {\color{red}$C_3=\{x_1,x_2,y_3,\dots, x_k\}$};
			
			%\path (c2) ++(0:28 mm) node (Lvc2) {\color{red}$C_2 = \{w,x_2,y_3,x_4\dots, x_k\}$};
			\path (c2) ++(0:5 mm) node (Lvc2) {\color{red}$C_2$};
			
			%	\path (Lvc2) ++(0:20 mm) node (Lvc2C) {\color{red} OR };
			%	\path (Lvc2C) ++(90:5 mm) node (Lvc2A) {\color{red} $\{y_1,x_2,y_3,\dots, x_k\}$};
			%	\path (Lvc2C) ++(-90:5 mm) node (Lvc2B) {\color{red} $\{x_1,y_2,y_3,\dots, x_k\}$};
			
			\path (c3) ++(0:5 mm) node (Lvc3) {\color{red}$C_3$};
			
			
		\end{tikzpicture}				
		\caption{$H=\thet{2,3,4}$ non-construction.}
		\label{fig:c:thet234}%
	\end{figure}
	
	
	\begin{proof}
		The construction for our contradiction begins similarly to that of $\thet{2,3,3}$ in Proposition \ref{prop:c:thet233}.  As before, we illustrate the graph  in Figure \ref{fig:c:thet234}, labelling the known sets in blue, and those yet to be determined in red.  Given the similarity of $\thet{2,3,3}$ and $\thet{2,3,4}$, many of the observations from Proposition \ref{prop:c:thet233} carry through to our current proof.  In particular, all of \ref{prop:c:thet233:a} - \ref{prop:c:thet233:d} hold here, including that $y_1\notin C_2$ from  \ref{prop:c:thet233:b}.  Moreover, the compositions of $Y$ and $B_2$ also hold, where $z$ is some vertex with $z \not\in \{y_1,x_2,y_2\}$.
		
		We now attempt to build $C_2$.  From Proposition \ref{prop:i:C4struct}, since $X \not\sim C_2$, $y_3 \in C_2$ (and $x_3 \not\in C_2$).  From the distance requirement of Observation \ref{obs:i:dist}, $|X - C_2| \leq 2$, and so at least one of $x_1$ or $x_2$ is in $C_2$.  Recall from the construction for Proposition \ref{prop:c:thet233} that $\edge{A,x_2,z,Y}$ and $\edge{B_1,x_1,z,B_2}$, and so $z$ is adjacent to both $x_1$ and $x_2$.  Hence, $z \not\in C_2$.  
		
		Gathering these results shows that none of $\{x_3,z,y_1\}$ are in $C_2$, and thus, $d(C_2, Y) \geq 3$, contradicting the distance requirement of Observation \ref{obs:i:dist}.  We conclude that no graph $G$ exists such that $\ig{G} = \thet{2,3,4}$.
	\end{proof}
	
	% <<< E: Prop {prop:c:thet234}
	
	
	
	
	
	
	
	
	
	%______________________SUBSUB SECTION:  theta (3,3,3) ______________________
	
	\subsubsection{$\thet{3,3,3}$ Is Not an $i$-Graph}  \label{subsubsec:c:333}
	
	
	%>>>S: Prop {prop:c:thet333}
	\begin{prop}	\label{prop:c:thet333}
		The graph $\thet{3,3,3}$ is not $i$-graph realizable.
	\end{prop}
	
	%~~~~~~~~~~~~FIG START~~~~~~~~~~~
	\begin{figure}[H]
		\centering
		\begin{tikzpicture}%[line width=0.3mm,scale=1]			
			
			%---------- REF-------------------
			\node(cent) at (0,0) {};			
			\path (cent) ++(0:60 mm) node(rcent)  {};		
			
			%----- left C4 ----------	
			\foreach \i/\j/\c in {x/X/90,y/Y/-90} {				
				\path (cent) ++(\c:20 mm) node [std] (v\i) {};
				%\path (v\i) ++(\c:5 mm) node (Lv\i) {${\j}$};
			}
			
			\path (vx) ++(90:5 mm) node (Lvx) {$\color{blue}X=\{x_1,x_2,x_3,\dots, x_k\}$};
			\path (vy) ++(-90:5 mm) node (Lvy) {$\color{red}Y$};
			%\path (vy) ++(-90:5 mm) node (Lvy) {$\color{blue}Y=\{y_1,y_2,x_3,\dots, x_k\}$};
			
			\path (cent) ++(180:8 mm) node (va) {};	
			
			%\path (va) ++(180:25 mm) node (Lva) {$A=\{y_1,x_2,x_3,\dots, x_k\}$};
			
			\path (va) ++(90:8 mm) node [std] (va1) {};
			\path (va1) ++(180:25 mm) node (Lva1) {\color{blue}$A_1=\{y_1,x_2,x_3,\dots, x_k\}$};
			
			\path (va) ++(90:-8 mm) node [std] (va2) {};
			\path (va2) ++(180:5 mm) node (Lva2) {\color{red}$A_2$};	
			
			
			
			\draw[thick] (vx)--(va1)--(va2)--(vy);		
			
			
			%------------ B Pathway
			
			\path (cent) ++(0:8 mm) node (vb) {};
			
			\path (vb) ++(90:8 mm) node [std] (vb1) {};
			\path (vb1) ++(0:25 mm) node (Lvb) {\color{blue}$B_1=\{x_1,y_2,x_3,\dots, x_k\}$};
			
			\path (vb) ++(90:-8 mm) node [std] (vb2) {};
			\path (vb2) ++(0:5 mm) node (Lvb) {\color{red}$B_2$};	
			%  \path (vb2) ++(0:25 mm) node (Lvb) {\color{blue}$B_2=\{x_1,y_2,x_3,\dots, x_k\}$};	
			
			\draw[thick](vx)--(vb1)--(vb2)--(vy); 
			
			
			%----- right P4 ----------
			\foreach \i/\c in {1/14,2/-14} {				
				\path (rcent) ++(90:\c mm) node [std] (c\i) {};
				%\path (c\i) ++(0:5 mm) node (Lc\i) {$C_{\i}$};
			}
			
			\draw[thick] (vx)--(c1)--(c2)--(vy);
			
			%\path (cent) ++(-90: 20mm) node (HL)  {$\mathcal{H}$};
			
			\path (c1) ++(0:25 mm) node (Lvc1) {\color{blue}$C_1=\{x_1,x_2,y_3,\dots, x_k\}$};
			%\path (c2) ++(0:25 mm) node (Lvc2) {\color{red}$C_2=\{x_1,x_2,y_3,\dots, x_k\}$};
			%\path (c3) ++(0:25 mm) node (Lvc3) {\color{red}$C_3=\{x_1,x_2,y_3,\dots, x_k\}$};
			\path (c2) ++(0:5 mm) node (Lvc2) {\color{red}$C_2$};
			
			
			
		\end{tikzpicture}				
		\caption{$H=\thet{3,3,3}$ non-construction.}
		\label{fig:c:thet333}%
	\end{figure}
	
	
	\begin{proof}
		Let $H$ be the theta graph $\thet{3,3,3}$, with vertices labelled as in Figure \ref{fig:c:thet333}.  Suppose to the contrary that there exists some graph $G$ such that $H$ is the $i$-graph of $G$;  that is, $\ig{G} = \thet{3,3,3}$.
		
		%From Observation \ref{obs:i:dist}, since $d_H(X,Y) = 3$, $ 2\leq |X-Y | \leq 3$. We consider the two case for $|X-Y|$ separately.
		
		%\noindent \textbf{Case 1:} $|X-Y|=3$. %Without loss of generality, say $Y=\{y_1,y_2,y_3,x_4,\dots,x_k\}$, where $y_1, y_2, y_3 \not\in V(G)-X$.  
		
		Since $d_H(A_1,Y)=2$,  by Observation  \ref{obs:i:d2}, $|A_1 - Y|=2$.  Similarly, $|B_1-Y|=2$ and $|C_1 - Y|=2$.  
		Suppose that, say, $x_4 \not\in Y$. Hence, by Observation \ref{obs:i:dist} $|\{x_1,x_2,x_3\} \cap Y | \geq 1$.  Without loss of generality, say $x_1 \in Y$.    Then since $y_1 \not\in Y$ and $x_4 \notin Y$, both $x_2$ and $x_3 \in Y$ to satisfy $|A_1 - Y|=2$.  However, then $Y=\{x_1,x_2,x_3,z,x_5,\dots,x_k\}$ for some vertex $z \sim x_4$, and so $\edge{X,x_4,z,Y}$, which is not so.  	
		We therefore conclude that $x_4 \in Y$, and likewise $x_i \in Y$ for $i\geq 4$.  Thus, $\{x_1,x_2,x_3\} \cap Y = \varnothing$.
		
		Returning to $A_1$, since $d(A_1,Y)= 2$ and  $x_2,x_3 \notin Y$,  we have that $y_1 \in Y$.  Similarly, $y_2, y_3 \in Y$.  Thus, $Y=\{y_1,y_2,y_3,x_3,\dots,x_k\}$.  Moreover, $A_2$ is obtained from $A_1$ by replacing one of $x_2$ or $x_3$, by $y_2$ or $y_3$,  respectively.  Say, $\edge{A_1,x_2,y_2,A_2}$ so that $A_2=\{y_1,y_2,x_3,\dots,x_k\}$.  Now, however, we have that $\edge{B_1,x_1,y_1,A_2}$, but clearly $B_1 \not\sim A_2$.  It follows that $\thet{3,3,3}$ is not an $i$-graph.
	\end{proof}
	
	% <<< E: Prop {prop:c:thet333}
	
	
	
	
	
	
	
	
	
	
	
	This completes the proof of Theorem \ref{thm:c:thetas}.
	
	
	
	
	%---------------------------------------SECTION: Other Results ----------------
	
	\section{Other Results}  \label{sec:c:other}
	In the final section of this chapter we first display a graph that is neither a theta graph nor an $i$-graph, and then use the method of graph complements to show that every cubic 3-connected bipartite planar graph is an $i$-graph.
	
	
	\subsection{A Non-Theta Non-$i$-Graph}  \label{subsubsec:c:nonThetnonI}
	
	
	So far, every non-$i$-graph we have observed is either one of the seven theta graphs from Theorem \ref{thm:c:thetas}, or contains one of those seven  as an induced subgraph (as per Corollary \ref{coro:i:notInduced}).  This leads naturally to the question of whether theta graphs provide a forbidden subgraph characterization for $i$-graphs.  Unfortunately, this is not the case.  
	
	Consider the graph $\ntni$ in Figure \ref{fig:c:nonThetnonI}: it is not a theta graph, and although it contains several theta graphs as induced subgraphs, none of those induced subgraphs are among the seven non-$i$-graph theta graphs.  In Proposition \ref{prop:c:nonThetnonI} we confirm  that $\ntni$ is not an $i$-graph.
	
	
	
	
	%~~~~~~~~~~~~FIG START~~~~~~~~~~~
	\begin{figure}[H]
		\centering
		\begin{tikzpicture}%[line width=0.3mm,scale=1]			
			
			%---------- REF-------------------
			\node(cent) at (0,0) {};			
			\path (cent) ++(0:65 mm) node(rcent)  {};		
			
			%----- left C4 ----------	
			\foreach \i/\j/\c in {x/X/90,y/Y/-90} {				
				\path (cent) ++(\c:20 mm) node [std] (v\i) {};
				%\path (v\i) ++(\c:5 mm) node (Lv\i) {${\j}$};
			}
			
			\path (vx) ++(90:5 mm) node (Lvx) {$\color{blue}X=\{x_1,x_2,x_3,x_4\dots, x_k\}$};
			\path (vy) ++(-90:5 mm) node (Lvy) {$\color{red}Y=\{y_1,y_2,y_3,x_4,\dots,x_k\}$};
			%\path (vy) ++(-90:5 mm) node (Lvy) {$\color{blue}Y=\{y_1,y_2,x_3,\dots, x_k\}$};
			
			\path (cent) ++(180:8 mm) node (va) {};	
			
			%\path (va) ++(180:25 mm) node (Lva) {$A=\{y_1,x_2,x_3,\dots, x_k\}$};
			
			\path (va) ++(90:8 mm) node [std] (va1) {};
			\path (va1) ++(180:25 mm) node (Lva1) {\color{blue}$A_1=\{y_1,x_2,x_3,\dots, x_k\}$};
			
			\path (va) ++(90:-8 mm) node [std] (va2) {};
			\path (va2) ++(180:25 mm) node (Lva2) {\color{red}$A_2=\{y_1,x_2,y_3,\dots,x_k\}$};	
			
			
			
			\draw[thick] (vx)--(va1)--(va2)--(vy);		
			
			
			%------------ B Pathway
			
			\path (cent) ++(0:8 mm) node (vb) {};
			
			\path (vb) ++(90:8 mm) node [std] (vb1) {};
			\path (vb1) ++(0:25 mm) node (Lvb) {\color{blue}$B_1=\{x_1,y_2,x_3,\dots, x_k\}$};
			
			\path (vb) ++(90:-8 mm) node [std] (vb2) {};
			\path (vb2) ++(0:25 mm) node (Lvb) {\color{blue}$B_2=\{y_1,y_2,x_3,\dots, x_k\}$};	
			%  \path (vb2) ++(0:25 mm) node (Lvb) {\color{blue}$B_2=\{x_1,y_2,x_3,\dots, x_k\}$};	
			
			\draw[thick](vx)--(vb1)--(vb2)--(vy); 
			
			
			%----- right P4 ----------
			\foreach \i/\c in {1/14,2/0,3/-13} {				
				\path (rcent) ++(90:\c mm) node [std] (c\i) {};
				%\path (c\i) ++(0:5 mm) node (Lc\i) {$C_{\i}$};
			}
			
			\draw[thick] (vx)--(c1)--(c2)--(c3)--(vy);
			
			%\path (cent) ++(-90: 20mm) node (HL)  {$\mathcal{H}$};
			
			\path (c1) ++(0:5 mm) node (Lvc1) {\color{red}$D_1$};
			%\path (c2) ++(0:25 mm) node (Lvc2) {\color{red}$C_2=\{x_1,x_2,y_3,\dots, x_k\}$};
			%\path (c3) ++(0:25 mm) node (Lvc3) {\color{red}$C_3=\{x_1,x_2,y_3,\dots, x_k\}$};
			\path (c2) ++(0:5 mm) node (Lvc2) {\color{red}$D_2$};
			\path (c3) ++(0:5 mm) node (Lvc3) {\color{red}$D_3$};
			
			
			\draw[thick](va1)--(vb2);
			
		\end{tikzpicture}				
		\caption{A non-theta non-$i$-graph $\ntni$.}
		\label{fig:c:nonThetnonI}%
	\end{figure}
	
	%>>> S: Prop {prop:c:nonThetnonI}
	\begin{prop} \label{prop:c:nonThetnonI}
		The graph $\ntni$ in Figure \ref{fig:c:nonThetnonI} is not an $i$-graph.
	\end{prop}
	
	
	\begin{proof}
		We proceed similarly to the proofs for the theta non-$i$-graphs in Section \ref{sec:c:nonthetas}.   Let $\ntni$ be the graph in Figure \ref{fig:c:nonThetnonI}, with vertices as labelled, and suppose to the contrary that there is some graph $G$ such that $\ig{G}\cong \ntni$.  
		
		To begin, we determine the vertices of the two induced $C_4$'s of $\ntni$.  Immediately from Proposition \ref{prop:i:C4struct}, the vertices of $X$, $A_1$, $B_1$, and $B_2$ are as labelled in Figure \ref{fig:c:nonThetnonI}.  Using a second application of Proposition \ref{prop:i:C4struct}, $A_2$ differs from $A_1$ in exactly one position, different from $B_2$.  Without loss of generality, say, $\edge{A_1, x_3, y_3, A_2}$.  Then again by the proposition, $Y=\{y_1, y_2, y_3, x_4 \dots, x_k\}$ as in Figure \ref{fig:c:nonThetnonI}.
		
		We now construct the vertices of $D_1$ through a series of claims:
		
		% From Lemma \ref{lem:i:claw}, $D_1$ differs from $X$ in one vertex, different from both $A_1$ and $B_1$.  
		
		%	By Observation \ref{obs:i:d2}, since $|D_1 - Y| =3$,
		
		\begin{enumerate}[label=(\roman*)]
			\item \label{prop:c:nonThetnonI:i} $x_3$ is not in $D_1$. 
			
			From Lemma \ref{lem:i:claw}, $D_1$ differs from $X$ in one vertex, different from both $A_1$ and $B_1$; moreover,  $x_1$ and $x_2$ are in $D_1$.    		
			Notice that $\{x_4,x_5,\dots,x_k\} \subseteq D_1$: suppose to the contrary that, say,  $x_4 \notin D_1$, so that $\edge{X, x_4,z,D_1}$.  Then $z \neq y_1$, since $y_1 \sim_G x_1$ and $D_1$ is independent.  Likewise $z \neq y_2$ and $z \neq y_3$. Thus $D_1 = \{x_1, x_2, x_3, z, x_5,\dots, x_k\}$ has $|Y \cap D_1| =4$, but $d(D_1,Y)=3$, contradicting Observation \ref{obs:i:d2}. 
			
			
			
			\item \label{prop:c:nonThetnonI:ii} $y_1$, $y_2,$ and $y_3$ are not in $D_1$.  
			
			
			As above, $y_1$ and $y_2$ are not in $D_1$, as $D_1$ is an independent set containing $x_1$ and $x_2$.  
			Suppose to the contrary that $\edge{X,x_3,y_3,D_1}$, so that $D_1 = \{x_1, x_2, y_3,  \dots, x_k\}$. Then, since $x_1 \sim_G y_1$, we have that $\edge{D_1,x_1,y_1,A_2}$, a contradiction.
			
			\item \label{prop:c:nonThetnonI:iii} $D_1 = \{x_1, x_2, z, x_4, \dots, x_k\}$, where $z \notin \{y_1,y_2,y_3\}$. 
			
			Immediate from \ref{prop:c:nonThetnonI:i} and \ref{prop:c:nonThetnonI:ii}.
			
			
		\end{enumerate}
		
		A contradiction for the existence of $G$ arises as we construct $D_2$.  Since $d_{\ntni}(D_1,Y)=3$ and $|D_1 \cap Y| = 3$, at each step along the path through $D_2, D_3,$ and $Y$, exactly one token departs  from a vertex of $D_1$  and moves to one of $Y-D_1=\{y_1,y_2,y_3\}$.
		However, $D_2 \neq \{y_1,x_2,z,x_4,\dots,x_k\}$, since otherwise, $\edge{A_1,x_3,z,D_2}$.  Likewise, $D_2 \neq \{x_1,y_2,z,x_4,\dots,x_k\}$.  Finally $D_2 \neq \{x_1,x_2,y_3,x_4,\dots,x_k\}$ as again we have $\edge{A_2,y_1,x_1,D_2}$.  Thus, we cannot build a set $D_2$ such that $|D_2 \cap Y| \leq 2$ as required.  We so conclude that no such graph $G$ exists, and that $\ntni$ is not an $i$-graph.
	\end{proof}
	
	Like the seven non-$i$-graph realizable theta graphs of Theorem \ref{thm:c:thetas},  $\ntni$ is a minimal obstruction to a graph being an $i$-graph; every induced subgraph of  $\ntni$ is a theta graph.

	
	
	
	%---------
	\subsection{Maximal Planar Graphs} \label{subsubsec:c:maxPlanar}
	
	
	We conclude this chapter with a result to demonstrate that certain planar graphs are $i$-graphs and $\agraph$-graphs.  Our proof uses the following three known results.
	
	
	
	
	%\nts{Fix reference}
	
	%>>> S: Theorem {thm:c:ref:planarDual}  
	\begin{theorem} \cite[Theorem 4.6]{CLZ} \label{thm:c:ref:cub3con}  A cubic graph is 3-connected if and only if it is 3-edge connected.
	\end{theorem}
	% <<< E: Theorem {thm:c:ref:planarDual}  
	
	
	
	
	
	%>>> S: Theorem {thm:c:ref:planarDual}  
	\begin{theorem} \cite{W69} \label{thm:c:ref:3col}  
		A connected planar graph $G$ is bipartite if and only if its dual $\dual{G}$ is Eulerian.
	\end{theorem}
	% <<< E: Theorem {thm:c:ref:planarDual}  
	
	
	
	
	%>>> S: Theorem {thm:c:ref:maxPlan}   
	\begin{theorem} \cite{H1898, TW11} \label{thm:c:ref:maxPlan}  
		A maximal planar graph $G$ of order at least 3 has $\chi(G) = 3$ if and only if ${G}$ is Eulerian.
	\end{theorem}
	% <<< E: Theorem {thm:c:ref:maxPlan}  
	
	
	
	In our proof of the following theorem, we consider a graph $G$ that is cubic, 3-connected, bipartite, and planar. We then examine its dual $\dual{G}$, and how those specific properties of $G$ translate to $\dual{G}$.  Then, we construct the complement of $\dual{G}$, which we refer to as $H$.  We claim that $H$ is a seed graph of $G$; that is, $\ig{H}$ contains an induced copy of $G$. 
	
	
	
	\begin{comment}
		%>>> S: Theorem {thm:c:ref:planarDual}  
		\begin{theorem} \cite{T1963} \label{thm:c:3conn}  
			Let $G$ be a 3-connected planar graph.  A cycle $C$ of $G$ is a facial cycle of some plane embedding of $G$ if and only if it is an induced cycle and non-separating.
		\end{theorem}
		% <<< E: Theorem {thm:c:ref:maxPlan}  
	\end{comment}
	
	%>>> S: Theorem {thm:c:3con}   
	\begin{theorem} \label{thm:c:3con}  
		Every cubic 3-connected bipartite planar graph  is an $i$-graph and an $\agraph$-graph.	
	\end{theorem}
	
	\begin{proof}
		Let $G$ be a cubic 3-connected bipartite planar graph and consider the dual $\dual{G}$ of $G$.  Since $G$ is bridgeless, $\dual{G}$ has no loops.  Moreover, since $G$ is 3-connected, Theorem \ref{thm:c:ref:cub3con} implies that no two edges separate $G$; hence, $\dual{G}$ has no multiple edges.  Therefore, $\dual{G}$  is a (simple) graph.  Further, since $G$ is cubic, each face of $\dual{G}$ is a triangle, and so $\dual{G}$ is a maximal planar graph.  
		
		We note the following two key observations.  First, since each face of $\dual{G}$ is a triangle,
		
		
		\begin{enumerate}[label=(\arabic*)]
			\item  \label{thm:c:3con:i}   each edge of $\dual{G}$ belongs to a triangle.
			
		\end{enumerate}
		
		\noindent For the second, note that since $G$ is bipartite, $\dual{G}$ is Eulerian (by Theorem \ref{thm:c:ref:3col}).  Then, by Theorem \ref{thm:c:ref:maxPlan}, $\chi(\dual{G})=3$, so $\dual{G}$ does not contain a copy of $K_4$.  Thus,
		
		\begin{enumerate}[label=(\arabic*),resume]
			\item \label{thm:c:3con:ii}   every triangle of $\dual{G}$ is a maximal clique.
		\end{enumerate}
		
		
		Now, by the duality of $\dual{G}$ and $G$, there is a one-to-one correspondence between the facial triangles of $\dual{G}$ and the vertices of $G$.   Let $H$ be the complement of $\dual{G}$.  By \ref{thm:c:3con:i} and \ref{thm:c:3con:ii}, $i(H) = \alpha(H)=3$, and every maximal independent set of $G$ corresponds to a triangle of $\dual{G}$.  But again, by duality, the facial triangles of $\dual{G}$ and their adjacencies correspond to the vertices of $G$ and their adjacencies.  Therefore, $\ig{H}$ contains $G$ as an induced subgraph.   Any additional unwanted vertices of $\ig{H}$ can be removed by applying the Deletion Lemma (Lemma \ref {lem:i:inducedI}).
	\end{proof}




